Reasoning-Driven Question-Answering for Natural Language Understanding

Natural language understanding (NLU) of text is a fundamental challenge in AI, and it has received significant attention throughout the history of NLP research. This primary goal has been studied under different tasks, such as Question Answering (QA) and Textual Entailment (TE). In this thesis, we investigate the NLU problem through the QA task and focus on the aspects that make it a challenge for the current state-of-the-art technology. This thesis is organized into three main parts: In the first part, we explore multiple formalisms to improve existing machine comprehension systems. We propose a formulation for abductive reasoning in natural language and show its effectiveness, especially in domains with limited training data. Additionally, to help reasoning systems cope with irrelevant or redundant information, we create a supervised approach to learn and detect the essential terms in questions. In the second part, we propose two new challenge datasets. In particular, we create two datasets of natural language questions where (i) the first one requires reasoning over multiple sentences; (ii) the second one requires temporal common sense reasoning. We hope that the two proposed datasets will motivate the field to address more complex problems. In the final part, we present the first formal framework for multi-step reasoning algorithms, in the presence of a few important properties of language use, such as incompleteness, ambiguity, etc. We apply this framework to prove fundamental limitations for reasoning algorithms. These theoretical results provide extra intuition into the existing empirical evidence in the field.

==> Daniel K - thesis - dissertation/0.acknowledgement.tex <==
I feel incredibly lucky to have Dan Roth as my advisor. 
I am grateful to Dan for trusting me, especially when 
% I approached him as \emph{``yet another student trying to apply his hammer (machine-learning knowledge) to a new problem''} with 
I had only a basic understanding of many key challenges in natural language. It took me a while to catch up with \emph{what is important} in the field and be able to communicate the challenges effectively. 
During these years, 
% Over the years, 
Dan's vision has always been the guiding principle to many of my works.   
His insistence on focusing on the long-term progress, rather than ``easy'' 
% short-term 
wins, shaped the foundation of many of the ideas I pursued. 
This perspective 
% , and 
pushed me to think differently than the popular trends. 
% In a long run, it changed my on
% I met Dan when I was looking for an application (namely NLP) to use the hammer I was familiar with (machine learning); little did I know that, in just a few years, the application itself turns more interesting than the hammer.    
It has been a genuine privilege to work together. 

I want to thank my thesis committee at UPenn, Mitch Marcus, Zach Ives and Chris Callison-Burch  for being a constant source of invaluable feedback and guidance. 
Additionally, I would like to thanks the many professors who have touched parts of my thinking: Jerry DeJong, for encouraging me read the classic literature; 
% on ``knowledge representation'';  
% Mitch Marcus, for his deep understanding of the literature; 
Chandra Chekuri and Avrim Blum, for their emphasis on intuition, rather than details; 
% and ``big picture''; % Avrim Blum, for his ability to attend to the ``big picture''; 
and my undergraduate advisor Hamid Sheikhzadeh Nadjar, for encouraging me to work on important problems. 

A huge thank you to the Allen Institute for Artificial Intelligence (AI2) for much support during my PhD studies. 
Any time I needed any resources (computing resources, crowdsourcing credits, engineering help, etc), without any hesitation, AI2 has provided me what was needed. 
Special thanks to Ashish Sabhwaral and Tushar Khot for being a constant source of wisdom and guidance, and investing lots of time and effort. They both have always been present to listen to my random thoughts, almost on a weekly basis. 
I am grateful to other members of AI2 for their help throughout my projects: Oren Etzioni, Peter Clark, Oyvind Tafjord, Peter Turney, Ingmar Ellenberger, Dirk Groeneveld,
% Niket Tandon, Bhavana Dalvi, 
Michael Schmitz, Chandra Bhagavatula and Scott Yih. 
Moreover, I would like to remember Paul Allen (1953-2018): his vision and constant generous support has tremendously changed our field (and my life, in particular).  

% Oren Etzioni with his strict management style and pushing us to be never stop being ambitious. His footsteps His vision has turned AI2 (and Seattle) into a leading hubs
% A big chunk of my work was done in collaboration with Allen Institute for Artificial Intelligence, at Seattle. 
% Mitch Marcus has been a constant source
% of wisdom and guidance, and his personality, in my mind, will always be synonymous with
% Penn NLP and the wonderful intellectual environment 
% \todo{cogcomp}

My collaborators, especially past and present CogComp members, have been major contributors and influencers throughout my works. I would like to thank Mark Sammons, Vivek Srikumar, Christos Christodoulopoulos, Erfan Sadeqi Azer, Snigdha Chaturvedi, Kent Quanrud, Amirhossein Taghvaei, Chen-Tse Tsai, and many other CogComp members. 
Furthermore, I thank Eric Horn and Jennifer Sheffield for their tremendous contributions to many of my write-ups. And thank you to all the friends I have made at Penn, UIUC, and elsewhere, for all the happiness you've brought me. Thanks to Whitney, for sharing many happy and sad moments with me, and for helping me become a better version of myself. 
% \todo{Especial thanks to Eric Horn and Jennifer Shefield for their significant efforts in reading my many write ups. }



Last, but never least, my family, for their unconditional sacrifice and support. I wouldn't have been 
% I will not be 
able to go this far without you.
% They convinced a three-year old me that scientists have all the fun in the world. I thank them for that, for everything else and a little more.
% Finally, I would like to thank my parents, for their unconditional sacrifice and support. I will not be able to go this far without you.

==> Daniel K - thesis - dissertation/0.introduction_new.tex <==
\chapter{Introduction}
\epigraph{ 
``To model this language understanding process in a computer, we need a program which combines grammar, semantics, and reasoning in an intimate way, concentrating on their interaction.''
}{--- \textup{T. Winograd}, Understanding Natural Language, 1972}


% \begin{chapquote}{Lewis Carroll, \textit{Alice in Wonderland}}
% \textsf{ 
% \footnotesize
% ``Begin at the beginning,'' the King said, gravely, ``and go on till you
% come to an end; then stop.''
% }
% \end{chapquote}

\section{Motivation}
%  is considered one of the ultimate goals in the natural language processing field. 
The purpose of \emph{Natural Language Understanding} (NLU) is to enable systems to interpret a given text, as close as possible to the many ways humans would interpret it. 


% The Natural Language Understanding (NLU) covers one of AI’s complex challenges. 
Improving NLU is increasingly changing the way humans interact with machines. 
% Improving NLU is increasingly changing human interface with machines.
The current NLU technology is already making significant impacts. 
For example, we can see it used by 
% NLU is used by 
speech agents, including Alexa, Siri, and Google Assistant. 
% Achieving NLU could unleash tremendous potentials for using  
% could enable current 
% impacts in the way different technology is being applied in our daily lives. 
% With this technology, computers would understand of natural human languages commands  
% and for computers to communicate back to humans in their own languages.
% Just to name a few,
In the near future, 
% In the coming year, 
with better NLU systems, we will witness a more active presence of these systems in our daily lives: social media interactions, in financial estimates, during the course of product recommendation, in accelerating of  scientific findings, etc. 

The importance of NLU was understood by many pioneers in Artificial Intelligence (starting in the '60s and '70s). The initial excitement about the field ushered a decade of activity in this area~\citep{McCarthy63,Winograd72,Schank72,Woods73,Zadeh78}. The beginning of these trends was overly positive at times, and it took years (if not decades) to comprehend and appreciate the real difficulty of language understanding. 
% While many pioneers in the Artificial Intelligence agreed on the importance of NLU, it's takes a longer time to comprehend and appreciate the complexity of this target. 
% While the importance of NLU was clear from early days of AI, its hardness was underestimated to the most part. 

\section{Challenges along the way to NLU}
\label{intro:challenges:nlu}
% \section{Why NLU is hard?}
\begin{figure}
    \centering
    \begin{tabular}{L{\textwidth}}
    \toprule
        \justify A 61-year-old furniture salesman was pushed down the shaft of a freight elevator yesterday in his downtown Brooklyn store by two robbers while a third attempted to crush him with the elevator car because they were dissatisfied with the \$1,200 they had forced him to give them.  \\ 
        The buffer springs at the bottom of the shaft prevented the car from crushing the salesman, John J. Hug, after he was pushed from the first floor to the basement. The car stopped about 12 inches above him as he flattened himself at the bottom of the pit.  \\ 
        Mr. Hug was pinned in the shaft for about half an hour until his cries attracted the attention of a porter. The store at 340 Livingston Street is part of the Seaman’s Quality Furniture chain. 
        \\ 
        Mr. Hug was removed by members of the Police Emergency Squad and taken to Long Island College Hospital. He was badly shaken, but after being treated for scrapes of his left arm and for a spinal injury was released and went home. He lives at 62-01 69th Lane, Maspeth, Queens.
        \\ 
        He has worked for seven years at the store, on the corner of Nevins Street, and this was the fourth time he had been held up in the store. The last time was about one year ago, when his right arm was slashed by a knife-wielding robber. \\ 
        \tabularnewline
    \bottomrule
    \end{tabular}
    \caption{A sample story appeared on the New York Times (taken from~\cite{McCarthy76}).  }
    \label{fig:mcarthy:example:paragraph}
\end{figure}

% Even kids are good at language understanding; so why is it so out of our reach? 
We, humans, are so used to using language that it's almost impossible to see its complexity, without a closer look into instances of this problem. 
As an example, consider the story shown in Figure~\ref{fig:mcarthy:example:paragraph}, which appeared in an issue of the New York Times (taken from~\cite{McCarthy76}). With relatively simple wording, this story is understandable to English speakers. Despite the simplicity, many nuances have to come together to form a coherent understanding of this story. 
% However, a true understanding of this story involves much more that combining shallow meaning individual words. 



We flesh out a few general factors which contribute to the complexity of language understanding in the context of the story given in Figure~\ref{fig:mcarthy:example:paragraph}:
\begin{figure}
    \centering
    \includegraphics[scale=0.4]{figures_intro/ambiguity_2.png}
    \caption{\emph{Ambiguity} (left) appears when mapping a raw string to its actual meaning; \emph{Variability} (right) is having many ways of referring to the same meaning. }
    \label{fig:ambiguity}
\end{figure}
\begin{itemize}
    \item \textit{Ambiguity} comes along when trying to make sense of a given string. While an average human might be good at this, it's incredibly hard for machines to map symbols or characters to their actual meaning. 
    % This results in \textbf{ambiguity} when interpreting natural language text.
    For example, the mention of ``car'' that appears in our story has multiple meanings (see Figure~\ref{fig:ambiguity}; left). In particular, this mention in the story refers to a sense other than its usual meaning (here refers to \emph{the elevator cabin}; the usual meaning is a \emph{road vehicle}).   
    % (referring to the elevator cabin) is used , which has a meaning other than its usual meaning. 
    \item \textit{Variability} of language means that a single idea could be phrased in many different ways. For instance, the same character in the story, ``Mr. Hug,'' has been referred to in  different ways: ``the salesman,'' ``he,'' ``him,'' ``himself,'' etc. 
    Beyond lexical level, there is even more variability in bigger constructs of language, such as phrases, sentences, paragraphs, etc. 
    % \includegraphics[scale=0.25]{figures_intro/variability.png}
    % This property is usually referred to as the \textbf{variability} of language. 
    \item Reading and understanding text involves an implicit formation of a mental structure with many elements. 
    % , some based on the given story and some based on our past experiences. 
    Some of these elements are directly described in the given story, but a significant portion of the understanding involves 
    % information \emph{implied} from the text (not directly mentioned).  
    information that is \emph{implied} based on a readers' background knowledge. 
    \textit{Common sense} refers to our (humans) understanding of everyday activities (e.g., sizes of objects, duration of events, etc), usually shared among many individuals. Take the following sentence from the story: 
    \begin{framed}
    \noindent
    The car stopped about 12 inches above him as he flattened himself at the bottom of the pit.
    \end{framed}
    There is a significant amount of imagination hiding in this sentence; each person after reading this sentence has a mental picture of the incident. And based on this mental picture, we have implied meanings: \emph{we know he is lucky to be alive now; if he didn't flatten himself, he would have died; he had nowhere to go at the bottom of the pit; the car is significantly heavier than the man}; etc. 
    % A major portion of our understanding is the result of  ... 
    % This phenomena is usually referred to as \textbf{common sense}. 
    Such understanding is common and easy for humans and rarely gets direct mention in text, since they are considered trivial (for humans). Humans are able to form such implicit understanding as a result of our own world model and past shared experiences.   
    \item \textit{Many small bits combine to make a big picture.}  
    % There are many small bits of information combine together to create a complex scenario. 
    We understand that ``downtown Brooklyn'' is probably not a safe neighborhood, since ``this was the fourth time he had been held up here.'' We also understand that despite all that happened to ``Mr. Hug,'' he likely goes back to work after treatment because similar incidents have happened in the past. Machines don't really make these connections (for now!). 
\end{itemize}


% \begin{comment}
%  - Ambiguities on the subject; The data may not be mathematically meaningful since it is textual data.
%  - Not complete data; Since the content of the textual content depends on the exact nature of the data, it also poses difficulties in modeling.
%  - The data is ambiguous; Due to the fact that textual data is not numerical, it is difficult to make meaning from texts precisely. 
%   Q1: time / commonsense 
%   Q2: variability  
%   Q3: event ordering / commonsense 
%   Q4: 
%   Abduction 
%  \end{comment}
Challenges in NLU don't end here; there are many other aspects to language understanding that we skip here since they go beyond the scope of this thesis. 
% Humans are used to being surrounded with so much  complexity. 
% The goal of this work (and any work towards NLU) is induce machines with such nuances. 


% \todo{talk about easier challenges: like coref, names, grouping, srl, etc.}

\begin{comment}
\section{Solving smaller pieces, one at a time}
\label{sec:pieace:by:pieace}
The hardness of NLU motivated the community to tackle the problem either as by chunking it into multiple subtask. 
There are numerous proposals as to what sub-tasks and what semantics and abstraction level to target. Below we briefly mention a few useful and well-established subtasks that could help us understanding this story. 
% Below, we briefly mention a few of the subtaks extensively studied in the field over the past one or two decades: 
% The field has shown more interest in some of these tasks,
% \begin{itemize}
%     \item Dependency Parsing: 
%     \item Named Entity Recognition: 
%     \item Coreference Resolution: 
%     % \item Quantity normalization: 
%     % \item Relation Extraction: 
%     \item Semantic Role Labeling: 
% \end{itemize}



Consider the phrase, ``\emph{61-year-old furniture salesman}'': many human readers would attribute ``61-years old'' to the ``salesman,'' and not to its adjacent term, ``furniture.'' Why should a computer know this? The \textbf{dependency-parse}~\citep{eisner1996three} could be used to infer this. 
% be useful in resolving such issues. In the figure below, .... As it can be seen in the 
As it can be seen in the dependency parse of the first sentence,  ``61-years old'' is a modifier of the ``salesman'': 

\resizebox{\textwidth}{!}{
\frame{
\includegraphics[scale=0.24,trim=0.3cm 6.5cm 24.9cm 0.4cm, clip=true]{figures_intro/modified_dependency.png}
}
}

% How does a computer know `M`
% \resizebox{\textwidth}{!}{
% \frame{
% \includegraphics[scale=0.24,trim=0.2cm 0.2cm 12cm 0.2cm, clip=true]{figures_intro/modified_ner.png}
% }
% }


Prepositions are likes connecting blocks between nouns and verbs, and there are many of them used in this story. Each preposition, depending on the context, they might carry a different meaning. For instance, ``for'' preposition alone has at least 15 different senses. Figure below, denotes the output of \textbf{preposition semantic roles}~\citep{litkowski2005preposition,SrikumarRo13} for two different phrases, each two different senses for the ``for'' preposition:

% \resizebox{\textwidth}{!}{
\begin{center}
\frame{
\centering
\includegraphics[scale=0.29,trim=0.2cm 0.4cm 21cm 0.4cm, clip=true]{figures_intro/modified_prep_srl.png}
}
% }
\end{center}
\end{comment}


\section{Measuring the progress towards NLU via Question Answering}
To measure machines' ability to understand a given text, one can create numerous questions about the story. A system that better understands language should have a higher chance of answering these questions.
% Having an effective protocol to measure the progress toward NLU is critical to the evolution of our field in this direction.
This approach has been a popular way of measuring NLU since its early days~\citep{McCarthy76,Winograd72,Lehnert77}. 
% We follow the same procedure established by the pioneers of the field: using natural language to issue queries about the assumed scenario. Probably an earliest version of of this is Turing's test~\cite{Turing50} or Winograd's conversational agents~\cite{Winograd72}. 
% Later in Chapter 2 (Section~\ref{}) we will provide better categorization of specific evaluation protocols. 


\begin{table}
    \centering
    \small
    \begin{tabular}{L{0.8 \textwidth}}
        \toprule
        \textbf{Question 1:} Where did the robbers push Mr. Hug?\\ 
        \textbf{Answer 1:} down the shaft of a freight elevator \\ 
        \midrule
        \textbf{Question 2:} How old is Mr. Hug? \\ 
        \textbf{Answer 2:} 61 years old \\ 
        \midrule
        \textbf{Question 3:} On what street is Mr. Hug's store located? \\ 
        \textbf{Answer 3:} 340 Livingston Street, on the corder of Nevins Street \\ 
        \midrule
        \textbf{Question 4:} How far is his house to work? \\ 
        \textbf{Answer 4:} About 30 minutes train ride \\ 
        \midrule
        \textbf{Question 5:} How long did the whole robbery take? \\ 
        \textbf{Answer 5:} Probably a few minutes \\ 
        \midrule
        \textbf{Question 6:} Was he trapped in the elevator car, or under? \\
        \textbf{Answer 6:} under  \\ 
        \midrule
        % \textbf{Q8:} Where is Mr. Hug’s home? \\
        % (A question whose answer requires a literal understanding of only one sentence of the story.) Does Mr. Hug live in Brooklyn? No,  
        % \textbf{A8:} he lives in Queens. \\ 
        % \midrule
        \textbf{Question 7:} Was Mr. Hug conscious after the robbers left?  \\ 
        \textbf{Answer 7:} Yes, he cried out and his cries were heard.  \\
        \midrule
        \textbf{Question 8:} How many floors does Mr. Hug's store have? \\
        \textbf{Answer 8:} More than one, since he has an elevator  
        % \tabularnewline
        \tabularnewline
        \bottomrule
    \end{tabular}
    \caption{Natural language questions about the story in Figure~\ref{fig:mcarthy:example:paragraph}. }
    \label{tab:mr:hug:questions}
\end{table}


Table~\ref{tab:mr:hug:questions} shows examples of such questions. 
Consider \textbf{Question 1}. The answer to this question is directly mentioned in text and the only thing that needs to be done is creating a representation to handle the variability of text. 
For instance, a reoresentation of the meaning that are conveyed by \emph{verb} predicates, since a major portion of meanings are centered around verbs. 
For example, to understand the various elements around a verb ``push,'' one has to figure out \emph{who pushed, who was pushed, pushed where}, etc. The subtask of \textbf{semantic role labeling}~\citep{PunyakanokRoYi04} is dedicated to resolving such inferences (Figure~\ref{fig:annotation:mrhug}; top). The output of this annotation of indicates that \emph{the location pushed to} is ``the shaft of a freight elevator.'' 
In addition, the output of  
% One only has to understand that ``Mr. Hug'' is the same as the ``A 61-year old furniture salesman''; such understanding comes from 
the \textbf{coreference} task~\citep{CarbonellBr88,McCarthy95} informs computers about such equivalences between the mentions of the main character of the story (namely, the equivalence between ``Mr. Hug'' and ``A 61-year-old furniture salesman'').  

% As it can be seen, this system has managed to resolve coreference relations of many different mentions in this paragraph. 
% For example ``Mr. Hug'', has been referred to in many different ways, such as ``the salesman'', ``he'', ``him'', ``himself'', etc. 


% \resizebox{\textwidth}{!}{
% \frame{
% \includegraphics[scale=0.24,trim=0.12cm 3.5cm 17cm 0.3cm, clip=true]{figures_intro/modified_verb_srl.png}
% }
% }

% \resizebox{\textwidth}{!}{
% \frame{
% \includegraphics[scale=0.24,trim=0cm 0cm 0cm -0.05cm]{figures_intro/coref-3-colored.png}
% }
% }

\begin{figure}
    \centering
    \frame{
        \resizebox{\textwidth}{!}{
            \includegraphics[scale=0.30,trim=0.19cm 3.5cm 17cm 0.2cm, clip=true]{figures_intro/modified_verb_srl.png}
        }
    }
    \frame{
        \resizebox{\textwidth}{!}{
            \includegraphics[scale=0.24,trim=0cm 0cm 0cm -0.05cm]{figures_intro/coref-3-colored.png}
        }
    }
    \caption{Visualization of two semantic tasks for the given story in Figure~\ref{fig:mcarthy:example:paragraph}. Top figure shows \emph{verb semantic roles}; bottom figure shows clusters of \emph{coreferred} mentions. 
    The visualizations use CogCompNLP~\citep{KSZRCSRRLDTRMFWYSGUANLR18} and AllenNLP~\citep{GGNTDLPSZ18}.
    }
    \label{fig:annotation:mrhug}
\end{figure}


Similarly the answers to \textbf{Question 2 and 3} are directly included in the paragraph, although they both require some intermediate processing like the coreference task. The system we introduce in Chapter 4 uses such representations (coreference, semantic roles, etc) and in principle should be able to answer such questions. 
% Such questions in principle could be address by the systems that will introduce here (see Chapter 4). 
The dataset introduced in Chapter 6 also motivates addressing questions that require chaining information from multiple pieces of text. In a similar vein, Chapter 8 takes a theoretical perspective on the limits of chaining information. 

The rest of the questions in Table~\ref{tab:mr:hug:questions} are harder for machines, as they require information beyond what is directly mentioned in the paragraph. For example, \textbf{Question 4} requires knowledge of the distance between ``Queens'' and ``Brooklyn,'' which can be looked up on the internet. 
Similarly, \textbf{Question 5} requires information beyond text; however, it is unlikely to be looked up easily on the web. 
% cannot be looked up anywhere. 
Understanding that ``the robbery'' took only a few minutes (and not hours or days) is part of our common sense understanding. The dataset that we introduce in Chapter 7 motivates addressing such understanding (temporal common sense). 
\textbf{Question 6 and 7} require different forms of common sense understanding, beyond the scope of this thesis. 
% which we do not address here. 

\begin{comment}
\begin{itemize}
    \item What is ``reasoning" \textit{in the context of natural language}, and whether it is possible to provide a definition for it? While other communities like logic and philosophy have had their definition for this for quite long time, such definitions (and their assumptions) often don't easily generalize to natural language.  
    \item How much reasoning ability does exist in the existing statistical systems? Many of the current systems leverage simple and shallow information. We have to understand the depth of their abilities. 
    \item Is it possible to (similar to humans) start with acquiring \textit{language ability} and then move on to \textit{question answering} ability? (unlike many current QA systems that equate the two).  
    % \item How can we create harmony between ``reasoning" (hard nature of language) and ``learning" (soft nature of language)? 
    % What is the ``right" interface between ``reasoning" (hard nature of language) and ``learning" (soft nature of language)? 
    % Almost any of the systems that put effort to model reasoning, they have to combine their system with a ``soft" knowledge so that their model does not suffer from brittleness. A challenge here is creating a good balance between the soft components and the reasoning elements. 
    \item How to deal with new (potentially contradictory) knowledge (or assumptions)? 
    % \item Are there any theoretical limitations/motivations for unification Reasoning and Learning?  
    % \item  What if the systems are missing some information/experiences? In other words, what is the right way to \textit{know what we don't know?}  % Many AI systems are dependent on their KB/experiences for making predictions.
    % \item Many Reasoning-based models are fragile when it comes to noisy data. How should we properly deal with false information? (4) There is a big literature on interactive learning with environment (e.g. contextual bandits \cite{auer2002nonstochastic}); is it possible to mingle such techniques with well-known supervised/semi-supervised algorithms for real applications? 
\end{itemize}


I propose to focus on \textit{reasoning} a key ingredient towards solving the question answering problem. This ingredient contains a wide spectrum of behaviors (induction, abduction, etc), many of which are actively in interaction with each other and are changing through the process. Loosely speaking the existing paradigms in the community often fall into limited forms of reasoning: learning-theoretic models can be thought of as \textit{induction}, Bayesian-nets perform \textit{abduction}, etc. 
It would be shortsighted to think that one can give an explicit definition for reasoning \underline{in natural language}, blindly following how it's been done conventionally in other communities like logic. Such definitions are often derived by introspection of personal experiences, and could be subject to biases and other flaws. Hence we argue that studying reasoning by trying to define a concrete definition for it might not be a good approach. Instead we try to study it in environments that it is forced to be exposed. 

The overarching theme on the subjects studied here is their connection to an aspect of reasoning. 
%, specifically when tacking natural language question answering. 
By studying each of these aspects, we show that understanding of the underlying process could substantially benefit our current technology and lead to better solutions. 
\end{comment}

In this thesis we focus on the task of Question Answering (QA), aiming to progress towards NLU. And for this goal, we study various representations and reasoning algorithms. 
% to address the common challenges in NLU. 
In summary, this thesis is centered around the following statement: 

%Instead we try to study it in scenarios where it is forced to reveal itself.  
\paragraph{Thesis Statement.} \emph{
% When designing QA systems``language understanding" should come before learning about questions. To enable machines answer natural questions, requires a diverse spectrum of ``reasoning" forms working in ``harmony". 
% Answering natural language questions, require a wide spectrum of reasoning abilities working together in harmony, while affecting each other. Focusing on creating this harmony and interplay is a key to making progress in question answering problem. 
% {\color{blue}Question answering} is one way to measure the progress in {\color{blue} natural language understanding}. 
% {\color{blue} Automating} natural language understanding requires {\color{blue} reasoning}.
% Effective {\color{blue} reasoning} requires a {\color{blue}wide spectrum} of {\color{blue}inter-dependent abilities} working together and {\color{blue} coherently}. 
% Question answering can be used to accurately measure progress in natural language understanding.
% {\color{blue}Question answering} can be used to measure the progress in {\color{blue} natural language understanding}. 
% {\color{blue} Automating} questions answering could be facilitated by incorporating a {\color{blue}wide spectrum} of {\color{blue}inter-dependent abilities} working together. 
Progress in {\color{blue}automated} question answering could be facilitated by incorporating the ability to {\color{blue}reason} over natural language {\color{blue}abstractions} and {\color{blue}world knowledge}. 
More {\color{blue}challenging, yet realistic} QA datasets pose problems to current technologies; hence, more {\color{blue}opportunities} for {\color{blue}improvement}.
}

\begin{comment}

\paragraph{Only the tip of the iceberg. } While these individual representations are effective at capturing some certain inferences about language, it's only a shallow representation of the complete phenomena. 

\todo{create connection here . . .  }
Below are a few ``easy'' interpretations (to humans) which are not directly mentioned in text and could be challenging for computers:  
% Take the following examples: 
\begin{itemize}
    \item The ``robbers'' certainly wanted \underline{more} than ``\$12,00,'' since they were ``dissatisfied'' with this amount. There is no explicit mention of this, but only implied. 
    \item ``Mr. Hug'''s store has multiple floors, since it  has  an ``elevator.'' 
    \item Probably none of ``Mr. Hug'''s friends were at the store, otherwise someone would have tried to help him. 
    \item The ``robbers'' probably think that ``Mr. Hug'' is dead, because they intended ``to crush him.'' 
\end{itemize}
% \todo{mention that, although these annotations give us something, these are just the tips of the iceberge.

Having known that the annotations (discussed in Section~\ref{sec:pieace:by:pieace}) only capture the surface of language understanding, solving each of these individual 
tasks should not be equated with NLU. In other words, these tasks are just means for a bigger end. 

\end{comment}

\section{Thesis outline}
In the thesis we use QA as a medium to tackle a few important challenges in the context of NLU. We start with an in-depth review of past work and its connections to our work in Chapter 2. The main content of the thesis is organized as follows (see also Figure~\ref{fig:contributions:table}): 
% We are addressing a few of the issues discussed above in three parts, followed by Chapter 2 where we review the literature and provide all the related work. 

\begin{figure}
    \centering
    % \resizebox{\textwidth}{!}{
    \includegraphics[scale=0.89,trim=5.5cm 14.2cm 0cm 1cm, clip=false]{figures_intro/chapters_and_issues4.pdf}
    \caption{An overview of the contributions and challenges addressed in each chapter of this thesis. 
    % Some of the terms will be defined in Chapter 2. 
    }
    \label{fig:contributions:table}
\end{figure}

\begin{itemize}
    \item Part 1: \emph{Reasoning-Driven QA System Design}
    % An Abductive Formulation for Question Answering
    % }
    \begin{itemize}
        \item Chapter 3 discusses \tableilp, a model for abductive reasoning over natural language questions, with internal knowledge available in tabular representation. 
        % , which internally uses models that are inductively-leaned models to create its abstractions.  
        % The model exploits the semantic structure of text to answer multiple-choice questions. We present a system that reasons over a wide range of semantic abstractions of the text, represented as families of graphs, based on which we translate question answering (QA) into a search for an optimal subgraph that satisfies certain global and local properties. The formalism can be seen as an \textit{abductive} reasoning. The proposed structured subgraph search system for this task is formulated and implemented as an Integer Linear Program (ILP). 
        % In out first system \tableilp, we use semi-automatically generated \textit{tables} as our knowledge representation and focus on multi-step inference and a combination of multiple facts across tables \cite{tableilp2016:ijcai}. 
%On a dataset science questions, our system significantly outperforms (+14\%) the best previous attempt at structured reasoning for this task, which used Markov Logic Networks (MLNs). 
        \item Chapter 4 presents \textilp, an extension of the system in the previous chapter to function on raw text knowledge. 
        % to use off-the-shelf and general-purpose natural language modules such as semantic role labelers, coreference resolvers, and dependency parsers to populate our graphical knowledge representation~\cite{semanticilp2018aaai}. 
        %The approach is especially suitable for domains that require reasoning over a diverse set of linguistic constructs but have limited training data. Our system demonstrates strong performance on two domains simultaneously. 
        % In particular, on a collection of challenging science QA datasets, it outperforms various state-of-the-art approaches, including neural models, broad coverage information retrieval, and specialized techniques using structured knowledge bases, by 2\%-6\%. 

        \item Chapter 5 %Question answering (QA) systems are easily distracted by irrelevant or redundant words in questions, especially when faced with long or multi-sentence questions in difficult domains. This paper introduces and 
        studies 
        % Second, we study 
        the notion of {\em essential question terms} with the goal of making QA solvers more robust to distractions and irrelevant information. 
        %We illustrate the importance of essential question terms by showing that humans' ability to answer questions drops significantly when essential terms are eliminated from questions. 
        % We develop a classifier that reliably 
        %(90\% mean average precision) 
        % identifies and ranks essential terms in questions, and use the classifier to demonstrate that the notion of question term essentiality allows state-of-the-art QA solvers for elementary-level science questions to make better and more informed decisions. % , improving performance by up to 5\%.
        % We also introduce a new dataset of over 2,200 crowd-sourced essential terms annotated science questions. 
        
    \end{itemize}
    \item Part 2: \emph{Moving the Peaks Higher: More Challenging QA datasets}
    % In this part, we propose two constructions for creating challenge QA datasets.
    \begin{itemize}
        \item Chapter 5 presents \multirc, a reading comprehension challenge which requires combining information from \underline{multiple sentences}.
%We solicit and verify questions and answers for this challenge through a 4-step crowdsourcing experiment.
%Enforcing the generated questions to depend on multiple sentences, results in questions with variety of reasoning phenomena.\todo{Do we show this? If not, remove this claim.}
%We do not limit ourselves to narrow classes of reasoning. 
% Our challenge dataset contains 6,500+ questions for 1000+ paragraphs across 7 different domains (elementary school science, news, travel guides, fiction stories, etc) bringing in linguistic diversity to the texts and to the questions wordings. On a subset of our dataset, we found human solvers to achieve an F1-score of $88.1\%$, while a range of baselines demonstrate the difficulty in this challenge. 
%\todo{Daniel update this number} %, an evidence for its high quality \todo{is it?!}.
% say that it is a majority vote of 3 humans? 

%for current computational models, 
% despite a high human performance.
%on this set. 
%The dataset is the first to study multi-sentence inference at scale, with an open-ended set of question types that requires reasoning skills.

        \item Chapter 6 presents \tacoqa, a reading comprehension challenge which requires  the ability to resolve \underline{temporal common sense}. 
    \end{itemize}
    \item Part 3: \emph{Formal Study of Reasoning in Natural Language}
    \begin{itemize}
        \item Chapter 7 presents a formalism, in an effort to provide \underline{theoretical grounds} to the existing intuitions on \underline{the limits and possibilities} in reasoning, in the context of natural language.
        % within the realm of its
        % in presence of properties like variability and ambiguity. 
    \end{itemize}
\end{itemize}




==> Daniel K - thesis - dissertation/1.background_new.tex <==
\chapter{Background and Related Work}
% \epigraph{ 
% ``A computer would deserve to be called intelligent if it could deceive a human into believing that it was human.''
% }{--- \textup{Alan Turing}, Computing Machinery and Intelligence, 1950}
% \label{chapter:background}

\epigraph{ 
``Whoever wishes to foresee the future must consult the past.''
}{--- \textup{Nicolo Machiavelli}, 1469-1527}
\label{chapter:background}


\section{Overview}
\label{sec:intro:qa:review}
% This chapter aims to provide a holistic view of the field. 
% % current and in the past. 
% As indicated in the previous chapter, we focus on \emph{natural language understanding} as the ultimate goal. In this chapter, we review the related literature that address different aspects of this target. 
In this chapter, we review the related literature that addresses different aspects of \emph{natural language understanding.}


Before anything else, we define the terminology (Section~\ref{sec:relate:terminology}). 
We divide the discussion into multiple interrelated axes: 
% the first in any effort towards NLU is to having an objective measure of progress this problem. 
Section~\ref{sec:related:protocols} discusses 
% first we discuss
various evaluation protocols and datasets introduced in the field. 
We then provide an overview of the field from the perspective of \emph{knowledge representation and abstraction} in Section~\ref{sec:related:kr}. Building on the 
% What is build on top of 
discussion of representation, we provide a survey of \emph{reasoning} algorithms, in Section~\ref{sec:related:reasoning}. We end the chapter with 
% an overview of NLU datasets (Section~\ref{sec:related:datasets}) and 
a short section on the technical background necessary for the forthcoming chapters (Section~\ref{sec:background:notation:technical}). 

To put everything into perspective, we show a summary of the highlights of the field in Figure~\ref{fig:nlu:history}. Each highlight is color-coded to indicate its contribution type. In the following sections, we go over a select few of these works and explain the evolution of the field, especially those directly related to the focus of this work. 
% . Wherever possible, we clarify the connections of the works discussed with the focus of this thesis. 

\begin{figure}
    \centering
    \includegraphics[scale=0.5,trim=1cm 0.0cm 1cm 5cm, clip=false]{figures_background/nlu_history_6.png}
    \caption{
        Major highlights of NLU in the past 50 years (within the AI community). For each work, its contribution-type is color-coded. To provide perspective about the role of the computational resources available at each period, we 
        show the progress of CPU/GPU hardware over time. 
    }
    \label{fig:nlu:history}
\end{figure}

\section{Terminology}
\label{sec:relate:terminology}
Before starting our main conversation, we define the terminology we will be using throughout this document. 
% To keep the discussion clear, we first define the key terms. 
% \noindent \textbf{Key terms:}
%To begin with let us first precise definitions for some of the terms we will be using in this work.
%\footnote{Some of the definitions here might be a little less accurate or incomplete, although good enough for our purposes. Interested reader is encourage to follow the citations for more accurate statement of the definitions.}   
% We start with \text{proposition}. 
\begin{itemize}
    \item 
    % \noindent 
    \underline{Propositions} are \textit{judgments} or \textit{opinions} which can be true or false. A proposition is not necessarily a sentence, although a sentence can express a proposition (e.g., ``cats cannot fly"). 
    % For example the sentence that  contains the proposition that cats are not able to fly. Similarly this sentence ``Cats are unable to fly" and this declarative phrase with logic {\tt can-fly(cats)=false} convey the same proposition. A claim or a sentence can contain multiple \textit{atomic} propositions. For example ``Many think that cats can fly". 
    \item 
    % \noindent 
    A \underline{concept} is either a physical entity (like a \textit{tree, bicycle, etc}) or an abstract idea (like \textit{happiness, thought, betrayal, etc}). 
    % , which all are (usually) called concepts. 
    %\begin{itemize}[noitemsep]
    %\item Oxford: An abstract idea; a general notion. 
    %\item Merriam-Webster: an idea of what something is or how it works. 
    %\end{itemize}
    % \noindent  
    \item 
    a \underline{belief} is an expression of faith and/or trust in the truthfulness of a proposition. 
    % , although a belief might not necessarily be true. 
    We also use \emph{confidence} or \emph{likelihood} to refer to the same notion. 
    %\begin{itemize}[noitemsep]
    %\item Oxford: An acceptance that a statement is true or that something exists 
    %\item Merriam-Webster: a feeling of being sure that someone or something exists or that something is true 
    %\end{itemize}
    % For example ``Homer believed that the earth is flat" is an proposition which contains the belief of ``earth" being ``flat", which is not true. ``The weather forecast predicts a tornado for tomorrow." is another proposition which expresses another belief which might turn out to be true or false. 
    % \noindent \underline{Cognition: } Discussion of knowledge representation is closely related to the mental picture of the objects and concepts around us. Cognition is the mental action or process of acquiring knowledge and understanding through thought, experience, and the senses. Although cognition involves abstract mental representations of concepts, it can have 
    %Cognition although is referring to an abstract idea of a concept, it can have 
    % an outer physical source (like observation, hearing, touching, etc), or inner source (like thinking), or a combination of inner and outer sources. 
    %The dictionary definition is: 
    %\begin{itemize}[noitemsep]
    %\item Oxford: The mental action or process of acquiring knowledge and understanding through thought, experience, and the senses.
    %\item Merriam-Webster: Conscious mental activities : the activities of thinking, understanding, learning, and remembering.  
    %\end{itemize}
    \item 
    % \noindent 
    \underline{Knowledge} is information, facts, understanding acquired through experience or education. 
    % ; the theoretical or practical understanding of a subject. 
    % Perhaps the right question to start with is what is \textit{knowledge}? 
    %We start by giving dictionary definitions, which might not be completely accurate, but are the common understanding of what it is: 
    %\begin{itemize}[noitemsep]
    %\item Oxford: Facts, information, and skills acquired by a person through experience or education; the theoretical or practical understanding of a subject. 
    %\item Merriam-Webster:  information, understanding, or skill that you get from experience or education; awareness of something : the state of being aware of something
    %\end{itemize}
    The discussion on the philosophical nature of knowledge 
    % has long been studied in 
    % , where it has been been classified into different categories
    and its various forms is studied under \textit{epistemology} \citep{Steup14}. 
    % based on its nature, and its inherent connection to \textit{belief}, \textit{truth}, \textit{justification}, etc is analyzed. %Informally, knowledge is any information about a domain that can be used to solve problems defined in that domain. 
    \item 
    % \noindent 
    \underline{Representation} 
    % To solve many problems there is a need to use some form of information which might be implicit in the problem definition or even not mentioned; therefore this
    is a medium through which knowledge is provided to a system. 
    % knowledge must be provided to the solver (which can be a computer or any other machine) in order to be used when needed. In other words, representation is a surrogate for a concept, belief, knowledge or propositions. 
    For example, the number 5 could be represented as the string ``5", as bits {\tt 101}, or 
    %Arabic script ``", or 
    Roman numeral ``V", etc. 
    % As part of designing a program to solve a problem, we must define how to represent the required knowledge. The theory of Knowledge Representation is concerned with the formalization of how to represent propositions, beliefs, etc. 
    % \item 
    % \noindent 
    % \underline{Representation Scheme} is the definition of the representations. 
    % the form of the knowledge saved in a knowledge base. 
    \item 
    % \noindent 
    \underline{Abstraction} 
    % Any representation is an \textit{abstraction} of the world and its objects. 
     defines the level of granularity in a representation. For example, the mentions ``New York City'', ``Buenos Aires'', ``Maragheh'' could all be \emph{abstracted} as {\tt \small city}.  
    % The abstraction level of a representation might be too detailed, or too coarse with only high-level information. 
    %\underline{Inference: }  
    %\begin{itemize}[noitemsep]
    %\item Oxford: A conclusion reached on the basis of evidence and reasoning. 
    %\item Merriam-Webster: The act or process of reaching a conclusion about something from known facts or evidence. 
    %\end{itemize}
    \item 
    % \noindent 
    \underline{Knowledge acquisition} is the process of identifying and acquiring the relevant knowledge, according to the representation. 
    % 
    \item 
    % \noindent 
    \underline{Reasoning} is the process of drawing a conclusion based on the given information. 
    % is the heart of AI, the decision making system for solving a problem or the action of thinking about something in a logical and sensible way in order to form a conclusion. 
    We sometimes refer to this process as \emph{decision-making} or \emph{inference}. 
    % \noindent \underline{Supervised learning: }
    % \noindent \underline{Unsupervised learning: }
\end{itemize}
\section{Measuring the progress towards NLU}
\label{sec:related:protocols}
\subsection{Measurement protocols}
% Machine reasoning is a fundamental challenges in AI, particularly in natural language processing (NLP) it has received significant attention throughout the AI history \cite{Greene1959AnAT,mccarthy1990example,reiter1976semantically,Winograd1980ExtendedIM}. 
Evaluation protocols are critical in incentivizing the field to solve the right problems. 
% In addition, for the protocols to become widely-used, they better be computationally inexpensive. 
% those objectives that are computationally inexpensive, tend to more convenient for becoming widely-used. 
% are ``cheaper'' to compute makes them easier to use. 
% Some of the earliest tests in AI address focus on the former aspect, while ignoring the latter, i.e. computational tractability.
% more on the deep philosophical aspects of the problem, and mostly ignore its computational tractability. 
% Perhaps 
One of the earliest proposals is due to Alan Turing: if you had a pen-pal for years, you would not know whether you're corresponding to a human or a machine~\citep{Turing50,Harnad92}. A major limitation of this test (and many of its extensions) is that it is ``expensive'' to compute~\citep{Hernandez-Orallo00,French00}. 
% This proposal has seen many supports, criticisms, and extensions; see for example, \citep{Hernandez-Orallo00,French00,lacurts2011criticisms}. 
% We refer the interested reader to the relevant literature~


The protocol we are focusing on in this work is through answering natural language questions; if an actor (human or computer) understands a given text, it should be able to answer any questions about it. Throughout this thesis, we will refer to this protocol as \textbf{Question Answering} (QA). 
This has been used in the field for many years~\citep{McCarthy76,Winograd72,Lehnert77}. 
There are few other terms popularized in the community to refer 
% We would like to note that the task we're solving here is sometimes referred 
the same task we are solving here. 
The phrase \textbf{Reading Comprehension} is borrowed from standardized tests (SAT, TOEFL, etc.), usually refers to the scenario where a paragraph is attached to the given question. Another similar phrase is  \textbf{Machine Comprehension}. Throughout this thesis, we use these phrases interchangeably to refer to the same task. 

To make it more formal, for an assumed scenario described by a paragraph $P$, a system $f$ equipped with NLU should be able to answer any questions $Q$ about the given paragraph $P$. One can measure the expected performance of the system on a set of questions $\mathcal{D}$, via some distance measure $d(., .)$ between the predicted answers $f(Q; P)$ and the correct answers $f^*(Q; P)$ (usually a prediction agreed upon by multiple humans): 
$$
\mathfrak{R}(f; \mathcal{D}) = \mathbb{E}_{(Q, P) \sim \mathcal{D}} \Big[ d \Big( f\left(Q; P\right), f^*\left(Q; P\right) \Big) \Big] 
$$
% Answering questions posed in natural language is a fundamental AI task, with a large number of impressive QA systems built over the years. 
% A chief goal in NLP is to have machines with similar reasoning abilities as humans (at least when looking from the outside). 
% Question answering (QA) is a fundamental challenge in AI, particularly in natural language processing (NLP) and reasoning.  
% for question answering systems that operate with a natural language interface.
% This protocol requires system to ``understand'' what a question is really about and how it has to be answered. This protocol has long been in the field: for example, McCarthy, after proving a story, argues, 
% ``an intelligent person or program should be able to answer ... 
% questions based on the information in the story''~\cite{McCarthy76}. 
% Similarly, 
% In a similar fashion, 
% Winograd uses natural language questions to measure the ability of artificial agents in NLU and connecting it to an environment. 
% Machine Comprehension of natural language text is a fundamental challenge in AI and it has received significant attention throughout the history of AI \citep{Greene1959AnAT,mccarthy1990example,reiter1976semantically,Winograd1980ExtendedIM}.
% the field has created over the years. 
% Over the years, the field has created many static datasets used to evaluate the progress of different NLU models. 
% For the remaining of this section, we review examples of each versions of QA. 
% The two variations tend appeart in two aspects 

A critical question here is the choice of question set $\mathcal{D}$ so that $\mathfrak{R}(f; \mathcal{D})$ is an effective measure of $f$'s progress towards NLU. 
% all the nuances of language understanding? 
Denote the set of all the possible English questions as $\mathcal{D}_u$. This is an enormous set and, in practice it is unlikely that we could write them all in one place. Instead, it might be more practical to sample from this set. In practice, this sampling is replaced with \emph{static} datasets. This introduces a problem: datasets are hardly a uniform subset of $\mathcal{D}_u$; instead, they are heavily skewed towards more simplicity. 


Figure~\ref{fig:question:manifold} depicts a hypothetical high-dimensional manifold of all the natural language questions in terms of an arbitrary representation (bytes, characters, etc.) 
Unfortunately, datasets are usually biased samples of the universal set $\mathcal{D}_u$. And they are often biased towards simplicity. This issue makes the dataset design of extra importance since performance results on a single set might not be a true representative of our progress. Two chapters of this work are dedicated to the construction of QA datasets. 

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.35,trim=1cm 0cm 0cm 0cm, clip=false]{figures_background/NLU_manifold4.png}
    \caption{A hypothetical manifold of all the NLU instances. Static datasets make it easy to evaluate our progress but since they usually give a biased estimate, they limit the scope of the challenge.}
    \label{fig:question:manifold}
\end{figure}

There are few flavors of QA in terms of their answer representations (see Table~\ref{tab:sample:questions:background}): 
% studied various versions of QA in the forms of 
% \begin{itemize}
    % \item 
     (i) questions with multiple candidate-answers, a subset of which are correct; %  and the correct one(s) have to be indicated; 
    % \item 
    (ii) extractive questions, where the correct answer is a  substring of a given paragraph; 
    % \item 
    (iii) Direct-answer questions; a hypothetical system has to \emph{generate} a string for such questions. 
% \end{itemize}
The choice of answer-representation has direct consequences for the representational richness of the dataset and ease of evaluation. The first two settings (multiple-choice and extractive questions) are easy to evaluate but restrict the richness of the dataset. Direct-answer questions can result in richer datasets but are more expensive to evaluate. 

\begin{table}[]
    \centering
    \small
    \begin{tabular}{c|L{0.93 \textwidth }}
        \toprule 
        \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\footnotesize Multiple-choice \hspace{-0.5cm} }}}  & Dirk Diggler was born as Steven Samuel Adams on April 15, 1961 outside of Saint Paul, Minnesota. His parents were a construction worker and a boutique shop owner who attended church every Sunday and
        believed in God. Looking for a career as a male model, Diggler dropped out of school at age 16 and left home. He was discovered at a falafel stand by Jack Horner. Diggler met his friend, Reed Rothchild, through Horner in 1979 while working on a film. \\ 
        & \textbf{Question:} How old was Dirk when he met his friend Reed?\\ 
        & \textbf{Answers:} *(A) 18 \hspace{0.75cm} (B) 16 \hspace{0.75cm} (C) 22  \\ 
        % \tabularnewline
        \midrule
        \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\footnotesize Extractive}}} & The city developed around the Roman settlement Pons Aelius and was named after the castle built in 1080 by Robert Curthose, William the Conqueror's eldest son. The city grew as an important centre for the wool trade in the 14th century, and later became a major coal mining area. The port developed in the 16th century and, along with the shipyards lower down the River Tyne, was amongst the world's largest shipbuilding and ship-repairing centres. \\ 
        % Newcastle's economy includes corporate headquarters, learning, digital technology, retail, tourism and cultural centres, from which the city contributes £13 billion towards the United Kingdom's GVA. 
        % Among its icons are Newcastle Brown Ale; Newcastle United football club; and the Tyne Bridge. It has hosted the world's most popular half marathon, the Great North Run, since it began in 1981. 
        & \textbf{Question:} Who built a castle in Newcastle in 1080? \\ 
        & \textbf{Answers:} ``Robert Curthose'' \\
        % \tabularnewline
        \midrule
        \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{{\footnotesize Direct-answer}}}} & \\ 
         & \textbf{Question:} Some birds fly south in the fall. This seasonal adaptation is known as migration. Explain why these birds migrate.  \\ 
        & \textbf{Answers:} ``A(n) bird can migrate, which helps cope with lack of food resources in harsh cold conditions by getting it to a warmer habitat with more food resources.'' \\ 
        % \tabularnewline
        \bottomrule
    \end{tabular}
    \caption{Various answer representation paradigms in QA systems; examples selected from \cite{KCRUR18,RZLL16,CEKSTTK16}. }
    \label{tab:sample:questions:background}
\end{table}


% In some settings there is no knowledge accompanying the questions. Hence the solvers are expected to bring in their own knowledge; for example elementary-level science exams~\citep{ClarkEt16}. In another popular scenario the relevant knowledge (a paragraph, a table, a graph, etc) is provided; for example \processBank~\citep{BSCLHHCM14} has paragraphs and WikiTables~\citep{Pasupat2015CompositionalSP} has knowledge provided as tables.  

% Having \textit{multiple-choices with single correct} is probably the oldest and most-popular way of writing questions.
% While they are easy to grade, it’s not always to generate them such that the answer is not trivial. In addition, assuming that there exactly one correct answer is often an extra help given to the machine. Regents science exam~\citep{CEKSTTK16} is an example dataset with of this kind. 
% In a different approach it is assumed to have answers as a contiguous substring of a paragraph. A prominent example is SQuAD where answers must be a span of the passage. This paradigm brings multiple limitations: first, the paragraph is guaranteed to contains the answer, while it might not be the
% case in realistic examples of comprehension. Second, since the answer has to be a span of the paragraph, it limits the questions to the classes with answers in the paragraphs, and rules out any questions which have answers implied by the text and require deeper understanding of it. 

% We give an extensive overview different datasets in Section~\ref{sec:related:datasets}. 
% \section{Datasets}
% \label{sec:related:datasets}
Datasets 
% are important in the sense that they 
make it possible to automate the evaluation of the progress towards NLU and 
be able to compare systems to each other on fixed problems sets. 
% unify the evaluation across systems to compare them. 
% In this section we provide an outline of various \emph{Question Answering} datasets introduced in the field. 
%  In particular, in natural language processing (NLP) it has been studied under various settings, such as multiple-choice Question-Answering (QA)~\citep{green1961baseball}, Reading Comprehension (RC)~\citep{HLBB99}, 
One of the earliest NLU datasets published in the field is the Remedia dataset~\citep{HLBB99} which contains 
% is a small dataset of 
short-stories written in simple language for kids provided by Remedia Publications. 
% for reading comprehension. 
Each story has 5 types of questions (\emph{who, when, why, where, what}). 
Since then, there has been many suggestions as to what kind of question-answering dataset is a better test of NLU. 
\cite{BGBGHF05} suggests SAT exams as a challenge for AI. \cite{Davis14} proposes 
% hand-construction of 
multiple-choice challenge sets that are easy for children but difficult for computers.  In a similar spirit, \cite{ClarkEt16} advocate elementary-school science tests. Many science questions have answers that are not explicitly stated in text and instead, require combining information together. 
In Chapter 2, 3 we use 
% will be using 
elementary-school science tests as our target challenge.
% MCTest~\citep{RichardsonBuRe13}, SQuAD~\citep{RZLL16} and TriviaQA \citep{JCWZ17} to name a few, are some of the datasets that were  released recently with the goal of facilitating research in machine comprehension. 


% Conversely, while there are AI systems for formal scientific reasoning (e.g., \citep{aura,isaac}), they require questions to be posed in logic or restricted English.

% An issue with Davis's proposal is that, 
% Despite Davis' claim on simplicity of his target questions, 
% it is not clear how easy it is to generate such questions, as he doesn't provide any reasonably-sized dataset matching his proposal. 
% \cite{weston2015towards}~present a relatively small dataset of 10 reasoning categories, and propose to build a system that uses a world model and a linguistic model. The fundamental limitation of the dataset is that it is generated according to a restricted set of reasoning categories, which possibly limits the complexity and diversity of questions.

% Some other recent datasets proposed for machine comprehension also pay attention to type of questions and reasoning required. 
% For example, MCTest~\citep{RichardsonBuRe13} is one of the earliest efforts to encourage reasoning with multiple sentences. 
% , and claims that about half of the questions require multi-sentence reasoning. That is, turkers were asked to generate multi-sentence questions. However, it was not systematically ensured that more than one sentences are indeed required to answer such questions. In Section~\ref{sec:analysis}, we empirically show that only about half of the questions annotated as `multi-sentence' actually require information from multiple sentences. 
% Another dataset, SQuAD \citep{RZLL16}, provides a collection of 100k+ questions composed for Wikipedia documents.  The questions are meant to be answered by extracting spans of text from the relevant paragraphs. 

% RACE~\citep{LXLYH17} is also a collection of about 100k+ questions extracted from text books. The language used in these paragraphs are somewhat simple because they were meant for students who learn English as a foreign language.  
% MS MARCO~\citep{NRSGTMD16} is another such large dataset, where questions are anonymized queries issued through Bing or Cortana and the passages are related web pages. For each question in the dataset, several related passages are provided.  The CNN/Daily Mail dataset \citep{HKGEKSB15} contains questions and passages from news domain. However, the questions were automatically generated by removing an entity from a human written summary of the corresponding news article.  WikiQA~\citep{YangYiMe15} is a Chinese dataset with 42k QA pairs and 580k evidences. All questions are factoid questions, and the evidences are also retrieved using a search engine. Nearly $2/3^{rd}$ of the questions have no correct answer in the candidate sentences. TriviaQA \citep{JCWZ17} contains a big collection of trivia questions and noisy evidence paragraphs extracted from the web. Due to the nature of many trivia questions, the majority of them are are limited to named-entities.

% Despite all the excitement fueled by that large data sets and the ability to directly train statistical learning models, current QA systems do not have capabilities comparable to elementary school or younger children~\citep{ClarkEt16}. 

While the field has produced many datasets in the past few years, many of these datasets are either too restricted in terms of their linguistic richness or they contain annotation biases~\citep{GSLSBS18,PNHRD18}. 
% These datasets differ in their linguistic richness. In fact, 
For many of these datasets, 
% researchers 
it has been pointed out
that many of the high-performing models neither need to `comprehend' in order to correctly predict an answer, nor learn to `reason' in a way that generalizes across datasets~\citep{ChenBoMa16,JiaLi17,KaushikLi18}. In Section~\ref{subsec:perturbation} we show that 
adversarially-selected candidate-answers 
result in a significant drop in performance of a few state-of-art science QA systems. 
To address these weaknesses, in Chapter 4, 5 we 
propose two new challenge datasets which, we believe, pose better challenges for systems.  
% , as we experimentally show, captures the kind of reasoning problems that are challenging for the current state-of-the-art. 
% will propose two different ideas to create NLU datesets. 
% Similarly, \citep{JiaLi17} show that adding an adversarially selected sentence to the instances in the SQuAD datasets drastically reduces the performance of many of the existing baselines. 
% \citep{ChenBoMa16} show that in the CNN/Daily Mail datasets, ``the required reasoning and inference level \ldots is quite simple'' and that a relatively simple algorithm can get almost close to the upper-bound. 

% \textbf{Question:} In New York State, the longest period of daylight occurs during which month? \\ 
%   \textbf{Answers:}  *(A) June   \hspace{0.5cm}   (B) March \hspace{0.5cm}    (C) December \hspace{0.5cm}   (D) September \\ 

% \todo{move it to reasoning}
A closely related task is the task of Recognizing Textual Entailment (RTE)~\citep{KSZRCSRRLDTRMFWYSGUANLR18,DRSZ13}, as QA can be cast as entailment (Does {\it $P$} entail {\it $Q+A$}? \citep{BCDG08}). 
While we do not directly address this task, in some cases we use it as a component within out proposed QA systems (in Chapter 3 and 4). 
% However, RTE has primarily focused on the task of {\it linguistic equivalence}, and has not addressed questions where some form of scientific reasoning is required. 
% Recent work on Natural Logic~\citep{angeli2014NLI,maccartney2009:thesis} has extended RTE to account for the {\it logical structure} within language.
% Our work can be seen as going one step further, to add a layer of structured reasoning on top of this; in fact, we use an RTE engine as a basic subroutine for comparing individual table cells in our ILP formulation.
% Recognizing Textual Entailment (RTE)~\citep{DRSZ13} etc. 


% \subsection{Evaluation. }
% A collection of question sets containing elementary-level science questions from standardized tests \citep{CEKSTTK16}. Here is an example question from \regentsFourth: 

% Proposed by \cite{BSCLHHCM14},

% We consider the multiple-choice setting where $Q$ is a question, $A$ is a set of answer candidates, and the knowledge required for answering $Q$ is available in the form of raw text $P$. 

% In particular, in natural language processing (NLP) it has been studied under various settings, such as multiple-choice Question-Answering (QA)~\citep{green1961baseball}, Reading Comprehension (RC)~\citep{HLBB99}, 

% Test scores are reported as percentages. For each multiple-choice question, a system gets a score of $1$ if it chooses the correct answer, $1/k$ if it reports a $k$-way tie that includes the correct answer, and $0$ otherwise.


\section{Knowledge Representation and Abstraction for NLU}
\label{sec:related:kr}
The discussion of knowledge representation has been with AI since its beginning and it is central to the progress of language understanding. 
Since directly dealing with the raw input/output complicates the reasoning stage, historically researchers have preferred to devise 
a  
% intermediate input/output to be 
middleman between the 
% natural 
raw 
information and the reasoning engine. 
% (Figure \ref{fig:representation:reasoning:sample:withKB}). 
Therefore, the need for an intermediate level seems to be essential. In addition, in many problems, there is a significant amount of knowledge that is not mentioned directly, but rather  implied from the context. Somehow the extra information has to be provided to the reasoning system. 
% , which is usually modeled as a \textit{knowledge base}. 
As a result, the discussion goes beyond just creating formalism for information, and also includes issues like, how to \emph{acquire}, \emph{encode} and \emph{access} it.
The issue of representations applies to both \emph{input} level information and the \emph{internal} knowledge of a reasoning system. 
% Such separation of knowledge from reasoning system is inherited to us from the very early AI projects. 
% and nowadays many accept it as the right way of modeling problems. Whether this is definitely the right way or not, there are debates; at least this is the popular way of doing it. 
We refer to some of the relevant debates in the forthcoming sections.  

% In this work we give a relatively comprehensive review on the long-standing works on knowledge representation with emphasis on natural language systems. The review will start from relatively fundamental issues on representation, and will continue to exemplary practical advancements. 
% Due to the close ties between representation and reasoning, various reasoning frameworks have appeared; we briefly explore them in conjunction with representation techniques.

\subsection{Early Works: ``Neats vs Scruffies''\protect\footnote{
Terms originally made by Roger Schank to characterize two different camps: the first group that represented commonsense knowledge in the form of large amorphous semantic networks, as opposed to another from the camp of whose work was based on logic and formal extensions of logic. 
}}
% \subsection{Knowledge Representations}
% In the early history of AI, there was big series of oppositions to the idea of ``abstract representation of thought" among psychology researchers.
% An early work that created a separate representation of the knowledge from the solver engine was the General Problem Solver (GPS) system of \cite{newell1961gps}. This system was intended to be a universal solver for any problem formalized in \textit{symbolic} form, like chess playing or theorem proving. The idea of symbolic reasoning was developed centuries earlier by Descartes, Pascal, Leibniz and some other pioneers in philosophy of mind. The use of \textit{symbols} as the fundamental elements of the representation---the \textit{physical symbol system hypothesis}~\citep{newell1961gps}---has widely been debated. 
% is a debatable assumption which has continued its way until now. 
% \todo{emphasize universl}
% Scalability was a big issue for GPS, due to 
% After the early scalablity issues of GPS, it soon became clear that a system designed for solving any formalized problem is impractical due to the 
% combinatorial explosion of intermediate states in many problems. 
% Also, it became apparent that 
% One of the main problems was how to represent the knowledge needed to solve a problem. Since then, the trend moved towards limiting the scope and focusing on specific problems, or narrower domains. 
An early trend emerged as the family of symbolic and logical representations, such as propositional and 1st-order logic~\citep{McCarthy63}.
This approach has deep roots in \emph{philosophy} and \emph{mathematical logic}, where the theories have evolved since Aristotle's time. Logic, provided a general purpose, clean and uniform language, both in terms of representations and reasoning. 


The other closely-related school of thought evolved from \emph{linguistics} and \emph{psychology}. This trend was less concerned with mathematical rigor, but more concerned with richer psychological and linguistic motivations. For example, \emph{semantic networks}~\citep{Quillan66}, a network of concepts and links, was based on the idea that memory consists of associations between mental entities. In 
Chapter 8 we study a formalism for reasoning with such graph-like representations. 
\emph{Scripts} and \emph{plans} are representational tools to model frequently encountered activities; e.g., going to a restaurant~\citep{SchankAb75,Lehnert77}. 
Minsky and Fillmore, separately and in parallel, advocated \emph{frame}-based representations~\citep{Minsky74,Fillmore77}. 
% they are all part of the  
% The two approaches were even given nicknames  due to their distinctions: \emph{neats} and \emph{scruffies}, respectively. 
% The nicknames  shows the depth of distinction between these approaches in the seventies. 
% There were distinction in terms of program design: One defines in a \emph{declarative} way, and has a \emph{procedural} views. 
% Frames can be seen as a restricted form of 1st-order knowledge.
The following decades, these approaches have evolved into fine-grained representations and hybrid systems for specific problems. 
% \textsc{LISP} was a declarative programming language ~\citep{McCarthyLe65}. 
One of the first NLU programs was the \textsc{STUDENT} program of~\cite{Bobrow64}, written in \textsc{LISP}~\citep{McCarthyLe65}, which could read and solve high school algebra problems expressed in natural language. 
% Similarly increased focus on specific applications gave rise to the popularity of \textit{Expert Systems} (i.e. systems which are good on a specific set of problems, rather than everything)~\citep{hayes1984building}. 
% The \textsc{Shrdlu} system of~\cite{winograd1971procedures} with a restricted natural language world model, could discuss and perform tasks in a simulated Blocks World, a famous planning domain with a set of objects (e.g. colored cubes, pyramids, etc). A user could ask for building stacks of blocks or moving them. 

% Programming languages like FRL~\citep{roberts1977frl} and KRL \citep{bobrow1977overview} we developed to support frame-models with default assignments, while borrowing elements from logic. 
% , are the early exemplar usages of frame-based knowledge bases, although tailored for limited problems. \todo{phrasing}

\begin{figure}
    \centering
    \includegraphics[scale=0.294,trim=1cm 0cm 0cm 0cm 0cm, clip=false]{figures_background/frame_example2.png}
    \caption{Example frames used in this work. Generic basic science frames (left), used in Chapter~3;  event frames with values filled with the given sentence (right), used in Chapter~4. }
    \label{fig:frame:example}
\end{figure}

Intuitively, a \emph{frame} induces a grouping of concepts and creates abstract hierarchies among them. 
For example, \emph{``Monday'', ``Tuesday'', ...} are distinct concepts, but all members of the same conceptual frame. 
A frame consists of a group of slots and fillers to define a stereotypical object or activity. A slot can contain values such as rules, facts, images, video, procedures or even another frame~\citep{FikesKe85}. 
Frames can be organized hierarchically, where the default values can be inherited the value directly from parent frames. 
% \citep{mccarthy1968some}
This is part of our underlying representation in Chapter 3, where the reasoning is done over tables of information (an example in Figure~\ref{fig:frame:example}, left). 
Decades later after its proposal, the frame-based approach resulted in resources like FrameNet~\citep{BakerFiLo98}, or tasks like Semantic Role Labeling~\citep{GildeaJu02,PalmerGiKi05,PunyakanokRoYi04}. 
This forms the basis for some of the key representations we use in Chapter 4 (see Figure~\ref{fig:frame:example}, right).  
% On Framesemantics: For example, one would not be able to understand the word "sell" without knowing anything about the situation of commercial transfer, which also involves, among other things, a seller, a buyer, goods, money, the relation between the money and the goods, the relations between the seller and the goods and the money, the relation between the buyer and the goods and the money and so on. 

% The differences perspectives was to the extend that 
% The two groups Roger Schank coined the two groups the neats and the scruffies, respectively.

% Frames later on evolved to other representational forms many of which are strict subsets of 1st-order logic and some are decidable and closely related to other formalisms such as modal logics~\citep{schild1991correspondence,schmidt1991attributive}.\todo{what?}
% One of such extensions is Description Logics (also called \textit{concept languages} or \textit{attributive description languages}~\citep{schmidt1991attributive}) that model the declarative part of frames using a logic-based semantics. One of the reasons for such extension was adding more mathematical 
% rigor in hierarchical definition of knowledge. 
% Description Logic~\citep{borgida1989classic} guarantee polynomial-time decision algorithms by using operators on concept descriptions (in contrast to the use of quantifiers in 1st-order logic).


\subsection{Connectionism}
\label{sec:connectionism}
There is another important trend  inspired by the apparent brain function emergent from interconnected networks of neural units~\citep{Rosenblatt58}.  
It lost many of its fans after \cite{MinskyPa69} showed representational limitations of shallow networks in approximating few functions. 
However, a series of events reinvigorated this thread: 
% gave another energy to neurally inspired models; 
Notably, \cite{RumelhartHiWi88} found a formalized way to train networks with more than one layer (nowadays known as Back-Propagation algorithm). This work emphasized the \textit{parallel} and \textit{distributed} nature of information processing and  gave rise to the ``connectionism" movement.
Around the same time \citep{Funahashi89} showed the universal approximation property for feed-forward networks (any continuous function on the real numbers can be uniformly approximated by neural networks). Over the past decade, this school has enjoyed newfound excitement by effectively exploiting parallel processing power of GPUs and harnessing large datasets to show progress on certain datasets.
%Since then, although there has been much effort on creating powerful and computationally efficient statistical models (like Support Vector Machines) based on feature-representation, \textit{Knowledge Representation} became a side focus of AI research, until the recent repopularization of Neural Networks, which moved the attention to \textit{unsupervised representation learning}. 
%The GPS paradigm eventually evolved into the Soar architecture for Artificial Intelligence. \cite{laird1987soar} \cite{laird2012soar}


\subsection{Unsupervised representations}
\label{sec:representations:intro}
Unsupervised representations are one of the areas that have shown tangible impacts across the board. A pioneering work is \cite{BDMPL92} which creates binary term representations based on co-occurrence information. Over the years, a wide variety of such representations emerged; using Wikipedia concepts~\citep{GabrilovichMa07}, word co-occurrences~\citep{TurneyPa10}, co-occurrence factorization~\citep{MCCD13,LevyGo14,PenningtonSoMa14,LXTJZC15}, and using context-sensitive representation~\citep{PNIGCLZ18,DCLT18}. In particular, the latter two are inspired by the connectionist frameworks in the 80s and have shown to be effective across a wide range of NLU tasks. In this thesis we use unsupervised representations in various ways: In Chapter 3 and 4 we use such representations for phrasal semantic equivalence within reasoning modules. In Chapter 5 we use as features of our supervised system. In Chapter 6, 7 we create NLU systems based on such representations in order to create baselines for the datasets we introduce. 
% , where we propose two challenge datasets, we create systems with such representations 
% \todo{Add a paragraph on unsupervised representations: BERT, W2V, etc. }
% It is important to mention that, there has been a surge of interest in creating distributed representations for natural language; for example {\tt Word2Vec } 
% \cite{MCCD13,PenningtonSoMa14} 
% and many other ongoing works. 

% \todo{The discussion of building blocks: Transformers, Attention, Seq2Seq}

% Much progress has been made, but still many problems are unsolved to a large extent. 
% , for some of which there are fundamental barriers. 
% \todo{simplify this paragraph}


% \subsection{Abstractions}
% \todo{phrasing:} 

% One of the issues which is arises as a result of representation of facts and rules is the  issue which, unfortunately, has little  direct literature. 

% For example, suppose in a database of people, a reasoning algorithm's function depends on  whether people are engineers or not. Consider these two scenarios: having a database of people with (1) with more abstracted form of job title, i.e. ``engineer" or ``non-engineer", or (2) full job names, such as ``psychologist", ``mathematician", ``chemical engineer", etc. In abstraction (1) the decision is relatively easier that abstraction (2), in which the decision needs further collapsing of the job-names into ``engineer" and ``non-engineer". 
% Therefore, usually the more detailed the information is, the more computationally difficult it is to reason with. 

% \todo{add figure?}
%A central issue for KR formalisms is the tradeoff between expressive power and deductive complexity. 
%At one extreme, propositional logic restricted to Horn clauses (disjunctions of atomic propositions with at most one negation) admits a very efficient decision procedure 
%but cannot ex-press any generalizations; 
%at another, full second-order logic is capable of expressing most of mathematics but has no complete inference procedure. 
%Most KR formalisms adopt various compromises. 

% What if in the previous example, the goal is a decision dependent on the exact job name? Then abstraction (2) would be the right abstraction level and abstraction (1) a bad approximation to the information needed. This shows that the right level of abstraction depends on what is needed. The abstraction level should be in a way that it is ``expressive enough" to find the answer, without further additional complications.  
% \todo{or it could be the responsibility of a reasoning algorithm to find ... }

% This is because a solution with detail involves more steps and many more possible courses of action exist from which to choose. 
% For example rather than specifying the property of ``fly" to each bird (e.g. ``geese", ``swan", ``eagle", etc), one can specify this property to any the more abstract level of ``birds". 

A more recent highlight along this path is the emergence of new unsupervised representations that have been shown to capture many interesting associations in freely available data~\citep{PNIGCLZ18,DCLT18}. 

\subsection{Grounding of meanings}
A tightly related issue to the abstraction issue is \emph{grounding} natural language surface information to their actual meaning~\citep{Harnad90}, as discussed in Section~\ref{intro:challenges:nlu}.
% Th \emph{symbol grounding problem}~, which is the problem of accurately mapping symbols into its underlying meaning representation.
Practitioners often address this challenging by enriching their representations; 
for example by mapping textual information to Wikipedia entries~\citep{MihalceaCs07}. 
% or grounding text to executable rules via semantic parsing~\citep{RTPSL17}. 
In Chapter 4 we use the disambiguation of semantic actions and their roles~\citep{PunyakanokRoYi04,DangPa05}. 
% Building upon such representations, the community has produced various reasoning systems that essentially work by combining local information. 
Chapter 8 of this thesis provides a formalism that incorporates elements of the symbol-grounding problem and shed theoretical light on existing empirical intuitions. 


% A major roadblock has been  the problem of \emph{symbol grounding}, or grounding free-form texts to a higher-level meaning. Example proposals to deal with this issue are, extracting semantic parses~\cite{KaplanBrot82,SteedmanBa11,BBCGGHKPS13}, linking to the knowledge bases~\cite{MihalceaCs07}, mapping to semantic frames~\cite{PunyakanokRoYi04}, etc. All such techniques can be thought of as approximate solutions for A tightly relatesymbolic information to some \emph{meaning}. 



% \todo{Add a paragraph on WSD and add wordnet there}
% \subsection{WordNet (1985--present)}
% WordNet~\citep{Miller95,fellbaum1998wordnet} is arguably one of the impactful resource used in NLP community. The resource is optimized for lexical categorization. 
% It contains (mostly) nouns, verbs, adjectives and adverbs\footnote{It ignores determiners, prepositions, pronouns, conjunctions, and particles.}, labeled with `sense' classes.  
% Meaning in Wordnet is defined through synsets, which are the set of synonyms. In addition, the elements are linked with small set of semantic relations, e.g. `is-a', synonym, hyponym, etc. For example here, the hierarchy of hypernyms  of {\tt happiness} is shown bellow: 

% \begin{framed}
% \begin{verbatim}
% abstraction 
%   => attribute 
%     => state 
%       => feeling 
%         => emotion 
%           => spirit 
%             => emotional_state
%               => happiness 
% \end{verbatim}
% \end{framed}


% \todo{this paragraph could be simplified}
% Another issue is the ``binding" of variables, which has a close connection to the ``systematicity" issue raised by Fodor and Pylyshyn \todo{year?}. Binding is the act of representing conjunctions of properties. A property can be anything being sensed, for example: color, shape, orientation, etc. To visually detect a red circle, among a blue circle and a blue rectangle, one must visually bind each object's color to its shape \cite{treisman1980feature}.  Similarly, one can imagine \textit{thematic roles} for groups of words in sentences which binds them together \cite{fodor1983modularity}. For example, in order to understand the statement, ``Jack feels Kate is angry" one must bind ``Jack" to the agent role of ``feels". Binding is the backbone of symbolic representation. The real world is full of concepts with complex combinations of properties which require efficient dynamic binding mechanisms in order to generate representations of perceptual objects and movements. However it is not obvious how to do dynamic binding in a mathematical framework. One of the popular trends following neuroscientists' observations of the human body \cite{gray1989stimulus}, is the binding base on \textit{temporal synchrony} of the connected units: if two units are bound, then they fire synchronously; otherwise they fire asynchronously. 
%Some researches suggest that the human visual system uses both static and dynamic codes for binding in the representation of object shape, and these separate codes manifest themselves, among other ways, as differing patterns of priming for attended and ignored object images.
% \todo{common sense and bringing knowledge from the outside}

\subsection{Common sense and implied meanings}
A major portion of our language understanding is only implied in language and not explicitly mention (examples in  Section~\ref{intro:challenges:nlu}). 
This difficulty of this challenge has historically been under-estimated. 
Early AI, during the sixties and onward, experienced a lot of interest in modeling common sense knowledge. McCarthy, one of the founders of AI, believed in formal logic as a solution to common sense reasoning~\citep{McCarthyLi90}. 
\cite{Minsky88} estimated that ``... commonsense is knowing maybe 30 or 60 million things about the world and having them represented so that when something happens, you can make analogies with others". There have been decade-long efforts to create knowledge bases of common sense information, such as Cyc~\citep{Lenat95} and ConceptNet~\citep{LiuSi04}, but none of these have yielded any major impact so far. 
% been shown to be a good solution to NLP problems, at least to a reasonable extent.
A roadblock in progress towards such goals is the lack of \emph{natural end-tasks} that can provide an objective measure of progress in the field. 
To facilitate research in this direction, in Chapter 6 we provide a new natural language QA dataset that performing well on it requires significant progress on multiple \emph{temporal} common sense tasks.


% There are works focusing on elementary-school level story comprehension, which is full  of commonsense facts (for example, \newcite{charniak1972toward} and \newcite{dejong1979skimming}). Unfortunately many of such efforts were tested on very limited problems, like the Block World problem. There have been famous decade-long efforts to create knowledge bases which contain commonsense, such as Cyc \cite{Lenat95} and ConceptNet \cite{LiuSi04} (explained in the last section), but none of these have been shown to be a good solution to NLP problems, at least to a reasonable extent. 
% In 80's Cyc~\citep{lenat1985cyc} started off with the goal of compiling a large collection of common sense knowledge-base. The project is still active, despite not having any significant industrial impact so far. 


\subsection{Abstractions of the representations}
\emph{Abstraction} of information is one of the key issues in any effort towards an effective representation. 
Having coarser abstraction could result in better generalization. However, too much abstraction could result in losing potentially-useful details. 
In general, there is a trade-off between the expressive level of the representation and the reasoning complexity. 
We also deal with this issue in multiple ways: (i) we use unsupervised representations that have been shown to indirectly capture  abstractions~\citep{MahabalRoMi18}. 
(ii) we use systems pre-trained with annotations that abstract over raw text; for example, in Chapter 4 we use semantic roles representations of sentences, which abstract over low-level words and map the argument into their high-level thematic roles. 


For a given problem instance, how does a system internally choose the right level of abstraction?
The human attention structure is extremely good in abstracting concepts~\citep{JohnsonPr04,JanzenVi97}, although automating this is an open question. 
% finding out what are the right abstraction for answering each question, but for computers, it might need a further pre-processing on the question to decide where to look for information. The issue of accessing knowledge goes beyond abstraction levels; in general it can be about accessing multiple knowledge bases, possibly with contradictions, etc. 
One way of dealing with such issues is 
% A few works in the fields have given a partial answer to this by 
to use multiple levels of abstraction and let the reasoning algorithm use the right level of abstraction when available~\citep{Rasmussen85,BisantzVi94}. 
In Chapter 4, we take a similar approach by using a collection of different abstractions.
% A few past works have the effectiveness of using multi
% Since many levels of abstraction might be necessary for reasoning, it might be a good idea to model an environment at multiple levels of abstraction
% \citep{Rasmussen85,BisantzVi94}. 
% Such hierarchical abstract can be modeled in various ways, 1st-order logic, frames, semantic graphs, etc, and the properties are inherited from parent nodes to more refined nodes (for example work with frames \cite{bobrow1977overview}). \todo{mind the transition} One issue with the default pass of properties to children is how model exceptions. For example, if  any ``bird" can ``fly", any entity of type ``bird" will inherit the ``fly" property. What is the right way handle the exception that ``chicken" does not fly?




\section{Reasoning/Decision-making Paradigms for NLU}
\label{sec:related:reasoning}
\subsection{Early formalisms of reasoning}
The idea of automated reasoning dates back before AI itself and can be traced to ancient Greece. Aristotle's syllogisms paved the way for \emph{deductive} reasoning formalism. It continued its way with philosophers like Al-Kindi, Al-Farabi, and Avicenna~\citep{Davidson92}, before culminating as the modern mathematics and logic. 
% are often seen as the first example of a formalisation of valid reasoning.
% With the separation of mind and body in the 17th century by Descartes, and in common sense, the road was opened up to apply newly found mathematical insights to model and
% imitate parts of human thought as mechanistic processes. 
% Perhaps the most appealing examples are Pascal’s arithmetic machine for addition and subtraction, and Leibniz’ improvements to it to support multiplication, division and computing the square root
% Innovations by pioneering 
% {
% \color{red}
% Some issues are far more foundational in AI, like authors who have claimed that human-level reasoning is not achievable via purely computational means; e.g. \citep{dreyfus1992computers,searle1980minds,boden1996philosophy}. 

% Automated reasoning, especially within the context of natural language at the problems, is arguably one of the major problems in contemporary AI research. 
Within AI research, \cite{McCarthy63} pioneered the use of logic for automating reasoning for language problems, which over time branched into other classes of reasoning~\citep{HHNT89,EvansNeBy93}.  
% In modern philosophy, the earlier notions were mixed with mathematical logic, resulting in formal theories of reasoning, 
% such as deductive~\citep{EvansNeBy93}, inductive~\citep{HHNT89}, etc.

A closely related reasoning to what we study here is \emph{abduction}~\citep{Peirce83,HSAM93}, which is the process of finding \textit{the best minimal explanation} from a set of observations (see Figure~\ref{fig:abduction:example}). 
% Abductive reasoning starts with an observation then seeks to find the simplest and most likely explanation. 
Unlike in deductive reasoning, in abductive reasoning the premises do not guarantee the conclusion. 
% One can understand abductive reasoning as inference to the best explanation, although not all uses of the terms abduction and inference to the best explanation are exactly equivalent
Informally speaking, abduction is inferring cause from effect (reverse direction from deductive reasoning). The two reasoning systems in Chapter 3 and 4 can be interpreted as abductive systems. 
%Abduction is widely used in finding explanations for events and actions of agents, scientific theory formulation, medical diagnosis etc. 
%For example, in plan recognition, actions are observed and the underlying plan that the agent is executing is abduced.

We define the notation to make the exposition slightly more formal. 
Let $\vdash$ denote entailment and $\bot$ denote contradiction. Formally, (logical) abductive reasoning is defined as follows:
\begin{framed}
\noindent Given background knowledge $B$ and observations $O$, find a hypothesis $H$, 
%also a set of logical formulae, 
such that $B \cup H \nvdash \bot$ (consistency with the given background) and $B \cup H \vdash O$ (explaining the observations).
\end{framed}

\begin{figure}
    \centering
    \includegraphics[scale=0.5,trim=0cm 0cm 0cm 0cm]{figures_background/abduction_example.png}
    \caption{Brief definitions for popular reasoning classes and their examples.}
    \label{fig:abduction:example}
\end{figure}

% In real problems,  
% Despite being intuitive, when it comes to practice, 
In practical settings,  
this purely logical definition has many limitations: (a) There could be multiple hypotheses $H$ that explain a particular set of observations given the background knowledge. The best hypothesis has to be selected based on some measure of goodness and the simplicity of the hypothesis (Occam's Razor). (b) Real life has many uncertain elements, i.e. there are degrees of certainties (rather than binary assignments) associated with observations and background knowledge. Hence the decision of consistency and explainability has to be done with respect to this fuzzy measure. (c) The inference problem in its general form is computationally intractable; often assumptions have to be made to have tractable inference (e.g., restricting the representation to Horn clauses). 


% From a pragmatic perspective, natural language understanding
% (NLU) can be thought of as first-order abduction [Hobbs
% et al., 1993; Ovchinnikova et al., 2014]. The sentence we
% want to interpret is what is “observed” and the “best” abductive
% proof tells us what the sentence actually means. Abductive
% reasoning is ampliative, that is, what we conclude cannot
% be proved deductively, but it extends our background knowledge
% in a coherent way.

% Abduction is intractable (cf. [Appelt and Pollack, 1992],
% “even in the case of propositional Horn clause theories, the
% problem of computing an explanation for an arbitrary proposition
% is NP hard”). Propositional abduction is known to
% be implementable as stable model enumeration [Gelfond and
% Kahl, 2014] but in the case of NLU the underlying theory
% is first-order. 

% In early experiments with interpretation as
% (weighted, i.e., cost-based) abduction, a Prolog-based abductive
% theorem prover was used [Hobbs et al., 1993]

%  Later
% a more efficient algorithm based on integer linear programming
% was developed [Inoue et al., 2012; Ovchinnikova et al.,
% 2014]. But neither approach allows for seamless integration
% of abduction with full-fledged deduction. In this contribution
% we present a method for comparatively efficient first-order
% abduction based on answer-set solving. We use the solver
% described in [Gebser et al., 2012].

%In some formalisms, a set of predicates are declared by the user as abducibles [Kakas et al., 1993], which are the only predicates that can be used in assumptions.
%Several first-order logic based approaches to abduction have been developed [Poole et al., 1987; Stickel, 1988; Ng and Mooney, 1991; Kakas et al., 1993]. 
%These approaches perform first-order logical reasoning to determine the set of assumptions sufficient to deduce the observations. 
%Their search is heuristically guided in accordance with the goodness criteria desired of the set of assumptions. 
%In many real-world applications, clauses in the provided background knowledge may be true in most cases but sometimes violated. 
% Therefore, it may be desirable to choose an explanation even though it violates some uncertain clauses in the background knowledge but is otherwise a very good explanation. 
%However, in purely logical approaches to abduction, such an explanation is ruled out because it contradicts the background knowledge. 
%A probabilistic form of abduction is needed in order to account for uncertainty in the background knowledge and to handle noisy and incomplete observations.

% \todo{talk about uncertainty}
% Later on, effort shifted towards a softer notion of symbols, by incorporating uncertainty into symbolic models~\cite{Zadeh75,Pearl1989ProbabilisticRI,SelmanLe90}. 
% The uncertainty of real problems~\cite{schutze1996ambiguity} pushed for development of systems which rely on relative truths. This resulted in theories like fuzzy-logic~\cite{Zadeh75}, or probabilistic Bayesian networks~\cite{Neapolitan1990ProbabilisticRI,Dechter2013ReasoningWP}, default reasoning~\cite{HSME88,SelmanLe90,Poole90}. 
% , and the theory of PAC-learning~\cite{valiatnt1984theory}. 
% approximate learning of concepts with probabilistic guarantees 
% In this work we disregard the issue of uncertainty and focus on the scenarios where the correct (but hidden) decision is certain. 

% Dealing with 
\subsection{Incorporating ``uncertainty'' in reasoning}
Over the years, a wide variety of \textit{soft} alternatives have emerged for reasoning algorithms, by incorporating uncertainty into symbolic models. 
 This resulted in theories like fuzzy-logic~\citep{Zadeh75}, or probabilistic Bayesian networks~\citep{Pearl88,Dechter13}, soft abduction~\citep{HSME88,SelmanLe90,Poole90}. 
% There are many \textit{soft} alternatives of abductive reasoning. % A popular soft alternative framework for abduction is based on
In Bayesian networks, the (uncertain) background knowledge is encoded in a graphical structure and upon receiving observations, the probabilistic explanation is derived by maximizing a posterior probability distribution. These models are essentially based on propositional logic and cannot handle quantifiers~\citep{KateMo09}. 
% , hence preventing their use in situations that involve an unbounded number of entities with a variety of relations between them~\citep{KateMo09}.
%In these networks, the background knowledge with its uncertainties is encoded in a directed graph. 
%Then, given a set of observations, probabilistic inference over the graph structure is done to compute the posterior probability of alternative explanations. 
%However, a major limitation of Bayesian networks is that they are essentially based on propositional logic and cannot handle structured representations, hence preventing their use in situations that involve an unbounded number of entities with a variety of relations between them.
Weighted abduction combines the weights of relevance/plausibility  with first-order logic rules~\citep{HSME88}. 
% is an alternative proposal to incorporate relevance and plausibility for the assumptions. 
However, unlike probability theoretic frameworks, their weighting scheme does not have any solid theoretical basis and does not lend itself to a complete probabilistic analysis. Our framework in Chapter 3,4 is also a way to perform abductive reasoning under uncertainty. Our proposal is different from the previous models in a few ways:  (i) Unlike Bayesian network our framework is not limited to propositional rules; in fact, there are first-order relations used in the design of \tableilp\ (more details in Chapter 3). 
% (ii) The uncertainty is not explicitly limited to probability theory. While making it easier to perform inference, it is hard to interpret the overall uncertainty score or provide provable statements. 
(ii) unlike many other previous works, we do not make representational assumptions to make the inference simpler (like limiting to Horn clauses, or certain independence assumptions). In fact, the inference might be NP-hard, but with the existence of industrial ILP solvers this is not an issue in practice. 
Our work is inspired by a prior line of work on inference on structured representations to reason on (and with) language; see \cite{CRRR08,CGRS10,ChangRaRo12}, among others.



\subsection{Macro-reading vs micro-reading}
With increased availability of  information (especially through the internet) \textbf{macro-reading} systems have emerged with the aim of leveraging 
% Depending on the perspective towards the goal of QA, there are different approaches to design of systems~\cite{MBCHW09}. 
% \textbf{Macro-reading} aims to find answers of questions from 
a large variety of resources and exploiting the redundancy of information~\citep{MBCHW09}. Even if a system does not understand one text, there might be many other texts that convey a similar meaning. Such systems derive significant leverage from relatively shallow statistical methods with surprisingly strong performance~\citep{CEKSTTK16}. 
Today's Internet search engines, for instance, can successfully retrieve \emph{factoid} style answers to many natural language queries by efficiently searching the Web. Information Retrieval (IR) systems work under the assumption that answers to many questions of interest are often explicitly stated somewhere~\citep{KwokEtWe01}, and all one needs, in principle, is access to a sufficiently large corpus. Similarly, statistical correlation based methods, such as those using Pointwise Mutual Information or PMI~\citep{ChurchHa89}, work under the assumption that many questions can be answered by looking for words that tend to co-occur with the question words in a large corpus.
% Many QA systems in such domains derive significant leverage from relatively shallow Information Retrieval (IR) and statistical correlation techniques operating on large unstructured corpora~\citep{KwokEtWe01,CEKSTTK16}.
While both of these approaches help identify correct answers, they
are not suitable for questions requiring language understanding and reasoning, such as chaining together multiple facts in order to arrive at a conclusion. 
% Arguably, such reasoning is a cornerstone of human intelligence, and is a key ability evaluated by standardized science exams given to students.
On the other hand, \textbf{micro-reading} aims at \emph{understanding} a piece of evidence given to the system, without reliance of \emph{redundancy}. The focus of this thesis is \emph{micro-reading} as it directly addresses NLU; that being said, whenever possible, we use macro-reading systems as our baselines. 


\subsection{Reasoning on ``structured'' representations}
With increasing knowledge resources and diversity of the available knowledge representations, 
% In parallel, there are 
numerous QA systems are developed to operate over large-scale \textit{explicit} knowledge representations. These approaches perform reasoning over \textit{structured} (discrete) abstractions. For instance, \cite{CGRS10} address RTE (and other tasks) via inference on structured representations), 
% \cite{KhotSaCl17} use Open IE subject-verb-object relations~\citep{BCSBE07}, 
\cite{BBCGGHKPS13} use AMR annotators~\citep{WXPP15}, 
\cite{UBLNGC12} use RDF knowledge~\citep{YZWYW17}, 
 \cite{ZettlemoyerCo05,CGCR10,GoldwasserRo14,KrishnamurthyTaKe16}  
use semantic parsers to answer a given question, and \cite{DoChRo11,DoLuRo12} employ constrained inference for temporal/causal reasoning. 
The framework we study in Chapter 3 is a reasoning algorithm functioning over  tabular knowledge (frames) of basic science concepts. 
% using executable formulas~\cite{RTPSL17,AngeliMa14}
% Majority of the existing work in QA, specially the ones claim to do structured reasoning have to make strong assumptions on how the input knowledge is represented. System introduced in \cite{UBLNGC12} needs RDF knowledge, \cite{YZWYW17} requires knowledge graphs, and so on. 
% \todo{mention chapter 4 here }
% Curating the input knowledge for many of these systems is often a costly process. 
% On other hand, some QA systems work on a knowledge representation which can be extracted in an automated way, making them them more extensible. 

% \todo{use this to explain chapter 4:}
% Unlike such works, our systems combines different layers of annotations, including the raw-text itself, to form a reasoning problem. The use of diverse set of knowledge representations, lets our system to be more robust to possible losses that annotators might have on certain inputs or domains.

% \todo{mention khot'16 in macroreading:}
% Recently proposed by \cite{KhotSaCl17}, this is a state-of-the-art system designed for science questions. It uses Open IE~\citep{BCSBE07} tuples derived from the text as the knowledge representation, and performs reasoning over it via an ILP. It has access to a large knowledge base of Open IE tuples, and exploits redundancy to overcome challenges introduced by noise and linguistic variability.



% chaining information 
% \todo{use this to motivate multi-hop}
An important limitation of IR-based systems is their inability to connect distant pieces of information together. 
% In factoid QA tasks this is not an issue, since the answers to many questions are repeated in many places in different forms. 
However, many other realistic domains (such as science questions or biology articles) have answers that are not explicitly stated in text, and instead require combining facts together. 
% A generation of recent systems developed to address this issue under the label of \textit{mutli-hop} reasoning\footnote{}
\cite{KhotSaCl17} creates an inference system capable of combining Open IE tuples~\citep{BCSBE07}. \cite{JSSC17} propose reasoning by aggregating sentential information from multiple knowledge bases. \cite{SCMN13,MNDB17} propose frameworks for chaining relations to infer new (unseen) relations. Our work in Chapter 3 creates chaining of information over multiple tables. The reasoning framework in Chapter 4 investigates reasoning over multiple peaces of raw text. The QA dataset in Chapter 5 we propose also encourages the use of information from different segments of the story. Chapter 8 proposes a formalism to study limits of chaining long-range information. 


% While in our formalism, we also propose way to chain information together, our system works with multiple knowledge representations. \todo{make it refer to the chapter:} \cite{tableilp2016:ijcai} propose a solution for this by creating alignment rules between cells, rows, columns of different knowledge tables.  
% \cite{JSSC17} shows that while this strategy improves over baselines with no reasoning (showing the effectiveness of reasoning), with aggregation of more than 2-3 sentences the quality declines (showing a limitation for reasoning).
% Our analysis covers any algorithm for inferring patterns that can be formulated in graph-based knowledge, e.g.,  
% In our work we study a special family of algorithms where the discovery of the event of interest can be formulated as a 
% chaining local information, often referred to as \emph{multihop} reasoning~\cite{JBSC16,JWMM18,LinRX2018:MultiHopKG}. 

% Our work is inspired by empirical observations of ``semantic drift'' of reasoning algorithms, as the number of hops is increased. There are series of works sharing this empirical observation; for example, \namecite{FJHSC15} show modest benefits up to 2-3 hops, and then decreasing performance; \namecite{Jansen16,JWMM18} made similar observations in graphs built out of larger structures such as sentences, where the performance drops off around 2 hops. This pattern has interestingly been observed in a number of results with a variety of representations, including word-level representations, graphs, and traversal methods. 
% The question we are after in this work is whether the field might be hitting a fundamental limit on multi-hop information aggregation using existing methods and noisy knowledge sources.

% Our ``impossibility'' results are reaffirmations of the empirical intuition in the field. This means that multi-hop inference (and any algorithm that can be cast in that form), as we've been approaching it, is exceptionally unlikely to breach the few-hop barrier predicted in our analysis. 

% }

\begin{comment}
Similarly on the representation level, there are many issues that still are subject to debate. For example, \textit{the frame problem} \citep{mccarthy1968some} in logical representation, which is the need for a compact way of expressing states which do not change in an environment as a result of some actions. For example, coloring a table, definitely does not change its position but when using classical logical reasoning, the independence between `color' property and `location' property needs to be explicitly encoded. Rather than encoding exceptions in the knowledge base, there has been proposals in the form of non-monotonic reasoning for the frame problem. In nonmonotonic reasoning it is possible to jump to a conclusion and retract some of the conclusions previously made, as further information becomes available (which is the reason for being called \textit{nonmonotonic}). 

%Thus, as the set of premises and input information grows, the set of conclusions may shrink.
%Nonmonotonic logics are used to formalize plausible reasoning. 
%They allow more general reasoning than standard logics, which deal with universal statements. 
%For example, standard logics can easily represent the argument:
%-All men are mortal
%-Socrates is a man
%Therefore, Socrates is mortal
%but cannot represent reasoning such as:
%-Birds typically fly
%-Tweety is a bird
%Therefore, Tweety (presumably) flies
%Such arguments are characteristic of commonsense reasoning, where default rules and the absence of complete information are prevalent.
Despite the initial promise of the nonmonotonic reasoning methods, many of such reasoning frameworks suffered from the issue of consistency, i.e. ensuring that conclusions drawn are consistent with one another and with the assumptions. 
% but also none of these have been fully satisfactory. 
Some other works group properties into independent categories to encode causal independence of actions on properties; for example grouping properties with temporal and spatial boundaries~\cite{Hayes:phyriscsManifesto}.


An early work that created a separate representation of the knowledge from the solver engine was the General Problem Solver (GPS) system of \cite{newell1961gps}. This system was intended to be a universal solver for any problem formalized in \textit{symbolic} form, like chess playing or theorem proving. The idea of symbolic reasoning was developed centuries earlier by Descartes, Pascal, Leibniz and some other pioneers in philosophy of mind. The use of \textit{symbols} as the fundamental elements of the representation---the \textit{physical symbol system hypothesis}~\citep{newell1961gps}---has widely been debated. 
% is a debatable assumption which has continued its way until now. 
\todo{emphasize universl}
Scalability was a big issue for GPS, due to 
% After the early scalablity issues of GPS, it soon became clear that a system designed for solving any formalized problem is impractical due to the 
combinatorial explosion of intermediate states in many problems. 
% Also, it became apparent  that 


\todo{mention that we skip the repeated  content}
Since the issue of reasoning is directly connected to the representation, we, to the most part, skip the notable works were mentioned in the previous section. 
\end{comment}


\subsection{Models utilizing massive annotated data}
A  highlight over the past two decades is the advent of statistical techniques into NLP~\citep{HLBB99}. Since then, a wide variety of supervised-learning algorithms have shown strong performances on different datasets. 


The increasingly large amount of data available for recent benchmarks make it possible to train neural models (see ``Connectionism''; Section~\ref{sec:connectionism})~\citep{SKFH16,PTDU16,WYW18,LSDG18,HPHXWZ2018}.
%  More recently, the field has seen increased activity on neural architectures on a couple of popular reading comprehension datasets  . 
Moreover, an additional technical shift was using distributional representation of words (word vectors or embeddings) extracted from large-scale text corpora~\citep{MCCD13,PenningtonSoMa14} (see Section~\ref{sec:representations:intro}). 

Despite all the decade-long excited about supervised-learning algorithms, the main progress, especially in the past few years, has mostly been due to the re-emergence of \emph{unsupervised} representations~\citep{PNIGCLZ18,DCLT18}.\footnote{\emph{Unsupervised} in the sense that they are constructed with freely available data, as opposed to task-specific annotated data. } 


\section{Technical background and notation}
\label{sec:background:notation:technical}
In this section, we provide the relevant mathematical background used throughout this thesis. We cover three main areas used widely across this document. 

\subsection{Complexity theory}
% We use common terms and notations from complexity theory. 
We follow the standard notation for asymptotic comparison of functions: 
$O(.), o(.), \Theta(.), \Omega(.),$ and $\omega(.)$~\citep{CLRS09}.


We use \emph{P} and \emph{NP} to refer to the basic complexity classes. We briefly review these classes: \emph{P} consists of all problems that can be solved efficiently (in polynomial time). \emph{NP} (non-deterministic polynomial time) includes all problems that given a solution, one can efficiently \emph{verify} the solution.   
When a problem is called \emph{intractable}, it refers to its complexity class being at least \emph{NP}-hard. 
% \emph{NP}-hard is a class of problems that are at least as hard as the hardest problem in \emph{NP}-complete~\citep{karp1972reducibility}.  


\subsection{Probability Theory}
\label{background:probability:theory}
% \paragraph{Probability Theory.}
$X \sim f(\theta)$ denotes a random variable $X$ distributed according to probability distribution $f(\theta)$, paramterized by $\theta$. The mean and variance of $X$ are denoted as 
$\mathbb{E}_{X \sim f(\theta)}[X]$ and $\mathbb{V}[X]$, resp.
$\bern{p}$ and $\bin{n,p}$ denote the Bernoulli and Binomial distributions, resp.

\subsection{Graph theory}
\label{sec:graph:theory}
We denote an undirected graph with $G(V, E)$ where $V$ and $E$ are the sets of nodes and edges, resp. We use the notations $V_G$ and $E_G$ to  refer to the nodes and edges of a graph $G$, respectively. 

A \emph{subgraph} of a graph $G$ is another graph formed from a subset of the vertices and edges of $G$. The vertex subset must include all endpoints of the edge subset, but may also include additional vertices. 
% A spanning subgraph is one that includes all vertices of the graph; an induced subgraph is one that includes all the edges whose endpoints belong to the vertex subset.

A \emph{cut} $C = (S,T)$ in $G$ is a partition of the nodes $V$ into subsets $S$ and $T$. The \emph{size} of the cut $C$ is the number of edges in $E$ with one endpoint in $S$ and the other in $T$.

% \todo{subgraph selection}

\subsection{Optimization Theory}
\label{sec:optimization:background}

As it is widely known an ILP can be written as the following: 
\begin{align}
& \text{maximize}   \hspace{-3cm} & \mathbf{w}^\mathrm{T} \mathbf{x} &  \label{eq:ilp:obj}\\
& \text{subject to} \hspace{-3cm} & A \mathbf{x} \le \mathbf{b}, & \label{eq:ilp:cons} \\
& \text{and} \hspace{-3cm} & \mathbf{x} \in \mathbb{Z}^n. & \label{eq:ilp:ints}
\end{align}
We first introduce the basic variables, and define the full definition of the ILP program: define the weights in the objective function ($\mathbf{w}$ in Equation \ref{eq:ilp:obj}), and the constraints ($A$ and $\mathbf{b}$ in Equation \ref{eq:ilp:cons}).

This formulation is incredibly powerful and has been used for many  problems. In the context of NLP problems, ILP based discrete optimization was introduced by \citet{RothYi04} and has been successfully  used~\citep{CGRS10,BerantDaGo10,SrikumarRo11,GoldwasserRo14}. 
In Chapter 3 and 4 also, we formalize our desired behavior as an optimization problem. 

This optimization problem with integrality constraint and its general form, is an NP-hard problem. That being said, the industrial solvers (which use cutting-plane and other heuristics) are quite fast across a wide variety of problems. 
% Integer programming is NP-complete. In particular, the special case of 0-1 integer linear programming


% \todo{subgraph selection as optimization}
% \todo{ilp optimization}
% \todo{approximation theory: relaxations}
% \todo{mention the use of solvers}
% \todo{auxilary variables .... }


==> Daniel K - thesis - dissertation/1.tableilp_new.tex <==
\chapter{QA as Subgraph Optimization on Tabular Knowledge}
\label{chapter:tableilp}
\epigraph{ 
``The techniques of artificial intelligence are to the mind what bureaucracy is to human social interaction.''
}{--- \textup{Terry Winograd}, Thinking Machines: Can there be? 1991}


\newif\ifarxiv

\arxivtrue

%%%%%%%%%%%%%% INTRODUCTION %%%%%%%%%%%%%%
\section{Overview}
\label{sec:intro}


Consider a question from the NY Regents 4th Grade Science Test:\footnote{This chapter is based on the following publication: \cite{KKSCER16}.}
\begin{myquote}
{In New York State, the longest period of daylight occurs during which month? \ \\ (A) June \ (B) March \ (C) December \ (D) September}
\end{myquote}

\noindent
We would like a QA system that, even if the answer is not explicitly stated in a document, can \emph{combine basic scientific and geographic facts} to answer the question, e.g., New York is in the north hemisphere; the longest day occurs during the summer solstice; and the summer solstice in the north hemisphere occurs in June (hence the answer is June). Figure~\ref{fig:ny-example:tableilp} illustrates how our system approaches this, with the highlighted support graph representing its line of reasoning.

% \begin{enumerate}
% \item Longest daylight corresponds to summer solstice.
% \item New York is in the United States.
% \item United States is in the northern hemisphere.
% \item Summer solstice in the northern hemisphere happens in the month of June.
% \end{enumerate}

\begin{wrapfigure}{r}{0.69\textwidth}
% \begin{figure}[tb]
\centering
%\includegraphics[width=0.48\textwidth]{figures_tableilp/ny-example}
%\begin{framed}
\includegraphics[trim=2.2cm 18.4cm 1cm 2.5001cm, clip=true, scale=0.76]{figures_tableilp/alignment7-7.pdf}
%\end{framed}
%\vspace{-0.25in}
\caption{
\footnotesize
\tableilp\ searches for the best support graph (chains of reasoning)
%, shown with red and implicitly used green elements) 
connecting the question to an answer, in this case June.
%\ashish{seemed like too much detail at this point. simplified.}
%Red cells and edges denote active unary and pairwise elements in the support graph, respectively. Green nodes/edges are not part of the support graph, although they are used in its calculation. 
Constraints on the graph define what constitutes valid support and how to score it (Section~\ref{subsec:ilp:tableilp}).} 
\label{fig:ny-example:tableilp}
% \end{figure}
\end{wrapfigure}
Further, we would like the system to be \emph{robust under simple perturbations}, such as changing New York to New Zealand (in the southern hemisphere) or changing an incorrect answer option to an irrelevant word such as ``last'' that happens to have high co-occurrence with the question text.


To this end, we propose a structured reasoning system, called \tableilp,
%(QUestion-answering via Integer Programming),
%\ashish{better name?? TILP / TIP / QUIP / QAILP / QUAIL / ...}, 
that operates over a semi-structured knowledge base derived from text and answers questions by chaining multiple pieces of information and combining parallel evidence.\footnote{{A preliminary version of our ILP model was used in the ensemble solver of \cite{CEKSTTK16}. We build upon this earlier ILP formulation, providing further details and incorporating additional syntactic and semantic constraints that improve the score by 17.7\%.}}
The knowledge base consists of \emph{tables}, each of which is a collection of instances of an $n$-ary relation defined over natural language phrases. E.g., as illustrated in Figure~\ref{fig:ny-example:tableilp}, a simple table with schema \emph{(country, hemisphere)} might contain the instance \emph{(United States, Northern)} while a ternary table with schema \emph{(hemisphere, orbital event, month)} might contain \emph{(North, Summer Solstice, June)}. \tableilp\ treats lexical constituents of the question $Q$, as well as cells of potentially relevant tables $T$, as nodes in a large graph $\mathcal{G}_{Q,T}$, and attempts to find a subgraph $G$ of $\mathcal{G}_{Q,T}$ that ``best'' supports an answer option. The notion of best support is captured via a number of structural and semantic constraints and preferences, which are conveniently expressed in the Integer Linear Programming (ILP) formalism. We then use an off-the-shelf ILP optimization engine called SCIP~\citep{Achterberg09} to determine the best supported answer for $Q$.

Following a recently proposed AI challenge~\citep{Clark15}, {we evaluate \tableilp\ on unseen elementary-school science questions from standardized tests. Specifically, we consider a challenge set \citep{CEKSTTK16} consisting of all non-diagram multiple choice questions from 6 years of NY Regents 4th grade science exams.}
%, an expanded version of the dataset used by \cite{KBGSCE15}. 
In contrast to a state-of-the-art structured inference method~\citep{KBGSCE15} for this task, which used Markov Logic Networks (MLNs)~\citep{RichardsonDo06}, \tableilp\ achieves a significantly (+14\% absolute) higher test score. 
%
This suggests that a combination of a rich and fine-grained constraint language, namely ILP,
even with a publicly available solver
%with an industrial strength solver
is more effective in practice than various MLN formulations of the task. Further, while the scalability of the MLN formulations %explored by \cite{KBGSCE15} 
 was limited to very few (typically one or two) selected science rules at a time, our approach easily scales to hundreds of relevant scientific facts.
% \dan{This reads as if the only issue is computational power, but it really has to do with the formulation and with propsitionalization, right? Maybe worth a clarification sentence, either here or when discussing it in the eperimental section.} \ashish{agreed! will do}  
%
It also complements the kind of questions amenable to IR and PMI techniques, as is evidenced by the fact that a combination (trained using simple Logistic Regression {\citep{CEKSTTK16}}) of \tableilp\ with IR and PMI results in a significant (+10\% absolute) boost in the score compared to IR alone.

Our ablation study suggests that
%\daniel{Better adjective?: say ``chaining facts for reasoning'', ``reasoning on top of facts'', ``reasoning by joining facts'' or just ``reasoning'' instead of ``non-trivial reasoning''}
%\ashish{good suggestion!}
combining facts from multiple tables or multiple rows within a table plays an important role in \tableilp's performance. 
We also show that \tableilp\ benefits from the table structure, by comparing it with an IR system using the same knowledge (the table rows) but expressed as simple sentences; \tableilp\ scores significantly (+10\%) higher. Finally, we demonstrate that our approach is robust to a simple perturbation of incorrect answer options: while the simple perturbation results in a relative drop of 20\% and 33\% in the performance of IR and PMI methods, respectively, it affects \tableilp's performance by only 12\%.

%%%%%%%%%%%%%% RELATED WORK %%%%%%%%%%%%%%

\section{Related Work}
\label{sec:related-work}
In this section, we provide additional related work, and augment our review related work provided in Section~\ref{sec:intro:qa:review}. 

{\cite{CEKSTTK16} proposed an ensemble approach for the science QA task, demonstrating the effectiveness of a combination of information retrieval, statistical association, rule-based reasoning, and an ILP solver operating on semi-structured knowledge. Our ILP system extends their model with additional constraints and preferences (e.g., semantic relation matching), substantially improving QA performance.}

A number of systems have been developed for answering factoid questions with short answers (e.g., ``What is the capital of France?'') using document collections or databases (e.g., Freebase~\citep{BEPST08}, NELL~\citep{CBKSJM10}), for example~\citep{BrillDuBa02,FaderZeEt14,FBCFGKLMNPo10,KoNySi07,YihHeMe14,YaoDu14,ZHWYHZ14}. However, many science questions have answers that are not explicitly stated in text, and instead require combining information together. Conversely, while there are AI systems for formal scientific reasoning (e.g., \citep{GCCBCG10,Novak77}), they require questions to be posed in logic or restricted English.
%rather than in natural language. 
Our goal here is a system that operates between these two extremes, able to combine information while still operating with natural language.


There is a relatively rich literature in the databases community, on executing different commands on the tablular content (e.g., searching, joining, etc) via a user commands issued by a semi-novice user~\cite{TJMCIPG08,TalukdarIvPe10}. 
A major distinguishing perspective is that 
% factor between the two problem is that, 
in our problem the queries are generated completely independent of the the table content. However, in a database system application, a user is at-least partially  informed of the common keywords, could observe the outputs of the queries and adjust the commands accordingly. 
% according to the output 
%  (usually keyword-based queries). 
% \cite{cohen2000:joins} studied tables with natural language text requiring soft matching, with a focus on efficiently computing the top few candidates given a database query.  In contrast, our system, given a natural language question, (implicitly) seeks to generate a query that produces the most supported answer.
% While our ILP formulation also operates on natural language text, our focus is on the use of a specific semi-structured table representation for QA.%
% \todo{mention Zack's works; Peter Jansen's works}



%%%%%%%%%%%%%% ILP APPROACH %%%%%%%%%%%%%%

\section{QA as Subgraph Optimization}

We begin with our knowledge representation formalism, followed by our treatment of QA as an optimal subgraph selection problem over such knowledge, and then briefly describe our ILP model for subgraph selection.
% ; full details of the ILP are deferred to the Appendix.

%%%%%%%%%%%%%%
\subsection{Semi-Structured Knowledge as Tables}
\label{subsec:tables}

We use semi-structured knowledge represented in the form of $n$-ary predicates over natural language text {\citep{CEKSTTK16}}. Formally, a $k$-column table in the knowledge base is a predicate $r(x_1, x_2, \ldots, x_k)$ over strings, where each string is a (typically short) natural language phrase. The column headers capture the table schema, akin to a relational database. Each row in the table corresponds to an instance of this predicate. For example, a simple country-hemisphere table represents the binary predicate $r_{\text{ctry-hems}}(c,h)$ with instances such as (Australia, Southern) and (Canada, Northern). Since table content is specified in natural language, the same entity is often represented differently in different tables, posing an additional inference challenge.

thAlthough techniques for constructing this knowledge base are outside the scope of this paper, we briefly mention them. Tables were constructed using a mixture of manual and semi-automatic techniques. First, the table schemas were manually defined based on the syllabus, study guides, and training questions. Tables were then populated both manually and semi-automatically using {IKE~\citep{DalviBhCl16}}, a table-building tool that performs interactive, bootstrapped relation extraction over a corpus of science text. In addition, to augment these tables with the broad knowledge present in study guides that doesn't always fit the manually defined table schemas, we ran an Open IE~\citep{BCSBE07} pattern-based \textit{subject-verb-object} (SVO) extractor from~\cite{CBBHKST14} over several science texts to populate three-column Open IE tables. Methods for further automating table construction are under development.
%\dan{It would be good to mention somewhere that the same entity could be represented differently in different tables, posing an additional inference challenge}\ashish{added to the previous paragraph.}

% \daniel{FYI, I haven't included a few constraints for SKIP columns. Do we want to include them? (and consequently mention ``fillers'' here?) I guess they might be necessary for relation alignment as well? } \ashish{filler/skip columns are an implementation technicality. I wouldn't mention them. For relation alignment, we can say the table schema specifies relevant relations that exist between columns (this is more general than filler columns anyway, as relation need not be among consecutive columns)}
% \daniel{Agreed with both. I suppose ``relations'' should be mention in this section; right?}
% \ashish{yes! will add it here. Where do we / should we describe Relation Matching constraints?}\tushar{They are in the long list of constraints and I have one bullet in the 3.3 list now. Should there be a small paragraph/subsection (mainly to clarify what do we mean, how do we match relations to the question, etc)?} \ashish{seems like a good idea, since we refer to it specifically later. Also, see above --- I started to write the part (relations, patterns, etc.) that comes with the table schema. May be you can fill it in?}
% \tushar{I can fill in the semantic relations here and create a subsection in 3.3. Maybe we can cluster some of the other proof graph properties  into their subsections too. }
% \ashish{agreed! that's one section I haven't actually looked at much. Will make a pass over it now, especially in the light of some stuff already present in 3.2.}

%%%%%%%%%%%%%%
\subsection{QA as a Search for Desirable Support Graphs}
\label{subsec:qa-as-subgraph-selection}

We treat question answering as the task of pairing the question with an answer such that this pair has the best support in the knowledge base, measured in terms of the strength of a ``support graph'' defined as follows.

Given a multiple choice question $Q$ and tables $T$, we can define a labeled undirected 
%\daniel{``undirected'' bugs me a bit; the directionality in some edges is important for us; however you might say that it comes into play when we assign weights, not in the graph itself.} \ashish{right, in our case I do see it more of a weight computation thing rather than inherent in the graph. hmm. will rethink.}
graph $\mathcal{G}_{Q,T}$ over nodes $\mathcal{V}$ and edges $\mathcal{E}$ as follows. We first split $Q$ into lexical constituents (e.g., non-stopword tokens, or chunks) $\mathbf{q} = \{\qCons\}$ and answer options $\mathbf{a} = \{\option\}$. For each table $\tableVar$, we consider its cells $\mathbf{t} = \{\tableCell\}$ 
%\daniel{Very minor issue; change \textbf{c} to \textbf{t} so that we don't confused it with ``question constituents''?}
%\ashish{done!}
as well as column headers $\mathbf{h} = \{\header\}$. The nodes of $\mathcal{G}_{Q,T}$ are then $\mathcal{V} = \mathbf{q} \cup \mathbf{a} \cup \mathbf{t} \cup \mathbf{h}$.
% where, with some abuse of notation, with 
For presentation purposes, we will equate a graph node with the lexical entity it represents (such as a table cell or a question constituent). The undirected edges of $\mathcal{G}_{Q,T}$ are $\mathcal{E} = ((\mathbf{q} \cup \mathbf{a}) \times (\mathbf{t} \cup \mathbf{h})) \cup (\mathbf{t} \times \mathbf{t}) \cup (\mathbf{h} \times \mathbf{h})$ excluding edges both whose endpoints are within a single table.

%\peter{I added this to try and explain *why* the entailment relation is introduced}
Informally, an edge denotes (soft) equality between a question or answer node and a table node, or between two table nodes. To account for lexical variability (e.g., that \emph{tool} and \emph{instrument} are essentially equivalent) and generalization (e.g., that a \emph{dog} is an \emph{animal}), we replace string equality with a phrase-level entailment or similarity function $w : \mathcal{E} \to [0,1]$ that labels each edge $e \in \mathcal{E}$ with an associated score $w(e)$. We use entailment scores (directional) from $\mathbf{q}$ to $\mathbf{t} \cup \mathbf{h}$ and from $\mathbf{t} \cup \mathbf{h}$ to $\mathbf{a}$, and similarity scores (symmetric) between two nodes in $\mathbf{t}$.\footnote{In our evaluations, $w$ for entailment is a simple WordNet-based \citep{Miller95} function that {computes the best word-to-word alignment between phrases, scores these alignments using WordNet's hypernym and synonym relations normalized using relevant word-sense frequency, and returns the weighted sum} of the scores. $w$ for similarity is the {maximum of the entailment score in both directions}. Alternative definitions for these functions may also be used.}
In the special case of column headers across two tables, the score is (manually) set to either 0 or 1, indicating whether this corresponds to a meaningful join. 
% In order to incorporate basic lexical information in this graph, such as a \emph{dog} is an \emph{animal} or that a \emph{tool} and an \emph{instrument} are essentially equivalent, we define a function $w : \mathcal{E} \to [0,1]$ that labels each edge $e \in \mathcal{E}$ with an associated entailment or similarity score $w(e)$. We use directional entailment scores from $\mathbf{q}$ to $\mathbf{t} \cup \mathbf{h}$ and from $\mathbf{t} \cup \mathbf{h}$ to $\mathbf{a}$, and a symmetric similarity score between two nodes in $\mathbf{t}$. The score between column headers in two tables is set to either 0 or 1, indicating whether this corresponds to a meaningful join. In our evaluations, $w$ is derived from Hypernym and Synonym relations in WordNet~\citep{Miller95}, although any other lexical resource may be used.

% \peter{I don't understand the intuition behind row-augmenting subgraph. Can you explain?}\ashish{added some explanation. helpful?} \peter{yes!}
Intuitively, we would like the support graph for an answer option to be connected, and to include nodes from the question, the answer option, and at least one table. Since each table row represents a coherent piece of information but cells within a row do not have any edges in $\mathcal{G}_{Q,T}$ (the same holds also for cells and the corresponding column headers), we use the notion of an augmented subgraph to capture the underlying table structure. Let $G = (V,E)$ be a subgraph of $\mathcal{G}_{Q,T}$. The \emph{augmented subgraph} $G^+$ is formed by adding to $G$ edges $(v_1,v_2)$ such that $v_1$ and $v_2$ are in $V$ and they correspond to either the same row (possibly the header row) of a table in $T$ or to a cell and the corresponding column header.
%\daniel{I didn't quite catch why we defined augmented graph (and why it is augmented only with row variables. )}

\begin{definition}
\label{def:support-graph:tableilp}
A \emph{support graph} $G = G(Q,T,\option)$ for a question $Q$, tables $T$, and an answer option $\option$ is a subgraph $(V,E)$ of $\mathcal{G}_{Q,T}$ with the following basic properties:
%(1) $V \cap \mathbf{a} = \option$, (2) $V \cap \mathbf{q} \neq \phi$, (3) $V \cap \mathbf{t} \neq \phi$, (4) $w(e) > 0$ for all $e \in E$, (5) if $e \in E \cap (\mathbf{t} \times \mathbf{t})$ then there exists a corresponding $e' \in E \cap (\mathbf{h} \times \mathbf{h})$ involving the same columns, and (6) the row-augmented subgraph $G_r$ is connected.
\begin{enumerate}
\item $V \cap \mathbf{a} =  \lbrace \option \rbrace, \ V \cap \mathbf{q} \neq \phi, \ V \cap \mathbf{t} \neq \phi$;
\item $w(e) > 0$ for all $e \in E$;
\item if $e \in E \cap (\mathbf{t} \times \mathbf{t})$ then there exists a corresponding $e' \in E \cap (\mathbf{h} \times \mathbf{h})$ involving the same columns; and
\item the augmented subgraph $G^+$ is connected.
\end{enumerate}
\end{definition}

%\daniel{Having these bullets in the definition bug me tad bit. Here we define the ``support graph'' and later we talk about  `` the desirable support graph''. One can ask what's the point of defining ``support graph'', while we only care about the ``desirable support graph''? I suggest we keep the definition of the support graph a little informal, say by mentioning ``it shows the trace of reasoning using different elements in the problem and external knowledge''. And later we can say ``In the ILP formulation we intent to formulate and find a sensible support graph for a given question'' (hence we never talk about ``desirable support graph". )}\dan{I think it's ok to have a definition for support graphs; only say immediately after something like: A given question and a collection of tables give rise to a large number of support graphs, and the role of the inference process will be to choose the ``best" one under a definition of best developed next.}\ashish{I am with Dan on this; will add his phrasing}

A support graph thus connects the question constituents to a unique answer option through table cells and (optionally) table headers corresponding to the aligned cells. A given question and tables give rise to a large number of possible support graphs, and the role of the inference process will be to choose the ``best" one under a notion of \emph{desirable} support graphs developed next. We do this through a number of additional structural and semantic properties; the more properties the support graph satisfies, the more desirable it is.
%Our ILP formulation in the next section will make the measure of desirability or \emph{strength} of a support graph more precise.

%\daniel{I am worried that some readers might think that the whole ILP formulation is supposed to model the 4 properties mentioned earlier. However we know that the full formulation is very detailed and not easy to express in a few bullets. Maybe we can somehow say that the result of our ILP is an instance that belongs to the family of valid support graphs? In other words the space of feasible solutions for ILP program is much smaller that the space of the space of valid support graphs.}

% \tushar{Would be nice to somehow connect the proof graphs with multiple row inference, relation matching to fit the ablation study.}
% \daniel{I think these properties will/should be mentioned in the next section where we talk about ``desirable properties'' of the support graph. }\tushar{Agreed. At some point, this section was going to introduce some broad proof/support graph properties.} \ashish{Right, might revisit that tomorrow, but currently easier to leave it all in 3.3. But we should add some sentence about Relation Matching (as it appears in ablation) in 3.3. May be a bullet?}

%%%%%%%%%%%%%%
\subsection{ILP Formulation}
\label{subsec:ilp:tableilp}
We model the above support graph search for QA as an ILP optimization problem, i.e., as maximizing a linear objective function over {a finite set of}
%integer- and continuous-valued \daniel{do we want to keep it? in the default setting no continuous variables are active} 
variables, subject to a set of linear inequality constraints (see Section~\ref{sec:optimization:background} for a premier on ILP formulation). 
A summary of the model is given below.\footnote{Details of the ILP model may be found in Appendix~\ref{appendix:optimization:details:tableilp}.}	

We note that  the ILP objective and constraints aren't tied to the particular domain of evaluation; they represent general properties that capture what constitutes a well supported answer for a given question.

\begin{wrapfigure}{r}{0.6\textwidth}
% \begin{table}[tb]
\centering
\setlength\tabcolsep{5pt}
\setlength\doublerulesep{\arrayrulewidth}
\small
\setlength\extrarowheight{-7pt}
%\begin{tabular}{|c|L{40ex}|} 
\begin{tabular}{c|l}
\textsc{Element} & \multicolumn{1}{c}{\textsc{Description}} \\ 
\hline\hline
\bigstrut[t] $\tableVar$ & table $i$ \\ 
%$\tableLen$ & Number of tables \\ 
$\header $  & header of the $k$-th column of $i$-th table \\
$\tableCell $ & cell in row $j$ and column $k$ of $i$-th table \\ 
$\rowVar$ & row $j$ of $i$-th table \\ 
$\columnVar$ & column $k$ of $i$-th table \\ 
$\qCons$ & $\ell$-th lexical constituent of the question $Q$ \\
%$\qLen$ & Length of a question \\ 
$\option$ & $m$-th answer option \\ 
\hline
\end{tabular}
\makeatletter\def\@captype{table}\makeatother% "Change float to table"
\caption{Notation for the ILP formulation. }
\label{table:summary-notation}
% \end{table}
\end{wrapfigure}
Table~\ref{table:summary-notation} summarizes the notation for various elements of the problem, such as $\tableCell$ for cell $(j,k)$ of table $i$. All core variables in the ILP model are binary, i.e., have domain $\{0,1\}$. For each element, the model has a unary
%\daniel{drop ``activity'' in this sentence? And right before this sentence add ``We can a variable ``active'' if its value in our optimization problem is 1.''?}
%\ashish{dropped ``activity''; seems better to relate the variable's meaning to the support graph rather than to its value in the ILP}
variable capturing whether this element is part of the support graph $G$, i.e., it is ``active''. For instance, row $r_{ij}$ is active if at least one cell in row $j$ of table $i$ is in $G$. The model also has pairwise ``alignment'' variables, capturing edges of $\mathcal{G}_{Q,T}$. The alignment variable for an edge $e$ in $\mathcal{G}_{Q,T}$ is associated with the corresponding weight $w(e)$, and captures whether $e$ is included in $G$. To improve efficiency, we create a pairwise variable for $e$ only if $w(e)$ is larger than a certain threshold. These unary and pairwise variables are then used to define various types of constraints and preferences, as discussed next.

{ 
To make the definitions clear, we introduce the variables used in our optimization, which we will use later to define constraints explicitly. 
%Table~\ref{table:variables-and-description} summarizes our notation to refer to various elements of the problem, such as $\tableCell$ for cell $(j,k)$ of table $i$, as defined in Section 3. 
We define variables over each element by overloading $\xOne{.}$ or $\xTwo{.}{.}$ notation to refer to a binary variable on a single elements or their pair, respectively. Table~\ref{table:ilp-variables} contains the complete list of the variables, all of which are binary, i.e. they are defined on $\{0,1\}$ domain. 
The unary variables represent presence of a specific element in the support graph as a node. For example $\xOne{\tableVar} = 1$ if and only if the table $\tableVar$ is active. Similarly basic variables are defined between pairs of elements; e.g., $\xTwo{\tableCell}{\qCons}$ is a binary variable that takes value 1 if and only if the corresponding edge is present in the support graph, which can alternatively be referred to as an \emph{alignment} between cell $(j,k)$ of table $i$ and the $\ell$-th constituent of the question. 
\begin{wrapfigure}{r}{0.45\textwidth}
% \begin{table}[htb]
\centering 
\small
\setlength\extrarowheight{-16pt}
\begin{tabular}{r | L{30ex}} 
\multicolumn{2}{c}{\textsc{Basic Pairwise Activity Variables \bigstrut}} \\
\hline \hline 
$\xTwo{\tableCell}{\tableCellPrime} $ & \text{cell to cell} \\
$\xTwo{\tableCell}{\qCons} $ & cell to question constituent \\
$\xTwo{\header}{\qCons} $ & header to question constituent \\
$\xTwo{\tableCell}{\option}$ & cell to answer option \\ 
$\xTwo{\header}{\option}$ & header to answer option \\
$\xTwo{\columnVar}{\option}$ & column to answer option \\
$\xTwo{\tableVar}{\option}$ & table to answer option \\
$\xTwo{\columnVar}{\columnVarPrime}$ & column to column relation \\
\hline
\multicolumn{2}{c}{\textsc{High-level Unary Variables \bigstrut}}   \\
\hline \hline 
$\xOne{\tableVar}$ & active table \\ 
$\xOne{\rowVar}$  & active row \\
$\xOne{\columnVar} $ &  active column \\  
$\xOne{\header} $ & active column header  \\ 
$\xOne{\qCons}$ & active question constituent  \\ 
$ \xOne{\option} $ & active answer option \\ 
\hline
\end{tabular}
\makeatletter\def\@captype{table}\makeatother% "Change float to table"
\caption{Variables used for defining the optimization problem for \tableilp\ solver. All variables have domain $\{0,1\}$.
%\tushar{Do we need column to answer option and table to answer option?} \daniel{Yea these last two are used in definition of constraints. }
}
\label{table:ilp-variables}
% \end{table}
\end{wrapfigure}

As previously mentioned, in practice we do not create all possible pairwise variables. Instead we choose the pairs which have the alignment score $w(e)$ exceeding a threshold. For example we create the pairwise variables   $\xTwo{\tableCell}{\tableCellPrimePrime}$ only if the score $w(\tableCell, \tableCellPrimePrime) \geq  \textsc{MinCellCellAlignment} $. 
\ifarxiv 
\footnote{An exhaustive list of the minimum alignment thresholds for creating pairwise variables is in Table~\ref{table:pairwise-thresholds} in the appendix. }   
\else
\footnote{An exhaustive list of the minimum alignment thresholds for creating pairwise variables is in Table~10
%\ref{table:pairwise-thresholds} 
of \citep{tableilp2016:arxiv}. }   
\fi 
% Table~\ref{table:ilp-variables} also includes some high level unary variables, which help conveniently impose structural constraints on the support graph $G$ we seek. An example is an \emph{active row} variable $\xOne{\tableVar}$ which takes value 1 if and only if at least a cell in row $j$ of table $i$ is in the support graph.
%\footnote{We say an element is ``active" if and only if the value of binary variable corresponding to this element is one.} 

%\textbf{Objective function: }
The objective function is a weighted linear sum of all the variables we instantiate for a given problem. 
\ifarxiv 
\footnote{The complete list of weights for the pairwise and unary variables are included in Table~\ref{table:objective-details} in the appendix.}
\else
\footnote{The complete list of weights for the pairwise and unary variables are included in Table~9
%\ref{table:objective-details} 
of \citep{tableilp2016:arxiv}.}
\fi 
%\footnote{There is a small set of auxiliary variables which are used for modeling complicated constraints, which will later introduce among constraints.}
%The weights for each The only detail about remaining to explain is how the weights for variables are set in the objective function (i.e. the vector $\textbf{w}$ in Eq. \ref{eq:ilp:obj}). 
There is a small set of auxiliary variables defined for linearizing complicated constraints, which will later introduce among constraints.
% In addition to the current set of variables, there are  some auxiliary variables which we define when we talk about constraints. Defining auxiliary variables is a common trick for linearizing more intricate constraints at the cost of having more variables. 

Constraints are a significant part of our model, which impose our desired behavior on the support graph. 
%There is a long set of constraints defined in our model, 
 However due to lack of space we only show a representative subset here.
\ifarxiv 
\footnote{The complete list of the constraints is explained in Table~\ref{table:constraints} in the appendix.}
\else
\footnote{The complete list of the constraints is explained in Table~13
%\ref{table:constraints}
of \citep{tableilp2016:arxiv}.}
\fi 
%Different groups of constraints are defined for different purposes, however it is hard to classify them into disjoint groups of constraints. We briefly mention a couple of important classes of constraints.

Some constraints relate variables to each other. The unary variables are defined through constraints that relate them to the pairwise basic variables. For example, for active row variable $\xOne{\tableVar}$, we ensure that it is active if and only if any cell in row $j$ is active:
$$
\xOne{\rowVar}  \geq \xTwo{\tableCell}{*}, \forall (\tableCell, *) \in \mathcal{R}_{ij}, \forall i, j, k, 
$$
where $\mathcal{R}_{ij}$ is collection of pairwise variables with one end in row  $j$ of table $i$. 
%(constraint~\ref{cons:rowIsActiveIfAnyCellInRowIsActive}, Table~\ref{table:constraints}). 

% Some constraints force the basic correctness principles on the final answer. For example $G$ should contain exactly one answer option which is expressed by the following: 
% $$
% \sum_{m}\xOne{\option} \leq 1, \quad  \sum_{m}\xOne{\option} \geq 1 
% $$
%constraint~\ref{cons:ifEdgeConnectedToTableIsActiveTableIsActive}, Table~\ref{table:constraints}. 
% Similarly $G$ should contain at least a certain number of elements in the question: 
% $$
%   \sum_{l} \xOne{\qCons} \geq \textsc{MinActiveQCons}  
% $$
%, which is modeled by constraint~\ref{cons:atLeastOneActiveEdgeConnectedToOption}, Table~\ref{table:constraints}.

% Another group of constraint induce simplicity (sparsity) in the output. For example $G$ should use at most a certain number of knowledge base table, since letting the inference use any table could lead to unreasonably long, and likely error-prone, answer chains. Also $G$ should use at most a certain number of cells in each table, since freedom to align with any number of cells in the table could lead to noisy and unreasonable alignments: 

In what follows we outline the some of the important behaviors we expect from our model which come out with different combination of the active variables. 
}

\subsubsection{Basic Lookup}
Consider the following question:
\begin{myquote}
Which characteristic helps a fox find food?
(A) sense of smell (B) thick fur (C) long tail (D) pointed teeth
\end{myquote}
In order to answer such lookup-style questions, we generally seek a row with the highest aggregate alignment to question constituents. We achieve this by 
%boosting the objective function based on \peter{"based on" - vague! What does this mean?} the question-table alignment scores and the number of active question constituents. 
incorporating the question-table alignment variables with the alignment scores, $w(e)$, as coefficients and the active question constituents variable with a constant coefficient in the objective function. Since any additional question-table edge with a positive entailment score (even to irrelevant tables) in the support graph would result in an increase in the score, we disallow tables with alignments only to the question (or only to a choice) and add a small penalty for every table used in order to reduce noise in the support graph. We also limit the maximum number of alignments of a question constituent and {  table cells to prevent one constituent or cell from having a large influence on the objective function and thereby the solution: 
$$
\sum_{(*, \qCons) \in \mathcal{Q}_l } \xTwo{*}{\qCons} \leq \textsc{MaxAlignmentsPerQCons}, \forall l
$$
where $\mathcal{Q}_l$ is the set of all pairwise variables with one end in question constituent $\ell$. 
}

\subsubsection{Parallel Evidence}
For certain questions, evidence needs to be combined from multiple rows of a table. For example,
\begin{myquote}
Sleet, rain, snow, and hail are forms of (A) erosion (B) evaporation (C) groundwater (D) precipitation
\end{myquote}
To answer this question, we need to combine evidence from multiple table entries from the weather terms table, \textit{(term, type)}, namely (sleet, precipitation), (rain, precipitation), (snow, precipitation), and (hail, precipitation). To achieve this, we allow multiple active rows in the support graph. Similar to the basic constraints, we limit the maximum number of active rows per table and add a penalty for every active row to ensure only relevant rows are considered for reasoning{:
$$
\sum_{j} \xOne{\rowVar} \leq \textsc{MaxRowsPerTable}, \forall i
$$
}
%Since our tables have well-defined schemas and few columns, 
To encourage only coherent parallel evidence within a single table,
we limit our support graph to always use the same columns across multiple rows within a table, i.e., every active row has {the active cells corresponding to the same  set of columns}.

\subsubsection{Evidence Chaining}
Questions requiring chaining of evidence from multiple tables, such as the example in Figure~\ref{fig:ny-example:tableilp}, are typically the most challenging in this domain.
%especially for simple IR-based approaches. One such question was discussed in Section~\ref{sec:intro} which required chaining of tables about geographical locations, orbital events and their properties.
Chaining can be viewed as performing a \emph{join} between two tables. We introduce alignments between cells across columns %\tushar{I think this is resolved now, right ?} \daniel{Add ``conditioned on alignment of their corresponding header cell, "?}\tushar{It's now completely controlled by the allowed joins, right?}\ashish{It is; also Def.~\ref{def:support-graph:tableilp} now explicitly already requires this}  
 in pairs of tables to allow for chaining of evidence. %\daniel{Now here we can again talk about red cells/edges in Fig 1, which are the active variables; also mention the green cells/edges which are used for alignment of the red stuff. How is that? }\tushar{That makes perfect sense. Also the same example question.} 
 To help minimize potential noise introduced by chaining irrelevant facts, we add a penalty for every inter-table alignment and also rely on the 0/1 weights of header-to-header edges
 %(shown in green in Figure \ref{fig:ny-example:tableilp})
 to ensure only semantically meaningful table joins are considered.
%constrain the inter-table alignments to manually specified column pairs of similar type where the tables are from similar domains.  

\subsubsection{Semantic Relation Matching}
Our constraints so far have only looked at the content of the table cells, or the structure of the support graph, without explicitly considering the \emph{semantics} of the table schema. By using alignments between the question and column headers (i.e., type information), we exploit the table schema to prefer alignments to columns relevant to the ``topic'' of the question. In particular, for questions of the form ``which X $\ldots$'', we prefer answers that directly entail X or are connected to cells that entail X. However, this is not sufficient for questions such as:
\begin{myquote}
What is one way to change water \underline{from} a liquid \underline{to} a solid? (A) decrease the temperature (B) increase the temperature (C) decrease the mass (D) increase the mass
\end{myquote}
Even if we select the correct table, say $r_\text{change-init-fin}(c, i, f)$ that describes the initial and final states for a phase change event, both choice (A) and choice (B) would have the exact same score in the presence of table rows (increase temperature, solid, liquid) and (decrease temperature, liquid, solid). The table, however, does have the initial vs.\ final state structure. To capture this semantic structure, we annotate pairs of columns within certain tables with the semantic relationship present between them. In this example, we would annotate the phase change table with the relations: changeFrom$(c, i)$, changeTo$(c, f)$, and fromTo$(i, f)$. 

Given such semantic relations for table schemas, we can now impose a preference towards question-table alignments that respect these relations. We associate each semantic relation with a set of linguistic patterns describing how it might be expressed in natural language. \tableilp\ then uses these patterns to spot possible mentions of the relations in the question $Q$. We then add the soft constraint that for every pair of active columns in a table (with an annotated semantic relation) aligned to a pair of question constituents, there should be a valid expression of that relation in $Q$ between those constituents. In our example, we would match the relation fromTo(liquid, solid) in the table to ``liquid \underline{to a} solid'' in the question via the pattern ``X to a Y" associated with fromTo(X,Y), and thereby prefer aligning with the correct row (decrease temperature, liquid, solid).
%\ashish{moved this over from 3.1, to shrink+merge with the paragraph below} Moreover, we extend the table schema by defining a semantic structure over the columns in the table to capture important latent structure.  For example, a table describing phase change contains relationships between the arguments (e.g. changeFrom(melting, solid), changeTo(melting, liquid)) that are critical to question answering. Without this semantic structure, a simple matching-based approach would not be able to differentiate melting from freezing. We capture this structure by annotating pairs of columns in certain tables with the semantic relationship present between them. We defined a closed set of relations observed in our tables for annotation: typeOf, partOf, hasProperty, in,  provides, performs, purpose, requires, helpsWith, causes, unitOf, measures, changeFrom, changeTo, fromTo.  \tushar{Maybe the entire list is not needed}

%Apart from using the column headers to capture the table semantics, we also use the relation structure defined over the table schema to go beyond simple row matching. For every pair of columns with an annotated relation, $\xTwo{\columnVar}{\columnVarPrime}$ and an expression of the relation in the question $\xTwo{\qCons}{\qConsPrime}$, we create a relation match variable $r(\columnVar, \columnVarPrime, \qCons, \qConsPrime)$. To find the expressions of a relation in a question, we first find the various syntactic patterns of the relationship in our corpus using our table-building tool. We manually simplify these patterns to a small set of regular expressions that are then used to find parts of the question, $(\qCons, \qConsPrime)$ that match these patterns as expressions of the relation in the question. For simplicity of exposition, we assume that all expressions of a relation are always preceded by the first argument of the relation (and followed by the second), but it is easy to extend our constraints to the general case.








%%%%%%%%%%%%%% EXPERIMENTS %%%%%%%%%%%%%%

\section{Evaluation}
\label{sec:experiments:tableilp}

We compare our approach to three existing methods, demonstrating that it outperforms {the best previous} structured approach~\citep{KBGSCE15} and produces a statistically significant improvement when used in combination with IR-based methods~\citep{CEKSTTK16}. For evaluations, we use a 2-core 2.5 GHz Amazon EC2 linux machine with 16 GB RAM.

% \ashish{TODO: include ancillary experiments that provide insights: proof graph stats (e.g., on average uses X rows and Y tables), score on questions that IR + PMI doesn't get right (arguably harder; of course, we lose some easy ones too)}
% \tushar{Not very sure if its worth making a section of its own. I have added some basic statistics about the overlap between tableilp and salience/lucene to motivate the solver combination. Regards to questions that lucene+salience gets wrong (both are wrong), tableilp gets a score of 26.75 of the total 51 points.
% Other stats:\\
% Average \#cells: 3.43\\
% Average \#qCons: 2.1 \\
% Average \#tables: 0.95 (counting unanswered options as 0)\\
% }
% \ashish{to double-check, 26.75 of total 51 points means effective a score of 52.5\%, right? compared to a random baseline, which would get 25\%?}\tushar{Yup, that is correct. That would be a nice way to presenting them in the solver combination.}
% \ashish{can't say much about 0.95 tables used on average. Might be more interesting if we know the average number of tables used for the top scoring answer only? (the rest of the proof graphs are just to get confidence scores for the combiner)}\tushar{Only for the top scoring option (ignoring correctness), we use on an average 1.3 tables for each choice. Still not a huge number, I will take a look at the \#rows (harder to do as it is not a feature)}
% \daniel{52.5\% is very interesting, although the avg number of tables used sounds odd.}
%\ashish{combination stuff (questions that \lucene/\salience\ get incorrect) is incorporated. looks like it might be difficult to make a strong point about average number of rows/tables. commenting it out for now.}\tushar{Requires some minor changes to the code to get the average \#rows, but my guess is that it would highlight that higher number of questions need parallel evidence vs chaining (based on the $\sim$ 1 avg \#tables needed)}
%\tushar{avg \#rows = 2.35 Vs avg \#tables = 1.35. Not very large numbers but slight preference towards parallel evidence.}

%\paragraph{Question set.}
%
%As our goal is to answer real exam questions, exactly as written, we use questions from the NY Regents\footnote{
%Similar to prior work\citep{CEKSTTK16}, 
\vspace{1ex}
\noindent \textbf{Question Set.}
{We use the same question set as \cite{CEKSTTK16}, which consists of all non-diagram multiple-choice questions from 12 years of the NY Regents 4th Grade Science exams.\footnote{These are the only publicly available state-level science exams. http://www.nysedregents.org/Grade4/Science/home.html} The set is split into 108 development questions and 129 hidden test questions based on the year they appeared in (6 years each).} All numbers reported below are for the hidden test set, except for question perturbation experiments which relied on the 108 development questions.
%Although the low number of publicly released, real exam questions makes the dataset small, it provides sufficient signal for evaluation.

Test scores are reported as percentages. For each question, a solver gets a score of $1$ if it chooses the correct answer and $1/k$ if it reports a $k$-way tie that includes the correct answer. On the 129 test questions, a score difference of 9\% (or 7\%) is statistically significant at the 95\% (or 90\%, resp.) confidence interval based on the binomial exact test~\citep{Howell12}.

%%%%%%%%%%%%%
%\subsection{Corpora, Rules, and Tables}
%
%\paragraph{Corpora}

\vspace{1ex}
\noindent \textbf{Corpora.}
We work with three knowledge corpora:
\begin{enumerate}
%\item Elementary Science Corpus: ~80k sentences about elementary science, consisting of a Regents study guide, CK12 textbooks,\footnote{www.ck12.org} and automatically collected Web sentences of similar style and content to that material.

\item Web Corpus: This corpus contains $5 \times 10^{10}$ tokens (280 GB of plain text) extracted from Web pages. {It was collected by Charles Clarke at the University of Waterloo, and has been {used previously by~\cite{Turney13}} and \cite{CEKSTTK16}.} We use it here to compute statistical co-occurrence values for the \salience\ solver.

\item Sentence Corpus {\citep{CEKSTTK16}}: This includes sentences from the Web corpus above, as well as around 80,000 sentences from various domain-targeted sources for elementary science:
%to create a corpus of sentences for the IR-based solver. For the domain-targeted corpus, we collected 
a Regents study guide, CK12 textbooks (www.ck12.org), and web sentences with similar content as the course material.

\item Table Corpus (cf.~Section~\ref{subsec:tables}): This includes 65 tables totaling around 5,000 rows, designed based on the development set and study guides, as well as 4 Open IE-style~\citep{BCSBE07} automatically generated tables totaling around 2,600 rows.\footnote{{Table Corpus and the ILP model are available at allenai.org}.} 
%We also converted sentences from Regents study guide into OpenIE-style~\citep{EBSW08} tuples to create a 3-column table. 
%\tushar{Might be better to describe the tables (what extractor, etc) in more detail in the main section.}\tushar{Reduced the description here after I added more details in the main section.}

\end{enumerate}

%From the Elementary Science corpus, a rulebase of 45,000 rules was automatically extracted for \praline, and a datastore of 45 tables (total 10k rows, 40k cells) was built using an interactive table-building tool and manually, for \tableilp. The \salience\ solver uses the Web Corpus and a window of 10 words to compute PMI values.

%\daniel{Shall we add a little more explanation about the auto-generated tables? We need to refer to them in the ablation study. Here is what I wrote; see if are happy to fit it somewhere:  } \ashish{yes, should add a little about tables, hopefully without using the word `manually' much; ok to say manually defined schema.}\tushar{Maybe we don't need the Elementary science Corpus as we are referring to the OpenIE tuples here and we don't have RULE solver as a baseline.}
%\ashish{tushar: that makes sense. should we just have two corpora, the Web Corpus and the Table Corpus in the bullets above? Oh. do we need something for MLN or shd we just refer to the EMNLP implementation? probably the latter.}\tushar{I was thinking of just mentioning the MLN solver as the solver with its corpora. The tricky part is also the Lucene solver which has a mixture of both the corpora and more.}
%{\color{red}
%Some of the tables are automatically modeled as relations and OpenIE-style tuples~\citep{OPENIE} extracted from Barron's syllabus, using ``NameOfATool" (and some references here?). These tables help in bringing more coverage to the solver (compared to the manually generated tables, which were mostly based on the training data). }

%%%%%%%%%%%
\subsection{Solvers}
\label{section:baslines:tableilp}

\vspace{1ex}
\noindent \textbf{\tableilp} (our approach). 
Given a question $Q$, we select the top 7 tables from the Table Corpus using the the standard TF-IDF score of $Q$ with tables treated as bag-of-words documents. For each selected table, we choose the 20 rows that overlap with $Q$ the most. This filtering improves efficiency and reduces noise. We then generate an ILP and solve it using the open source SCIP engine~\citep{Achterberg09}, returning the active answer option $\option$ from the optimal solution. To check for ties, we disable $\option$, re-solve the ILP, {and compare the score of the second-best answer, if any, with that of $a_m$}.

%We compare our approach to three baseline solvers:
%Apart from three statistical baseline methods, we use the state-of-the-art structured method from prior work~\citep{KBGSCE15} to compare against our approach

\vspace{1ex}
\noindent \textbf{MLN Solver} (structured inference baseline). 
We consider the current state-of-the-art structured reasoning method developed for this specific task by~\cite{KBGSCE15}. We compare against their best performing system, namely Praline, which uses Markov Logic Networks~\citep{RichardsonDo06} to (a) align lexical elements of the question with probabilistic first-order science rules and (b) to control inference. We use {the entire set of} 47,000 science rules from their original work, which were also derived from same domain-targeted sources as the ones used in our Sentence Corpus.
%\daniel{This last phrase sounds odd to me: ``rule-based science knowledge, and to control inference.'' Anything missing from here?}

\vspace{1ex}
\noindent \textbf{\lucene\ Solver} (information retrieval baseline).
{We use the IR baseline by \cite{CEKSTTK16},} {which selects the answer option that has} the best matching sentence in a corpus. {Specifically,} for each answer option $a_i$, the \lucene\ solver sends $q + a_i$ as a query to a search engine (we use Lucene) on the Sentence Corpus, and returns the search engine's score for the top retrieved sentence $s$, where $s$ must have at least one non-stopword overlap with $q$, and at least one with $a_i$. The option with the highest Lucene score is returned as the answer.

\vspace{1ex}
\noindent \textbf{\salience\ Solver} (statistical co-occurrence baseline).
{We use the PMI-based approach by \cite{CEKSTTK16}}, {which selects} the answer option that most frequently co-occurs with the question words in a corpus. Specifically, it extracts unigrams, bigrams, trigrams, and skip-bigrams from the question and each answer option.
%We use the SMART stop word list \citep{salton1971smart} to filter the extracted n-grams, but allow trigrams to have a stop word in the middle.
For a pair $(x,y)$ of $n$-grams, their pointwise mutual information (PMI)~\citep{ChurchHa89} in the corpus is defined as $\log \frac{p(x,y)}{p(x)p(y)}$ where $p(x,y)$ is the co-occurrence frequency of $x$ and $y$ (within some window) in the corpus.
The solver returns the answer option that has the largest average PMI in the Web Corpus, calculated over all pairs of question $n$-grams and answer option $n$-grams.

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Results}

We first compare the accuracy of our approach against the previous structured (MLN-based) reasoning solver. We also compare against \lucene(tables), an IR solver using table rows expressed as sentences, thus embodying an unstructured approach operating on the same knowledge as \tableilp.
%\daniel{cite \citep{Howell12}?} \ashish{hmm. psychology :-) Is there a pure stats or CS reference?} \daniel{I tried to find another CS-ish reference, but couldn't find a significant highly cited reference. (This work is highly cited; beside hypothesis testing is the cornerstone of the psycology! :) )}
%\ashish{Howell it is, then!}
%\ashish{adding 90\% confidence interval too, to avoid people thinking nothing else besides one result is statistically significant} 

% \begin{table}[htb]
% \centering
% \setlength\tabcolsep{10pt}
% \setlength\doublerulesep{\arrayrulewidth}
% \begin{tabular}{c|l|c}
% %\textbf{Solver} & \textbf{Test score} \\
% Solver type & Solver & Test Score \\
% \hline\hline \bigstrut[t]
% \multirow{3}{*}{Unstructured} & \lucene (tables) & 51.2 \\
% & \lucene & 58.5 \\
% & \salience & 60.7 \\
% \hline \bigstrut[t]
% \multirow{2}{*}{Structured} \bigstrut[t]  % leave some gap (?)
% & \praline & 47.5 \\
% & \tableilp & {\bf 61.5} \\
% \hline
% \end{tabular}
% \caption{Test score comparison of the solvers using structured and unstructured data. \lucene(tables) uses the table rows as input sentences for the \lucene\ approach.}
% \label{tab:eval}
% \end{table}

\begin{wrapfigure}{r}{0.35\textwidth}
% \begin{table}[htb]
\centering
\small
\setlength\extrarowheight{-10pt}
\setlength\tabcolsep{10pt}
\setlength\doublerulesep{\arrayrulewidth}
\begin{tabular}{l|c}
Solver & Test Score (\%) \\
\hline\hline \bigstrut[t]
\praline & 47.5 \\
\lucene (tables) & 51.2 \\
\tableilp & {\bf 61.5} \\
\hline
\end{tabular}
\makeatletter\def\@captype{table}\makeatother% "Change float to table"
\caption{\tableilp~significantly outperforms both the prior MLN reasoner, and IR using identical knowledge as \tableilp}
% \caption{Test score comparison: structured reasoning methods and IR using identical knowledge as \tableilp}
\label{tab:eval}
% \end{table}
\end{wrapfigure}

As Table \ref{tab:eval} shows, among the two structured inference approaches, \tableilp\ outperforms the MLN baseline by 14\%. {The preliminary ILP system reported by \cite{CEKSTTK16} achieves only a score of 43.8\% on this question set.} Further, given the same semi-structured knowledge (i.e., the Table Corpus), \tableilp\ is substantially (+10\%) better at exploiting the structure than the \lucene(tables) baseline, {which, as mentioned above,} uses the same data expressed as sentences.
%Finally, \tableilp's score is comparable to the unstructured baselines that utilized much larger corpora. This closes, for the first time, the rather large gap between unstructured and structured approaches for this QA domain.

%\tableilp has significantly better performance compared to the IR baseline limited to the same knowledge base, although IR baseline gets very close to \tableilp when it uses significant amount of free data crawled from the web, as well as PMI baseline. \tableilp  has significantly better performance compared to a rival structured model MLN. 


\subsubsection{Complementary Strengths}
\begin{wrapfigure}{r}{0.5\textwidth}
% \begin{table}[htb]
\centering
\small
\setlength\tabcolsep{10pt}
\setlength\doublerulesep{\arrayrulewidth}
\setlength\extrarowheight{-10pt}
\begin{tabular}{l|c}
%\textbf{Solver} & \textbf{Test score} \\
Solver & Test Score (\%) \\
\hline\hline \bigstrut[t]
\lucene & 58.5 \\
\salience & 60.7 \\
\tableilp & 61.5  \\
\tableilp\ + \lucene & 66.1 \\
\tableilp\ + \salience & 67.6 \\
\tableilp\ + \lucene + \salience & {\bf 69.0} \\
\hline
\end{tabular}
\makeatletter\def\@captype{table}\makeatother% "Change float to table"
\caption{Solver combination results}
\label{tab:combination}
% \end{table}
\end{wrapfigure}
%Not all the solvers have the same behavior on the same problems; a question might be easy for one, meanwhile hard for the other. 
While their overall score is similar, \tableilp\ and IR-based methods clearly approach QA very differently. To assess whether \tableilp\ {adds} any new capabilities, we considered the 50 (out of 129) questions incorrectly answered by \salience\ solver (ignoring tied scores). On these unseen but arguably more difficult questions, \tableilp\ answered 27 questions correctly, achieving a score of 54\% compared to the random chance of 25\% for 4-way multiple-choice questions. Results with \lucene\ solver were similar: \tableilp\ scored 24.75 on the 52 questions incorrectly answered by \lucene\ (i.e., 47.6\% accuracy).
%For example, out of the 74 questions correctly answered by the \tableilp \ solver, \lucene\ solver also answers 50 of these questions and \salience \ answers 48 questions in the hidden set. 



{This analysis highlights the} complementary strengths of these solvers. {Following \cite{CEKSTTK16}, we create an ensemble of \tableilp, \lucene, and \salience\ solvers, combining their answer predictions} using a simple Logistic Regression model trained on the development set. {This model uses} 4 features derived from each solver's score for each answer option, and 11 features derived from \tableilp's support graphs.
\ifarxiv 
\footnote{Details of the 11 features may be found in the Appendix B.}
\else
\footnote{Details of the 11 features may be found in the extended version~\citep{tableilp2016:arxiv}.}
\fi Table \ref{tab:combination} shows the results,
%two top performing solvers from Table \ref{tab:eval}. 
%The addition of each solver to \tableilp\ leads to an increase in the score, 
with the final combination at 69\% representing a significant improvement over individual solvers.
%being statistically significantly better than \lucene\ alone. 
%\tushar{TODO: Use the statistics from the solver overlap to make this point stronger.}\tushar{This is taken care of by the earlier para, right?}

%%%%%%%%%%%%%%
\subsubsection{ILP Solution Properties}
Table~\ref{tab:stats:tableilp} summarizes various ILP and support graph statistics for \tableilp, averaged across all test questions.

The optimization model has around 50 high-level constraints, which result, on average, in around 4000 inequalities over 1000 variables. Model creation, which includes %a large number of 
computing pairwise entailment scores using WordNet, takes 1.9 seconds on average per question, and the resulting ILP is solved by the SCIP engine in 2.1 seconds (total for all four options), using around 1,300 LP iterations for each option.\footnote{Commercial ILP solvers (e.g., CPLEX, Gurobi) are much faster than the open-source SCIP solver we used for evaluations.} 

\begin{wrapfigure}{r}{0.55\textwidth}
% \begin{table}[htb]
\centering
\small
\setlength\tabcolsep{10pt}
\setlength\doublerulesep{\arrayrulewidth}
\setlength\extrarowheight{-12pt}
\begin{tabular}{llc}
Category & Quantity & Average \\
\hline\hline \bigstrut[t]
\multirow{3}{*}{ILP complexity} & \#variables & 1043.8 \\
& \#constraints & 4417.8 \\
& \#LP iterations & 1348.9 \\
\hline \bigstrut[t]
%\multirow{3}{*}{Alignments} &\#question constituents & 3.34 \\
%& \#rows & 2.32 \\
\multirow{2}{*}{Knowledge use} & \#rows & 2.3 \\
& \#tables & 1.3 \\
\hline \bigstrut[t]
\multirow{2}{*}{Timing stats} & model creation & 1.9 sec \\
& solving the ILP & 2.1 sec \\
\hline
\end{tabular}
\makeatletter\def\@captype{table}\makeatother% "Change float to table"
\caption{\tableilp\ statistics averaged across questions}
\label{tab:stats:tableilp}
% \end{table}
\end{wrapfigure}
Thus, \tableilp\ takes only 4 seconds to answer a question using multiple rows across multiple tables (typically 140 rows in total), as compared to 17 seconds needed by the \praline\ solver for reasoning with four rules (one per answer option).  


While the final support graph on this question set relies mostly on a single table to answer the question, it generally combines information from more than two rows (2.3 on average) for reasoning. This suggests parallel evidence is more frequently used on this dataset than evidence chaining.
%\tableilp\ relies on roughly three question constituents to answer the questions which have XXX constituents on an average. \ashish{hmm. this doesn't sound that great and is probably one of the biggest weakness of the solver --- that it ignores a large part of the question! commenting it out until we have a better solution :-)}


%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Ablation Study}

\begin{wrapfigure}{r}{0.5\textwidth}
% \begin{table}[htb]
\centering
\small
\setlength\tabcolsep{7pt}
\setlength\extrarowheight{-6pt}
\setlength\doublerulesep{\arrayrulewidth}
\begin{tabular}{ll|cc}
%\multicolumn{1}{c|}{\textbf{Approach}} & \textbf{Test score} & \textbf{\% drop} \\
\multicolumn{2}{c|}{Solver} & Test Score (\%) \\
\hline\hline
\multicolumn{2}{l|}{\bigstrut[t] \tableilp} & 61.5  \\
  & No Multiple Row Inference & 51.0 \\
  & No Relation Matching & 55.6 \\
  \cline{2-3} \bigstrut[t] 
  & No Open IE Tables & 52.3  \\
  & No Lexical Entailment & 50.5  \\
\hline 
\end{tabular}
\makeatletter\def\@captype{table}\makeatother% "Change float to table"
\caption{Ablation results for \tableilp}
\label{tab:ablation:tableilp}
% \end{table}
\end{wrapfigure}
To quantify the importance of various components of our system, we performed several ablation experiments, summarized in Table~\ref{tab:ablation:tableilp} and described next.
% We start with two components related to structured inference, and then discuss the impact of coverage of knowledge and lexical alignment scores.
%\ashish{it's better to order these in terms of what's most relevant. Putting Lexical Entailment upfront can be troublesome, as we don't say much about it. Reordering.} \daniel{ok; fine by me.}



\vspace{1ex}
\noindent \textbf{No Multiple Row Inference}: We modify the ILP constraints to limit inference to a single row (and hence a single table), thereby disallowing parallel evidence and evidence chaining (Section~\ref{subsec:ilp:tableilp}). This drops the performance by 10.5\%, highlighting the importance of being able to combine evidence from multiple rows (which would correspond to multiple sentences in a corpus) from one or more tables.

\vspace{1ex}
\noindent \textbf{No Relation matching}: To assess the importance of considering the semantics of the table, we remove the requirement of matching the semantic relation present between columns of a table with its lexicalization in the question (Section~\ref{subsec:ilp:tableilp}). The 6\% drop indicates \tableilp\ relies strongly on the table semantics to ensure creating meaningful inferential chains.
%gets similar performance to the IR-based solver on the table corpus, since it also picks the best matching sentences (corresponding to a row in a table) for a question.

\vspace{1ex}
\noindent \textbf{No Open IE tables}: To evaluate the impact of relatively unstructured knowledge from a large corpus, we removed the tables containing Open IE extractions (Section~\ref{subsec:qa-as-subgraph-selection}). The 9\% drop in the score shows that this knowledge is important and \tableilp\ is able to exploit it even though it has a very simple triple structure. This opens up the possibility of extending our approach to triples extracted from larger knowledge bases.

\vspace{1ex}
\noindent \textbf{No Lexical Entailment}: Finally, we test the effect of changing the alignment metric $w$ (Section~\ref{subsec:qa-as-subgraph-selection}) from WordNet based scores to a simple asymmetric word-overlap measured as $\mathit{score}(T, H) = \frac{|T \cap H|}{|H|}$. Relying on just word-matching results in an 11\% drop, which is consistent with our knowledge often being defined in terms of generalities.% and not overfit to the questions.

%\tushar{Daniel: Does my change look okay ? I have used most of your text with some changes.}
%There are interesting points can be inferred from the comparison in Table~\ref{tab:ablation:tableilp}: (1) We test effect of replacing the entailment-based alignment metric \daniel{Better name? I don't want to use similarity metric since it implies symmetricity} with simple word-matching. Using entailment for connecting facts/cells helps significantly (compared to a naive similarity metrics). (2) Chaining facts (rather than looking up a fact in a single row)  is the second helping important component. (3) The auto-generated tables help the solver to generalize over the unseen test data, and hence the final performance. (4) The relation alignment adds a non-trivial amount to the final combination. 


%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Question Perturbation}
\label{subsec:perturbation}

One desirable property of QA systems is robustness to simple variations of a question, \emph{especially when a variation would make the question arguably easier for humans}. 
%\tushar{I like the point being made in the following line, but it highlights the limited nature of our test set :). is there a different way of saying it? -- A solver might get very good results on a limited dataset, but it is not clear if it generalizes well beyond that dataset. } \ashish{probably not. it's a sticky point. commenting it out.}
%
%In this experiment we test generalizability against a 

To assess this, we {consider a simple, automated way to perturb} each 4-way multiple-choice question: (1) query Microsoft's Bing search engine (www.bing.com) with the question text and obtain the text snippet of the top 2,000 hits; (2) create a list of strings by chunking and tokenizing the results; (3) remove stop words and special characters, as well as any words (or their lemma) appearing in the question; (4) sort the remaining strings based on their frequency; and (5) replace the three incorrect answer options in the question with the most frequently occurring strings, thereby generating a new question. For instance:
\begin{quote}
{In New York State, the longest period of daylight occurs during which month? (A) \emph{eastern} (B) June (C) \emph{history} (D) \emph{years}}
\end{quote}

\begin{wrapfigure}{r}{0.65\textwidth}
% \begin{table}[htb]
\centering
\small
\setlength\tabcolsep{10pt}
\setlength\doublerulesep{\arrayrulewidth}
\setlength\extrarowheight{-10pt}
\begin{tabular}{l|cccc}
 & Original & \multicolumn{2}{c}{\% Drop with Perturbation} \\
 \cline{3-4}
Solver & Score (\%) & \bigstrut[t] absolute & relative \\
\hline\hline \bigstrut[t]
\lucene & 70.7 & 13.8 & 19.5 \\
\salience & 73.6 & 24.4 & 33.2 \\
\tableilp & 85.0 & {\bf 10.5} & {\bf 12.3} \\
\hline
\end{tabular}
\makeatletter\def\@captype{table}\makeatother% "Change float to table"
\caption{Drop in solver scores (on the development set, rather than the hidden test set) when questions are perturbed}
\label{tab:perturbation}
% \end{table}
\end{wrapfigure}

%
%As can be seen here, the options (except for the correct one) are sometimes not even of the correct type, making it often \emph{easier} for humans. Surprisingly, such simple perturbations can often throw computers off. 
As in this example, the perturbations (italicized) are often not even of the correct ``type'', {typically making them much easier for humans. They, however, still remain difficult for solvers.}

For each of the 108 development questions, we generate 10 new perturbed questions, using the 30 most frequently occurring words in step (5) above. {While this approach can introduce new answer options that should be considered correct as well, only 3\% of the questions in a random sample exhibited this behavior.} Table~\ref{tab:perturbation} shows the performance of various solvers on the resulting 1,080 perturbed questions. As one might expect, the \salience\ approach suffers the most at a 33\% relative drop. \tableilp's score drops as well (since answer type matching isn't perfect), but only by 12\%, attesting to its higher resilience to simple question variation.


\section{Summary and Discussion}
This chapter proposed a reasoning system for question answering on elementary-school science exams, using a semi-structured knowledge base. 
We formulate QA as an Integer Linear Program (ILP), that answers natural language questions using a semi-structured knowledge base derived from text, including questions requiring multi-step inference and a combination of multiple facts. On a dataset of real, unseen science questions, our system significantly outperforms (+14\%) the best previous attempt at structured reasoning for this task, which used Markov Logic Networks (MLNs). When combined with unstructured inference methods, the ILP system significantly boosts overall performance (+10\%).  Finally, we show our approach is substantially more robust to {a simple answer} perturbation compared to statistical correlation methods.
% We presented \tableilp, a system that can answer such questions, 
% The system in this chapter does not not address a few aspects 

There are a few factors that limit the ideas discussed in this chapter. In particular,  the knowledge consumed by this system are in the form of curated tables;
% of elementary science facts; 
constructing such knowledge is not always easy. In addition, not everything might be representable in that form. 
% raw text itself could be much richer representation. 
% We address this limitation in Chapter 4, where we introduce a system that can consume raw text as input knowledge. 
% Second, the solver has a relatively shallow understanding of 
Another limitation stems from the nature of multi-step reasoning: larger number of reasoning steps could result in more brittle decisions. We study this issue in Chapter 8. 


\begin{comment}
We treat QA as a subgraph selection problem and then formulate this as an ILP optimization. 
Most importantly, this formulation allows multiple, semi-formally expressed facts to be combined to answer questions, a capability outside the scope of IR-based QA systems.
In our experiments, this approach significantly outperforms both the previous best attempt at structured reasoning for this task,  and an IR engine provided with the same knowledge. It also significantly boosts performance {when combined with} unstructured methods (IR and PMI). 
% These results suggest that the approach is both viable and promising for natural language question answering.
Our effort has had multiple impacts since publication.  Our work has inspired others to to build systems based on our design and to improve the state of the art in other domains; e.g., \cite{KhotSaCl17}.
In addition, the system has been incorporated into Allen Institute's reading-comprehension project\footnote{\url{https://allenai.org/aristo/}} and was shown to give a significant boost to their performance~\citep{CEKSTTK16}. 
Even after two years, the system was shown to be 
% The system was later on, after a two years, shown to be 
among the best systems on a recently-proposed reading comprehension task~\citep{CCEKSST18}.  
% Previous work has examined the use of Markov Logic Networks (MLNs) to represent the requisite background knowledge and interpret test questions, but did not improve upon an information retrieval (IR) baseline.
\end{comment}



==> Daniel K - thesis - dissertation/2.semanticilp_new.tex <==
\chapter{QA as Subgraph Optimization over Semantic Abstractions}
\epigraph{ 
``It linked all the perplexed meanings \\ 
Into one perfect peace.''
}{--- \textup{Procter and Sullivan}, The Lost Chord, 1877}
\label{chapter:semantic:ilp}

%%%%%%%%%%%%%%%%%%
%%\input{intro}
%% inline intro for camera-ready
\section{Overview}
In this chapter, we consider the multiple-choice setting where $Q$ is a question, $A$ is a set of answer candidates, and the knowledge required for answering $Q$ is available in the form of raw text $P$.\footnote{This chapter is based on the following publication: \cite{KKSR18}.} A major difference here with the previous chapter is that, the knowledge given a system is \textit{raw-text}, instead of of being represented in tabular format. 

We demonstrate that we can use existing NLP modules, such as semantic role labeling (SRL) systems with respect to multiple predicate types (verbs, prepositions, nominals, etc.), to derive multiple semantic views of the text and perform reasoning over these views to answer a variety of questions.

As an example, consider the following snippet of sports news text and an associated question:
\begin{framed}
%\vspace{-1.5ex}
\noindent\footnotesize\emph{\noindent$P$: Teams are under pressure after PSG purchased Neymar this season. \textbf{Chelsea purchased Morata}. The Spaniard looked like he was set for a move to Old Trafford for the majority of the summer only for Manchester United to sign Romelu Lukaku instead, paving the way for Morata to finally move to Chelsea for an initial \pounds 56m.
%The 24-year-old is in line to make his full Chelsea debut on Sunday against Tottenham at Wembley on Sunday having come off the bench in the season’s curtain raiser against Burnley last weekend.   
%He made a positive start to life in west London with a goal and an assist despite that defeat and Conte insisted that given today market – where Liverpool are rejecting £110m+ offers for Philippe Coutinho – Morata is a bargain signing for the Blues. After signing Morata, Conte spoke publically of how Spurs striker Kane would have been is ideal signing but he tried to clarify those comments by insisting Morata can have a similar impact to the Englishman. 
% }
% \end{framed}
% And consider the following question: 
% \begin{framed}
% \small
\\
\noindent
$Q$: Who did Chelsea purchase this season?  \\ 
$A$: \{\checkmark Alvaro Morata, Neymar, Romelu Lukaku \}%  \;  (D) Manchester United
}
\end{framed}

Given the bold-faced text $P'$ in $P$, simple word-matching suffices to correctly answer $Q$. However, $P'$ could have stated the same information in many different ways. As paraphrases become more complex, they begin to involve more linguistic constructs such as coreference, punctuation, prepositions, and nominals. This makes understanding the text, and thus the QA task, more challenging.

\begin{figure}[ht]
    \centering
% \begin{wrapfigure}{r}{0.53\textwidth}
  \includegraphics[trim=-0.00cm 0cm 0cm -0.00cm, scale=0.55]{figures_semanticilp/cropped_morata-simplfied-cropped.pdf}
  \caption{Depiction of \textilp\ reasoning for the example paragraph given in the text.
    Semantic abstractions of the question, answers, knowledge snippet are shown in different colored boxes (blue, green, and yellow, resp.). Red nodes and edges are the elements that are aligned (used) for supporting the correct answer. There are many other unaligned (unused) annotations associated with each piece of text that are omitted for clarity. 
    }
    \label{fig:morata-visualization}
% \end{wrapfigure}
\end{figure}

For instead, $P'$ could instead say \emph{Morata is the recent \textbf{acquisition} by Chelsea}. This simple looking transformation can be surprisingly confusing for highly successful systems such as \bidaf~\citep{SKFH16}, which produces the partially correct phrase \emph{``Neymar this season.\ Morata''}. On the other hand, one can still answer the question confidently by abstracting relevant parts of $Q$ and $P$, and connecting them appropriately. Specifically, a verb SRL frame for $Q$ would indicate that we seek the object of the verb \emph{purchase}, a nominal SRL frame for $P'$ would capture that the \emph{acquisition} was of Morata and was done by Chelsea, and textual similarity would align \emph{purchase} with \emph{acquisition}.

% \begin{figure}[ht]
%     \centering
%     \includegraphics[trim=-0.00cm 0cm 0cm -0.00cm, scale=0.55]{figures_semanticilp/cropped_morata-simplfied-cropped.pdf}
%     \caption{Depiction of \textilp\ reasoning for the example paragraph given in the text.
%     Semantic abstractions of the question, answers, knowledge snippet are shown in different colored boxes (blue, green, and yellow, resp.). Red nodes and edges are the elements that are aligned (used) for supporting the correct answer. There are many other unaligned (unused) annotations associated with each piece of text that are omitted for clarity. 
%     }
%     \label{fig:morata-visualization}
% \end{figure}

Similarly, suppose $P'$ instead said \emph{Morata\textbf{,} the recent acquisition \textbf{by} Chelsea\textbf{,} will start for the team tomorrow.} \bidaf\ now incorrectly chooses Neymar as the answer, presumably due to its proximity to the words \emph{purchased} and \emph{this season}. However, with the right abstractions, one could still arrive at the correct answer as depicted in Figure~\ref{fig:morata-visualization} for our proposed system, \textilp. This reasoning uses comma SRL to realize that the Morata is referring to the \emph{acquisition}, and a preposition SRL frame to capture that the acquisition was done \emph{by} Chelsea.

One can continue to make $P'$ more complex. For example, $P'$ could introduce the need for coreference resolution by phrasing the information as: \emph{\textbf{Chelsea} is hoping to have a great start this season by actively hunting for new players in the transfer period. Morata, the recent acquisition by the team, will start for \textbf{the team} tomorrow.} Nevertheless, with appropriate semantic abstractions of the text, the underlying reasoning remains relatively simple. 

% such as:
% \begin{framed}
% \vspace{-3ex}
% \footnotesize
%     \emph{ 
%     \begin{enumerate}[leftmargin=0.3cm]
%         \item Chelsea acquired Alvaro Morata.  
%         \item Real Madrid sold Alvaro Morata to Chelsea. 
%         % \item Alvaro Morata's recent acquisition by Chelsea has given extra hope for its fans.  
%         \item Chelsea broke its previous record by purchasing Morata from Real Madrid. \ashish{SQuAD: Morata from Real Madrid}
%         \item Morata hinted at his purchase. Later that day Chelsea announced the purchase.  
%         \item Recent purchase for Chelsea, Alvaro Morata, will start for Chelsea tomorrow.
%         \item Chelsea is hoping to have a great start this season by actively hunting for new players in the transfer period. Morata, the recent acquisition by the team, will start for the team tomorrow.
%     \end{enumerate}
%     }
% \vspace{-2ex}
% \end{framed}

% The first paraphrasing of $P'$ relies on synonymy between \emph{purchased} and \emph{acquired}, a gap easily bridged using resources such as WordNet~\citep{Miller95} or low-dimensional word embeddings~\citep{mikolov2013distributed}. The second requires understanding that \emph{X purchased Y} is the same as \emph{Y was sold to X}, which methods using contextual verb embeddings, such as LSTM based neural models~\citep{?}, may be able to address. \daniel{instead of this I would say, ``The second requires understanding that \emph{X purchased Y} is the same as \emph{Y was sold to X}, which resources like PropBank~\citep{KingsburyPa02} would help to answer."} \ashish{Agreed with the explanation, although, especially since even we don't use PropBank and get it right, I would instead change the rephrasing of $T'$ so that it requires more than just soft word distance but a state-of-the-art system like BiDAF \emph{can} get it correct. Then say what it cannot get.}
% \dan{Are you sure that LSTM based  systems get it for the right reason? Or only because it's the only NE option? Can you try to add deceiving entities?}
% \ashish{Not sure about LSTM. The text does have all other answer options (also NEs) mentioned in the second sentence of the paragraph.}
% \dan{Maybe it's sufficient to say: "requires understanding that \emph{X purchased Y} is the same as \emph{Y was sold to X}"; [or add also] a lexico-structural pattern that can be learned from a large QA collection only for the most common lexical items.}
% \ashish{I like the fancy last sentence, in part because it yields that existing systems \emph{can} do this, at least for common terms.}
% % side note: Propbank indeed helps us answer this. If you go to the "sell" frame, it labels subject as "buyer": https://github.com/propbank/propbank-frames/blob/master/frames/sell.xml#L21
% % }


Given sufficiently large QA training data, one could conceivably perform end-to-end training (e.g., using a deep learning method) to address these linguistic challenges. However, existing large scale QA datasets such as SQuAD~\citep{RZLL16} often either have a limited linguistic richness or do not necessarily need reasoning to arrive at the answer~\citep{JiaLi17}. 
% \ashish{update citation to point to EMNLP (I think)} 
%\danchange{
Consequently, the resulting models do not transfer easily to other domains.
%}
%\dan{is there a reference to cite here?; can we give the performance of a good Squad system on Aristo?} \ashish{added SQuAD-trained BiDAF performance on Aristo. Helpful or risky claim?}. 
For instance, the above mentioned BiDAF model trained on the SQuAD dataset performs substantially worse than a simple IR approach on our datasets. On the other hand, many of the QA collections in domains that require some form of reasoning, such as the science questions we use, are small  
%, suffer from the issue of \emph{data sparsity}. Their small size 
(100s to 1000s of questions). This brings into question the viability of the aforementioned paradigm that attempts 
%makes it difficult, if not impossible, 
to learn everything from only the QA training data.

Towards the goal of effective structured reasoning in the presence of data sparsity, we propose to use a rich set of general-purpose, pre-trained NLP tools to create various \emph{semantic abstractions} of the raw text\footnote{This applies to all three inputs of the system: $Q$, $A$, and $P$.} in a domain independent fashion, as illustrated for an example in Figure~\ref{fig:morata-visualization}.
We represent these semantic abstractions as \emph{families of graphs}, where the family (e.g., trees, clusters, labeled predicate-argument graphs, etc.) is chosen to match the nature of the abstraction (e.g., parse tree, coreference sets, SRL frames, etc., respectively). The collection of semantic graphs is then augmented with inter- and intra-graph edges capturing lexical similarity (e.g., word-overlap score or word2vec distance).

This semantic graph representation allows us to formulate QA as the search for an optimal \emph{support graph}, a subgraph $G$ of the above augmented graph connecting (the semantic graphs of) $Q$ and $A$ via $P$. The reasoning used to answer the question is captured by a variety of requirements or constraints that $G$ must satisfy,
as well as a number of desired properties, encapsulating the ``correct'' reasoning, that makes $G$ preferable over other valid support graphs. For instance, a simple requirement is that $G$ must be connected and it must touch both $Q$ and $A$. Similarly, if $G$ includes a verb from an SRL frame, it is preferable to also include the corresponding subject. Finally, the resulting constrained optimization problem is formulated as an Integer Linear Program (ILP), and optimized using an off-the-shelf ILP solver (see Section~\ref{sec:optimization:background} for a review of ILP). 

This formalism may be viewed as a generalization of the systems introduced in the previous chapter: 
% that reason over tables of knowledge~\citep{cohen2000:joins,tableilp2016:ijcai} :
instead of operating over table rows (which are akin to labeled sequence graphs or predicate-argument graphs), we operate over a much richer class of semantic graphs. It can also be viewed as a generalization of the recent \tupleinf\ system~\citep{KhotSaCl17}, which converts $P$ into a particular kind of semantic abstraction, namely Open IE tuples~\citep{BCSBE07}.

This generalization to multiple semantic abstractions poses two key technical challenges: (a) unlike clean knowledge-bases (e.g., \cite{DWZX15}) used in many QA systems, abstractions generated from NLP tools (e.g., SRL) are noisy; and (b) even if perfect, using their output for QA requires delineating what information in $Q$, $A$, and $P$ is relevant for a given question, and what constitutes valid reasoning. The latter is especially challenging when combining information from diverse abstractions that, even though grounded in the same raw text, may not perfectly align. We address these challenges via our ILP formulation, by using our linguistic knowledge about the abstractions to design requirements and preferences for linking these abstractions.

We present a new QA system, \textilp,\footnote{Code available at: {https://github.com/allenai/semanticilp}} based on these ideas, and evaluate it on multiple-choice questions from two domains involving rich linguistic structure and reasoning: elementary and middle-school level science exams, and early-college level biology reading comprehension. Their data sparsity, as we show, limits the performance of state-of-the-art neural methods such as BiDAF~\citep{SKFH16}. \textilp, on the other hand, is able to successfully capitalize on existing general-purpose NLP tools in order to outperform existing baselines by 2\%-6\% on the science exams, leading to a new state of the art. It also generalizes well, as demonstrated by its strong performance on biology questions in the \processBank\ dataset~\citep{BSCLHHCM14}. Notably, while the best existing system for the latter relies on domain-specific structural annotation and question processing, \textilp\ needs neither.


\subsection{Related Work}
\label{subsec:related-work}
We provide a brief review of the related work, in additional to the discussion provided in Section~\ref{sec:intro:qa:review}. 


Our formalism can be seen as an extension of the previous chapter. 
% , which was focused on 
% some of the prior work on structured reasoning over semi-structured text. 
For instance, in our formalism, each table used by \tableilp\ 
% \cite{tableilp2016:ijcai} 
can be viewed as a semantic frame and represented as a predicate-argument graph. The table-chaining rules used there are equivalent to the reasoning we define when combining two annotation components. Similarly, Open IE tuples used by~\citep{KhotSaCl17} can also be viewed as a predicate-argument structure.



% Semantic Role Labeling 
One key abstraction we use is the predicate-argument structure provided by Semantic Role Labeling (SRL).
% Semantic role labeling, is the detection of the semantic arguments associated with the predicate  of a sentence and their classification into their specific roles. 
%Semantic Role Labeling (SRL) is one of the important NLP problems %and to this date, there are 
 Many SRL systems have been designed \citep{GildeaJu02,PunyakanokRoYi08} using linguistic resources such as FrameNet~\citep{BakerFiLo98}, PropBank~\citep{KingsburyPa02}, and NomBank~\citep{MRMSZYG04}. These systems are meant to convey high-level information about predicates (which can be a verb, a noun, etc.) and related elements in the text. The meaning of each predicate is conveyed by a frame, the schematic representations of a situation. Phrases with similar semantics ideally map to the same frame and roles. Our system also uses other NLP modules, such as for coreference resolution~\citep{LCPCSJ13} and dependency parsing~\citep{CUCSR15}.


% Understanding events and their participants is a key part of understanding natural
% language. At a high level, understanding an event means being able to answer the
% question “Who did what to whom” (and perhaps also “when and where”). The
% answers to this question may be expressed in many different ways in the sentence.
% For example, if we want to process sentences to help us answer question about a
% purchase of stock by XYZ Corporation, we need to understand this event despite
% many different surface forms. The event could be described by a verb (sold, bought)
% or a noun (purchase), and XYZ Corp can be the syntactic subject (of bought) the
% indirect object (of sold), or in a genitive or noun compound relation (with the noun
% purchase), in the following sentences, despite having notationally the same role in
% all of them:
% • XYZ corporation bought the stock.
% • They sold the stock to XYZ corporation.
% • The stock was bought by XYZ corporation.
% • The purchase of the stock by XYZ corporation...
% • The stock purchase by XYZ corporation...

While it appears simple to use SRL systems for QA~\citep{PalmerGiKi05}, this has found limited success~\citep{KaisserWe07,PizzatoMo08,MLBP11}. The challenges earlier approaches faced were due to making use of VerbSRL only, while QA depends on richer information, not only verb predicates and their arguments, along with some level of brittleness of all NLP systems. \cite{ShenLa07} have partly addressed the latter challenge with an inference framework that formulates the task as a bipartite matching problem over the assignment of semantic roles, and managed to slightly improve QA. In this work we address both these challenges and go beyond the limitations of using a single predicate SRL system; we make use of SRL abstractions that are based on verbs, nominals, prepositions, and comma predicates, as well as textual similarity. We then develop an inference framework capable of exploiting combinations of these multiple SRL (and other) views, thus operating over a more complete semantic representation of the text.


% Our work is not limited or focused on using SRL, but SRL is indeed a key ingredient of our work.
% Often QA is cited as one of the important potential applications of SRL \citep{PalmerGiKi05}. \addedT{While it seems intuitive and simple to use SRL for question answering, there has been limited work on using SRL for such problems \citep{ShenLa07,KaisserWe07,PizzatoMo08,MLBP11}.}
% %On simple examples, it often feels very intuitive and simple to use SRL to improve QA, however there are very few works using SRL for QA and similar problem. 
%  There are a couple of reasons for this: (1) Even with improvements to SRL systems over years, these systems are still noisy across different domains. (2) Often realistic QA problems are not as simple and need additional reasoning, possibly beyond the information provide by one single SRL system. \cite{ShenLa07}'s work is among the few who use FrameNet-based SRL in order to improve QA. They formulated the problem as a bipartite matching problem which incorporates assignment of semantic roles. In this work, we manage to go beyond limitations of using single SRL annotations by creating combinations among them and with other annotations bring in an extra level of robustness to noise in knowledge. %against how the knowledge is phrased. 


%\ashish{are these still to be included?}
%\citep{novischi2006question,KaisserWe07,PizzatoMo08,MLBP11,BarHaim2008EfficientSD,szpektor2009augmenting}

%Another aspect of our work is search over space of possible textual variations (rewrites). Our system works by solving an optimization problem which models potential equivalences classes of text.

A key aspect of QA is handling textual variations, on which there has been prior work using dependency-parse transformations~\citep{PunyakanokRoYi04}. 
These approaches often define inference rules, which can generate new trees starting from a base tree. \cite{Bar-HaimDaBe15} and \cite{SSDF12} search over a space of a pre-defined set of text transformations (e.g., coreference substitutions, passive to active). Our work differs in that we consider a much wider range of textual variations by combining multiple abstractions, and make use of a more expressive inference framework.


%\section{Formulation}
\section{Knowledge Abstraction and Representation}
\label{subsec:kr}
We begin with our formalism for abstracting knowledge from text and representing it as a family of graphs, followed by specific instantiations of these abstractions using off-the-shelf NLP modules.

\subsection{Semantic Abstractions}
The pivotal ingredient of the abstraction is raw text. This representation is used for question $Q$, each answer option $A_i$ and the knowledge snippet $P$, which potentially contains the answer to the question. The KB for a given raw text, consists of the text itself, embellished with various \semanticGraph s attached to it, as depicted in Figure~\ref{fig:layers}.  
\begin{wrapfigure}{r}{0.4\textwidth}
% \begin{figure}[ht]
% \resizebox{\linewidth}{!}{
    % \centering\includegraphics[trim=0cm 10.6cm 0cm 0.0cm, clip=false, scale=0.92]{figures_semanticilp/cropped_layers-side-text2-cropped.pdf}
    \centering\includegraphics[trim=0cm 0cm 0cm 0.0cm, width=0.4 \textwidth]{figures_semanticilp/cropped_layers-side-text2-cropped.pdf}
    % }
    % \begin{framed}
        % \includegraphics[trim=10cm 2.5cm 2.6cm 15.3cm, clip=true]{figures_semanticilp/layers3.pdf}
        % \vspace{-0.72cm}
    % \end{framed}
    \caption{
    \small
    Knowledge Representation used in our formulation. Raw text is associated with a collection of \semanticGraph s, which convey certain information about the text.
    %Each layer contains a \semanticGraph.
    There are implicit similarity edges among the nodes of the connected components of the graphs, and from nodes to the corresponding raw-text spans. }
    \label{fig:layers}
% \end{figure}
\end{wrapfigure}


Each \semanticGraph\ is representable from a family of graphs. In principle there need not be any constraints on the permitted graph families; however for ease of representation we choose the graphs to belong to one of the 5 following families:
\sequence\ graphs represent labels for each token in the sentence.
\spann\ family represents labels for spans of the text.  
\treeView, is a tree representation of text spans. 
\clusterView\ family, contain spans of text in different groups. 
\predArgView\ family represents predicates and their arguments; in this view edges represent the connections between each single predicates and its arguments. Each \semanticGraph\ belongs to one of the graph families and its content is determined by the semantics of the information it represents and the text itself.

% \subsection{Representation}
We define the knowledge more formally here. For a given paragraph, $T$, its representation $\know{T}$ consists of a set of semantic graphs  $\know{T} = \setOf{g_1, g_2, \hdots}$. 
% \daniel{this might need clarification; help me fix it; basically I'm trying to say that, \verbSRL\ graph is dictated by the input text, the fact that it's a predicate argument, the fact that it is ``verb-srl" view, and it has to contain verbs and noun-phrases as its argument} 
We define $\nodes{g} = \setOf{c_i}$ and $\edges{g} = \setOf{(c_{i}, c_{j})} $ to be the set of nodes and edges of a given graph, respectively. 
% Also define the set of all nodes and edges across all annotations as $\mathcal{C}(T) = \bigcup_{g \in \know{T}} \nodes{g} $ and $\mathcal{E}(T) = \bigcup_{g \in \know{T}} \edges{g}$, respectively. 
% Given this representation, we create different classes of reasoning. 
%For each view $v$, we consider its nodes $\textbf{c}_v = \setOf{c_{j}}$ and edges $\textbf{e}_v = \setOf{(c_{i}, c_{j})}$. For a given text $T$, define the set of all nodes and edges, across all views as $\mathcal{C}(T)$ and $\mathcal{E}(T)$, respectively. 

\subsection{Semantic Graph Generators}

Having introduced a graph-based abstraction for knowledge and categorized it into a family of graphs, we now delineate the instantiations we used for each family. Many of the pre-trained extraction tools we use are available in \cogcompnlp.\footnote{Available at: http://github.com/CogComp/cogcomp-nlp}

% \vspace{-0.15cm}
\begin{itemize}[leftmargin=0.25cm]
    \item 
         \sequence\, or labels for sequence of tokens; for example \lemmaa\ and \pos\  \citep{RothZe98}. 
    \item
        \spann\ which can contains labels for spans of text; we instantiated \shallowP\ \citep{PunyakanokRo01}, \quantities\ \citep{RoyViRo15}, \ner\  \citep{RatinovRo09,RedmanSaRo16}).   
    \item 
        \treeView, a tree representation connecting spans of text as nodes; for this we used \dep\ of \cite{CUCSR15}. 
    \item 
        \clusterView, or spans of text clustered in groups. An example is \coref\ \citep{LPCCSJ11}. 
    \item 
        \predArgView; for this view we used \verbSRL\ and \nomSRL \citep{PunyakanokRoYi08,RothLa16}, \prepSRL\ \citep{SrikumarRo13}, \commaSRL\ \citep{ArivazhaganChRo16}.
\end{itemize}

Given \semanticGraph\ generators we have the question, answers and paragraph represented as a collection of graphs. Given the instance graphs, creating augmented graph will be done implicitly as an optimization problem in the next step. 



\section{QA as Reasoning Over Semantic Graphs}

We introduce our treatment of QA as an optimal subgraph selection problem over knowledge. 
We treat question answering as the task of finding the best support in the knowledge snippet, for a given question and answer pair,
measured in terms of the strength of a ``support graph'' defined as follows.

The inputs to the QA system are, a question $\know{Q}$, the set of answers $\setOf{\know{A_i}}$ and given a knowledge snippet $\know{P}$.\footnote{For simplicity, from now on, we drop ``knowledge"; e.g., instead of saying ``question knowledge", we say ``question". } Given such representations, we will form a reasoning problem, which is formulated as an optimization problem, searching for a ``support graph" that connects the question nodes to a unique answer option through nodes and edges of a snippet. 

Define the instance graph $I = I(Q, \setOf{A_i}, P)$ as the union of knowledge graphs: $I \triangleq \know{Q} \cup \paran{\know{A_i}} \cup \know{P}$. Intuitively, we would like the support graph to be connected, and to include nodes from the question, the answer option, and the knowledge. Since the \semanticGraph\ is composed of many disjoint sub-graph, we define \emph{augmented graph} $I^+$ to 
model a bigger structure over the instance graphs $I$. 
Essentially we \textit{augment} the instance graph and weight the new edges. Define a scoring function $f:(v_1, v_2) $ labels pair of nodes $v_1$ and $v_2$ with an score which represents their phrase-level entailment or similarity. 

% Next we define augmented graph: 
% Before defining such augmentation, let us first define a graph operator ``node multiplier", given a function $s$ which encodes whether two nodes are eligible alignable.  
%The \emph{augmented graph} $I^+$ is formed by adding to $I$ edges. 
% Let $G = (V,E)$ be a subgraph of $\mathcal{G}_{Q,P}$. 

% \begin{definition}[Node Multiplier]
% \label{def:graph-multiplication}
%Given a graph $G_1(V_1, E_1)$ and $G_2(V_2, E_2)$, and a constrained set $s: (.,.) \rightarrow \setOf{0, 1}$. 
%$V_1 \star_s V_2 \triangleq \setOf{ (v_1, v_2): v_1 \in V_1, v_2 \in V_2, s(v_1, v_2) = 1} $
%The multiplied graph $G'$ is defined as $G(V_1 \cup V_2, V_1 \star_S V_2 \cup E_1, \cup E_2)$
%\end{definition}

%Next we define augmented graph, given a set of functions $S = \setOf{s_1, s_2, s_3, \hdots;  s_i: (., .) \rightarrow \setOf{0, 1} }$: 

\begin{definition}
\label{def:augmented-graph}
An \emph{augmented graph} $I^+$, for a question $Q$, answers $\setOf{A_i}$ and knowledge $P$, is defined with the following properties: 
\begin{enumerate}
    \item Nodes: $\nodes{I^+} = \nodes{I(Q, \setOf{A_i}, P)}$
    \item Edges:\footnote{Define $\know{T_1} \otimes \know{T_2} \triangleq \bigcup_{\substack{ (g_1, g_2) \in \\ \know{T_1} \times \know{T_2}} } \nodes{g_1} \times \nodes{g_2}$, where $\nodes{g_1} \times \nodes{g_2} = \setOf{ (v, w); v \in \nodes{g_1}, w \in \nodes{g_2} }. $} 
    \begin{align*} 
     \edges{I^+} &= \edges{I} \cup  \know{Q} \otimes \know{P} \cup \brac{\cup_i \know{P} \otimes \know{A_i} }
    %  \bigcup_{\substack{ (X, Y) \in  \\ \setOf{(Q, P), (P, A)} } }  \bigcup_{\substack{ (g_1, g_2) \in \\ \know{X} \times \know{Y}} }\nodes{g_1} \times \nodes{g_2}    
     % \\
     %     \bigcup_{\substack{ (g_1, g_2) \in \\ \know{Q} \times \know{P}} }& \nodes{g_1} \times \nodes{g_2}  \cup \brac{ 
     %     \bigcup_{i} \bigcup_{\substack{ (g_1, g_2) \in   \know{P} \times \know{A_i}}} \nodes{g_1} \times \nodes{g_2}}     
    \end{align*} 
    % $\edges{I^+} = \edges{I(Q, \setOf{A_i}, P)} 
    % \cup \paran{ \cup_{g_1, g_2 \in (\know{Q}, \know{P})} \nodes{g_1} \times \nodes{g_2} } 
    % \cup \paran{ \cup_{g_1, g_2 \in (\know{P}, \know{A})} \nodes{g_1} \times \nodes{g_2} } 
    % $ 
    % \daniel{don't you want to constrain this set? }
    \item Edge weights: for any $e \in I^+$: 
    \begin{itemize}
      \item If $e \notin I$, the edge connects two nodes in different connected components: 
      $$
      \forall e = (v_1, v_2) \notin I : w(e) = f(v_1, v_2) 
      $$
      \item If $e \in I$, the edge belongs to a connected component, and the edge weight information about the reliability of the \semanticGraph\ and semantics of the two nodes. 
      $$
        \forall g \in I, \forall e \in g: w(e) = f'(e, g)
      $$
    \end{itemize}
\end{enumerate}
\end{definition}

Next, we have to define \textit{support graphs}, the set of graphs that support the reasoning of a question. For this we will apply some structured constraints on the augmented graph. 

\begin{definition}
\label{def:support-graph}
A \emph{support graph} $G = G(Q,\setOf{A_i}, P)$ for a question $Q$, answer-options $\setOf{A_i}$ and paragraph $P$, is a subgraph $(V,E)$ of $I^+$ with the following properties:
\begin{enumerate}
\item $G$ is connected.
\item $G$ has intersection with the question, the knowledge, and exactly one answer candidate:\footnote{$\onlyOne$ here denotes the uniqueness quantifier, meaning ``there exists one and only one".} 
$$
G \cap \know{Q} \neq \emptyset,
\hspace{0.3cm}  G \cap \know{P} \neq \emptyset,
\hspace{0.3cm}  \onlyOne \; i: G \cap \know{A_i} \neq \emptyset 
$$
% $$
% \begin{aligned}
%         & G \cap \know{Q} \neq \emptyset  \\ 
%         & G \cap \know{Q} \neq \emptyset  \\ 
%         & G \cap \know{A_i} \neq \emptyset, \;\;  \onlyOne \; i
% \end{aligned}
% $$
\item $G$ satisfies structural properties per each connected component, as summarized in Table~\ref{table:structural-properties}. 
\end{enumerate}
\end{definition}

\begin{table}
    \centering
    \small 
    \setlength\tabcolsep{10pt}
    \setlength\doublerulesep{\arrayrulewidth}
    % \resizebox{\linewidth}{!}{
    \begin{tabular}{C{2.5cm}|L{5.1cm}}
        Sem. Graph &  Property \\
        \hline\hline \bigstrut[t]
         \predArgView & Use at least (a) a predicate and its argument, or (b) two arguments  \\ 
         \hline 
         \clusterView & Use at least two nodes  \\
         \hline 
         \treeView & Use two nodes with distance less than $k$ \\ 
         \hline 
         \spanLabelView & Use at least $k$ nodes   
    \end{tabular}
    % }
    % \vspace{-0.3cm}
    \caption{Minimum requirements for using each family of graphs. Each graph connected component (e.g. a \predArgView\ frame, or a \coref\ chain) cannot be used unless the above-mentioned conditioned is satisfied. }
    \label{table:structural-properties}
\end{table}

Definition~\ref{def:support-graph} characterizes what we call a potential solution to a question. A given question and paragraph give rise to a large number of possible support graphs. We define the space of feasible support graphs as $\mathcal{G}$ (i.e., all the graphs that satisfy Definition~\ref{def:support-graph}, for a given $(Q, \setOf{A_i}, P)$).
To rank various feasible support graphs in such a large space, we define a scoring function $\score{G}$ as:
\begin{equation}
\label{eq:score-function}
%\small
%\score{G} = 
\sum_{v \in \nodes{G}} w(v) + \sum_{e \in \edges{G}} w(e) - \sum_{c \in \mathcal{C} } w_c \, \eye{c \text{ is {violated}}}
\end{equation}
for some set of preferences (or soft-constraints) $\mathcal{C}$.
{When $c$ is violated, denoted by the indicator function $\eye{c \text{ is violated}}$ in Eq.~(\ref{eq:score-function}), we penalize the objective value by some fixed amount $w_c$.}
The second term is supposed to bring more sparsity to the desired solutions, just like how regularization terms act in machine learning models \citep{Natarajan95}. The first term is the sum of weights we defined when constructing the augmented-graph, and is supposed to give more weight to the models that have better and more reliable alignments between its nodes. 
% We do this through a number of additional structural and semantic properties; the more properties the support graph satisfies, the more desirable it is. 
The role of the inference process will be to choose the ``best" one under our notion of \emph{desirable} support graphs: 
\begin{equation}
\label{eq:objective}
G^* =\argmax_{G \in \mathcal{G}}
\end{equation}

\subsection{ILP Formulation}
\label{subsec:ilp}

Our QA system, \textilp, models the above support graph search of Eq.~(\ref{eq:objective}) as an ILP optimization problem, i.e., as maximizing a linear objective function over a finite set of variables, subject to a set of linear inequality constraints. A summary of the model is given below. % \footnote{Details of the ILP model may be found in the appendix.}	

The augmented graph is not explicitly created; instead, it is implicitly created. The nodes and edges of the augmented graph are encoded as a set of binary variables. The value of the binary variables reflects whether a node or an edge is used in the optimal graph $G^*$. The properties listed in Table~\ref{table:structural-properties} are implemented as weighted linear constraints using the variables defined for the nodes and edges. 

As mentioned, edge weights in the augmented graph come from a function, $f$, which captures (soft) phrasal entailment between question and paragraph nodes, or paragraph and answer nodes, to account for lexical variability.
In our evaluations, we use two types of $f$. (a) Similar to \cite{KKSCER16}, we use a WordNet-based \citep{Miller95} function to score word-to-word alignments, and use this as a building block to compute a phrase-level alignment score as the weighted sum of word-level alignment scores.
%that computes the best word-to-word alignment between phrases, scores these alignments
Word-level scores are computed using WordNet's hypernym and synonym relations, and weighted using relevant word-sense frequency.
%, and returns the weighted sum of the scores.
$f$ for similarity (as opposed to entailment) is taken to be the average of the entailment scores in both directions. (b) For longer phrasal alignments (e.g., when aligning phrasal verbs) we use the Paragram system of \cite{WBGLR15}.


The final optimization is done on Eq.~(\ref{eq:score-function}). The first part of the objective is the sum of the weights of the sub-graph, which is what an ILP does, since the nodes and edges are modeled as variables in the ILP. The second part of Eq.~(\ref{eq:score-function}) contains a set of preferences $\mathcal{C}$, summarized in Table~\ref{tab:preferences}, meant to apply \textit{soft} structural properties that partly dependant on the knowledge instantiation. These preferences are soft in the sense that they are applied with a weight to the overall scoring function (as compare to a hard constraint). For each preference function $c$  there is an associated binary or integer variable with weight $w_c$, and we create appropriate constraints to simulate the corresponding behavior. 

\begin{table}
    \small
    \begin{framed}
    \noindent - Number of sentences used is more than $k$\\ 
    - Active edges connected to each chunk of the answer option, more than $k$ \\ 
    - More than k chunks in the active answer-option \\ 
    - More than k edges to each question constituent  \\ 
    - Number of active question-terms  \\ 
    - If using \predArgView of $\know{Q}$, at least an argument should be used  \\ 
    - If using \predArgView(\verbSRL) of $\know{Q}$, at least one predicate should be used.
    \end{framed}
    % \vspace{-0.25cm}
    \caption{The set of preferences functions in the objective. }
    % \vspace{-0.1cm}
    \label{tab:preferences}
\end{table}

We note that the ILP objective and constraints aren't tied to the particular domain of evaluation; they represent general properties that capture what constitutes a well supported answer for a given question.




%%%%%%%%%%%%%%%%%%%%%%%
\section{Empirical Evaluation}
\label{sec:experiments:semanticilp}

We evaluate on two domains that differ in the nature of the supporting text (concatenated individual sentences vs.\ a coherent paragraph), the underlying reasoning, and the way questions are framed. We show that \textilp\ outperforms a variety of baselines, including retrieval-based methods, neural-networks, structured systems, and the current best system for each domain. These datasets and systems are described next, followed by results.


\subsection{Question Sets}

For the first domain, we have a collection of question sets containing elementary-level science questions from standardized tests \citep{CEKSTTK16,KhotSaCl17}. Specifically, \regentsFourth\ contains all non-diagram multiple choice questions from 6 years of NY Regents 4th grade science exams (127 train questions, 129 test). \regentsEighth\ similarly contains 8th grade questions (147 train, 144 test). The corresponding expanded datasets are \publicFourth\ (432 train, 339 test) and \publicEighth\ (293 train, 282 test).\footnote{AI2 Science Questions V1 at http://data.allenai.org/ai2-science-questions}

For the second domain, we use the \processBank\footnote{https://nlp.stanford.edu/software/bioprocess} dataset for the reading comprehension task proposed by \cite{BSCLHHCM14}. It contains paragraphs about biological processes and two-way multiple choice questions about them. We used a broad subset of this dataset that asks about events or about an argument that depends on another event or argument.\footnote{These are referred to as ``dependency questions" by \cite{BSCLHHCM14}, and cover around 70\% of all questions.}. The resulting dataset has 293 train and 109 test questions, based on 147 biology paragraphs.

Test scores are reported as percentages. For each question, a system gets a score of $1$ if it chooses the correct answer, $1/k$ if it reports a $k$-way tie that includes the correct answer, and $0$ otherwise.


\subsection{Question Answering Systems}
\label{section:baslines}
%
We consider a variety of baselines, including the best system for each domain.

% \vspace{0.5ex}
\textbf{\lucene} (information retrieval baseline).
We use the IR solver from \cite{CEKSTTK16}, which selects the answer option that has the best matching sentence in a corpus. The sentence is forced to have a non-stopword overlap with both $q$ and $a$.


% \vspace{0.5ex}
\textbf{\textilp} (our approach). 
Given the input instance (question, answer options, and a paragraph), we invoke various NLP modules to extract semantic graphs. We then generate an ILP and solve it using the open source SCIP engine~\citep{Achterberg09}, returning the active answer option $\option$ from the optimal solution found. To check for ties, we disable $\option$, re-solve the ILP, and compare the score of the second-best answer, if any, with that of the best score.

For the science question sets, where we don't have any paragraphs attached to each question, we create a passage by using the above \lucene\ solver to retrieve scored sentences for each answer option and then combining the top 8 unique sentences (across all answer options) to form a paragraph.

{
While the sub-graph optimization can be done over the entire augmented graph in one shot, %\ashish{`we choose to create' begs the question of pros, cons, etc. Changing to something less assertive.} 
our current implementation uses multiple simplified solvers, each performing reasoning over augmented graphs for a commonly occurring annotator combination, as listed in Table~\ref{tab:combinations}. For all of these annotator combinations, we let the representation of the answers be $\know{A}=\{\shallowP, \tokens\}$. Importantly, our choice of working with a few annotator combinations is mainly for simplicity of implementation and suffices to demonstrate that reasoning over even just two annotators at a time can be surprisingly powerful. 
% \ashish{changed `due to computational issues', which sounds more serious than it is; at least we haven't run into the scalability bottleneck of the ILP itself. I think it's really more a simplicity-of-implementation issue. Rewording accordingly.} 
There is no fundamental limitation in implementing \textilp\ using one single optimization problem as stated in Eq.~(\ref{eq:objective}). 

\begin{table}
% \begin{wrapfigure}{r}{0pt}
    \small 
  \setlength\tabcolsep{2pt}
  \setlength\doublerulesep{\arrayrulewidth}
    \centering
    % \resizebox{244pt}{!}{
    % \resizebox{\linewidth}{!}{
    \begin{tabular}{c|l}
        Combination & \multicolumn{1}{c}{Representation}   \\
        \hline\hline \bigstrut[t]
         \multirow{2}{*}{
        %  \simple-alignment
            Comb-1
         } 
         
         & $\know{Q}=\{\shallowP, \tokens\}$  \\ 
           &  $\know{P}=\{\shallowP, \tokens, \dep\}$  \\ 
           \hline 
         \multirow{2}{*}{
        %  \verbSRL-alignment
            Comb-2
         } &$\know{Q}=\setOf{\verbSRL, \shallowP}$    \\ 
          & $\know{P}=\setOf{ \verbSRL }$ \\ 
         \hline 
          \multirow{2}{*}{
          % \verbSRL+\coref
            Comb-3 
          } & $\know{Q}=\setOf{\verbSRL, \shallowP}$    \\  
          &   $\know{P}=\{\verbSRL, \coref \}$  \\  
         \hline 
         \multirow{2}{*}{
            Comb-4
            % \verbSRL+\commaSRL
         } & $\know{Q}=\setOf{ \verbSRL,\shallowP}$    \\ 
          &  $\know{P}=\setOf{\commaSRL }$ \\ 
         \hline 
         \multirow{2}{*}{
        %  \verbSRL+\prepSRL
            Comb-5 
         } & $\know{Q}=\setOf{\verbSRL,\shallowP }$  \\ 
          & $\know{P}=\setOf{ \prepSRL }$ \\ 
    \end{tabular}
    % }
    % }
    % \vspace{-0.3cm}
    \caption{The semantic annotator combinations used in our implementation of \textilp. 
    % \ashish{changed; emphasizing limitation of the implementation rather than of the concept.}
    }
    %\vspace{-0.3cm}
    \label{tab:combinations}
\end{table}
% \end{wrapfigure}

Each simplified solver associated with an annotator combination in Table~\ref{tab:combinations} produces a confidence score for each answer option. We create an \emph{ensemble} of these solvers as a linear combination of these scores, with weights trained using the union of training data from all questions sets. 
%\ashish{rephrased this paragraph. I think it was not totally obvious what the ensemble is over... that we get confidence scores from each simplified solver, and use that instead of just the answer selected by each solver. Please double-check that this is accurate!}\tushar{It would help to add how the QA dataset was converted into training examples.}
}


\textbf{\bidaf} (neural network baseline).
We use the recent deep learning reading comprehension model of \cite{SKFH16}, which is one of the top performing systems on the SQuAD dataset and has been shown to generalize to another domain as well~\citep{MinSeHa17}. Since \bidaf\ was designed for fill-in-the-blank style questions, we follow the variation used by \cite{KSSCFH17} to apply it to our multiple-choice setting. Specifically, we compare the predicted answer span to each answer candidate and report the one with the highest similarity.
%\footnote{We report number for the SQuAD-trained \bidaf\ system. We also tried continuous training to fine-tune its parameters by further providing (small) training data from our domain, but that did not improve performance.}

We use two variants: the original system, \bidaf, pre-trained on 100,000+ SQuAD questions, as well as an extended version, \bidafTrained, obtained by performing continuous training to fine-tune the SQuAD-trained parameters using our (smaller) training sets. For the latter, we convert multiple-choice questions into reading comprehension questions by generating all possible text-spans within sentences, with token-length at most \textit{correct answer length + 2}, and choose the ones with the highest similarity score with the correct answer. We use the \allennlp\ re-implementation of \bidaf\footnote{Available at: https://github.com/allenai/allennlp}, train it on SQuAD, followed  by training it on our dataset. We tried different variations (epochs and learning rates) and selected the model which gives the best average score across all the datasets. As we will see, the variant that was further trained on our data often gives better results. 

\textbf{\tupleinf} (semi-structured inference baseline).
Recently proposed by \cite{KhotSaCl17}, this is a state-of-the-art system designed for science questions. It uses Open IE~\citep{BCSBE07} tuples derived from the text as the knowledge representation, and performs reasoning over it via an ILP. It has access to a large knowledge base of Open IE tuples, and exploits redundancy to overcome challenges introduced by noise and linguistic variability.

\textbf{\proread} and \textbf{\syntprox}. 
\proread is a specialized and best performing system on the \processBank\ question set. \cite{BSCLHHCM14} annotated the training data with events and event relations, and trained a system to extract the process structure. Given a question, \proread\ converts it into a query (using regular expression patterns and keywords) and executes it on the process structure as the knowledge base. Its reliance on a question-dependent query generator and on a process structure extractor makes it difficult to apply to other domains.

\syntprox\ is another solver suggested by \citep{BSCLHHCM14}. It aligns content word lemmas in both the question and the answer against the paragraph, and select the answer tokens that are closer to the aligned tokens of the questions. The distance is measured using dependency tree edges. To support multiple sentences they connect roots of adjacent sentences with bidirectional edges. 


\subsection{Experimental Results}
We evaluate various QA systems on datasets from the two domains. The results are summarized below, followed by some some insights into \textilp's behavior and an error analysis. 
\paragraph{Science Exams.}
The results of experimenting on different grades' science exams are summarized in Table~\ref{table:science}, which shows the exam scores as a percentage.  
The table demonstrates that \textilp\ consistently outperforms the best baselines in each case by 2\%-6\%. 

Further, there is no absolute winner among the baselines; while \lucene\ is good on the 8th grade questions, \tupleinf\ and \bidafTrained\ are better on 4th grade questions. This highlights the differing nature of questions for different grades. 
\begin{table}[htb]
  \centering
  \small
  \setlength\tabcolsep{2pt}
  \setlength\doublerulesep{\arrayrulewidth}
%   \resizebox{\linewidth}{!}{
  \begin{tabular}{l|cccc|c}
  Dataset & \bidaf & \bidafTrained & \lucene & \tupleinf & \textilp \\ 
  \hline\hline \bigstrut[t]
  \regentsFourth  & 56.3 & 53.1 & 59.3 & \emph{61.4} & {\bf 67.6} \\ 
  \publicFourth   & 50.7 & \emph{57.4} & 54.9 & 56.1 & {\bf 59.7} \\ 
  \regentsEighth  & 53.5 & 62.8 & \emph{64.2} & 61.3 & {\bf 66.0} \\ 
  \publicEighth   & 47.7 & 51.9 & \emph{52.8} & 51.6 & {\bf 55.9} \\ 
  \hline
  \end{tabular}
%   }
%   \vspace{-0.15cm}
  \caption{Science test scores as a percentage. On elementary level science exams, \textilp\ consistently outperforms baselines. In each row, the best score is in \textbf{bold} and the best baseline is \emph{italicized}.  }
  \label{table:science}
\end{table}

\paragraph{Biology Exam.} 
The results on the \processBank\ dataset are summarized in Table~\ref{table:bio}. While \textilp's performance is substantially better than most baselines and close to that of \proread, it is important to note that this latter baseline enjoys additional supervision of domain-specific event annotations. This, unlike our other relatively general baselines, makes it limited to this dataset,
%for this reason we are separating it from other baselines which are relatively more general across datasets.
which is also why we don't include it in Table~\ref{table:science}.

We evaluate \lucene\ on this reading comprehension dataset by creating an ElasticSearch index, containing the sentences of the knowledge paragraphs. 

\begin{table}[htb]
  \centering
  \small
  \setlength\tabcolsep{2pt}
  \setlength\doublerulesep{\arrayrulewidth}
% \resizebox{\linewidth}{!}{
  \begin{tabular}{c|cccc|c}
  \proread &  \syntprox & \lucene &  \bidaf & \bidafTrained & \textilp \\ 
  \hline\hline \bigstrut[t]
  68.1  &  61.9 & 63.8 & 58.7 & 61.3 & {\bf 67.9 }\\ 
  \hline
  \end{tabular}
%   }
%   \vspace{-0.15cm}
  \caption{Biology test scores as a percentage. \textilp\ outperforms various baselines on the \processBank\ dataset and roughly matches the specialized best method.}
  \label{table:bio}
\end{table}


\subsection{Error and Timing Analysis}
For some insight into the results, we include a brief analysis of our system's output compared to that of other systems.

We identify a few main reasons for \textilp's errors.
Not surprisingly, some mistakes
%(cf.\ Figure~\ref{fig:annotation-mistake} in the Appendix)
(see the appendix figure of~\cite{KKSR18} for an example)
% \citep{2018a_aaai_semanticilp-extended}
 can be traced back to failures in generating proper annotation (\semanticGraph). Improvement in SRL modules or redundancy can help address this. 
% The issues in soft-matching (similarity) module's failures. 
Some mistakes are from the current ILP model not supporting the ideal reasoning, i.e., the requisite knowledge exists in the annotations, but the reasoning fails to exploit it. 
Another group of mistakes is due to the complexity of the sentences, and the system lacking a way to represent the underlying phenomena with our current annotators. 

A weakness (that doesn't seem to be particular to our solver) is reliance on explicit mentions. If there is a meaning indirectly implied by the context and our annotators are not able to capture it, our solver will miss such questions. There will be more room for improvement on such questions with the development of discourse analysis systems.   

When solving the questions that don't have an attached paragraph, relevant sentences need to be fetched from a corpus. A subset of mistakes on this dataset occurs because the extracted knowledge does not contain the correct answer. 


\subsubsection{ILP Solution Properties.}
% \tushar{Maybe separate the science question set numbers from process bank numbers. Especially if you are considering different configuration settings for both. It could highlight that your model is simpler on the science exams where the paragraphs contain independent sentences}

% Implementing conditions specified in formalized of support graphs are implemented using many constraints, 
% The optimization model has around  high-level constraints, which result, on average, in around \daniel{x} inequalities over \daniel{y}variables. Model creation, which includes a large number of 
% computing pairwise entailment scores using WordNet and \paragram, takes %  \daniel{y} seconds on average per question, and the resulting ILP is solved by the SCIP engine in % \daniel{x} seconds (total for all four options), using around \daniel{x} LP iterations for each option.\footnote{Commercial ILP solvers (e.g., CPLEX, Gurobi) are much faster than the open-source SCIP solver we used for evaluations.}

Our system is implemented using many constraints, requires using many linear inequalities which get instantiated on each input instanced, hence there are a different number of variables and inequalities for each input instance. There is an overhead time for pre-processing an input instance, and convert it into an instance graph. Here in the timing analysis we provide we ignore the annotation time, as it is done by black-boxes outside our solver.

Table~\ref{tab:stats} summarizes various ILP and support graph statistics for \textilp, averaged across \processBank\ questions. Next to \textilp\ we have included numbers from \tableilp\ which has similar implementation machinery, but on a very different representation. While the size of the model is a function of the input instance, on average, \textilp\ tends to have a bigger model (number of constraints and variables). The model creation time is significantly time-consuming in \textilp\ as involves many graph traversal operations and jumps between nodes and edges. 
We also providing times statistics for \tupleinf\, which takes roughly half the time of \tableilp, which means that it is faster than \textilp.

\begin{table}[htb]
\centering
\footnotesize
\setlength\tabcolsep{5pt}
\setlength\doublerulesep{\arrayrulewidth}
% \resizebox{\linewidth}{!}{
\begin{tabular}{llccc}
\multirow{2}{*}{Category} & 
\multirow{2}{*}{Quantity} & 
Avg. & Avg. & Avg.  \\
& & { \tiny (\textilp) } & { \tiny (\tableilp) } & { \tiny (\tupleinf) } \\ 
\hline\hline \bigstrut[t]
\multirow{3}{*}{ILP complexity} & \#variables & 2254.9 & 1043.8 & 1691.0 \\
& \#constraints & 4518.7 & 4417.8 & 4440.0 \\
% & \#LP iterations & & 1348.9 \\
\hline \bigstrut[t]
\multirow{2}{*}{Timing stats} & model creation & 5.3 sec  & 1.9 sec & 1.7 sec \\
& solving the ILP & 1.8 sec   & 2.1 sec &  0.3 sec\\
\hline
\end{tabular}
% }
% \vspace{-0.15cm}
\caption{\textilp\ statistics averaged across questions, as compared to  \tableilp\ and \tupleinf\ statistics.
% \tushar{Did we consider adding \tupleinf\ numbers too here or in a footnote?}
}
\label{tab:stats}
\end{table}


\subsection{Ablation Study}
In order to better understand the results, we ablate the contribution of different annotation combinations, where we drop different combination from the ensemble model. We retrain the ensemble, after dropping each combination.

The results are summarized in Table~\ref{tab:ablation}. While Comb-1
%\shallowA-alignment 
seems to be important for science tests, it has limited contribution to the biology tests. On 8th grade exams, the \verbSRL\ and \commaSRL-based alignments provide high value. Structured combinations (e.g., \verbSRL-based alignments) are generally more important for the biology domain. 

\begin{table}[htb]
\centering
\footnotesize
\setlength\tabcolsep{5pt}
\setlength\doublerulesep{\arrayrulewidth}
% \resizebox{\linewidth}{!}{
\begin{tabular}{lC{2.2cm}C{2.2cm}}
 %& \publicFourth 
 & \publicEighth & \processBank  \\ 
\hline\hline
Full \textilp\ & 
% 59.7 &	
55.9 &	67.9 \\ 
\hline 
no Comb-1  
% \simple-alignment 
&
% -4.5  &
 -3.1 &	-1.8 \\ 
no Comb-2 
% \verbSRL-alignment
% & +0.4 
& -2.0 &	-4.6 \\ 
no Comb-3  
% \verbSRL+\coref  
% & -0.1 
& -0.6 &	-1.8 \\ 
no Comb-4 
% \verbSRL+\commaSRL 
% & +0.5 
& -3.1 &	-1.8 \\ 
no Comb-5  
% \verbSRL+\prepSRL 
% & -0.1 
& -0.1 &	-5.1 \\ 
\hline
\end{tabular}
% }
% \vspace{-0.15cm}
\caption{Ablation study of \textilp\ components on various datasets. The first row shows the overall test score of the full system, while other rows report the change in the score as a result of dropping an individual combination. The combinations are listed in Table~\ref{tab:combinations}.}
\label{tab:ablation}
\end{table}



\paragraph{Complementarity to \lucene.}
\begin{wrapfigure}{r}{0pt}
% \begin{figure}[ht]
    \centering
    %\begin{framed}
    % \includegraphics[trim=1.6cm 1.4cm 2cm 1.1cm, clip=true, scale=0.55]{figures_semanticilp/fourht_standard.png}
    % \includegraphics[trim=0.0cm 1.0cm 0.4cm 0.3cm, clip=true, scale=0.75]{figures_semanticilp/forth_smaller.png}
    \includegraphics[scale=0.75]{figures_semanticilp/forth_smaller.png}
    %\includegraphics[trim=1.6cm 1.4cm 2cm 1.1cm, clip=true, scale=0.64]{figures_semanticilp/eight_standard.png}
    %\end{framed}
    % \vspace{-0.2cm}
    \caption{Overlap of the predictions of \textilp\ and \lucene\ on 50 randomly-chosen questions from \publicFourth.
    %\tushar{Generally bar graphs are considered better than pie charts for comparing 3+ classes. Maybe just a latex table ?}
    }
    \label{fig:piechart}
% \end{figure}
\end{wrapfigure}
Given that in the science domain the input snippets fed to \textilp\ are retrieved through a process similar to the \lucene\ solver, one might naturally expect some similarity in the predictions. 
%\tushar{dropped qualities}
The pie-chart in Figure~\ref{fig:piechart} shows the overlap between mistakes and correct predictions of \textilp\ and \lucene\ on 50 randomly chosen training questions from \publicFourth. While there is substantial overlap in questions that both answer correctly (the yellow slice) and both miss (the red slice), there is also a significant number of questions solved by \textilp\ but not \lucene\ (the blue slice), almost twice as much as the questions solved by \lucene but not \textilp\ (the green slice).  




\begin{figure*}
    \centering
    % \begin{framed}
    \hspace{0.8cm}
    % \resizebox{\linewidth}{!}{
    \includegraphics[scale=0.33]{figures_semanticilp/knowledge-ensemble-big4.png}
    % }
    \hspace{0.8cm}
    %\includegraphics[scale=0.35,trim=0.6cm 0.05cm 1.4cm 0.0cm, clip=true]{figures_semanticilp/knowledge-ensemble-big3.png}
    \includegraphics[scale=0.33]{figures_semanticilp/knowledge-length-per-combo6.png}
    % \end{framed}
    % \vspace{-0.2cm}
    \caption{Performance change for varying knowledge length.}
    \label{fig:knowledge-experiment}
\end{figure*}

\subsubsection{Cascade Solvers.}
In Tables~\ref{table:science} and~\ref{table:bio}, we presented one \textit{single} instance of \textilp\ with state-of-art results on multiple datasets, where the solver was an ensemble of semantic combinations (presented in Table~\ref{tab:combinations}). Here we show a simpler approach that achieves stronger results on individual datasets, at the cost of losing a little generalization across domains. 
Specifically, we create two ``cascades'' (i.e., decision lists) of combinations, where the ordering of combinations in the cascade is determined by the training set precision of the simplified solver representing an annotator combination (combinations with higher precision appear earlier). One cascade solver targets science exams and the other the biology dataset.

The results are reported in Table~\ref{table:cascade}. On the 8th grade data, the cascade solver created for science test achieves higher scores than the generic ensemble solver. Similarly, the cascade solver on the biology domain outperforms the ensemble solver on the \processBank\ dataset.

% \begin{table}[htb]
\begin{wrapfigure}{r}{0.6\textwidth}
  \centering
  \small
  \setlength\tabcolsep{5pt}
  \setlength\doublerulesep{\arrayrulewidth}
%   \resizebox{244pt}{!}{
% \resizebox{\linewidth}{!}{
\setlength\extrarowheight{-8pt}
  \begin{tabular}{cl|ccc}
  \multicolumn{2}{c|}{Dataset} & Ensemble & \specialcell{Cascade \\(Science)} & \specialcell{Cascade \\(Biology)} \\ 
  \hline\hline \bigstrut[t]
   \parbox[t]{2ex}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Science}}} 
   &  \regentsFourth  & {\bf 67.6} & 64.7 & 63.1 \\ 
   & \publicFourth   & {\bf 59.7} & 56.7 & 55.7\\ 
   & \regentsEighth  & 66.0 & {\bf 69.4} & 60.3 \\ 
   & \publicEighth   & 55.9 & {\bf 56.5 } & 54.3 \\ 
  \hline 
    & \processBank   & 67.9 & 59.6 & {\bf 68.8 } \\ 
  \hline
  \end{tabular}
%   }
    % \vspace{-0.2cm}
    \makeatletter\def\@captype{table}\makeatother% "Change float to table"
  \caption{
    Comparison of test scores of \textilp\ using a generic ensemble vs.\ domain-targeted cascades of annotation combinations. 
    %\ashish{updated to be more concrete}
  }
  \label{table:cascade}
% \end{table}
\end{wrapfigure}


\paragraph{Effect of Varying Knowledge Length.}
%
We analyze the performance of the system as a function of the length of the paragraph fed into \textilp, for 50 randomly selected training questions from the \regentsFourth\ set. Figure~\ref{fig:knowledge-experiment} (left) shows the overall system, for two combinations introduced earlier, as a function of knowledge length, counted as the number of sentences in the paragraph.

As expected, the solver improves with more sentences, until around 12-15 sentences, after which it starts to worsen with the addition of more irrelevant knowledge. While the cascade combinations did not show much generalization across domains, they have the advantage of a smaller drop when adding irrelevant knowledge compared to the ensemble solver. This can be explained by the simplicity of cascading and minimal training compared to the ensemble of annotation combinations. 

Figure~\ref{fig:knowledge-experiment} (right) shows the performance of individual combinations as a function of knowledge length.
It is worth highlighting that while Comb-1
% \shallowA\ alignment 
(blue) often achieves higher coverage and good scores in simple paragraphs (e.g., science exams), it is highly sensitive to knowledge length. On the other hand,  highly-constrained combinations have a more consistent performance with increasing knowledge length, at the cost of lower coverage. 

\section{Summary and Discussion}
This chapter extends our abductive reasoning system from Chapter 3 to consume raw text as input knowledge. This is the first system to successfully use a wide range of semantic abstractions to perform a high-level NLP task like Question Answering. 
% We propose a novel method for exploiting the semantic structure of text to answer multiple-choice questions. 
The approach is especially suitable for domains that require reasoning over a diverse set of linguistic constructs but have limited training data. To address these challenges, we present the first system, to the best of our knowledge, that reasons over a wide range of semantic abstractions of the text, which are derived using off-the-shelf, general-purpose, pre-trained natural language modules such as semantic role labelers. Representing multiple abstractions as a family of graphs, we translate question answering (QA) into a search for an optimal subgraph that satisfies certain global and local properties. This formulation generalizes several prior structured QA systems. Our system, \textilp, demonstrates strong performance on two domains simultaneously. In particular, on a collection of challenging science QA datasets, it outperforms various state-of-the-art approaches, including neural models, broad coverage information retrieval, and specialized techniques using structured knowledge bases, by 2\%-6\%. 

A key limitation of the system here is that its abstractions are mostly extracted from explicit mentions of in a given text. However, a major portion of our understanding come is only implied from text (not directly mention). We propose a challenge dataset for such questions (limited to the \emph{temporal} domain) in Chapter 7. Additionally, the two systems discussed in Chapter 3 and here, lack explicit explicit attention mechanism to the content of the questions. We study this topic in Chapter 5.


% The system makes use of a wide range of semantic abstractions of the text, which are derived using off-the-shelf and general-purpose natural language modules such as semantic-role labelers. This is the first system that †hat successfully uses a wide  
% Departing from the currently popular paradigm of generating a very large dataset and learning ``everything'' from it in an end-to-end fashion, we  demonstrate that one can successfully leverage pre-trained NLP modules to extract a sufficiently complete linguistic abstraction of the text that allows answering interesting questions about it. This approach is particularly valuable in settings where there is a small amount of data. Instead of exploiting peculiarities of a large but homogeneous dataset, as many state-of-the-art QA systems end up doing, we focus on confidently performing certain kinds of reasoning, as captured by our semantic graphs and the ILP formulation of support graph search over them. Bringing these ideas to practice, our system, \textilp, achieves state-of-the-art performance on two domains with very different characteristics. 
% , outperforming both traditional and neural models.
    




==> Daniel K - thesis - dissertation/3.essentialterms_new.tex <==
\chapter{Learning Essential Terms in Questions}
\epigraph{ 
``The trouble with Artificial Intelligence is that computers don't give a damn-or so I will argue by considering the special case of understanding natural language.''
}{--- \textup{John Haugeland}, 1979}


\newcommand\T{\rule{0pt}{2.6ex}}       % Top strut
\newcommand\B{\rule[-1.2ex]{0pt}{0pt}} % Bottom strut

%%%%%%%%%%%
\section{Overview}

Many of today's QA systems 
% These QA systems, however, 
often struggle with seemingly simple questions because they are unable to reliably identify which question words are redundant, irrelevant, or even intentionally distracting.\footnote{This chapter is based on the following publication: \cite{KKSR17}} This reduces the systems' precision and results in questionable ``reasoning'' even when the correct answer is selected among the given alternatives. The variability of subject domain and question style makes identifying essential question words challenging. Further, essentiality is context dependent---a word like `animals' can be critical for one question and distracting for another.
%
% These QA systems, however, generally do not exploit the diverse value of information of different elements of the question, especially as the questions get longer. The variability of subject domain and question style makes it difficult to identify what the question is really about, and which terms\footnote{The word `term' here refers to question words or tokens. The ideas apply equally well to chunks, phrases, etc.} in the question are redundant, irrelevant, or even intentionally distracting. This reduces the system's precision and yields questionable ``reasoning'' even when the correct answer is selected among the given alternatives.
%
Consider the following example:
%
%\vspace{-0.20cm}
\FrameSep2pt
\begin{framed}
\small 
\noindent 
One way animals usually respond to a sudden drop in temperature is by (A) sweating (B) shivering (C) blinking (D) salivating. 
\end{framed}
%\vspace{-0.20cm}
%
\noindent 
The system we discussed in Chapter 3, 
% A state-of-the-art optimization based QA system called 
\tableilp~\citep{KKSCER16}, which performs reasoning by aligning the question to semi-structured knowledge, aligns only the word `animals' when answering this question. Not surprisingly, it chooses an incorrect answer. The issue is that it does not recognize that ``drop in temperature" is an \ess\ aspect of the question. 
%Ideally to induce such an attentive decision making into a solver one has to have the knowledge is the key elements of the question. 

\begin{wrapfigure}{r}{0.48\textwidth}
% \begin{figure}[tb]
  \centering
  \vspace{-1.1cm}
  \includegraphics[trim={0.1cm 0.1cm 0.1cm 1.6cm}, clip=true, scale=0.7]{figures_essential_terms/essentiality2.pdf}
  %\vspace*{-0.6cm}
  \vspace{-.5cm}
  \caption{\label{fig:scores-example} 
  \footnotesize
  Essentiality scores generated by our system, which assigns high essentiality to ``drop" and ``temperature".
  }
% \end{figure}
\end{wrapfigure}
Towards this goal, we propose a system that can assign an essentiality score to each term in the question. For the above example, our system generates the scores shown in Figure~\ref{fig:scores-example}, where more weight is put on ``temperature" and ``sudden drop". A QA system, when armed with such information, is expected to exhibit a more informed behavior.



We make the following contributions:

(A) We introduce the notion of \emph{question term \essty} and release a new dataset of 2,223 crowd-sourced essential term annotated questions (total 19K annotated terms) that capture this concept.\footnote{\label{footnote1} Annotated dataset and classifier available at
\url{https://github.com/allenai/essential-terms}
} We illustrate the importance of this concept by demonstrating that humans become substantially worse at QA when even a few essential question terms are dropped.

(B) We design a classifier that is effective at predicting question term essentiality. The F1 (0.80) and per-sentence mean average precision (MAP, 0.90) scores of our classifier supercede the closest baselines by 3\%-5\%. Further, our classifier generalizes substantially better to unseen terms.

(C) We show that this classifier can be used to improve a surprisingly effective IR based QA system~\citep{CEKSTTK16} by 4\%-5\% on previously used question sets and by 1.2\% on a larger question set.
We also incorporate the classifier in \tableilp~\citep{KKSCER16}, resulting in fewer errors when sufficient knowledge is present for questions to be meaningfully answerable.

% We also explore \tableilp, whose semi-structured reasoning already performs well. While there wasn't an overall improvement, we show 42\% error reduction on a small synthetic set of questions with sufficient knowledge to be meaningfully ``answerable'' by \tableilp.


\ignore{
We take a supervised learning approach for identifying \emph{terms of a question that are \ess\ to answering it correctly}. Arguably, whether a particular term is \ess\ or not is somewhat subjective. Instead of attempting to define this concept formally, we use crowdsourcing based on certain broad guidelines in order to obtain an annotated dataset, thereby capturing human intuition about what is essential. 
%\ashish{Drop the rest of this paragraph and go straight to the contribution bullets, which repeat the same info?} We then train a max-margin based classifier on this dataset. Finally, we demonstrate that the resulting information can be incorporated in multiple systems to improve end-to-end QA performance.

We make three contributions:
%
(1) \textbf{Term-Essentiality Dataset}:
%We study 
%\ashish{Didn't like `define' or `introduce'. `Study' is a possibility.}
%    the notion of \textit{term-essentiality} for question answering, and
We introduce a dataset of over 2,200 questions with annotated \ess\ terms.
    %\ashish{1. is 2K `large' enough by today's standards? 2. is the contribution the annotation or the release of an annotated dataset?} \daniel{1. With this level of annotation, I think 2K is `relatively large`. 2. The latter.  } \ashish{1. I would say drop 'relatively large'; just say 'a dataset'. 2. Let's then change 'we annotate' to 'we introduce/release/provide an annotated dataset of ...'}
    We also validate the notion of term essentiality via a more refined (but expensive to annotate) notion of term-group essentiality.
%
    (2) \textbf{ET Classifier}: We demonstrate that a new max-margin essential terms (ET) classifier trained on the above dataset significantly outperform supervised and unsupervised baselines.
     %\ashish{here and elsewhere: the footnote command should start after the punctuation mark \emph{without} a space; changed here}
    %We create a system that is able to learn this dataset \ashish{`learn a dataset': odd phrase} to a large extent.\footnote{Both the dataset and the trained classifier will be made publicly available.}
%
    (3) \textbf{Enhancing QA Systems}: First, we illustrate sensible behavior of the above ET classifier as a sub-component of a model-agnostic ``oracle'' QA system that has humans in the loop. Second, for a state-of-the-art \lucene\ based QA system mentioned earlier, we demonstrate improved performance across multiple datasets. Third, for \tableilp, a constraint-based solver mentioned earlier, we didn't achieve an overall improvement in score but provide a tunable precision-recall tradeoff and a detailed analysis in support of more informed QA.
    %we used our system to tune it towards higher precision. 
    % \ashish{investigation is generally not a contribution; the outcome / insights from it are. we should articulate that here instead}
    % \daniel{Updated; how about now?}
    %\ashish{Once \tableilp\ story is clear, add the main claim about it in this bullet or as a 4th bullet.}
}

% The paper is structured as follows: \s2 describes our annotation process, \s3 delineates our \et\ classifier trained on the annotated data, and \s4 discusses how to effectively use this as a sub-component of QA systems. 


%%%%%%%%%%%%%%%%
\subsection{Related Work}

Our work can be viewed as the study of an intermediate layer in QA systems.
%To the best of our knowledge, there is no prior work modelling or analyzing this layer directly \tushar{The remaining related work section contradicts this line. Drop it ?}. 
Some systems implicitly model and learn it, often via indirect signals from end-to-end training data. For instance, Neural Networks based models \citep{WangLiZh16,TymoshenkoBoMo16,YinEbSc16} implicitly compute some kind of \emph{attention}. While this is intuitively meant to weigh key words in the question more heavily,
%whether this actually happens in practice 
this aspect hasn't been systematically evaluated, in part due to the lack of ground truth annotations.
%\ashish{Does attention (e.g., memory networks) generally apply to the background knowledge? or does it apply to the question as well?}

There is related work on extracting \emph{question type} information \citep{LiRo02,LZYZ07} and applying it to the design and analysis of end-to-end QA systems \citep{MPHS03}. 
%, which is often followed by extraction of key question terms, according to the type of the question. 
The concept of term \essty\ studied in this work is
%broader\tushar{Its a different task, not necessarily broader. It would be broader if we extracted answer type and other information from the question.} than question type. Also, 
different, and so is
our supervised learning approach compared to the typical rule-based systems for question type identification.
%This is often used in the rule-based systems, which tend to suffer from poor recall.

% harabagiu2000falcon  


Another line of relevant work is sentence  compression \citep{ClarkeLa08}, where the goal is to minimize the content while maintaining grammatical soundness. These approaches typically build an internal importance assignment component to assign significance scores to various terms, which is often done using language models, co-occurrence statistics, or their variants \citep{KnightMa02,HoriSa04}. We compare against unsupervised  baselines inspired by such importance assignment techniques. 

In a similar spirit,~\cite{ParkCr15} use translation models to extract key terms to prevent semantic drift in query expansion.

One key difference from general text summarization literature is that we operate on questions, which tend to have different essentiality characteristics than, say, paragraphs or news articles. As we discuss in Section~\ref{subsec:dataset}, typical indicators of essentiality such as being a proper noun or a verb (for event extraction) are much less informative for questions. Similarly, while the opening sentence of a Wikipedia article is often a good summary, it is the last sentence (in multi-sentence questions) that contains the most pertinent words.

In parallel to our effort, \citet{JSSC17} recently introduced a science QA system that uses the notion of \emph{focus words}. Their rule-based system incorporates grammatical structure, answer types, etc. We take a different approach by learning a supervised model using a new annotated dataset. 

%\daniel{review the subsection again, and potentially re-order the paragraphs. }


%%%%%%%%%%%%%%%%%
%\section{Dataset of \Ess\ Terms}
\section{Essential Question Terms}
\label{sec:essential-terms}

In this section, we introduce the notion of \emph{essential question terms}, present a dataset annotated with these terms, and describe two experimental studies that illustrate the importance of this notion---we show that when dropping terms from questions, humans' performance degrades significantly faster if the dropped terms are essential question terms.

Given a question $q$, we consider each non-stopword token in $q$ as a candidate for being an essential question term. Precisely defining what is essential and what isn't is not an easy task and involves some level of inherent subjectivity. We specified  \emph{three broad criteria}: 1) altering an \ess\ term should change the intended meaning of $q$,  2) dropping non-\ess\ terms should not change the correct answer for $q$, and 3) grammatical correctness is not important. We found that given these relatively simple criteria, human annotators had a surprisingly high agreement when annotating elementary-level science questions. Next we discuss the specifics of the crowd-sourcing task and the resulting dataset.


\subsection{Crowd-Sourced Essentiality Dataset}
\label{subsec:dataset}

We collected 2,223 elementary school science exam questions for the annotation of \ess\ terms. This set includes the questions used by \citet{CEKSTTK16}\footnote{These are the only publicly available state-level science exams. http://www.nysedregents.org/Grade4/Science/} and additional ones obtained from other public resources such as the Internet or textbooks. %$^{1}$
%\footnotemark[\getrefnumber{footnote1}] 
For each of these questions, we asked crowd workers\footnote{We use Amazon Mechanical Turk for crowd-sourcing.} to annotate essential question terms based on the above criteria as well as a few examples of essential and non-essential terms. \f\ref{fig:mturk:interface} depicts the annotation interface.

\begin{figure*}[tb]
    \centering
    \begin{framed}
        \includegraphics[trim=0cm 0.6cm 0cm 0.3cm, clip=true, scale=0.25]{figures_essential_terms/mturk2.png}
    \end{framed}
    %\vspace{-0.5cm}
    \caption{Crowd-sourcing interface for annotating \ess\ terms in a question, including the criteria for \essty\ and sample annotations.}
    \label{fig:mturk:interface}
\end{figure*}

%Given these guidelines, the group intelligence of annotators 
% implicitly defines the notion of \essty, as long as there is agreement among annotators.
% \f\ref{fig:mturk:interface} depicts the interface shown to the annotators.
%which includes our guidelines and examples.
% For each question, we ask annotators to mark each non-stopword token that they believe to be essential as per the above criteria.

\ignore{
\begin{table}[t]
    \setlength\doublerulesep{\arrayrulewidth}
    \small
    \centering
    \begin{tabular}{lc}
        \multicolumn{1}{c}{Statistic} & Value \\ 
        \hline 
        \hline 
        \# of annotated questions &  2,223 \\ 
        \# of annotated question terms & 19,380 \\ 
        \hline
        most frequent essential POS & NN \\
        question terms marked essential (avg.) & 29.9\%\\
        science terms marked essential & 76.6\%\\
        \ashish{add more}
        \\
        % \# of questions with at least\footnote{Due to unintentional repetition of question, 79 questions received 10 annotators.} 5 annotators & 2,199 \\ 
        % \# of questions with 4 annotators & 21 \\ 
        % \# of questions with 3 annotators & 4 \\ 
        % \# of questions with 1 or 2 annotators & 0 \\ 
        %\# of terms with 1 annotators & \\ 
        %\hline 
        %avg. agreement with maj. vote &  0.91 \\
        %avg. agreement with maj. vote, when it is \ess\ & 0.84  \\
        \hline 
    \end{tabular}
    % \vspace{-.3cm}
    \caption{Annotation statistics. 2,199 questions received at least 5 annotations (79 received 10 annotations due to unintended question repetition), 21 received 4 annotations, and 4 received 3 annotations.     \daniel{Ashish: The percentage for NN is, among the essential terms, how often its label is NN. Although it can be misinterpreted as how often a word with POS=NN was essential. } }
    \label{tab:annotationStatistics}
\end{table}

\ta\ref{tab:annotationStatistics} summarizes key statistics of the annotated data.
}

The questions were annotated by 5 crowd workers,\footnote{A few invalid annotations resulted in about 1\% of the questions receiving fewer annotations. 2,199 questions received at least 5 annotations (79 received 10 annotations due to unintended question repetition), 21 received 4 annotations, and 4 received 3 annotations.} and resulted in 19,380 annotated terms. The Fleiss' kappa statistic \citep{Fleiss71} for this task was $\kappa$ = 0.58, indicating a level of inter-annotator agreement very close to `substantial'. In particular, all workers agreed on 36.5\% of the terms and at least 4 agreed on 69.9\% of the terms. We use the proportion of workers that marked a term as essential to be its annotated essentiality score.

On average, less than one-third (29.9\%) of the terms in each question were marked as essential (i.e., score $>$ 0.5). This shows the large proportion of distractors in these science tests (as compared to traditional QA datasets), further showing the importance of this task.
%64.47\% of the non-stopword tokens marked as essential.
%63.3\% of the essential terms were common nouns (NN, NNS) and 19.3\% were verbs.
Next we provide some insights into these terms.

We found that part-of-speech (POS) tags are not a reliable predictor of \essty, making it difficult to hand-author POS tag based rules. Among the proper nouns (NNP, NNPS) mentioned in the questions, fewer than half (47.0\%) were marked as essential. This is in contrast with domains such as news articles where proper nouns carry perhaps the most important information.
Nearly two-thirds (65.3\%) of the mentioned comparative adjectives (JJR) were marked as essential, whereas only a quarter of the mentioned superlative adjectives (JJS) were deemed essential. Verbs were marked essential less than a third (32.4\%) of the time. This differs from domains such as math word problems where verbs have been found to play a key role \citep{HHEK14}.

The best single indicator of essential terms, not surprisingly, was being a scientific term\footnote{We use 9,144 science terms from \citet{KKSCER16}.} (such as \emph{precipitation} and \emph{gravity}). 76.6\% of such terms occurring in questions were marked as essential. 


% In order to assess task clarity and annotator agreement, we consider majority vote as a metric. This dataset turns out to have a reasonable level of agreement. Specifically, the average agreement with majority vote is 0.91 across all terms, and  0.84 over the ones with a majority vote of \ess.\footnote{We average across the terms in a sentence and then average across all sentences.}
% %This indicates a reasonable level of agreement between annotators.
% %On similar study, we plot the scores we get from the annotations. Based the total number of people annotated a term as \Ess\ and the total number of annotations, we create an raw/gold \essty\ for each terms. 
% Finally, for each term, we consider the fraction of annotators that marked it as \ess\ as its ground truth \essty\ score. \f\ref{fig:scoreHistogram} shows the distribution of these scores across all terms. E.g., all 5 annotators agreed that XX out of YY terms are highly essential.\ashish{Change figure to have fractional scores on the x-axis; or change discussion to match figure.}
% %A significant number of the annotation scores are close to the two extremes, further confirming the high level of agreement between the annotators. 
% %This indicates that Turkers were generally able to discriminate between the two classes and the annotations can be used to learn a classifier.

In summary, we have a term essentiality annotated dataset of 2,223 questions. We split this into train/development/test subsets in a 70/9/21 ratio, resulting in 483 test sentences
%where statistical significance at p $<$ 0.05 is 4.5\%.
%\daniel{Ashish: test set was bigger; update the sig. margin?}\tushar{AS: doesn't it depend on the actual mean for the binomial test}\ashish{indeed, tricky as it's not a binary task; commenting it out}
used for per-question evaluation.

We also derive from the above an annotated dataset of 19,380 terms by pooling together all terms across all questions. Each term in this larger dataset is annotated with an essentiality score in the context of the question it appears in. This results in 4,124 test instances (derived from the above 483 test questions)%, statistical significance over which at p $<$ 0.05 is 1.4\% \tushar{Cite/verify}.
. We use this dataset for per-term evaluation.


% \begin{figure}[ht]
%     \centering
%     %  \begin{framed}
%     \includegraphics[trim=4.6cm 11.1cm 4cm 11.25cm, clip=true, scale=0.47]{figures_essential_terms/hist.pdf}
% %    \includegraphics[trim=4.6cm 11.0cm 0cm 11.5cm, clip=true, scale=0.6]{histogramOfLabels2.pdf}
%     %  \end{framed}
%     %\begin{framed}
%     % \includegraphics[trim=3.3cm 8.7cm 0cm 9.1cm, clip=true, scale=0.3]{histogramOfLabels2.pdf}
%     % \end{framed}
%     \vspace{-0.4cm}
%     \caption{Distribution of the terms based on the number of times marked as \ess. 
%     %Histogram of the crowdsourced scores \todo{larger fonts} %\daniel{replaced the fig; see if it's better now. }
%     }
%     \label{fig:scoreHistogram}
% \end{figure}

%In overall it seems there is some agreement among the annotators, which at least indicates the different people have similar understanding of the task defined, which is clearly a necessary condition for learnabitliy of the output annotations.


%\subsection{Essentiality for Human QA}
\subsection{The Importance of \Ess\ Terms}

Here we report a second crowd-sourcing experiment that validates our hypothesis that the question terms marked above as essential are, in fact, essential for understanding and answering the questions. Specifically, we ask: \emph{Is the question still answerable by a human if a fraction of the essential question terms are eliminated?}
%\tushar{Added to combine old 4.1 with 2.2}
%While the Turkers label the terms in the question based on their assumptions of essentiality, the marked terms are actually essential for answering the question. Ideally the essential terms, when dropped, would make the question unanswerable for a human.
For instance, the sample question in the introduction is unanswerable when ``drop'' and ``temperature'' are removed from the question: \textit{One way animals usually respond to a sudden * in * is by \_\_\_?}
%Here, we show that our annotations as well as the learned classifier (presented in Section \ref{sec:ET}) scores do capture such sets based on the per-token labels. 

\begin{figure*}[ht]
    \centering
    \begin{framed}
            \includegraphics[trim=0cm 1.3cm 0cm 0.4cm, clip=true, scale=0.307]{figures_essential_terms/mturk-experiment.png}
    \end{framed}
    %\vspace{-0.5cm}
    \caption{Crowd-sourcing interface for verifying the validity of \essty\ annotations generated by the first task. Annotators are asked to answer, if possible, questions with a group of terms dropped.}
    \label{fig:mturk:interface:group}
\end{figure*}

To this end, we consider both the annotated essentiality scores %\footnote{Fraction of annotators that marked a term as essential.} 
 as well as the score produced by our trained classifier (to be presented in Section \ref{sec:ET}).
We first generate candidate sets of terms to eliminate using these \essty\ scores based on a threshold $\xi \in \{0, 0.2, \hdots, 1.0\}$: (a) \textbf{essential set}: terms with score $\geq \xi$; (b) \textbf{non-essential set}: terms with score $< \xi$.
%We perform a second crowdsourcing task to verify that the essential set is needed for answering a question and the non-essential set has little impact on the question answering ability of humans.  Specifically,
We then ask crowd workers to try to answer a question after replacing each candidate set of terms with ``***". In addition to four original answer options, we now also include ``I don't know. The information is not enough" (cf.\ Figure~\ref{fig:mturk:interface:group} for the user interface).\footnote{It is also possible to directly collect essential term groups using this task. However, collecting such sets of essential terms would be substantially more expensive, as one must iterate over exponentially many subsets rather than the linear number of terms used in our annotation scheme.} For each value of $\xi$, we obtain 
$5 \times 269$ 
annotations for 
269
questions. We measure how often the workers feel there is sufficient information to attempt the question and, when they do attempt, how often do they choose the right answer.


\begin{wrapfigure}{r}{0.5\textwidth}
% \begin{figure}[ht]
%\begin{framed}
    %\includegraphics[trim={2.5cm 8cm 0cm 8.9cm}, clip=true, scale=0.44]{figures_essential_terms/questionLevelExperiment.pdf}
    %\includegraphics[trim={3.6cm 9.9cm 0cm 9.7cm}, clip=true, scale=0.55]{figures_essential_terms/questionLevelExperiment2.pdf}
    %\includegraphics[trim={4cm 10.3cm 0cm 9.7cm}, clip=true, scale=0.58]{figures_essential_terms/questionLevelExperiment3.pdf}
    \includegraphics[trim={4cm 10.2cm 0cm 9.9cm}, clip=true, scale=0.60]{figures_essential_terms/questionLevelExperiment4.pdf}
%\end{framed}
    \caption{
        \footnotesize
        The relationship between the fraction of question words dropped and the fraction of the questions attempted (fraction of the questions workers felt comfortable answering). Dropping most essential terms (blue lines) results in very few questions remaining answerable, while least essential terms (red lines) allows most questions to still be answerable. Solid lines indicate human annotation scores while dashed lines indicate predicted scores. 
        %\tushar{Daniel can you relabel this figure to use "drop" instead of "keep" in the legend ? Everywhere in text and axis we refer to terms being dropped, so it would help to use the same verb.}\ashish{also, increase font size} \daniel{done. Good?}
    }
    \label{fig:combinedDropTerms}
% \end{figure}
\end{wrapfigure}
Each value of $\xi$ results in some fraction of terms to be dropped from a question; the exact number depends on the question and on whether we use annotated scores or our classifier's scores. In Figure~\ref{fig:combinedDropTerms}, we plot the average fraction of terms dropped on the horizontal axis and the corresponding fraction of questions attempted on the vertical axis. Solid lines indicate annotated scores and dashed lines indicate classifier scores. Blue lines (bottom left) illustrate the effect of eliminating essential sets while red lines (top right) reflect eliminating non-essential sets.

We make two observations. First, the solid blue line (bottom-left) demonstrates that dropping even a small fraction of question terms marked as essential dramatically reduces the QA performance of humans. E.g., dropping just 12\% of the terms (with high  essentiality scores) makes 51\% of the questions unanswerable. The solid red line (top-right), on the other hand, shows the opposite trend for terms marked as not-essential: even after dropping 80\% of such terms, 65\% of the questions remained answerable.

Second, the dashed lines reflecting the results when using scores from our \et\ classifier are very close to the solid lines based on human annotation. This indicates that our classifier, to be described next, closely captures human intuition.

% If we have a good definition of essentiality, dropping even a small fraction of terms from the \textbf{essential set} would leave most of the questions unanswerable as we see with the blue curve for both the MTurk and learned scores. Similarly, dropping a large fraction of terms from a \textbf{non-essential set} should result in most questions being answerable as seen with the red curves. %If we drop only 12\% of the terms based on the annotation score, the workers were unable to answer 51\% of the questions, showing the value of these annotations.
%  This verifies that our per-term annotations are a cost-effective yet useful \emph{approximation} of the essential group of terms for a question.
 



\ignore{
% \subsection{Verifying the correctness of annotation}
\subsection{Validation via Group Essentiality} 

\tushar{Do we need the next sub-section ?}

There is no a priori guarantee that our annotation mechanism will result in well-defined %\ashish{`reasonable' is fuzzy; but I'm not sure what else to put here. do we want consistency? meaningfulness?} %\daniel{not sure how not to be fuzzy here. Maybe the example later will clarify things?} \daniel{Dan suggested `well-defined`} \ashish{Sounds better. Changing.}
scores. It's quite possible that per-token annotations might not capture correlation between terms. In fact, a clearer definition of \ess\ terms is perhaps via term-\textit{groups} (rather than per-token judgments): \emph{a term-group $G$ is essential for a question $Q$ if dropping $G$ from $Q$ leaves insufficient information to answer $Q$}.
%The groups resulting in the least number of correct answers are arguably more \ess. 
%\daniel{give example?} \ashish{definitely! re-use a previously introduced question so readers can see the contrast} \daniel{added the followings; see if it reads well?} 
Clearly, if $G$ is essential, so are its supersets, but not necessarily its subsets. For instance, here are a few annotated term-groups for the example discussed in the introduction: 
%For the example discussed in the introduction, one might want the following \esty\ group annotations:
%To illustrate this point, here are essentiality scores \ashish{Where are these scores coming from? Annotation or estimated using per-token scores?} for a few term-groups: 

{
\small 
\indent $\set{\text{``animals"}} \rightarrow$ not essential\\
\indent $\set{\text{``animals", ``sudden drop"}} \rightarrow$ essential \\ 
\indent $\set{\text{``animals", ``temperature"}}\rightarrow$ not essential \\
\indent $\set{\text{``animals", ``sudden drop", ``temperature"}}\rightarrow$ essential
}

%The last row in the example above shows an essential-term group, however the subsets of this set might be essential.
%\ashish{Reworded a few things in this para and the next.} 
While such a group-based representation is more natural, its annotation mechanism is substantially more expensive, as one must iterate over exponentially many subsets rather than a linear number of individual terms.
%An ideal annotation mechanism for such a representation is to drop a \textit{group} of terms and ask workers to answer it, which would result in exponentially many annotation candidates.

To address this challenge, we use our per-token annotation and a per-token learning model (next section) to create candidates for essential groups. 
%as an \emph{approximation}, and 
We then perform a smaller scale crowdsourcing task to verify that term-groups composed of terms marked essential during per-term annotation are indeed essential for answering the question. This verifies that our per-term annotations provide a cost-effective yet useful \emph{approximation} of term-group annotation.

Specifically, in this second task, we ask annotators to answer a question after replacing some of the terms with ``***". In addition to four original answer options, we include ``I don't know. The information is not enough" (Figure~\ref{fig:mturk:interface:group}). 
Candidate term-groups are generated in two ways: For a threshold $\xi$, we keep terms with per-token \essty\ score (a) at least $\xi$ and (b) less than $\xi$.
For each of these settings and for $\xi \in \{0, 0.2, \hdots, 1.0\}$, we repeat the experiment, keeping track of the number of questions attempted, i.e., where the new ``I don't know'' option wasn't selected.

Intuitively, we expect a much higher number of question attempted in scenario (a) compared to scenario (b). 
Figure~\ref{fig:droppQuestionTerms} shows the relationship between the fraction of question words dropped and the resulting number of questions workers felt comfortable answering. 
%\todo{say sth more interesting about the figure?} \ashish{may be point out a couple of specific numbers that quantify the message?}
Interestingly, when term-groups comprising only 12\% of the terms, marked ``highly essential'', were dropped from the question, the workers felt there wasn't enough information left to answer 51\% of the questions, showing the value of these annotations. On the other hand, even after dropping 80\% of the terms, ranking low on the essentiality score, the workers answered around 65\% of the questions.
%We show that we can approximate the essential term-group by just using the top K essential terms with linear annotation cost.
%Tushar: I changed this line to the one above. Indeed, seeing that workers answered only 49\% of the questions when 12\% of the ``highly essential" terms were dropped is a good signal that there is value in these annotations. This attest to the value of our per-token annotations. 

% \begin{figure}[ht]
%     \centering 
%     %\begin{framed}    
%         %\includegraphics[scale=0.16]{figures_essential_terms/questionLevelExperiment.png}
%         %\includegraphics[trim={2.5cm 8.3cm 0cm 9cm}, clip=true, scale=0.44]{figures_essential_terms/questionLevelExperiment-onlyAnnotation.pdf}
%     %\end{framed}
%     %\begin{framed}
%         \includegraphics[trim={4.9cm 10.3cm 0cm 11cm}, clip=true, scale=0.65]{figures_essential_terms/questionLevelExperiment-onlyAnnotation2.pdf}
%     %\end{framed}
%     \vspace{-0.8cm}
%     \caption{
%     %\ashish{increase font size} 
%     %\ashish{The caption repeats info from the relevant paragraph. Skip that, instead say one sentence about the main outcome/message} Verifying the validity of our \essty\ annotations. 
%     %We ask the annotators to answer questions with some of the terms dropped. We devise two strategies for dropping terms: dropping terms with score above some certain threshold (red lines) and dropping terms with score below some certain threshold (blue lines).
%     %We run this experiment on two types of scores: raw scores \essty\ scores (solid lines; right figure) and the confidence values extracted from classifiers (dashed lines; right figure). 
%      With fixed ratio of the terms dropped, dropping terms with bigger \essty scores results in lesser tendency to answer the questions.
%      }
%     \label{fig:droppQuestionTerms}
%     \vspace{-0.2cm}
% \end{figure}

%\daniel{explain this more}
}



%%%%%%%%%%%%%%%%%%
\section{\Ess\ Terms Classifier}
\label{sec:ET}

Given the dataset of questions and their terms annotated with \ess\ scores,
%we investigate the learnability of this annotation.
is it possible to learn the underlying concept? Towards this end,
given a question $q$ , answer options $a$, and a question term $q_l$, we seek a classifier that predicts whether $q_l$ is essential for answering $q$. We also extend it to produce an \essty\ score $et(q_l, q, a) \in
[0,1]$.\footnote{The \essty\ score may alternatively be defined as $et(q_l, q)$, independent of the answer options $a$. This is more suitable for non-multiple choice questions. Our system uses $a$ only to compute PMI-based statistical association features for the classifier. In our experiments, dropping these features resulted in only a small drop in the classifier's performance.}
We use the annotated dataset from \s2, where real-valued \essty\ scores are binarized to 1 if they are at least 0.5, and to 0 otherwise.
%We choose a threshold of 0.5 on the annotated \essty\ scores to binarize the real-valued confidence scores (\ess\ vs non-\ess) resulted from the annotations, and feed them to our classifier. 
%The training is done on 70\% randomly selected questions, choose 40\% of the remaining as development set, and the remainder as the test set 

We train a linear SVM classifier \citep{Joachims98}, henceforth referred to as \textbf{\et\ classifier}. Given the complex nature of the task, the features of this classifier include syntactic (e.g., dependency parse based) and semantic (e.g., Brown cluster representation of words \citep{BDMPL92}, a list of scientific words) properties of question words, as well as their combinations.
%\daniel{give example?} \ashish{yes! especially since we are highlighting the complex nature. given broad categories and/or specific examples in 2-3 lines.}
In total, we use 120 types of features (cf.~Appendix of~\cite{KKSR17}).

% \begin{table*}[t]
%     \setlength\doublerulesep{\arrayrulewidth}
%     \centering 
%     \begin{tabular}{c||ccc|c|cc}
%           & \multicolumn{3}{c|}{Avg.\ over Tokens}  & \multicolumn{3}{c}{Avg.\ over Sentences}    \\ 
%           \hline 
%             & \multicolumn{4}{c|}{0/1 Predictions}  & \multicolumn{2}{c}{Term Ranking}    \\ 
%           Metric & Prec.  & Rec. & F1 & Avg. Hamming Dist. & MAP & MP@3  \\ 
%         \hline 
%         \hline 
%         PMI-based (unsupervised) & & & & & & \\ 
%         Majority label (supervised) & & & & & & \\ 
%         ET Classifier  & & & & & & \\ 
%     \end{tabular}
%     \caption{\todo{add caption}}
%     \label{tab:results:et:classifier}
% \end{table*}


\paragraph{Baselines.}
%
To evaluate our approach, we devise a few simple yet relatively powerful baselines.

First, for our supervised baseline, given $(q_l, q, a)$ as before, we ignore $q$ and compute how often is $q_l$ annotated as essential in the entire dataset. In other words, the score for $q_l$ is the proportion of times it was marked as essential in the annotated dataset. If the instance is never observer in training, we choose an arbitrary label as prediction.
%A relatively simple supervised baseline is counting the number of the times a certain label has appeared for a given input (hence proportion of \ess\ labels as confidence score) 
%\ashish{both of the above sentences were confusing to me. try using some notation, like: given $(q_l, q, a)$, we ignore $q$ and compute how often is $q_l$ annotated as essential in the entire dataset. or something specific like this. relate it to the word 'proportion' that's used in the baseline name}
We refer to this baseline as \emph{label proportion baseline} and create two variants of it: \wordBaseline based on surface string and \lemmaBaseline based on lemmatizing the surface string. For unseen $q_l$, this baseline makes a random guess with uniform distribution. 

Our unsupervised baseline is inspired by work on sentence compression \citep{ClarkeLa08} 
%\ashish{can we cite the Clarke-Lapata work here?}
and the PMI solver of \citet{CEKSTTK16}, which compute word importance based on co-occurrence statistics in a large corpus. 
In a corpus $\mathcal{C}$ of 280 GB of plain text ($5 \times 10^{10}$ tokens) extracted from Web pages,\footnote{Collected by Charles Clarke at the University of Waterloo,
and used previously by \citet{Turney13}.} 
%We use it here to compute statistical co-occurrence values for the PMI solver. 
we identify unigrams, bigrams, trigrams, and skip-bigrams from $q$ and each answer option $a_i$. For a pair $(x, y)$ of $n$-grams, their pointwise mutual information (PMI) \citep{ChurchHa89} in $\mathcal{C}$ is defined as $\log \frac{p(x,y)}{p(x)p(y)}$ where $p(x, y)$ is the co-occurrence frequency of $x$ and $y$ (within some window) in $\mathcal{C}$. For a given word $x$, we find all pairs of question $n$-grams and answer option $n$-grams. \maxSalience and \sumSalience
score the importance of a word $x$ by max-ing or summing, resp., PMI scores $p(x,y)$ across all answer options $y$ for $q$. A limitation of this baseline is its dependence on the existence of answer options, while our system makes essentiality predictions independent of the answer options. 

We note that all of the aforementioned baselines produce real-valued confidence scores (for each term in the question), which can be turned into binary labels (\ess\ and non-\ess) by thresholding at a certain confidence value. 


%%%%%%%%%
\subsection{Evaluation}

%We consider two types of downstream usage for \Ess\ classifier: one based on its real-valued confidence scores, and the generated discrete classification results.
%Following the usage of \Ess\ classifier in the next section, we present two evaluations: 
%Here we present two evaluations scenarios: 
We consider two natural evaluation metrics for essentiality detection, first treating it as a binary prediction task at the level of individual terms and then as a task of ranking terms within each question by the degree of essentiality.


\paragraph{Binary Classification of Terms. }
%
We consider all question terms pooled together as described in Section~\ref{subsec:dataset}, resulting in a dataset of 19,380 terms annotated (in the context of the corresponding question) independently as essential or not. The \et\ classifier is trained on the train subset, and the threshold is tuned using the dev subset.

% \begin{wrapfigure}{r}{0.55\textwidth}
\begin{table}[ht]
    \setlength\doublerulesep{\arrayrulewidth}
    \centering 
    \small
    \setlength\extrarowheight{-10pt}
    \begin{tabular}{l|cc|ccc}
           &  AUC & Acc & P  & R   & F1   \\ 
        \hline \hline 
        \maxSalience$^\dagger$ & 0.74 & 0.67 & 0.88 & 0.65 & 0.75\\
        \sumSalience$^\dagger$ & 0.74 & 0.67 & 0.88 & 0.65 & 0.75\\
        \wordBaseline & 0.79 & 0.61 & 0.68 & 0.64 & 0.66 \\
        \lemmaBaseline & 0.80 & 0.63 & 0.76 & 0.64 & 0.69 \\
        {\bf \et\ Classifier} & \textbf{0.79} & \textbf{0.75} & \textbf{0.91} & \textbf{0.71} & \textbf{0.80} \\
        \hline
    \end{tabular}
    % \vspace{-0.3cm}
    \makeatletter\def\@captype{table}\makeatother% "Change float to table"
    \caption{
    \small
    Effectiveness of various methods for identifying essential question terms in the test set, including area under the PR curve (AUC), accuracy (Acc), precision (P), recall (R), and F1 score. \et\ classifier substantially outperforms all supervised and unsupervised (denoted with $^\dagger$) baselines.}
    \label{tab:results:classifier}
\end{table}
% \end{wrapfigure}

For each term in the corresponding test set of 4,124 instances, we use various methods to predict whether the term is essential (for the corresponding question) or not. Table~\ref{tab:results:classifier} summarizes the resulting performance. For the threshold-based scores, each method was tuned to maximize the F1 score based on the dev set. The \et\ classifier achieves an F1 score of 0.80, which is 5\%-14\% higher than the baselines. Its accuracy at 0.75 is statistically significantly better than all baselines based on the Binomial\footnote{Each test term prediction is assumed to be a binomial.} exact test~\citep{Howell12} at $p$-value 0.05.

% \begin{wrapfigure}{r}{0.5\textwidth}
\begin{figure}[htb]
    \centering
        %\includegraphics[trim=4.8cm 9.3cm 4.8cm 10cm, clip=true, scale=0.63]{figures_essential_terms/pr_curve_ranking_3.pdf}
        \includegraphics[trim=4.7cm 9.85cm 4.8cm 10.2cm, clip=true, scale=0.63]{figures_essential_terms/pr_curve_ranking_4.pdf}
        %\vspace{-0.8cm}
    \caption{
    \small
    Precision-recall trade-off for various classifiers as the threshold is varied.
    \et\ classifier (green) is significantly better throughout.
    }
    \label{fig:pr:differentSolvers}
\end{figure}
%\end{wrapfigure}
As noted earlier, each of these essentiality identification methods are parameterized by a threshold for balancing precision and recall. This allows them to be tuned for end-to-end performance of the downstream task. We use this feature later when incorporating the \et\ classifier in QA systems. Figure~\ref{fig:pr:differentSolvers} depicts the PR curves for various methods as the threshold is varied, highlighting that the \et\ classifier performs reliably at various recall points. Its precision, when tuned to optimize F1, is 0.91, which is very suitable for high-precision applications. It has a 5\% higher AUC (area under the curve) and outperforms baselines by roughly 5\% throughout the precision-recall spectrum. 

% we illustrate in Figure~\ref{fig:pr:differentSolvers} the resulting precision-recall tradeoff on the test set of 4124 term instances, as each classifier's acceptance threshold is varied. 
% \daniel{AS: this is actually incorrect. The upper figure is for ranking based evaluation.}\ashish{Let's change the upper figure to have a standard PR curve for binary classification: rank all 4124 terms by classifier score, then follow Footnote 10 to compute various (p,r) points to plot.}
% We see that our \et\ classifier consistently outperforms all baselines.

% \begin{figure}[t]
%     \centering
%     \includegraphics[trim=4.4cm 9.6cm 5cm 10.0cm, clip=true, scale=0.6]{figures_essential_terms/f_alpha_curve_3.pdf}
%         \vspace{-0.4cm}
%     \caption{
%     % \small 
%     $F_\alpha$ values for various classifiers (with threshold optimized to maximize $F_\alpha$) as $\alpha$ is varied. 
%     \et\ classifier (green) makes a significantly better prediction throughout. 
%     %The majority vote baselines \wordBaseline and \lemmaBaseline are relatively worse when $\alpha > 1$ (due to their low recall), while the unsupervised baselines \maxSalience and \sumSalience are relatively worse when $\alpha < 1$ (due to their low precision).
%     }
%     \label{fig:calibratedF:differentSolvers}
% \end{figure}

% As a second study, we measure $F_\alpha$,\footnote{$F_\alpha \triangleq (1 + \alpha^2) \cdot \frac{\mathrm{precision} \cdot \mathrm{recall}}{(\alpha^2 \cdot \mathrm{precision}) + \mathrm{recall}}$.} where $\alpha$ controls the balance between precision and recall. Depending on the usage in a downstream application, one might prefer high precision ($\alpha < 1$) over high recall ($\alpha > 1$), or vice versa. In Figure~\ref{fig:calibratedF:differentSolvers}, for each classifier (different curves), for each $\alpha$ (horizontal axis), we compute the acceptance threshold that maximizes $F_\alpha$ on the 
% %\tushar{train/dev/test} 
% dev set, and plot the resulting value of $F_\alpha$ (vertical axis). We observe that the supervised baselines are relatively better on the precision side ($\alpha < 1)$, while the unsupervised baselines are relatively better on the recall side ($\alpha > 1)$. Most interestingly, our \et\ classifier outperforms all baselines by around 5\% across all values of $\alpha$. %(statistical significance, as mentioned earlier, is 1.5\% %\tushar{Isn't this margin only applicable for accuracy comparisons i.e. when each term prediction is sampled from a binomial?}\ashish{right, $F_\alpha$ is tricky; leaving stat. sign. implicit; 5\% should be convincing anyway given the test set size}) 

%\begin{wrapfigure}{r}{0.55\textwidth}
\begin{table}[tb]
    \setlength\doublerulesep{\arrayrulewidth}
    \centering 
    \small
    \setlength\extrarowheight{-10pt}
    \begin{tabular}{l|cc|ccc}
           &  AUC & Acc & P  & R   & F1   \\ 
        \hline \hline 
        \maxSalience$^\dagger$ & 0.75 & 0.63 & 0.81 & 0.65 & 0.72 \\
        \sumSalience$^\dagger$ & 0.75 & 0.63 & 0.80 & 0.66 & 0.72 \\
        \wordBaseline & 0.57 & 0.51 & 0.49 & 0.61 & 0.54 \\
        \lemmaBaseline & 0.58 & 0.49 & 0.50 & 0.59 & 0.54 \\
        {\bf \et\ Classifier} & \textbf{0.78} & \textbf{0.71} & \textbf{0.88} & \textbf{0.71} & \textbf{0.78} \\
        \hline
    \end{tabular}
    \makeatletter\def\@captype{table}\makeatother% "Change float to table"
    \caption{
    \small
    Generalization to unseen terms: Effectiveness of various methods, using the same metrics as in Table~\ref{tab:results:classifier}. As expected, supervised methods perform poorly, similar to a random baseline. Unsupervised methods generalize well, but the \et\ classifier again substantially outperforms them.}
    \label{tab:precisionRecallUnseenTerms}
\end{table}
% \end{wrapfigure}
As a second study, we assess how well our classifier \textbf{generalizes to unseen terms}. For this, we consider
%a variant of Figure~\ref{fig:pr:differentSolvers} that considers
only the 559 test terms that do not appear in the train set.\footnote{In all our other experiments, test and train questions are always distinct but may have some terms in common.} Table~\ref{tab:precisionRecallUnseenTerms} provides the resulting performance metrics. We see that the frequency based supervised baselines, having never seen the test terms, stay close to the default precision of 0.5.  
%\ashish{fix this to reflect what's implemented} 
The unsupervised baselines, by nature, generalize much better but are substantially dominated by our \et\ classifier, which achieves an F1 score of 78\%. This is only 2\% below its own F1 across all seen and unseen terms, and 6\% higher than the second best baseline.




 \ignore{   
\begin{figure}
    \centering
    \includegraphics[trim=3.4cm 9.3cm 1cm 10.0cm, clip=true, scale=0.54]{figures_essential_terms/rankingScorePRCurve_onConstituentsNotSeen.pdf}
    \caption{Our classifier generalizes to the unseen data. The supervised baselines stay close to the default precision of 0.5, while the unsupervised baselines generalize much better but are substantially dominated by our \et\ classifier.}
    \label{fig:precisionRecallUnseenTerms}
\end{figure}    
}    
\paragraph{Ranking Question Terms by Essentiality. }

% \begin{figure}
% %\begin{framed}
% \centering
% \includegraphics[scale=0.6, trim=5cm 9.3cm 4.7cm 10cm]{figures_essential_terms/pr_curve_ranking_2.pdf}
% %\end{framed}
% \vspace{-0.5cm}
% \caption{Precision-Recall curve for essential term predictors when evaluated using ranking-based measures. Our trained classifier \et\ attains higher precision at every recall point.}
% %produces a more sensible confidence scores than our baselines.}
% \label{fig:pr:curve:ranking}
% \end{figure}

%In addition to using \et\ as a binary classifier, %we use its real-valued confidence scores directly.
    %In order to evaluate the confidence scores we use ranking-based measures \citep{manning2008introduction}. 
    % We now evaluate \et's confidence scores using ranking-based measures \citep{manning2008introduction}. 
    % Figure~\ref{fig:pr:curve:ranking} shows precision 
    % % \ashish{the caption of that figure mentions precision, not average precision. clarify and consolidate.}
    % % \daniel{minor changes made; does it read better now?}
    % averaged across all terms \ashish{I don't understand what's in Figure~\ref{fig:pr:curve:ranking}. If we are ranking all terms by their essentiality score, computing precision at each rank, and taking the average, would we not just get a single AP number?} in the test set questions.\footnote{We rank all terms based on their essentiality scores.  For any positive instance at rank $k$, the precision at $k$ is defined to be the number of positive instances with rank no more than $k$, divided by $k$. Similarly, recall at $k$ is the number of the positive instances with rank no more than $k$, divided by the total number of positive instances.} We observe that our classifier results in roughly 5\% higher precision at each recall point. Thus, using the confidence scores directly can be beneficial for a downstream application. 
    

\begin{wrapfigure}{r}{0.4\textwidth}
% \begin{table}[t]
    \setlength{\tabcolsep}{12pt}
    \setlength\doublerulesep{\arrayrulewidth}
    \centering 
    \small
    \setlength\extrarowheight{-10pt}
    \begin{tabular}{l|c}
        System  &  MAP \\ 
        \hline 
        \hline 
        \maxSalience$^\dagger$ & 0.87 \\
        \sumSalience$^\dagger$ &  0.85 \\
        \wordBaseline & 0.85  \\ 
        \lemmaBaseline & 0.86 \\ 
        {\bf \et\ Classifier} & \textbf{0.90} \\
        \hline
    \end{tabular}
    \makeatletter\def\@captype{table}\makeatother% "Change float to table"
    \caption{
    \small
    Effectiveness of various methods for ranking the terms in a question by essentiality. $^\dagger$ indicates unsupervised method. Mean-Average Precision (MAP) numbers reflect the mean (across all test set questions) of the average precision of the term ranking for each question. \et\ classifier again substantially outperforms all baselines.}
    \label{tab:results:et:classifier}
% \end{table}
\end{wrapfigure}
Next, we investigate the performance of the \et\ classifier as a system that ranks all terms within a question in the order of essentiality. Thus, unlike the previous evaluation that pools terms together across questions, we now consider each question as a unit. For the ranked list produced by each classifier for each question, we compute the average precision (AP).\footnote{We rank all terms within a question based on their essentiality scores. For any true positive instance at rank $k$, the precision at $k$ is defined to be the number of positive instances with rank no more than $k$, divided by $k$.
%Similarly, recall at $k$ is the number of the positive instances with rank no more than $k$, divided by the total number of positive instances.
The average of all these precision values for the ranked list for the question is the \emph{average precision}.} We then take the mean of these AP values across questions to obtain the mean average precision (MAP) score for the classifier.


    
The results for the test set (483 questions) are shown in Table~\ref{tab:results:et:classifier}. Our \et\ classifier achieves a MAP of 90.2\%, which is 3\%-5\% higher than the baselines, 
%\tushar{DK: do we have the std.dev.\ across questions? then can compute stat.\ sign.}
%(statistical significance at p$<$ 0.05 for this data , as mentioned earlier, is 4.5\% \ashish{double-check}\tushar{If we are using Wilson's test, it is at 2.98 for mean value of 90.2 but I guess we can't use a binomial test here, right ? see ``A Comparison of Statistical Significance Tests for Information Retrieval Evaluation''}).
and demonstrates that one can learn to reliably identify essential question terms.


%%%%%%%%%%%
\section{Using \et\ Classifier in QA Solvers}
\label{sec:using:in:classifier}

In order to assess the utility of our \et\ classifier, we investigate its impact on two end-to-end QA systems. We start with a brief description of the question sets.


\paragraph{Question Sets.} We use three question sets of 4-way multiple choice questions.\footnote{Available at \url{http://allenai.org/data.html}}
%for evaluating end-to-end performance of QA systems with and without the \et\ classifier.
\regents\ and \aiTwoPublic\ are two publicly available elementary school science question set. \regents\ comes with 127 training and 129 test questions; \aiTwoPublic\ contains 432 training and 339 test questions that subsume the smaller question sets used previously \citep{CEKSTTK16,KKSCER16}.
%The \emph{Regents} set from \citet{CEKSTTK16} consists of 129 hidden New York state Regents 4th Grade Science exam questions. 
\regentsPerturbed\ set, introduced by \citet{KKSCER16}, has 1,080 questions obtained by automatically perturbing incorrect answer choices for 108 New York Regents 4th grade science questions. We split this into 700 train and 380 test questions. 
%Finally, the new \emph{Omnibus} dataset expands the Regents set and has a total of 1,304 4th grade science questions collected from standardized exams in states other than New York as well as from \todo{say something about Certica, Key Data Systems, etc., to get credibility for this question set.}

%Test scores are reported as percentages. 
For each question, a solver gets a score of 1 if it chooses the correct answer and $1/k$ if it reports a $k$-way tie that includes the correct answer. 

\paragraph{QA Systems.} We investigate the impact of adding the \et\ classifier to two state-of-the-art QA systems for elementary level science questions. Let $q$ be a multiple choice question with answer options $\{a_i\}$. The \emph{\lucene\ Solver} from \citet{CEKSTTK16} searches, for each $a_i$, a large corpus for a sentence that best matches the $(q,a_i)$ pair. It then selects the answer option for which the match score is the highest. The inference based \emph{\tableilp\ Solver} from \citet{KKSCER16}, on the other hand, performs QA by treating it as an optimization problem over a semi-structured knowledge base derived from text. It is designed to answer questions requiring multi-step inference and a combination of multiple facts.

%For a given QA system, incorporating \et\ information within the reasoning loop anything requires understanding of its internal structure. Therefore there is no general way of using such component which would work for all the systems. 
%There are multiple ways of \textbf{incorporating \et\ information} within a QA reasoning loop. We will discuss the specifics, along with our findings, for each of the QA systems, using the following common setup.
For each multiple-choice question $(q, a)$, we use the \et\ classifier to obtain \ess\ term scores $s_l$ for each token $q_l$ in $q$; $s_l = et(q_l, q, a)$.
We will be interested in the subset $\omega$ of all terms $T_q$ in $q$ with \essty\ score above a threshold $\xi$: 
$\omega(\xi; q) =  \{l \in T_q \mid s_l > \xi \}$.
Let $\overline{\omega}(\xi; q) = T_q \setminus \omega(\xi; q)$. For brevity, we will write $\omega(\xi)$ when $q$ is implicit. 


% %%%%%%%%%
% %tushar{commented out this section to move into 2.2}
% \iffalse
% \subsection{Humans as Generic QA Systems}

% Using an \et\ classifier within QA systems require model-specific engineering. 
% %\ashish{commented out the sentence about `may or may not show benefits'. doesn't add much value and may raise premature questions}
% %which depending on the properties of the target question set and the form of reasoning needed, may or may not show benefits.
% For a model-agnostic evaluation of our classifier, we consider \emph{humans} as the target reasoning engine. 
% Towards the goal of measuring
% %the meaningfulness \ashish{not very sure about `meaningfulness'; revisit}
% %\daniel{any suggestions?}
% how well-defined are our \essty\ scores, we perform experiments under two conditions: 
% %\ashish{rephrased the following using previously introduced notation; in general, can reduce verbosity in several places} 
% starting with a question $q$ and a threshold $\xi$, (A) drop all terms in $\omega(\xi; q)$ and (B) drop all terms in $\overline{\omega}(\xi; q)$. 
% %\ashish{`below' a threshold was vague; did you mean $<$ or $\leq$? The complement of $\omega$ isn't formally defined above, but intuitively points to $\leq$, which seems like the right thing to do.}
% %(A) drop terms with score above a certain threshold (B) drop terms with score below a certain threshold.
% % \ashish{added the task description} 
% We then created a crowdsourcing task where workers were asked to answer the question with dropped words, but only if they felt there still was enough information to do so.

% % \begin{enumerate}
% %     \item drop terms with score above a certain threshold 
% %     \item drop terms with score below a certain threshold 
% % \end{enumerate}

% \begin{figure}[ht]
% %\begin{framed}
% %    \includegraphics[trim={2.5cm 8cm 0cm 9cm}, clip=true, scale=0.44]{figures_essential_terms/questionLevelExperiment-onlyClassifier.pdf}    
% %\end{framed}
%     %\begin{framed}
%     \includegraphics[trim={4.6cm 10.1cm 1.2cm 10.2cm}, clip=true, scale=0.6]{figures_essential_terms/questionLevelExperiment-onlyClassifier5.pdf}
%     %\end{framed}
%     \vspace{-0.8cm}
%     \caption{
%     %\ashish{increase font size in the figure; change Number to Fraction in y-label} 
%     x-axis: fraction of question words dropped. y-axis: the resulting fraction of questions workers felt comfortable answering. }
%     \label{fig:humanAnnnotation:ET:classifier}
% \end{figure}

% Figure~\ref{fig:humanAnnnotation:ET:classifier} shows the relationship between the fraction $d$ of question words dropped (determined by $\xi$) and the fraction $p$ of questions workers 
% %\ashish{as on page 1 or 2, changing Turkers to workers, to keep the discussion platform independent} 
% felt comfortable answering. Their precision, when they did answer, was nearly constant at 70-80\%. (cf.\ Appendix II, Table~1
% %\ref{table:human-in-loop} 
% for detailed numbers) 

% In scenario (A) where we drop high scoring terms (blue curve), we see that dropping even a small fraction of terms made annotators not answering many questions. Specifically, when only 17\% of the top scoring terms are dropped, only 25\% of the questions were answered. 
% On the other hand, even when dropping as many as 60\% of the least valuable terms as in scenario (B) (red curve), annotators continued to answer 79\% of the questions. 
% %
% This indicates that the scores generated by our ET system are indeed meaningful and the top scoring terms are the most helpful when humans act as the underlying QA system.

% \fi


%%%%%%%%%%%%%%
\subsection{\lucene\  solver + \et}

To incorporate the \et\ classifier, we create a parameterized \lucene\ system called \queryFiltering($\xi$) where, instead of querying a $(q,a_i)$ pair, we query 
$(\omega(\xi; q),a_i)$.
%\ashish{can't we just say we query $(\omega(\xi; q),a_i)$ for some $\xi$? if so, drop the remainder of the sentence. in general, re-use previous notation whenever possible, or extend it so it is reusable} 
%$(\hat{q},a_i)$ pair, where $\hat{q}$ contains all the question terms which have \essty\ score above a threshold $\xi$. In our experiments we use $\xi = 0.36$.
% and refer to this variation of \lucene\ as \queryFiltering. 
 

While IR solvers are generally easy to implement and are used in popular QA systems with surprisingly good performance, they are often also sensitive to the nature of the questions they receive. \citet{KKSCER16} demonstrated that a minor perturbation of the questions, as embodied in the \regentsPerturbed\ question set, dramatically reduces the performance of IR solvers. Since the perturbation involved the introduction of distracting incorrect answer options, we hypothesize that a system with better knowledge of what's important in the question will demonstrate increased robustness to such perturbation.

\begin{wrapfigure}{r}{0.5\textwidth}
% \begin{table}[t]
\setlength{\tabcolsep}{8pt}
\setlength{\doublerulesep}{\arrayrulewidth}
\centering 
\small
% \begin{tabular}{lcc}
% Dataset & Setting & Test Score (\%)  \\ 
% \hline 
% \hline
% \T \regents & IR \baseline\ & 59.11 \\
% \regents & \queryFiltering\ & 63.37  \\
% \hline 
% \T \aiTwoPublic & IR \baseline\ & 57.90 \\
% %Lucene & Upper-Bound & 58.30 & 58.30 \\
% \B \aiTwoPublic & \queryFiltering\ & 59.10 \\
% \hline 
% \T \regentsPerturbed & IR \baseline\ & 61.84 \\
% \regentsPerturbed & \queryFiltering\ & 66.84  \\
% \end{tabular}
% \vspace{2cm}
\setlength\extrarowheight{-10pt}
\begin{tabular}{l|cc}
Dataset & Basic IR & \queryFiltering\  \\ 
\hline 
\hline
\T \regents &  59.11 & {\bf 60.85}  \\
\aiTwoPublic & 57.90 & {\bf 59.10} \\
\regentsPerturbed &  61.84 & {\bf 66.84}  \\
\hline
\end{tabular}
\vspace{-0.1cm}
\makeatletter\def\@captype{table}\makeatother% "Change float to table"
\caption{Performance of the \lucene\ solver without (Basic IR) and with (\queryFiltering) essential terms. The numbers are solver scores (\%) on the test sets of the three datasets. 
%\et, on \aiTwoPublic\  and  \regentsPerturbed\ datasets. Precision and score are reported as percentages.
%\ashish{drop precision from all tables? we don't discuss it and there isn't too much to say about it. Also, use a consistent number of decimal digits.}
}
\vspace{-0.1cm}
\label{table:public}
% \end{table}
\end{wrapfigure}

Table \ref{table:public} validates this hypothesis, showing the result of incorporating \et\ in \lucene, as \queryFiltering($\xi = 0.36$), where $\xi$ was selected by optimizing end-to-end performance on the training set. 
%\ashish{DK: add something here} 
We observe a 5\% boost in the score on \regentsPerturbed, showing that incorporating the notion of \essty\ makes the system more robust to perturbations.


Adding ET to \lucene\ also improves its performance on standard test sets.  On the larger \aiTwoPublic\ question set, we see an improvement of 1.2\%.
%On the smaller \regents\ set, introducing \et\ improves \lucene's score by 4.26\% to 63.4\% where the previous state-of-the-art solver, \tableilp, achieves a score of 61.5\%. Thus, combining \et\ with a simple \lucene\ solver achieves a new state of the art on this set.
On the smaller \regents\ set, introducing \et\ improves \lucene solver’s score by 1.74\%, bringing it close to the state-of-the-art solver, \tableilp, which achieves a score of 61.5\%.
%On the smaller \regents\ set, introducing \et\ improves \lucene's score by 4.26\% to 63.4\% where the previous state-of-the-art solver, \tableilp, achieves a score of 61.5\%. Thus, combining \et\ with a simple \lucene\ solver achieves a new state of the art on this set.
%Our modified system, \queryFiltering, indeed confirms the hypothesis: adding ET to \lucene\ makes it substantially more robust to perturbations. 
% Also on the \aiTwoPublic\ question set, \lucene's performance improves by 1.2\%, indicating that the \et\ classifier is effective in pruning out distracting question terms.
This demonstrates that the notion of essential terms can be fruitfully exploited to improve QA systems.


%%%%%%%%%%%%%
% \tushar{Attempt at rewriting 4.2; original in an ignore block below}
\subsection{\tableilp\  solver + \et}

Our essentiality guided query filtering helped the \lucene\ solver find sentences that are more relevant to the question. However, for \tableilp\ an added focus on essential terms is expected to help only when the requisite knowledge is present in its relatively small knowledge base. To remove confounding factors, we focus on questions that are, in fact, answerable.

To this end, we consider three (implicit) requirements for \tableilp\ to demonstrate reliable behavior:
%Reliable behavior of \tableilp\ implicitly requires
%The decisions made inside \tableilp\ are a complex combination of multiple aspects: 
(1) the existence of relevant knowledge, (2) correct alignment between the question and the knowledge, and (3) a valid reasoning chain connecting the facts together. Judging this for a question, however, requires a significant manual effort and can only be done at a small scale.

\paragraph{Question Set.} We consider questions for which the \tableilp\ solver does have access to the requisite knowledge and, as judged by a human, a reasoning chain to arrive at the correct answer. To reduce manual effort, we collect such questions by starting with the correct reasoning chains (`support graphs') provided by \tableilp.
%Since \tableilp\ already answers these questions,
A human annotator is then asked to paraphrase the corresponding questions or add distracting terms, while maintaining the general meaning of the question. Note that this is done independent of essentiality scores. For instance, the modified question below changes two words in the question without affecting its core intent:
\vspace{-0.1cm}
\begin{framed}
\small 
\noindent 
\textbf{Original question: } A {\color{blue}fox} grows thicker {\color{blue}fur} as a season changes. This adaptation helps the fox to (A) find food(B) keep warmer(C) grow stronger(D) escape from predators \\ 
\textbf{Generated question: } An {\color{blue} animal} grows thicker {\color{blue} hair} as a season changes. This adaptation helps to (A) find food(B) keep warmer(C) grow stronger(D) escape from predators
\end{framed}
\vspace{-0.1cm}

While these generated questions should arguably remain correctly answerable by \tableilp, we found that this is often not the case. To investigate this, we curate a small dataset $Q_R$ with 12 questions 
(see the Appendix)
on each of which,  despite having the required knowledge and a plausible reasoning chain, \tableilp\ fails. 

\paragraph{Modified Solver.} To incorporate question term essentiality in the \tableilp\ solver while maintaining high recall, we employ a \emph{cascade} system that starts with a strong essentiality requirement and progressively weakens it.

Following the notation of Chapter 3, let $x(q_l)$ be a binary variable that denotes whether or not the $l$-th term of the question is used in the final reasoning graph. We enforce that terms with \essty\ score above a threshold $\xi$ must be used:  $x(q_l) = 1$, $\forall l \in \omega(\xi) $. Let \tableilp+\et($\xi$) denote the resulting system which can now be used in a cascading architecture: 

\tikzstyle{b} = [rectangle, draw, fill=blue!20, text width=10em, text centered, rounded corners, minimum height=2.1em, thick]
%\tikzstyle{c} = [rectangle, draw, fill=blue!20, text width=2.6em, text centered, rounded corners, minimum height=2.5em, thick]

\vspace{0.1cm}
\begin{center}
\begin{tikzpicture}[auto]
    \node [b] (sys1)  {{\scriptsize \tableilp+\et($\xi_1$)}};
    \node [right=of sys1, xshift=-0.8cm](dots1) {$\rightarrow$};
    \node [b, right=of dots1, xshift=-0.8cm] (sys2) {{\scriptsize \tableilp+\et($\xi_2$)}};
    \node [right=of sys2, xshift=-0.8cm](dots2) {$\rightarrow$ \hspace{0.2cm} ... };
    %\node [c, right=of dots2, xshift=-0.95cm] (sys3) {{\scriptsize \tableilp}};
\end{tikzpicture}
\end{center}
\vspace{0.1cm}
where 
$\xi_1 < \xi_2 < \hdots < \xi_k$ is a sequence of thresholds. Questions unanswered by the first system are delegated to the second,
%those still unanswered are delegated to the third later,
and so on. 
%In our experiments we use cascades with thresholds $\xi_1=0.4, \xi_2=0.6, \xi_3=0.8, \xi_4=1.0$, with the last layer being vanilla \tableilp. 
The cascade has the same recall as \tableilp, as long as the last system 
is the vanilla \tableilp. We refer to this configuration as \cascades$(\xi_1, \xi_2, \hdots, \xi_k)$.

This can be implemented via repeated calls to \tableilp+\et($\xi_j$) with $j$ increasing from $1$ to $k$, stopping if a solution is found. Alternatively, one can simulate the cascade via a single extended ILP using $k$ new binary variables $z_j$ with constraints:
$|\omega(\xi_j)| * z_j  \leq \sum_{l \in \omega(\xi_j)} x(q_l)$
for $j \in \{1, \hdots, k\}$,
and adding $M * \sum_{j = 1}^k z_j$ to the objective function, for a sufficiently large constant $M$.
%We used \cascades($0.4, 0.6, 0.8, 1.0$) in our experiments. 

We evaluate \cascades($0.4, 0.6, 0.8, 1.0$) on our question set, $Q_R$. By employing essentiality information provided by the \et\ classifier, \cascades\ corrects 41.7\% of the mistakes made by vanilla \tableilp. This error-reduction illustrates that the extra attention mechanism added to \tableilp\ via the concept of essential question terms helps it cope with distracting terms. 


%%%%%%%%%%
\ignore {
\subsection{\tableilp\  solver + \et}

We now consider incorporating the notion of question term essentiality in the \tableilp\ solver. This can be done in many ways. We describe a \emph{cascade} system that starts with a strong essentiality requirement and progressively weakens it.

%We modify the constraints in the ILP model to prefer solutions that use the \ess\ terms predicted by the classifier. 
Following the notation of \citet{KKSCER16}, let $x(q_l)$ be a binary variable that denotes whether or not the $l$-th term of the question is used in the final reasoning graph. We enforce that terms with \essty\ score above a threshold $\xi$ must be used:  $x(q_l) = 1$, $\forall l \in \omega(\xi) $. Let \tableilp+\et($\xi$) denote the resulting system.
%This is a relatively harsh constraint especially when knowledge is incomplete, and is likely to often result in insufficient support for any answer choice for many questions when $\xi$ is small (most terms are marked as essential).
To maintain high recall for the solver in the presence of incomplete knowledge, we create a cascading architecture: 

\tikzstyle{b} = [rectangle, draw, fill=blue!20, text width=5em, text centered, rounded corners, minimum height=2.1em, thick]
%\tikzstyle{c} = [rectangle, draw, fill=blue!20, text width=2.6em, text centered, rounded corners, minimum height=2.5em, thick]

\vspace{0.1cm}
\begin{tikzpicture}[auto]
    \node [b] (sys1)  {{\scriptsize \tableilp+\et($\xi_1$)}};
    \node [right=of sys1, xshift=-0.8cm](dots1) {$\rightarrow$};
    \node [b, right=of dots1, xshift=-0.8cm] (sys2) {{\scriptsize \tableilp+\et($\xi_2$)}};
    \node [right=of sys2, xshift=-0.8cm](dots2) {$\rightarrow$ \hspace{0.2cm} ... };
    %\node [c, right=of dots2, xshift=-0.95cm] (sys3) {{\scriptsize \tableilp}};
\end{tikzpicture}
\vspace{0.1cm}
%
where 
%\ashish{double-check the direction of this inequality?}
%\daniel{good catch. I think it's correct now. }
$\xi_1 < \xi_2 < \hdots < \xi_k$ is a sequence of thresholds. Questions unanswered by the first system are delegated to the second,
%those still unanswered are delegated to the third later,
and so on. 
%In our experiments we use cascades with thresholds $\xi_1=0.4, \xi_2=0.6, \xi_3=0.8, \xi_4=1.0$, with the last layer being vanilla \tableilp. 
The cascade has the same recall as \tableilp, as long as the last system 
is the vanilla \tableilp. We refer to this configuration as \cascades$(\xi_1, \xi_2, \hdots, \xi_k)$.
%
%The simplest way to implement \cascades$(\xi_1, \xi_2, \hdots, \xi_k)$ is to make 
This can be implemented via repeated calls to \tableilp+\et($\xi_j$) with $j$ increasing from $1$ to $k$, stopping if a solution is found. Alternatively, one can simulate the cascade via a single extended ILP using $k$ new binary variables $z_j$ with constraints:
% \begin{align*}
%     |\omega(\xi_j)| * z_j & \leq \sum_{l \in \omega(\xi_j)} x(q_l)
%     & & \forall j \in \{1, \hdots, k\}
% \end{align*}
$|\omega(\xi_j)| * z_j & \leq \sum_{l \in \omega(\xi_j)} x(q_l)$
for $j \in \{1, \hdots, k\}$,
and adding $M * \sum_{j = 1}^k z_j$ to the objective function, for a sufficiently large constant $M$.
%This allows a single additional constraint to simulate the cascade.
 We used \cascades($0.4, 0.6, 0.8, 1.0$) on our question set, $Q_R$.


%In this section we provide results of evaluating \tableilp\  on \aiTwoPublic\ dataset.
%\ashish{We should just drop that table. It doesn't add useful information. Instead, could just mention in text here, e.g.: The baseline \tableilp\ solver scores 46.7\% on the \aiTwoPublic\ question set. We found that the \cascades\ system, while answering a different set of questions \ashish{is this correct?}, did not achieve a higher score.}

% \paragraph{\cascades\ on question sets}

% The baseline \tableilp\ solver scores 46.7\% on the \aiTwoPublic\ question set, while the \cascades\ system only achieved a score of \tushar{XX\%}. % We found that the \cascades\ system, while behaving differently than \tableilp, achieved a score of \tushar{XX\%}.
% %The results are summarized in Table~\ref{table:public:tableilp}. 
% %As it can be observed, the performance of ET with \tableilp\ is only on-par with its baseline.
% This is unexpected as the informative attention should generally improve the score of the solver. We present a possible explanation for this drop and verify it with additional experiments next.
%tushar{commented} This is somewhat counter-intuitive, as adding informative attention to questions should help  the performance of the system. Next, we present and verify a possible explanation for this drop. 

%(vs. vanilla \tableilp\ \ashish{do we need 'vs. vanilla \tableilp'? shouldn't it be obvious by this time, assuming it's the baseline?} which treats the question terms as bag of words, after dropping the stopwords \citep{KKSCER16}) In what follows next we do more careful analysis of the unexpected observation.

%in the previous section; adding more attentional information on what terms are informative doesn't seem to be helpful for our target structured reasoning system, \tableilp.

While essentiality guided query filtering helps the \lucene\ solver find sentences that are more relevant to the question, an added focus on essential terms is expected to help \tableilp\ only when the requisite knowledge is in fact present in its relatively small knowledge base. To remove confounding factors, we specifically focus on questions that are answerable.

To this end, we consider three (implicit) requirements for \tableilp\ to demonstrate reliable behavior:
%Reliable behavior of \tableilp\ implicitly requires
%The decisions made inside \tableilp\ are a complex combination of multiple aspects: 
(1) the existence of relevant knowledge, (2) correct alignment between the question and the knowledge, and (3) a valid reasoning chain connecting the facts together. Judging this for a question, however, requires a significant manual effort and can only be done at a small scale.

%\tushar{Drop the second hypothesis if we are not using PR curves ? Will wait for AS to finish.}Such lucky guesses can be eliminated by requiring the use of the essential terms, increasing the precision of the solver but dropping the overall score. We verify these two hypotheses in the next two sections. 

% For a complex QA system like \tableilp, it is insightful to understand the reasons across this entire spectrum, ranging from bad predictions by \et\ classifier, missing knowledge, out of scope reasoning mechanism (e.g., quantitative reasoning, comparison questions), or inaccurate fuzzy matching between knowledge phrases.

%We hypothesize, and in the remaining section attempt to substantiate for \cascades($0.4, 0.6, 0.8, 1.0$), that our counter-intuitive observation stems from the existence of different distracting factors that wash away the improvement gained from \et.
%In the this section we will study a few of these phenomena.

% \begin{table}[t]
% \centering 
% \small 
% \begin{tabular}{L{1.5cm}C{2.7cm}|C{0.8cm}|C{0.9cm}}
% Dataset & Setting & Test Score & Precision \\ 
% \hline 
% \hline
% \aiTwoPublic & \baseline\ & 46.7 & 49.5 \\ 
% \aiTwoPublic & \cascades($0.8, 1.0$) & 46.7 & 48.7 \\
% \aiTwoPublic & \cascades{ ($0.4, 0.6, 0.8, 1.0$)} & 46.0 & 48.0 \\ 
% \end{tabular}
% \caption{Performance of \tableilp\ solvers, with and without \et, on \aiTwoPublic\ dataset. Precision and score are reported as percentages. }
% \label{table:public:tableilp}
% \end{table}

% \begin{figure*}[ht]
%     \centering
%     \includegraphics[scale=0.5, trim=4.2cm 9.6cm 3.5cm 10.3cm, clip=true]{figures_essential_terms/tableilp-precision-recall.pdf}
%     \includegraphics[scale=0.5, trim=4.4cm 9.6cm 0cm 10.3cm, clip=true]{figures_essential_terms/fAlphaVsAlpha.pdf}
%     \vspace{-0.5cm}
%     \caption{
%     Using \tableilp+\et\ as a high-precison solver. The left figure shows the precision-recall trade-off of \tableilp+\et\ for different constraints. Right figure shows the $F_\alpha$ for \tableilp\ with and without \et: for smaller $\alpha$s, \tableilp+\et\ is a better solver. \tushar{Daniel: Can you add one point for \tableilp\ in the left figure ?}}
%     \label{precision:tableilp:et}
% \end{figure*}


%\paragraph{\cascades\ on answerable questions}
%

We hypothesize that the \cascades\ solver improves over \tableilp\ when the above requirements are met.\footnote{Note that when these requirements aren't met for a question, \tableilp\ may still choose the correct answer by luck.}
To validate this hypothesis, we create a question set, $Q_R$, where each question does have the requisite knowledge and, as judged by a human, a reasoning chain to arrive at the correct answer. To reduce manual effort, we collect such questions by starting with the correct reasoning chains (`support graphs') provided by the \tableilp\ solver.
%Since \tableilp\ already answers these questions,
A human annotator is then asked to paraphrase the corresponding questions or add distracting terms, while maintaining the general meaning of the question. Note that this is done independent of essentiality scores. For example, the modified question below changes two words in the question without affecting its core intent:
\vspace{-0.1cm}
\begin{framed}
\small 
\noindent 
\textbf{Original question: } A {\color{blue}fox} grows thicker {\color{blue}fur} as a season changes. This adaptation helps the fox to (A) find food(B) keep warmer(C) grow stronger(D) escape from predators \\ 
\textbf{Generated question: } An {\color{blue} animal} grows thicker {\color{blue} hair} as a season changes. This adaptation helps to (A) find food(B) keep warmer(C) grow stronger(D) escape from predators
\end{framed}
\vspace{-0.1cm}

While these generated questions should arguably remain correctly answerable by \tableilp, we found that this is often not the case. To investigate this, we curate a small dataset $Q_R$ with 12 questions 
(see the Appendix)
where,  despite having the required knowledge and a plausible reasoning chain, \tableilp\ fails. Interestingly, simply adding \et\ classifier via the \cascades\ system corrects 41.7\% of these mistakes. This error-reduction illustrates that the extra attention mechanism added to \tableilp\ via the concept of essential question terms helps it cope with distracting terms.
}

\iffalse
Following the above observations, we perform a controlled (albeit less-realistic)
% rather than: unrealistic 
experiment.
To reduce distracting factors, we synthesize a question set $Q$ such that for every question $q \in Q$, (1) \tableilp\ answers $q$ incorrectly; (2) doesn't create a proper alignment 
for $q$, i.e., doesn't use all essential terms; (3) does have the requisite knowledge to answer $q$. In other words, the misalignment happens due to distracting terms. 
%\ashish{could distraction in the question also be a factor, not just distracting knowledge? after all, \et\ will address distractions stemming from the question}
%\daniel{True; it's both ways. But I wouldn't blame it on the question tho, but rather the knowledge and/or the entailment/similarities.}
%\ashish{How about `distracting terms'? Will keep it ambiguous but that's probably our best guess anyway.}

In order to ensure the third property, we start off with a set of questions that \tableilp\ answers correctly for the right reason (i.e., correct reasoning alignment to the correct knowledge). A human annotator is then asked to paraphrase question terms or add distracting terms, while maintaining the general meaning of the question and its answer options.  
%\ashish{... such that \tableilp\ stops answering the question correctly? i.e., how do we ensure property (A)?}
Note that this generation process is done independent of the \et\ scores.  
Here is an example question \tableilp\ answers correctly for the right reason (i.e.,  we are sure that the solver has the right knowledge to answer it with almost correct alignment scores). We change two words, while retaining the general meaning of the questions, but that causes the solver to answer it incorrectly.
\vspace{-0.2cm}
\begin{framed}
\small 
\noindent 
\textbf{Original question: } A {\color{blue}fox} grows thicker {\color{blue}fur} as a season changes. This adaptation helps the fox to (A) find food(B) keep warmer(C) grow stronger(D) escape from predators \\ 
\textbf{Generated question: } An {\color{blue} animal} grows thicker {\color{blue} hair} as a season changes. This adaptation helps to (A) find food(B) keep warmer(C) grow stronger(D) escape from predators
\end{framed}
\vspace{-0.2cm}
Only the questions that result in an incorrect answer from \tableilp\ (first property) due to missing alignments (second property) are added to Q. Given the expensive nature of this process, we curate a small dataset $Q$ of 12 questions of this form 
(see the Appendix). 
% \begin{table}[t]
% \centering 
% \small 
% % \begin{tabular}{lc}
% % Setting & Test Score \\ 
% % \hline \hline
% % \baseline\ & 0.00  \\
% % \cascades & 41.67 \\
% % \end{tabular}
% \begin{tabular}{l|c|c}
% Setting & \baseline & \cascades \\ 
% \hline 
% Test Score \ & 0.00 & 41.67 \\
% \end{tabular}
% \vspace{-0.4cm}
% \caption{Comparing the performance of \tableilp, with and without \et, on a manually generated dataset of question. While all the these questions are answerable by \tableilp, it fails on all of them for various reasons. }
% \label{table:controlled:experiment}
% \vspace{-0.1cm}
% \end{table}

%Table~\ref{table:controlled:experiment} shows the result of running both \tableilp\ and \cascades\ on $Q$. 
By design, \tableilp\ has a score of zero. Note that all of these questions are answerable by this solver (i.e. the knowledge for answering them exists in the solver knowledge base), but the solver gets distracted for various noises along the reasoning chain. Adding \et, on the other hand, corrects 41.67\% of the mistakes. This shows that the extra attention mechanism induced in the behavior of the solver helps it cope with the distractors. \fi
%\ashish{this last phrase is not very helpful; what's the main conclusion from this controlled experiment? need to end the paragraph with a solid articulation of this conclusion.} 

% \paragraph{\cascades\ as high-precision solver.}
% While the \cascades\ system doesn't show a clear advantage over the vanilla \tableilp, %we observe that it has a more robust behavior on a synthesized dataset. 
%  we hypothesize that our modified solver is more robust in its predictions and is less likely to make lucky guesses.  However this higher precision comes at the cost of losing recall (fewer questions attempted) leading to no net impact on the score. %Such a system would be more useful in applications where mistakes are costly and we are willing to trade-off some recall for improved precision.

% %his might be interesting in scenarios that making mistakes is costlier than not answring it. 
% We show this behavior with two curves. Figure~\ref{precision:tableilp:et} (left) shows  the precision-recall of our system for different $\xi$ values of the hard constraint. As compared to \tableilp, \cascades\ solver is able to achieve much higher precision at the cost of lower recall. By changing the value of $\xi$, a user can select a suitable precision-recall tradeoff. Such a ``knob'' would be useful in applications where mistakes are costly and we are willing to trade-off some recall for improved precision.


% %By modifying this ``knob'' in our system, a user can select a suitable precision-recall tradeoff.% The more constrained it gets, the higher precison solver we have (while having lower recall). 

% \tushar{The next para is basically describing $F_\alpha$ for a particular value of precision and recall. I am not sure if it adds much more than what is communicated by the PR curve.}
% We can also observe the higher precision of \tableilp\ with \et\ using the $F_\alpha$ measure. $F_\alpha$ combines the precision and recall values where $\alpha$=1 gives equal weight to both precision and recall. As the $\alpha$ value goes closer to zero, $F_\alpha$ gives more importance to precision. Figure~\ref{precision:tableilp:et} (right) shows the $F_\alpha$ for different values of $\alpha$, for a single configuration of the solvers.\footnote{\tableilp+\et\ has a hard constraint where 85\% of the essential terms must be used with a slack of one term.} For smaller values of $\alpha$, where precision is more important, our configuration of \tableilp+\et\ outperforms vanilla \tableilp. 

% Depending on how much one cares about precision vs. recall, she may prefer one solver over another. Figure~\ref{precision:tableilp:et} (right) shows such a trade-off between precision and recall by depicting the $F_\alpha$ for different values of $\alpha$, for two solvers. For smaller values of $\alpha$ (where precision is more important), a fixed configuration of \tableilp+\et\ outweighs \tableilp alone.  

%\section*{Reproducibility}
%The code for ET classifier is available at \url{https://github.com/allenai/essential-terms} which can be used to reproduce our results for Section 3.  




\section{Summary}
% This chapter introduces the concept of essential question terms and demonstrates its importance for question answering. 
% Question answering (QA) systems are easily distracted by irrelevant or redundant words in questions, especially when faced with long or multi-sentence questions in difficult domains. 
This chapter introduces and studies the notion of {\em essential question terms} with the goal of improving such QA solvers.
% \footnote{This chapter is based on the following publication: \cite{essentialterms}.}  
We illustrate the importance of essential question terms by showing that humans' ability to answer questions drops significantly when essential terms are eliminated from questions. We then develop a classifier that reliably (90\% mean average precision) identifies and ranks essential terms in questions. Finally, we use the classifier to demonstrate that the notion of question term essentiality allows state-of-the-art QA solvers for elementary-level science questions to make better and more informed decisions, improving performance by up to 5\%.


% Since the publication, this work has been picked up by others to significantly improve other systems~\citep{NZCM18}. 

% via two empirical findings: (a) humans becomes substantially worse at QA even when a few essential question terms are dropped, and (b) state-of-the-art QA systems can be improved by incorporating this notion. While text summarization has been studied before, questions have different characteristics, requiring new training data to learn a reliable model of essentiality. 
% We introduce a dataset for this task and show that our classifier trained on this dataset substantially outperforms several baselines in identifying and ranking question terms by the degree of essentiality.
% Since the publication, this work has been picked up by others to significantly improve other systems~\citep{NZCM18}. 

% We also introduce a new dataset of over 2,200 crowd-sourced essential terms annotated science questions. 





==> Daniel K - thesis - dissertation/4.multirc_new.tex <==

\chapter{A Challenge Set for Reasoning on Multiple Sentences}
\label{chapter:multirc}
% \epigraph{ 
% ``I am convinced that the act of thinking logically cannot possibly be natural to the human mind. If it were, then mathematics would be everybody's easiest course at school and our species would not have taken several millennia to figure out the scientific method.''
% }{--- \textup{Neil deGrasse Tyson}, The Sky Is Not the Limit: Adventures of an Urban Astrophysicist}
\epigraph{ 
``Human beings, viewed as behaving systems, are quite simple. The apparent complexity of our behavior over time is largely a reflection of the complexity of the environment in which we find ourselves.''
}{--- \textup{Herbert A. Simon}, The Sciences of the Artificial, 1968}


\section{Overview}
%An important contributor for a lack of motivation for learning sophisticated reasoning could be the limited design of the existing datasets. For example \citep{ChenBoMa16} shows that in the CNN/Daily Mail datasets, ``the required reasoning and inference level of this dataset is quite simple'' and a relatively simple algorithm could get almost close to the upper-bound. 
In this chapter we 
% We propose to address this shortcoming by developing 
develop 
a reading comprehension challenge in which answering each of the questions requires reasoning over multiple sentences.\footnote{This chapter is based on the following publication: \cite{KCRUR18}.}

There is evidence that answering `single-sentence questions', i.e. questions that can be answered from a single sentence of the given paragraph, is easier than answering multi-sentence questions', which require multiple sentences to answer a given question. For example, \citep{RichardsonBuRe13} released a reading comprehension dataset that contained both single-sentence and multi-sentence questions; models proposed for this task yielded considerably better performance on the single-sentence questions than on the multi-sentence questions (according to \citep{NarasimhanBa15} accuracy of about $83\%$ and $60\%$ on these two types of questions, respectively). 



%One possible reason for the seemingly good performance of existing systems is that most of the existing datasets contain `single-sentence questions', i.e. questions that can be answered from a single sentence of the given paragraph, and existing systems have grown to be comfortable with such questions. On the other hand, `multi-sentence questions', that require multiple sentences to answer, can be more difficult for an automated system. For example, \citep{RichardsonBuRe13} released a reading comprehension dataset that contained both single-sentence and multi-sentence questions. Thereafter, several models were proposed for this task and most of them yielded considerably better performance on the single-sentence questions than on the multi-sentence questions. For example, \citep{NarasimhanBa15} get an accuracy of about $83\%$ and $60\%$ on these two types of questions, respectively. 

There could be multiple reasons for this. First, multi-sentence reasoning seems to be inherently a difficult task. Research has shown that while complete-sentence construction emerges as early as first grade for many children, their ability to integrate sentences emerges only in fourth grade~\citep{BerningerNaBe11}. Answering multi-sentence questions might be more challenging for an automated system because it involves more than just processing individual sentences but rather combining linguistic, semantic and background knowledge across sentences---a computational challenges in itself. Despite these challenges, multi-sentence questions can be answered by humans and hence present an interesting yet reasonable goal for AI systems \citep{Davis14}.

\begin{wrapfigure}{r}{0.55\textwidth}
% \begin{figure}[th]
% \scalebox{0.90}{
% \footnotesize{
\includegraphics[scale=0.25]{figures_multirc/examples_multirc.png}
% \begin{tabular}{|L{7.7cm}|}
% \hline
% \rowcolor{light-gray}S3: Hearing noises in the garage, Mary Murdock finds a bleeding man, mangled and impaled on her jeep's bumper.\\
% \rowcolor{light-gray}S5: Panicked, she hits him with a golf club.\\
% \rowcolor{light-gray}S10: Later the news reveals the missing man is kindergarten teacher, Timothy Emser.\\%, bipolar and unstable when he vanished.\\
% \rowcolor{light-gray}S12: It transpires that Rick, her boyfriend, gets involved in the cover up and goes to retrieve incriminatory evidence off the corpse, but is killed, replaced in Emser's grave.\\
% \rowcolor{light-gray}S13: It becomes clear Emser survived.\\
% \rowcolor{light-gray}S15: He stalks Mary many ways.\\
% \hline 
% Who is stalking Mary? \\
% A)* Timothy          \hspace{1.46cm} D) Rick\\
% B)   Timothy's girlfriend    \hspace{0.16cm} E)  Murdock\\  
% C)*  The man she hit \hspace{0.55cm} F)  Her Boyfriend\\
% %\hline \hline
% %\rowcolor{light-gray}Sent 4: Richard Wentworth, an amateur criminologist who is friendly with the police, is secretly  `The Spider', a masked vigilante equally determined to wipe the Octopus and his gang off the face of the earth.\\
% %\rowcolor{light-gray}Sent 5: Pleasant and smiling in civilian life, Wentworth is often ruthless as the Spider, slinging two guns against the public enemies who attack him.\\
% %\rowcolor{light-gray}Sent 6: Wentworth also masquerades as affable underworld lowlife Blinky McQuade.\\
% %\hline 
% %What are Wentworth's two alitases? \\
% %A)  Octopus and Spider  \\
% %B)*  `The Spider' and Blinky McQuade  \\
% \hline \hline
% \rowcolor{light-gray}S1: Most young mammals, including humans, play.\\
% \rowcolor{light-gray}S2: Play is how they learn the skills that they will need as adults.\\
% \rowcolor{light-gray}S6: Big cats also play.\\
% \rowcolor{light-gray}S8: At the same time, they also practice their hunting skills.\\
% %\rowcolor{light-gray}S8: At the same time, they are also practicing their hunting skills.\\
% %\rowcolor{light-gray}S9: The dogs are playing tug-of-war with a toy.\\
% \rowcolor{light-gray}S11: Human children learn by playing as well.\\
% \rowcolor{light-gray}S12: For example, playing games and sports can help them learn to follow rules.\\
% \rowcolor{light-gray}S13: They also learn to work together.\\
% \hline 
% What do human children learn by playing games and sports?\\
% A)*  They learn to follow rules and work together \\
% B) hunting skills \\
% C)*  skills that they will need as adult\\  
% %D) they learn about how to cheat  \\
% %D) tug-of-war  \\
% \hline 
% \end{tabular}
% }
% }
\vspace{-0.3cm}
\caption{
\small
Examples from our \fancyname corpus. Each example shows relevant excerpts from a paragraph; multi-sentence question that can be answered by combining information from multiple sentences of the paragraph; and corresponding answer-options. The correct answer(s) is indicated by a *. Note that there can be multiple correct answers per question.}
\vspace{-0.2cm}
\label{figure:intro}
% \end{figure}
\end{wrapfigure}
In this work, we propose a
%--> focus doesn't make it clear whether we solve them or not. 
% on other hand "introduce" makes it sound like we are the first to study it. MCTest has them too. 
multi-sentence QA challenge in which questions can be answered only using information from multiple sentences. Specifically, we present \fancyname\ (Multi-Sentence Reading Comprehension)\footnote{\url{http://cogcomp.org/multirc/}}---a dataset of short paragraphs and multi-sentence questions that can be answered from the content of the paragraph. Each question is associated with several choices for answer-options, out of which {\em one or more} correctly answer the question. Figure~\ref{figure:intro} shows two examples from our dataset. Each instance consists of a multi-sentence paragraph, a question, and answer-options. All instances were constructed such that it is not possible to answer a question correctly without gathering information from multiple sentences. Due to space constraints, the figure shows only the relevant sentences from the original paragraph. The entire corpus consists of $871$ paragraphs and about $\sim6$k multi-sentence questions. % 900 or 800? :)  871 coolb :)etter? yes!good
%\snigdha{Delete the following sentence? It is described later} On average, there are 5 answer-options per question out of which 2.1 are correct. 
% D: good by me
%\todo{clarify the issue on the size of the multi-sentence questions. }



The goal of this dataset is to encourage the research community to explore approaches that can do more than sophisticated lexical-level matching. To accomplish this, we designed the dataset with three key challenges in mind. (i) The number of correct answer-options for each question is not pre-specified. This removes the over-reliance of current approaches on answer-options and forces them to decide on the correctness of each candidate answer independently of others. In other words, unlike previous work, the task here is not to simply identify the best answer-option, but to evaluate the correctness of each answer-option individually. For example, the first question in Figure~\ref{figure:intro} can be answered by combining information from sentences 3, 5, 10, 13 and 15. It requires not only understanding that the stalker's name is Timothy but also that he is the man who Mary had hit. (ii) The correct answer(s) is not required to be a span in the text. For example, the correct answer, A, of the second question in Figure~\ref{figure:intro} is not present in the paragraph verbatim. It is instead a combination of two spans from 2 sentences: 12 and 13. Such answer-options force models to process and understand not only the paragraph and the question but also the answer-options. (iii) The paragraphs in our dataset have diverse provenance by being extracted from 7 different domains such as news, fiction, historical text etc., and hence are expected to be more diverse in their contents as compared to single-domain datasets. We also expect this to lead to  diversity in the types of questions that can be constructed from the passage.


Overall, we introduce a reading comprehension dataset that significantly differs from most other datasets available today in the following ways:
\begin{itemize}[topsep=0pt,itemsep=-3ex,partopsep=1ex,parsep=1ex,nolistsep]
    \item $\sim$6$k$ high-quality multiple-choice RC questions that are generated (and manually verified via crowdsourcing) to require integrating information from multiple sentences.\\[-1em]
    \item The questions are not constrained to have a {\em single} correct answer, %making them more challenging and 
    generalizing existing paradigms for representing answer-options.\\[-1em]
    \item Our dataset is constructed using 7 different sources, allowing more diversity in content, style, and possible question types.\\[-1em]
    \item We show a significant performance gap between current solvers and human performance, indicating an opportunity for developing sophistical reasoning systems. 
    %for real progress in RC using this dataset.
    %\snigdha{the phrase "real progress" is a bit weird (implies that till now people have been making `virtual progress'). How about `significant progress' or `opportunity for developing sophisticated reasoning potential'.}\daniel{meaningful progress? consequential progress?} \snigdha{hmm, I don't like these or `significant progress'. We are able to talk about multi-hop reasoning because lexical reasoning (paraphrasing etc.) is relatively easier for us now. However, we weren't always good at lexical reasoning. We got better at it by working on the datasets/problems that were proposed in the past. So, implying that the progress till now has been not-real/insignificant/meaningless/inconsequential is sort-of ungrateful. I would have chosen something like `more sophisticated/complicated/challenging progress'. That said, I feel we are unnecessarily spending too much time on this :) Feel free to do what you like.  }
\end{itemize}



\newif\ifshort
\shorttrue
\newif\iftable
\tablefalse 

\section{Relevant Work}
\label{sec:related}

Some recent datasets proposed for machine comprehension pay attention to type of questions and reasoning required. For example, RACE~\citep{LXLYH17} attempts to incorporate different types of reasoning phenomena, and MCTest~\citep{RichardsonBuRe13} attempted to contain at least $50\%$ multi-sentence reasoning questions. However, since the crowdsourced workers who created the dataset were only encouraged, and not required, to write such questions, it is not clear how many of these questions actually require multi-sentence reasoning (see Sec.~\ref{subsec:multi-other-data}).
Similarly, only about 25\% of question in the RACE dataset require multi-sentence reasoning as reported in their paper. Remedia~\citep{HLBB99} also contains $5$ different types of questions (based on question words) but is a much smaller dataset. Other datasets which do not deliberately attempt to include multi-sentence reasoning, like SQuAD \citep{RZLL16} and the CNN/Daily Mail dataset \citep{HKGEKSB15}, suffer from even lower percentage of such questions (12\% and 2\% respectively~\citep{LXLYH17}). There are several other corpora which do not guarantee specific reasoning types, including MS MARCO~\citep{NRSGTMD16}, WikiQA \citep{YangYiMe15}, and TriviaQA \citep{JCWZ17}.


The complexity of reasoning required for a reading comprehension dataset would depend on several factors such as the source of questions or paragraphs; the way they are generated; and the order in which they are generated (i.e. questions from paragraphs, or the reverse). Specifically, paragraphs' source could influence the complexity and diversity of the language of the paragraphs and questions, and hence  the required level of reasoning capabilities. Unlike most current datasets which rely on only one or two sources for their paragraphs (e.g. CNN/Daily Mail and SQuAD rely only on news and Wikipedia articles respectively) our dataset uses $7$ different domains. 

Another factor that distinguishes our dataset from previously proposed corpora is the way answers are represented. Several datasets represent answers as multiple-choices with a single correct answer. While multiple-choice questions are easy to grade, coming up with non-trivial correct and incorrect answers can be challenging. 
Also, assuming exactly one correct answer (e.g., as in MCTest and RACE) inadvertently changes the task from choosing the correct answer to choosing the most likely answer.
Other datasets (e.g MS-MARCO and SQuAD) represent answers as a contiguous substring within the passage. This assumption of the answer being a span of the paragraph, limits the questions to those whose answer is contained verbatim in the paragraph. Unfortunately, it rules out more complicated questions whose answers are only implied by the text and hence require a deeper understanding. Because of these limitations, we designed our dataset to use multiple-choice representations, but without specifying the number of correct answers for each question. 




\section{Construction of \fancyname}
\label{sec:construction}

In this section we describe our principles and methodology of dataset collection. This includes automatically collecting paragraphs, composing questions and answer-options through crowd-sourcing platform, and manually curating the collected data. We also summarize a pilot study that helped us design this process, and end with a summary of statistics of the collected corpus.


\subsection{Principles of design}
Questions and answers in our dataset are designed based on the following key principles:

\paragraph{Multi-sentenceness.} Questions in our challenge require models to use information from multiple sentences of a paragraph. This is ensured through explicit validation. We exclude any question that can be answered based on a single sentence from a paragraph.

\paragraph{Open-endedness.} Our dataset is not restricted to questions whose answer can be found verbatim in a paragraph. Instead, we provide a set of hand-crafted answer-options for each question. Notably, they can represent information that is not explicitly stated in the text but is only inferable from it (e.g. implied counts, sentiments, and relationships).

\paragraph{Answers to be judged independently.} The total number of answer options per question is variable in our data and we explicitly allow multiple correct and incorrect answer options (e.g. 2 correct and 1 incorrect options). As a consequence, correct answers cannot be guessed solely by a process of elimination or by simply choosing the best candidates out of the given options.\\

Through these principles, we encourage users to explicitly model the semantics of text beyond individual words and sentences, to incorporate extra-linguistic reasoning mechanisms, and to handle answer options independently of one another. 
% \snigdha{If we run out of space, we can delete this para.}
%\michael{Agreed. OTOH, space doesn't seem to be an issue so far.}

\paragraph{Variability.} We encourage variability on different levels. Our dataset is based on paragraphs from multiple domains, leading to  linguistically diverse questions and answers. Also, we do not impose any restrictions on the questions, to encourage different forms of reasoning.

\subsection{Sources of documents}
The paragraphs used in our dataset are extracted from various sources. Here is the complete list of the text types and sources used in our dataset, and the number of paragraphs extracted from each category (indicated in square brackets on the right):  
\begin{enumerate}[topsep=0pt,itemsep=-3ex,partopsep=1ex,parsep=1ex,nolistsep]
    \item News: \hfill [121] 
    \begin{itemize}[nolistsep]
        \item CNN  \citep{HKGEKSB15} 
        \item WSJ  \citep{IBFFP08}
        \item NYT  \citep{IBFFP08}
    \end{itemize}
    \item Wikipedia articles \hfill [92] 
    \item Articles on society, law and justice  \citep{IdeSu06} \hfill [91]
    \item Articles on history and anthropology \citep{IBFFP08} \hfill [65]
    \item Elementary school science textbooks~\footnote{https://www.ck12.org} \hfill [153]%, from Flexbook~\footnote{https://www.ck12.org} \hfill [155]
    \item 9/11 reports~\citep{IdeSu06} \hfill [72]
    \item Fiction: \hfill [277]
    \begin{itemize}[nolistsep]
        \item Stories from the Gutenberg project  
        \item Children stories from MCTest~\citep{RichardsonBuRe13} 
        \item Movie plots from CMU Movie Summary corpus~\citep{BammanO'Sm13}% \hfill [92]  
    \end{itemize}
\end{enumerate}


From each of the above-mentioned sources we extracted paragraphs that had enough content. To ensure this we followed a $3$-step process. In the first step we selected top few sentences from paragraphs such that they contained $1$k-$1.5$k characters. To ensure coherence, all sentences were contiguous and extracted from the same paragraph. In this process we also discarded paragraphs that seemed to deviate too much from third person narrative style. For example, while processing Gutenberg corpus we considered files that had at least $5$k lines because we found that most of them were short poetic texts. In the second step, we annotated~\citep{KSZRCSRRLDTRMFWYSGUANLR18} the paragraphs and automatically filtered texts using conditions such as the average number of words per sentence; number of named entities; number of discourse connectives in the paragraph. These were designed by the authors of this paper after reviewing a small sample of paragraphs. A complete set of conditions is listed in Table~\ref{tab:paragraph-selection-condition}. Finally in the last step, we manually verified each paragraph and filtered out the ones that had formatting issues or other concerns that seemed to compromise their usability.



% }
%We extract paragraphs from each source, and automatically ensure that the selected content have enough content \todo{``selected content have enough content''? Great. \snigdha{Haha! See fix above.}}. For this, we make use of lower-bound conditions regarding, for instance, the average number of words per sentence, number of named entities, and discourse connectives. The complete set of conditions is listed in Appendix II. We manually verify each text and filter ones that have formatting issues. 


% \begin{wrapfigure}{r}{0.56\textwidth}
\begin{table}
    \centering
    \footnotesize{
    \centering
    \setlength\tabcolsep{10pt}
    \setlength\doublerulesep{\arrayrulewidth}
% \resizebox{310px}{!}{
% \setlength\extrarowheight{-3pt}
    \begin{tabular}{@{}ll@{}}
        \toprule
        Condition  & bound  \\
        \midrule
        Number of sentences & $\geq 6$ \& $\leq 18$ \\
        Number of NER(CoNLL) mentions & $\geq 2$  \\
        Avg. number of NER(CoNLL) mentions  & $\geq 0.2$ \\
        Number of NER(Ontonotes) mentions & $\geq 4$ \\
        Avg. number of NER(Ontonotes) mentions & $\geq 0.25$ \\
        Avg. number of words per sentence  & $\geq 5$ \\
        Number of coreference mentions & $\geq 3$  \\
        Avg. number of coreference mentions & $\geq 0.1$ \\
        Number of coreference relations  & $\geq 3$ \\
        Avg. number of coreference relations  & $\geq 0.08$ \\
        Number of coreference chains & $\geq 2$ \\
        Avg. number of coreference chains & $\geq0.1$ \\
        Number of discourse markers & $\geq2$ \\
\bottomrule
    \end{tabular}
    % }
    }
    \vspace{-0.1cm}
    \makeatletter\def\@captype{table}\makeatother% "Change float to table"
    \caption{Bounds used to select paragraphs for dataset creation.}
    \vspace{-0.1cm}
    \label{tab:paragraph-selection-condition}
\end{table}
% \end{wrapfigure}

\subsection{Pipeline of question extraction}
In this section, we delineate details of the process for collecting questions and answers. Figure~\ref{fig:steps} gives a high-level idea of the process. The first two steps deal with creating multi-sentence questions, followed by two steps for construction of candidate answers.
% Interested readers can find more details on set-ups of each step in Appendix I.
%(supplementary material). 

\begin{figure*}[ht]
    \centering
    % \begin{framed}
    % \includegraphics[trim=0cm 10.7cm 0cm 0.55cm, clip=true,scale=0.5]{figures_multirc/steps.pdf}
    \includegraphics[trim=0cm 10.7cm 0cm 0.55cm, clip=true,scale=0.48]{figures_multirc/steps2.pdf}
    % \end{framed}
    \vspace{-0.4cm}
    \caption{Pipeline of our dataset construction.}
    \label{fig:steps}
    \vspace{-0.2cm}
\end{figure*}

\paragraph{Step 1: Generating questions.}

The goal of the first step of our pipeline is to collect multi-sentence questions. We show each paragraph to $5$ turkers and ask them to write $3$-$5$ questions such that:  
(1) the question is answerable from the passage, and
(2) only those questions are allowed whose answer cannot be determined from a single sentence. 
We clarify this point by providing example paragraphs and questions. In order to encourage turkers to write meaningful questions that fit our criteria, we additionally ask them for a correct answer and for the sentence indices required to answer the question. To ensure the grammatical quality of the questions collected in this step, we limit the turkers to the countries with English as their major language. 
After the acquisition of questions in this step, we filter out questions which required less than 2 or more than 4 sentences to be answered; we also run them through an automatic spell-checker\footnote{Grammarly: www.grammarly.com} and manually correct questions regarding typos and unusual wordings.


\paragraph{Step 2: Verifying multi-sentenceness of questions. }
In a second step, we verify that each question can only be answered using more than one sentence. For each question collected in the previous step, we create question-sentence pairs by pairing it with each of the sentences necessary for answering it as indicated in the previous step. For a given question-sentence pair, we then ask turkers to annotate if they could answer the question from the sentence it is paired with (binary annotation). The underlying idea of this step is that a multi-sentence question would not be answerable from a single sentence, hence turkers should not be able to give a correct answer for any of the question-sentence pair.
%The underlying idea behind this step is that a multi-sentence question would not be answerable from a single sentence, and so for each of the corresponding pairs, the turkers would say that they couldn't answer the question from the given sentence. 
Accordingly, we determine a question as requiring multiple sentences only if the correct answer cannot be guessed from any single question-sentence pair.
%\snigdha{Check the tex file. I think we should keep the part commented above because in my opinion, its not trivial to understand why this step achieves the desired effect (if someone is reading superficially, which most reviewers do).}
%\michael{Okay, I put it back in and rephrased stuff a little. Better? }\snigdha{Yes}
We collected at least 3 annotations per pair, and to avoid sharing of information across sentences, no two pairs shown to a turker came from the same paragraph. We aggregate the above annotations for each question-answer pair and
%... to determine if a question is a multi-sentence question or not. Specifically, for each question-sentence pair (q,s), we define the answerability, A (q,s), of the question, q, from a single sentence, s as the fraction of turkers who said that the question could be answered from s. At the end of this step, we discard all questions whose answerability for any of the sentences it was paired with was more than ⅓. In other words, 
retain only those questions for which no pair was judged as answerable by a majority of turkers.


\paragraph{Step 3: Generating answer-options.}
In this step, we collect answer-options that will be shown with each question. Specifically, for each verified question from the previous steps, we ask 3 turkers to write as many correct and incorrect answer options as they can think of. In order to not curb creativity, we do not place a restriction on the number of options they have to write. We explicitly ask turkers to design difficult and non-trivial incorrect answer-options (e.g. if the question is about a person, a non-trivial incorrect answer-option would be other people mentioned in the paragraph). 
% \daniel{read the previous sentence and see if it is better?}\snigdha{Made minor changes and removed 'animate' because animals can also be animate but wouldn't be good incorrect option}

After this step, we perform a light clean up of the candidate answers by manually correcting minor errors (such as typos), completing 
% \snigdha{did you mean 'completing' instead of `clarifying'?} 
incomplete sentences and rephrasing any ambiguous sentences.
We further make sure there is not much repetition in the answer-options, to prevent potential exploitation of correlation between some candidate answers in order to find the correct answer. For example, we drop obviously duplicate answer-options (i.e.\ identical options after lower-casing, lemmatization, and removing stop-words).   %\daniel{read this paragraph?}
% \snigdha{We need to clarify what we do with answer-options with major problems. Also, we probably need to clarify why this is not redundant given Step 4.} We also merge answer-options that are lexically identical or are substrings of one another after normalization (lowercasing, deleting stopwords and punctuation).
%Some of the questions obtained from the previous steps were not answerable at all from the paragraph or contained other types of errors. To identify (and later discard) such questions, we additionally asked the turkers to check a box indicating the "question is bad", and also correct it if possible. 

\paragraph{Step 4: Verifying quality of the dataset.}
%\daniel{read this paragraph}
%\michael{I find this way too vague. What is meant by "problematic" and what are the "issues"? How did we fix them? The paragraph is bla bla, but doesn't really explain anything.}
%\snigdha{Michael, read this now}
This step serves as the final quality check for both questions and the answer-options generated in the previous steps. We show each paragraph, its questions, and the corresponding answer-options to $3$ turkers, and ask them to indicate if they find any errors (grammatical or otherwise), in the questions and/or answer-options. We then manually review, and correct if needed, all erroneous questions and answer-options. This ensures that we have meaningful questions and answer-options. In this step, we also want to verify that the correct (or incorrect) options obtained from Step 3 were indeed correct (or incorrect). For this, we additionally ask the annotators to select all correct answer-options for the question. If their annotations did not agree with the ones we had after Step 3 (e.g. if they unanimously selected an `incorrect' option as the answer), we manually reviewed and corrected (if needed) the annotation. 

%This step serves as the final quality check for both questions and the answer-options generated in the previous steps. We show each paragraph, its questions and the answer-options to $3$ turkers and ask them to mark the problematic questions and candidate answers, as well as answering the questions (i.e. selecting all the answer-options which answer the question). After the process is done, first we manually go through all the questions and answer-options which are marked as problematic, study the issues and correct it depending on the type of the problem (such as minor typos, ambiguous questions, irrelevant question or candidate-answer). In addition, we inspect the answer options that answered incorrectly unanimously by the turkers and fix the issue if the candidate answer is mislabeled in the step 3, or it is ambiguous. 

%The step verifies the quality of questions and candidate answer-options jointly in the previous step. In this step we show the answer options in addition to the question and paragraph they belong to, and ask the turkers to judge their validity. 
%The step verifies the quality of answer-options generated in the previous step. In this step we show the answer options in addition to the question and paragraph they belong to, and ask the turkers to judge their validity. 
% \todo{give more details on how the aggregation is done}

\subsection{Pilot experiments}
% \snigdha{
The $4$-step process described above was a result of detailed analysis and substantial refinement after two small pilot studies. 

In the first pilot study, we ran a set of $10$ paragraphs extracted from the CMU Movie Summary Corpus through our pipeline. Our then pipeline looked considerably different from the one described above. We found the steps that required turkers to write questions and answer-options to often have grammatical errors, possibly because a large majority of turkers were non-native speakers of English. This probslem was more prominent in questions than in answer-options. Because of this, we decided to limit the task to native speakers. Also, based on the results of this pilot, we overhauled the instructions of these steps by including examples of grammatically correct---but undesirable (not multi-sentence)---questions and answer-options, in addition to several minor changes. 

Thereafter, we decided to perform a manual validation of the verification steps (current Steps 2 and 4). For this, we (the authors of this paper) performed additional annotations ourselves on the data shown to turkers, and compared our results with those provided by the turkers. We found that in the verification of answer-options, our annotations were in high agreement ($98\%$) with those obtained from mechanical turk. However, that was not the case for the verification of multi-sentence questions. We made several further changes to the first two steps. Among other things, we clarified in the instructions that turkers should not use their background knowledge when writing and verifying questions, and also included negative examples of such questions. Additionally, when turkers judged a question to be answerable using a single sentence, we decided to encourage (but not require) them to guess the answer to the question. This improved our results considerably, possibly because it forced  annotators to think more carefully about what the answer might be, and whether they \textit{actually} knew the answer or they just \emph{thought} that they knew it (possibly because of background knowledge or because the sentence contained a lot of information relevant to the question). Guessed answers in this step were only used to verify the validity of multi-sentence questions. They were not used in the dataset or subsequent steps.

After revision, we ran a second pilot study in which we processed a set of $50$ paragraphs through our updated pipeline. This second pilot confirmed that our revisions were helpful, but thanks to its larger size,  also allowed us to identify a couple of borderline cases for which additional clarifications were required. Based on the results of the second pilot, we made some additional minor changes and then decided to apply the pipeline for creating the final dataset. 
% }
% 10 paragraphs from Wiki movie summaries, results of all steps annotated by ourselves
% Step 1: Collection of questions (6 per paragraph)
% Step 2: Verification -- 50\% agreement with turkers on “multi-sentence-ness”
% Step 3: Collection of correct & incorrect answer options
% Step 4: Answer verification -- 98\% agreement on goodness with 4/5 turker majorities

% Steps 1&2 suffered from lack of proper definitions
% Forms on previous slides are a result of major revisions
% Agreement on a balanced subset now 75\%
% Steps 3&4 caused no major problems
% Forms and instructions remained largely unchanged

\subsection{Verifying multi-sentenceness}
\label{subsec:multi-other-data}
% \snigdha{
While collecting our dataset, we found that, even though Step 1 instructed turkers to write multi-sentence questions, not all generated questions indeed required multi-sentence reasoning. This happened even after clarifications and revisions to the corresponding instructions, and we attribute it to honest mistakes. Therefore, we designed the subsequent verification step (Step 2). 
%While collecting our dataset, we found that, even though in Step 1 we instructed turkers to write multi-sentence questions, not all generated questions indeed required multi-sentence reasoning. This happened even after clarifications and revisions to the corresponding instructions, and we attribute it to honest mistakes. Therefore, we designed the subsequent Step 2 which verified the multi-sentenceness of our questions. %%We found that a significant chunk of questions that we collected were not multi-sentence questions. 

There are other datasets which aim to include multi-sentence reasoning questions, especially MCTest. 
%and the one with the greatest fraction of such questions is MCTest. 
Using our verification step, we % decide to 
systematically verify their multi-sentenceness. For this, we conducted a small pilot study on about $60$ multi-sentence questions from MCTest. As for our own verification, we created question-sentence pairs for each question and asked annotators to judge whether they can answer a question from the single sentence shown. Because we did not know which sentences contain information relevant to a question, we created question-sentence pairs using all sentences from a paragraph. After aggregation of turker annotations, we found that about half of the questions annotated as multi-sentence could be answered from a single sentence of the paragraph. This study, though performed on a subset of the data, underscores the necessity of rigorous verification step for multi-sentence reasoning when studying this phenomenon.
%After aggregation of turker annotations, we found that only about half of what was claimed to be multi-sentence questions could be answered from a single sentence of the paragraph.\daniel{made some changes to the previous sentence; read it?} 
%This underscores the necessity of rigorous verification step for multi-sentence reasoning when studying this phenomena. 
% While this study is small in size, it confirms the need for verifying that questions intended to be ``multi-sentence'' actually require information from multiple sentences to be answered.
%\daniel{check the last sentence?} % first I didn't want to confess our weakness (small size). Also the 2nd part of the sentence was long and hard to read. 
% }
%\snigdha{Daniel, I think this is a sensitive issue. We are refuting a major claim by that paper based on a very small sample. So we should be careful. How about:  ``After aggregation of turker annotations, we found that about half of the questions annotated as multi-sentence could be answered from a single sentence of the paragraph. This study, though performed on a subset of the data, underscores the necessity of rigorous verification step for multi-sentence reasoning when studying this phenomena.'' I have deliberately replaced 'claimed' by 'annotated' and acknowledged that it was done on a subset.}


\subsection{Statistics on the dataset}
%\snigdha{THE DESCRIPTION LOOKS GOOD. HOWEVER, YOU NEED TO PROVIDE A CONCLUSION TO YOUR EXPERIMENTS. CURRENTLY YOU ONLY SHOW THE RESULTS BUT DON'T PROVIDE A CONCLUSION OF YOUR EXPERIMENT. ALSO, THE WRITING IS A BIT TOO DENSE. SEE SUGGESTIONS BELOW.}
%\daniel{did some paraphrasing here. Read it? }
% \snigdha{
We now provide a brief summary of \fancyname. %  collected after the above mentioned procedure. 
Overall, it contains roughly $\sim$~$6k$ multi-sentence questions collected for about $+800$ paragraphs.\footnote{We will also release the $3.7k$ questions that did not pass Step 2. Though not multi-sentence questions, they could be a valuable resource on their own.}  The median number of correct and total answer options for each question is $2$ and $5$, respectively. Additional statistics are given in Table~\ref{tab:statistics:multirc}.

\begin{wrapfigure}{r}{0.5\textwidth}
% \begin{table}[th]
    \footnotesize
    \centering
    \resizebox{210px}{!}{
    \setlength\extrarowheight{-3pt}
    \begin{tabular}{l|c}
        \toprule
        Parameter & Value \\ 
        \hline 
         \# of paragraphs & 871\\ 
        \# of questions & 9,872 \\ 
        \# of multi-sentence questions & 5,825  \\ 
        avg \# of candidates (per question) &  5.44 \\ 
         avg \# of correct answers (per question) & 2.58  \\ 
        \hline 
         avg paragraph length (in sentences) & 14.3 (4.1) \\  
         avg paragraph length (in tokens) & 263.1 (92.4) \\  
         avg question length (in tokens) & 10.9 (4.8) \\ 
         avg answer length (in tokens) & 4.7 (5.5) \\ 
        \hline         
        \% of yes/no/true/false questions & 27.57\% \\ 
        % \% of  questions & 0.54\% \\  % \snigdha{merge this with previous row?} 
        \hline 
        avg \# of sent. used for questions & 2.37 (0.63) \\ 
        avg distance between the sent.'s used & 2.4 (2.58) \\ 
        \hline
        \% of correct answers verbatim in paragraph & 34.96\%  \\ 
        \% of incorrect answers verbatim in paragraph & 25.84\%  \\ 
        \bottomrule
    \end{tabular}
    }
    \vspace{-0.1cm}
    \makeatletter\def\@captype{table}\makeatother% "Change float to table"
    \caption{Various statistics of our dataset. Figures in parentheses represent standard deviation.}
    % \vspace{-0.1cm}
    \label{tab:statistics:multirc}
% \end{table}
\end{wrapfigure}

In Step 1, we also asked annotators to 
% \snigdha{replace `provide indices of' with `identify' }
identify sentences required to answer a given question. We found that answering each question required $2.4$ sentences on average. Also, required sentences are often not contiguous, and the average distance between sentences is $2.4$. Next, we analyze the types of questions in our dataset. Figure~\ref{fig:first-chunk-distribution} shows the count of first word(s) for our questions. We can see that while the popular question words (\emph{What}, \emph{Who}, etc.) are very common, there is a wide variety in the first word(s) indicating a diversity in question types. About $28\%$ of our questions require binary decisions (true/false or yes/no). 

\begin{figure*}
    \includegraphics[scale=0.41]{figures_multirc/phenomena7.png}
    \includegraphics[scale=0.41]{figures_multirc/phenomena4.png}
    \caption{Distribution of (left) general phenomena; (right) variations of the ``coreference" phenomena.  }
    \label{fig:phenomena}
\end{figure*}

%Lastly, we do a series of experiments on the questions regarding the type of inferences they demand. We select 60 questions that are previously labeled to require multi-sentence reasoning. Each question is labeled by two independent annotators, and adjudicated by two other annotators. The annotation is multi-label (i.e. annotators assign any label that match the question). 
%The adjudication step is necessary since sometimes there are multiple ways to get to the correct answer(s). The adjudicators were asked  to (1) respect the labels agreed upon the previous two annotators (2) among the labels disagreed, include the ones that can be used in a solution to the question. 
%We study the questions in two stages: In the first stage, we classify the questions into a relatively coarse categories: mathematical and logical reasoning, spatio-temporal reasoning, list/enumeration, coreference resolution (including implicit references, abstract pronouns, event coreference, etc.), causal relations, paraphrases and contrasts (including lexical relations such as synonyms, antonyms), commonsense knowledge, and `other'. The results of this experiment in Figure~\ref{fig:phenomena} (left) shows a broad variety of phenomena. 
%Since the ``coreference" category in the first experiment is too coarse, in a follow-up we break it down into finer classes: entity coreference (between two entities), event coreference	(between two events), set inclusion coreference (one item is included in the other) and `other' (Figure~\ref{fig:phenomena} (right)).
% We provide some examples of questions along with the required reasoning phenomena in Appendix II of the supplementary material.

%\snigdha{HOW ABOUT: 
We randomly selected 60 multi-sentence questions from our corpus and asked two independent annotators to label them with the type of reasoning phenomenon required to answer them.\footnote{The annotations were  adjudicated by two authors of this paper.} During this process, the annotators were shown a list of common reasoning phenomena (shown below), and they had to identify one or more of the phenomena relevant to a given question. The list of phenomena shown to the annotators included the following categories: mathematical and logical reasoning, spatio-temporal reasoning, list/enumeration, coreference resolution (including implicit references, abstract pronouns, event coreference, etc.), causal relations, paraphrases and contrasts (including lexical relations such as synonyms, antonyms), commonsense knowledge, and `other'. The categories were selected after a manual inspection of a subset of questions by two of the authors. The annotation process revealed that answering questions in our corpus requires a broad variety of reasoning phenomena. The left plot in Figure~\ref{fig:phenomena} provides detailed results. 

The figure shows that a large fraction of questions require coreference resolution, and a more careful inspection revealed that there were different types of coreference phenomena at play here. To investigate these further, we conducted a follow-up experiment in which manually annotated all questions that required coreference resolution into finer categories. Specifically, each question was shown to two annotators who were asked to select one or more of the following categories:  entity coreference (between two entities), event coreference	(between two events), set inclusion coreference (one item is part of or included in the other) and `other'. Figure~\ref{fig:phenomena} (right) shows the results of this experiment. We can see that, as expected, entity coreference is the most common type of coreference resolution needed in our corpus. However, a significant number of questions also require other types of coreference resolution.
% We provide some examples of questions along with the required reasoning phenomena in Appendix II.
% of the supplementary material.
%}

%provide statistics and some related intuitions on generated dataset. 
% }
%\todo{(one of us) explain these statistics}

%\snigdha{Statistics to include: avg paragraph size, avg question size, avg number of answer-options per question, avg number of correct options per question, avg answer-length. also count what fraction of questions are binary(yes/no, true/false)  or start with who(m), what, when, where, why, how, or something else }

% \snigdha{How to measure multi-sentenceness? We could compute the average number of sentences required to answer a question (as reported by turkers). Also, compute how far these sentences are. I guess is that deep learning methods could still potentially combine information from neighboring sentences, but if a question requires combining sent 1 with sent 15, it might not be easy for them. We should have this information somewhere (either in intro or somewhere in the paper).}

% number of paragraphs 1006
% number of questions 10k 
% number of multi-sentence questions 6.5k 
% avg paragraph size: 271.57 
% var of paragraph size: 92.399 
% avg question size: Avg que length:10.33159268929504 
% var of question size: Var que length:4.2244123692449325 
% avg number of candidates = 5.049222797927461
% avg number of correct answers = 2.0906735751295336 
% avg answer-length: Avg ans length:3.8945974576271185 
% var of answer-length:Var ans length:4.0581071356483545 
% ratio of questions that contain at least one 
% ratio of questions which contains List(yes, no) in their answer: 0.28296564923944795
% ratio of questions which contains List(false, true) in their answer: 0.005439709882139619
% distribution of the first words 
% distribution of the first chunk
% distribution of the number of sentences indicated in the first step 
% avg number of sentences indicated: 
% sentenceSizeMean:2.3785900783289815
% sentenceSizeVar:0.6301900717094747 
% avg of pairwise distance between the sentences indicated - Avg distance:2.4941549668096106 
% var of pairwise distance between the sentences indicated - Var distance:2.5804470447095436 


% \begin{wrapfigure}{r}{0.55\textwidth}
\begin{figure}
    \centering
    % \begin{framed}
    % \includegraphics[trim=2.3cm 2.5cm 21.4cm 1.7cm, clip=true, scale=0.36]{figures_multirc/question-first-chunk-distribution.png}
    \includegraphics[trim=1.3cm 1.1cm 0.0cm 0.0cm, scale=0.36]{figures_multirc/question-first-chunk-distribution3.png}
    % \end{framed}
    % \vspace{-0.1cm}
    \caption{Most frequent first chunks of the questions (counts in log scale). }
    \label{fig:first-chunk-distribution}
    % \vspace{-0.1cm}
\end{figure}
% \end{wrapfigure}


\section{Analysis}
\label{sec:analysis}

In this section, we provide a quantitative analysis of several baselines for our challenge. %We describe evaluation metrics and benchmark systems, and present results based on the dataset described in Section \ref{sec:construction}.
%\snigdha{If we run out of space, we can delete the second sentence.}

\paragraph{Evaluation Metrics.}
We define precision and recall for a question $q$ as:
$\text{Pre}(q) = \frac{|A(q) \cap \hat{A}(q)|}{|\hat{A}(q)|}$ and $\text{Rec}(q) = \frac{|A(q) \cap \hat{A}(q)|}{|A(q)|}$, where $A(q)$ and $\hat{A}(q)$ are the sets of correct and selected answer-options. 
%Generalize these definitions for a given dataset of $\{q\}$ by averaging the values of precision and recall, weighted with $w(q)$.  %$\text{Pre}(\{q\}) = \frac{ \sum_q w(q) \text{Pre}(q)  }{ \sum_q w(q) }$ (Similarly for $\text{Pre}(\{q\})$).
%We define (macro-average) $F1$ as the harmonic mean of average precision and recall across all the questions, one for uniform weights $w(q) = 1$ (denote with $F1_{\text{u}}$) and another weighting $w(q) = |A(q)|$ to account for variable number of answer options in questions (denote with $F1_{\text{w}}$). 
We define (macro-average) F1$_m$ as the harmonic mean of average-precision $avg_{q \in Q}(\text{Pre}(q))$ and average-recall $avg_{q \in Q}(\text{Rec}(q))$ with $Q$ as the set of all questions. 

Since by design, each answer-option can be judged independently, we consider another metric, F1$_a$, evaluating binary decisions on all the answer-options in the dataset. We define F1$_a$ to be the harmonic mean of $\text{Pre}(Q)$ and $\text{Rec}(Q)$, with $\text{Pre}(Q) = \frac{|A(Q) \cap \hat{A}(Q)|}{|\hat{A}(Q)|}$; $A(Q)=\bigcup_{q \in Q} A(q)$; and similar definitions for $\hat{A}(Q)$ and $\text{Rec}(Q)$.
%\snigdha{Made minor modifications} -->cool 

\subsection{Baselines}

\paragraph{Human.} Human performance provides us with an estimate of the best achievable results on datasets. Using mechanical turk, we ask 4 people (limited to native speakers) to solve our data. We evaluate score of each label by averaging the decision of the individuals. 
% a subset of our data (386 questions from  32 paragraphs). 


\paragraph{Random.}
To get an estimate on the lower-bound we consider a random baseline, where each answer option is selected as correct with a probability of 50\% (an unbiased coin toss). The numbers reported for this baseline represent the expected outcome (statistical expectation). 

\paragraph{\lucene}(information retrieval baseline). This baseline selects answer-options that best match sentences in a text corpus~\citep{CEKSTTK16}. Specifically, for each question $q$ and answer option $a_i$, the \lucene\ solver sends $q + a_i$ as a query to a search engine (we use Lucene) on a corpus, and returns the search engine's score for the top retrieved sentence $s$, where $s$ must have at least one non-stopword overlap with $q$, and at least one with $a_i$. 

We create two versions of this system. In the first variation IR(paragraphs) we create a corpus of sentences extracted from all the paragraphs in the dataset. In the second variation, IR(web) in addition to the knowledge of the paragraphs, we use extensive external knowledge extracted from the web (Wikipedia, science textbooks and study guidelines, and other webpages), with $5 \times 10^{10}$ tokens (280GB of plain text). 

\paragraph{SurfaceLR}(logistic regression baseline). As a simple baseline that makes use of our small training set, we reimplemented and trained a logistic regression model using word-based overlap features. As described in \citep{MHBSZ18}, this baseline takes into account the lengths of a text, question and each answer candidate, as well as indicator features regarding the (co-)occurrences of any words in them.


\paragraph{SemanticILP}(semi-structured baseline). This state-of-the-art solver, originally proposed for science questions and biology tests, uses a semi-structured representation to formalize the scoring problem as a subgraph optimization problem over multiple layers of semantic abstractions~\citep{KKSR18}. Since the solver is designed for multiple-choice with single-correct answer, we adapt it to our setting by running it for each answer-option. Specifically for each answer-option, we create a single-candidate question, and retrieve a real-valued score from the solver.  

% \begin{table}
\begin{wrapfigure}{r}{0.5\textwidth}
\centering
\small {
\setlength\extrarowheight{-6pt}
\begin{tabular}{@{}lcc|cc@{}}
\toprule
                            & \multicolumn{2}{c}{Dev} & \multicolumn{2}{c}{Test} \\ 
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
                            & F1$_m$  & F1$_a$ & F1$_m$  & F1$_a$  \\
\midrule
Random                      & 44.3 & 43.8 & 47.1 & 47.6  \\
\lucene (paragraphs)	    & 64.3 & 60.0 &	54.8 &	53.9 \\
SurfaceLR            	    &  66.1 & 63.7  & 66.7 &	63.5 \\
\hline
Human 	                    & 86.4 & 83.8 & 84.3 & 81.8 \\ 
\bottomrule
\end{tabular}
}
\makeatletter\def\@captype{table}\makeatother% "Change float to table"
\caption{
\small
Performance comparison for different baselines tested on a subset of our dataset (in percentage). There is a significant gap between the human performance and current statistical methods. }
\label{table:mainResults}
% \end{table}
\end{wrapfigure}
\paragraph{BiDAF}(neural network baseline). As a neural baseline, we apply this solver by \cite{SKFH16}, which was originally proposed for SQuAD but has been shown to generalize well to another domain~\citep{MinSeHa17}. Since BiDAF was designed for cloze style questions, we apply it to our multiple-choice setting following the procedure by \cite{KSSCFH17}: Specifically, we score each answer-option by computing the similarity value of it's output span with each of the candidate answers, computed by phrasal similarity tool of \cite{WBGLR15}. 



\subsection{Results} 
\begin{wrapfigure}{r}{0.5\textwidth}
% \begin{figure}[ht]
    \centering
    % \includegraphics[trim=0.45cm 0.7cm 0cm 0cm, scale=0.63]{figures_multirc/pr-curve3.png}
    % \includegraphics[trim=0.45cm 0.7cm 0cm 0cm, scale=0.63]{figures_multirc/pr-curve4.png}
    % \includegraphics[trim=0.45cm 0.55cm 0cm 0.45cm, scale=0.63]{figures_multirc/pr-curve5.png}
    \includegraphics[trim=0.45cm 0.55cm 0cm 0.45cm, scale=0.63]{figures_multirc/pr-curve.png}
    \vspace{-0.1cm}
    \caption{PR curve for each of the baselines. There is a considerable gap with the baselines and human. }
    % \vspace{-0.2cm}
    \label{fig:pr-curve}
% \end{figure}
\end{wrapfigure}
To get a sense of our dataset's hardness, we evaluate both human performance and multiple computational baselines. Each baseline scores an answer-option with a real-valued score, which we threshold to decide whether an answer option is selected or not, where the threshold is tuned on the development set. Table~\ref{table:mainResults} shows performance results for different baselines. The significantly high human performance shows that humans do not have much difficulties in answering the questions. Similar observations can be made in Figure~\ref{fig:pr-curve} where we plot $avg_{q \in Q}(\text{Pre}(q))$ vs. $avg_{q \in Q}(\text{Rec}(q))$, for different threshold values. 



\section{Summary}
To motivate the community to work on more challenging forms of natural language comprehension, in this chapter we discussed  a dataset that requires reasoning over multiple sentences. 
% This chapter presents a reading comprehension dataset in which questions require reasoning over multiple sentences to be answered. 
% We present a reading comprehension challenge in which questions can only be answered by taking into account information from multiple sentences. 
We solicit and verify questions and answers for this challenge through a 4-step crowdsourcing experiment.
Our challenge dataset contains $\sim$6$k$ questions for $+800$ paragraphs across 7 different domains (elementary school science, news, travel guides, fiction stories, etc) bringing in linguistic diversity to the texts and to the questions wordings. On a subset of our dataset, we found human solvers to achieve an F1-score of $86.4\%$.
We analyze a range of baselines, including a recent state-of-art reading comprehension system, and demonstrate the difficulty of this challenge,
% despite a high human performance.
The dataset is the first to study multi-sentence inference at scale, with an open-ended set of question types that requires reasoning skills.

%%% MultiRC 
% This dataset contains $\sim6k$ questions extracted from about +800 paragraphs. For each question, it contains multiple answer-options out of which one or more can be correct. The paragraphs (and questions) originate from different domains and hence are amenable to a wide variety and complexity of required reasoning phenomena. We found human performance on this corpus to be about $88\%$ 
% while state-of-the-art machine comprehension models do not exceed a F1-score of $60\%$. We hope that this significant difference in performance will encourage the community to work towards more sophisticated reasoning systems. Since its publication, this dataset has been uses by a couple of works that are currently under review. 

An additional important aspect of this work is that we challenged the community to change the harmful ``fixed'' test set methodology, and committed to updating the test set every few months.  


==> Daniel K - thesis - dissertation/5.tacoqa_new.tex <==
\chapter{A Question Answering Benchmark for Temporal Common-sense}
\label{chapter:dataset:tacoqa:commonsense}
% \epigraph{ 
% ``Human beings, viewed as behaving systems, are quite simple. The apparent complexity of our behavior over time is largely a reflection of the complexity of the environment in which we find ourselves.''
% }{--- \textup{Herbert A. Simon}, The Sciences of the Artificial, 1969}
% \epigraph{ 
% ``Common sense is a wild thing, savage, and beyond rules.''
% }{--- \textup{G. K. Chesterton}, Charles Dickens: A Critical Study, 1906}
\epigraph{ 
``Everything changes and nothing stands still.''
}{--- \textup{Heraclitus}, 535 BC - 475 BC}


\section{Overview}

% talk about commonsense + time 
Automating natural language understanding requires models that are informed
by commonsense knowledge and the ability to reason with it in both common and unexpected
situations. The NLP community has started in the last few year to investigate how to acquire such knowledge \cite{ForbesCh17,ZRDD17,YBWD18,RSASC18,BauerWaBa18,TDGYBC18,ZBSC18}.

%for many applications, such as design of dialogue assistants~\cite{ram2018conversational,mostafazadeh2017image}, document summarization~\cite{aslam2013trec}, and timeline construction~\cite{do2012joint}.\qiangcomment{I think there we should cite those more recent commonsense papers like SWAG and VerbPhysics. Will do so soon.}
This work studies a specific type of commonsense, {\em temporal commonsense}.\footnote{This chapter is based on the following publication: \cite{ZKNR19}.} For instance, given two events \emph{``going on a vacation''} and \emph{``going for a walk,''} most humans would know that a vacation is typically longer and occurs less often than a walk, but our programs currently do not know that. 

\begin{figure}
    \centering
    % \includegraphics[scale=0.35,trim=0cm 1cm 0cm 2cm]{figures/examples6.png}
    \includegraphics[width=0.8\textwidth]{figures_temporal_common_sense/examples10.pdf}
    \caption{\small Five types of temporal commonsense in \datasetname. Note that a question may have multiple answers. \ignore{Correct answers marked by `x'.}}
    \label{fig:intro:example}
\end{figure}


% qiang's first revision
% \qiang{Easy interpretations of natural language for humans can still be hard for a computer due to its lack of commonsense. For instance, given two events \emph{E1:``going on a vacation''} and \emph{E2:``going for a walk''}, it is easy for humans to figure out that a vacation is typically longer and less often than a walk, but not necessarily easy for computers. Due to the reporting bias that people usually do not say the obvious, it is crucial for a computer to acquire such knowledge and incorporate it into its decision making process for many applications, such as design of dialogue assistants~\cite{ram2018conversational,mostafazadeh2017image}, document summarization~\cite{aslam2013trec}, and timeline construction~\cite{do2012joint}.}

% old version
% The easiest interpretations for humans, can be extremely hard for computers:
% many individuals have a \emph{common} understanding of the differences between two events \emph{E1:``going on a vacation''} and \emph{E2:``going for a walk''}. 
% In particular, humans can easily pinpoint different \emph{temporal}  attributes of events~\cite{KozarevaHo11}. For instance, understanding that $E1$ usually takes longer than $E2$ (duration), or that $E2$ likely to happen more often than $E1$ (frequency), etc. 
% Understanding \emph{time} and reasoning with it is crucial for many natural language applications, like personal  assistants~\cite{}. We (humans) conveniently understand that the duration 
% Since \emph{commonsense} interpretations are typically easy for humans, they often go unmentioned, due to their triviality (for humans). Hence, for a system to solve this task, they have to be able to bring in world knowledge (as a result of knowledge acquisition, or other means) and incorporate it within their decision making. This capability, to understand and reasoning about {\em time}, is crucial for many applications, such as design of dialogue assistants~\cite{ram2018conversational,mostafazadeh2017image}, document summarization~\cite{aslam2013trec}, and timeline construction~\cite{do2012joint}. 
% and causality inference \qiang{(refs)}, for which commonsense is also very important. 
% \ben{I think maybe we can reference a few down-stream tasks here? Then we somehow argue, in order to solve those tasks, people should be able to answer our questions first.}

Temporal commonsense has received limited attention so far. \textbf{Our first contribution} is that, to the best of our knowledge, we are the first to systematically study and quantify performance on a range of temporal commonsense phenomena. Specifically, we consider five temporal properties: \emph{duration} (how long an event takes),  \emph{temporal ordering} (typical order of events), \emph{typical time} (when an event happens), \emph{frequency} (how often an event occurs), and \emph{stationarity} (whether a state holds for a very long time). Previous works have investigated some of them, either explicitly or implicitly (e.g., duration \cite{DivyeKhilnaniJu11,Williams12} and ordering \cite{ChklovskiPa04,NWPR18}), but none of them have defined or studied all aspects of temporal commonsense in a unified framework. \cite{KozarevaHo11} came close, when they defined a few temporal aspects to be investigated, but failed short of distinguishing in text and quantifying performances on these.

% old version
\ignore{
In this work, we examine the existing systems in their ability to handle \emph{temporal commonsense} or such world knowledge. 
% In particular, we focus on \emph{temporal} aspects of commonsense understanding. 
In particular, we consider five temporal properties: \emph{duration} (typical event duration), \emph{stationarity} (whether an event lasts long-enough), \emph{temporal ordering} (typical order of events), \emph{typical time} (when do events usually happen), and \emph{frequency} (\qiang{how often an event occurs}). Our goal is to study how existing methods could understand all these attributes.
}


% \todo{``the definition of the temporal aspects (we can appeal to the Hovy paper)''}

Given the lack of an evaluation standards and datasets for temporal commonsense, \textbf{our second contribution} is the collection of a new dataset dedicated for it, \datasetname{} (short for \textbf{t}empor\textbf{a}l \textbf{co}mmon-sense \textbf{q}uestion \textbf{a}nswering).\footnote{The dataset and code will be released upon publication.}
\datasetname{} is constructed via crowdsourcing with three meticulously-designed stages to guarantee its quality. 
An entry in \datasetname{} contains a \emph{sentence} providing context information, a \emph{question} requiring temporal commonsense, and \emph{candidate answers} with or without correct ones (see Fig.~\ref{fig:intro:example}).
More details about \datasetname{} are  in Sec.~\ref{sec:tacoqa}.

% old version
\ignore{
To have a natural evaluation to such properties, this paper introduces \datasetname, \textbf{t}empor\textbf{a}l \textbf{co}mmon-sense \textbf{q}uestion \textbf{a}nswering dataset, to serve as a diagnostic environment for further investigations dedicated to temporal commonsense. 
Our dataset is constructed with three meticulously-designed crowdsoursing stages. 
Figure~\ref{fig:intro:example} shows some examples for each class in \datasetname. 
The input contains a \emph{sentence} providing context information, a \emph{question} asking for temporal information, and \emph{candidate answers} with or without the correct ones in it.
To ensure the answers requires commonsense, no questions can be answered with a phrase explicitly contained in the context. 
% Note that we intentionally require that the answers to those questions should not be mentioned explicitly in the sentence, but humans can still infer them.
Moreover, we made sure that the question can still be answered with high agreement by human.
For example, \emph{Q1} asks whether that Mark is still on the farm. Given somebody being at some place's transient property, in addition to Mark is now a judge, humans can agree that he is no longer on the farm, even though the answer is not explicitly mentioned in \emph{S1}.
Similarly, \emph{Q5} asks for the frequency of large mammals' rest, and humans know that they usually rest every day, not too frequent (``once a minute'') or too infrequent (``once every three days'').
\qiangcomment{I feel that this paragraph can be shortened. It's too detailed right now.}
}

\textbf{Our third contribution} is that we propose multiple systems, including \emph{ESIM}, \bert{} and their variants, for this task. \datasetname{} allows us to investigate how state-of-the-art NLP techniques do on temporal commonsense tasks. Results in Sec.~\ref{sec:exp} show that, despite a significant improvement over random-guess baselines, \bert{} is still far behind human performance on temporal commonsense reasoning, indicating that existing NLP techniques still have limited capability of capturing high-level semantics like time.

% difference with the typical time. 
\ignore{
The temporal problems we are interested here are different from what has been investigated in the field. 
While there are many works on understanding \emph{time}, a vast majority of efforts focus on problems that mostly involve semi-direct mentions in text: 
for instance, extraction and normalization of \emph{temporal mentions}, \emph{events}, and \emph{relations}, %etc.~
% "such as" cannot be followed by "etc."
\cite{Str{\"o}tgenGe10,chang2012sutime,ning2017structured}. 
% This problem has been addressed in different levels, such as the extraction of \emph{temporal mentions}, \emph{events}, and \emph{relations}, %etc.~
% "such as" cannot be followed by "etc."
% \cite{Str{\"o}tgenGe10,chang2012sutime,ning2017structured}.
However, many instances we consider here contains involve a  variety of temporal phenomena that appear implicitly, without direct temporal references. 
% (hence, temporal commonsense). 
% This implicit understanding is usually referred to as \emph{commonsense} understanding, as it is widely known by many people and rarely get direct mentions in text.
\qiangcomment{I feel that this discussion is not in the right position.}
}


\begin{comment}
\daniel{OLD: 
Understanding \emph{time} and reasoning with it is crucial for many natural language 
% understanding 
tasks. This problem has been addressed in different levels, such as the extraction of \emph{temporal mentions}, \emph{events}, and \emph{relations}, %etc.~
% "such as" cannot be followed by "etc."
\cite{Str{\"o}tgenGe10,chang2012sutime,ning2017structured}. 
However, a wide variety of temporal phenomena appear implicitly, without direct temporal references. This implicit understanding is usually referred to as \emph{commonsense} understanding, as it is widely known by many people and rarely get direct mentions in text. % For instance,
% The easiest problems for humans are usually the hardest for computers. Such problems often go unmentioned,
% due to their triviality (for humans). 
For instance, humans trivially know that there are many differences between ``going to college'' and ``going to the movies'' (e.g., duration and prerequisites)
%, etc). 
% again, "e.g.," cannot be followed by "etc."
% Our current technologies so far don’t have any responses to such problems.
% Solving high-level natural language end-tasks, such as dialogue, machine comprehension, textual entailment, requires an extensive use of \emph{commonsense} knowledge and reasoning~\cite{}. 
}



commonsense has been an active topic in NLP due to its importance for reasoning, but the acquisition of commonsense is challenging because it is rarely explicitly mentioned in text. 
\ben{I think rarely mentioned in text is inaccurate \qiangcomment{agreed; I think we can simply delete the discourse of "but"} (e.g, we can use ``for" pattern to collect huge amounts of knowledge on duration). I believe the real difficulty here is that there will never be enough supervision on this, and learning from unsupervised objectives are noisy, thus the representations are not ideal. }
Much attention has been paid to this area over the years, including open concepts \cite{HavasiSpAl07}, sentiments \cite{CambriaOlRa14},  adjective intensities \cite{CWPAC18}, and physical properties of actions and objects \cite{ForbesCh17,YBWD18}.
\qiangcomment{add more references.}

The capability of understanding and reasoning over {\em time} is crucial for many tasks, such as timeline construction \qiang{(refs)}, summarization \qiangcomment{don't know the refs here}, and causality inference \qiang{(refs)}, for which commonsense is also very important. 
\todo{
``concrete examples of upstream tasks that make use
  of systems that tackle the task/dataset in this paper.'' + 
  ``a more crisp connection between the task/dataset and these
  would make things more concrete.''
}
For example, to answer, {\em did Aristotle have a laptop?} one needs to at least reason about when Aristotle lived, when laptop was invented, and a person who had died could not have a laptop. 
However, such cases have hardly been studied.
\ben{I think we should change the example. \qiangcomment{agreed} Dead person cannot have new things is not strictly an aspect that we care in this work. What about one of our extended questions in Appendix A.2?}

\todo{Better (formal?) definition of the categories, somewhere near here?}
\todo{Related: ``define the scope of the task''}

To fill this gap, this paper introduces \datasetname, short for \textbf{t}empor\textbf{a}l \textbf{co}mmonsense \textbf{q}uestion \textbf{a}nswering dataset, to serve as a benchmark for further investigations dedicated to temporal commonsense.
% \todo{``the definition of the temporal aspects (we can appeal to the Hovy paper)'',}
Specifically, for the first time, we systematically categorize the phenomena in temporal commonsense into five classes: \emph{duration,  stationarity, temporal ordering, typical time, and frequency}.
\ben{Yes, I think we can include here some bullet points for definitions. Alternatively we can have a section just for temporal commonsense?}
Figure~\ref{fig:intro:example} shows some examples for each class in \datasetname. 
The input contains a \emph{sentence} providing context information, a \emph{question} asking for temporal information, and \emph{candidate answers} with or without the correct ones in it.
\ben{To ensure the answers requires commonsense, no questions can be answered with a phrase contained in the context. Moreover, we made sure that the question can still be answered with high agreement by human.}
Note that we intentionally require that the answers to those questions should not be mentioned explicitly in the sentence, but humans can still infer them.
For example, \emph{Q1} asks whether that ``she is known as Fontaine'' still holds true at a later time (i.e., a {\em transient} state or a {\em stationary} fact).
Although the answer is not explicitly mentioned in \emph{S1}, most humans can tell that a person does not change his/her name if not stated otherwise.
Similarly, \emph{Q5} asks for the frequency of people making trips, and humans know it is unlikely to happen every night.
\ben{I think we should select better examples, and provide better explanations.}
\ben{In addition, we do not provide training data for this dataset, only a small dev set that provides the definition of the task. This is because the test set heavily evaluates system's ability to acquire commonsense knowledge, so that end-to-end training makes no sense, as there will never be enough direct supervision. We expect a system to be capable of acquiring temporal commonsense from other sources (e.g. pre-training), then use the dev data to derive a reasoning/QA model. }
% about duration of a ``laughing'' event described in \emph{S3}. Any human knows that ``laughter'' usually last less than a few minutes or seconds (and not ``20 minutes'').

\todo{
This might be a good place to defend this criticism: 
``Has the author tried any time/number recognizing and normalization preprocessing (for sentences / questions / answers)?''
}
\end{comment}

\ignore{
\textbf{The contributions of this work can be summarized as follows.}\qiangcomment{I'm going to move the bullets below to different places in-text. Will work on it in the afternoon.}
\begin{itemize}[noitemsep,leftmargin=0.4cm]
    \item A high-quality dataset on \emph{temporal commonsense}, \datasetname, is collected via crowdsourcing, which can significantly facilitate further research along this direction.\footnote{The dataset and codes will be released upon publication.}
    \ignore{To facilitate this research towards the problem of \emph{temporal commonsense}, we create a high-quality dataset for this task using crowdsourcing.}
    
    \item Multiple systems based on the state-of-the-art (including \emph{ESIM} and \bert) are proposed and evaluated on \datasetname. 
    % , showing the current state-of-the-art on this problem.
    \ignore{We  develop
    % \ben{can we say create here?}
    multiple competitive systems using state-of-the-art machinery available in the field. Additionally we show that humans are able to achieve significantly higher score on this task. }
    
    \item We show that there remains a significant performance gap between the proposed systems and humans, indicating the limitations of current NLP techniques and pointing out potential research directions.
    \ignore{We provide extra analysis on limitations of current techniques and remaining open challenges.} 
    % We create competitive systems for each sub-task, using state-of-the-art techniques. 
    % We observe that complexity of the datset to machine solvers, 
    % for our dataset and show its complexity, 
    % as indicated by the performance gap with human.
    
\end{itemize}
}

% \daniel{ 
% OLD: 
% In this work we introduce \datasetname, a \underline{t}empor\underline{a}l \underline{co}mmon-sense \underline{q}uestion \underline{a}nswering dataset. The goal of this dataset is to provide a natural language testbed, 
% % in order 
% to measure the progress towards acquiring and applying \emph{temporal commonsense}. Figure~\ref{fig:intro:example} provides a few examples questions from our dataset. The inputs include a \emph{sentence} describing a situation, a \emph{temporal question} and collection of \emph{candidate answers}. None of the questions have explicit answers in the sentence; instead, their answers need to be 
% % have to 
% be \emph{inferred} from the given input. For example, \emph{Q1} is asking about the age of a ``structure'' described in \emph{S1}. While there is no direction mention of the answer in \emph{S1}, many humans are able guess how many years can a ``structure'' age and answer this question. Similarly, \emph{Q3} is asking about duration of a ``laughing'' event described in \emph{S3}. Any human knows that ``laughter'' usually last less than a few minutes or seconds (and not ``20 minutes''). 
% }


% To facilitate further analysis, each question comes with its reasoning category, such as \emph{event frequency, event duration, etc}. 
% A few sampled questions in our dataset are depicted in Figure~\ref{fig:intro:example}. For example, 
% A system, in order to answer such questions, it has to be equipped with the 

% sciene exams 
% textual entailment 
% The importance of real-world knowledge for natural language understanding has been well-understood. 
% For example, Winograd's
% Representing knowledge and automating reasoning about times, durations, and
% time intervals is a largely solved problem.
% For instance, if one knows that Mozart was born earlier and died younger than Beethoven, one can infer that Mozart died earlier than Beethoven. 
% If one knows the Battle of Trenton occurred during the Revolutionary War, the Battle of Gettysburg occurred during the Civil War, and the Revolutionary War was over before the Civil War started, then one can infer the Battle of Trenton occurred before the Battle of Gettysburg. The inferences involved here in almost all cases reduce to solving
% systems of linear inequalities, usually small and of a very simple form. Integrating such reasoning with specific applications, such as natural language interpretation, has been much more problematic. Natural language expressions for time are com

% \qiangcomment{I think we need to discuss the following things in intro: (1) Why is temporal common sense important? (2) How to formally define temporal common sense? (3) What are (and how do we position) our contributions? I feel that we did not do well in address all the three points.}


\section{Related Work}
% temporal information extraction 
\begin{comment}
\daniel{
OLD: 
Temporal information and inference is an important component in natural language understanding. There are multiple popular tasks related to temporal inference, such as temporal relation \cite{NFWR18} and script generation \cite{leeuwenberg2018temporal} \cite{granroth2016happens}. These works have shown that temporal reasoning is essential yet challenging, as human performances are still much better than state-of-the-art systems across multiple benchmarks.
}

\daniel{
OLD: 
commonsense understanding has a long history as a critical part of machine reasoning as well, for both vision \cite{lin2015don} and NLP communities. Early work to address commonsense in languages are mostly focusing on acquiring commonsense information. \cite{LiuSi04} proposed a large knowledge base of commonsense relations between entities. \cite{ForbesCh17} proposed a way to generate large scale commonsense knowledge of physical properties. \cite{williams2012extracting} proposed an early work on acquiring large-scale temporal duration information. With the acquired information, there has been recent successes in applying commonsense information for downstream tasks. \cite{YBWD18} proposed a model to learn physical relationships among properties, \cite{NFWR18} ...
}

\daniel{
OLD: 
If we want to evaluate systems' abilities of acquiring and reasoning with commonsenses, it is natural to use question answering as the end task. People have done a lot in terms of gathering QA datasets as machine reading comprehension benchmarks. Most existing QA datasets for reading comprehension require the answer to have direct supporting evidences in the provided text, such as \cite{RichardsonBuRe13} and \cite{KCRUR18}. We have seen more datasets that address the use of commonsense, in which the answers are not directly supported by the evidence. \cite{ZBSC18} proposed a work of ending completion.
}
\end{comment}

% general commonsense  
commonsense has been a very popular topic in recent years and existing NLP works have mainly investigated the acquisition and evaluation of commonsense in the physical world, including but not limited to, size, weight, and strength \cite{ForbesCh17}, roundness and deliciousness \cite{YBWD18}, and intensity \cite{CWPAC18}. In terms of commonsense on ``events'', \citet{RSASC18} investigated the intent and reaction of participants of an event, and \citet{ZBSC18} tried to select the most likely subsequent event. As far as we know, no existing work has focused on temporal commonsense yet.

% old
\ignore{
\paragraph{commonsense understanding.}
The majority of the work in this area has focused on formalizing and acquisition of commonsense \emph{knowledge}, either in the form of manually curated knowledge-bases~\cite{LiuSi04}, exploiting weak signals from sensors like vision~\cite{lin2015don,ZBSC18} or  
% formalisms like network of commonsense relation
a combination of weak signals incorporated within relational frameworks ~\cite{ForbesCh17}. Within this literature, to the best of our knowledge, this 
is the first work along the commonsense thread which systematically focuses on the commonsense understanding of \emph{time}.
}
% is the first work among to address commonsense understanding of \emph{temporal} events. 
% \cite{LiuSi04} -> ConceptNet—a practical commonsense reasoning tool-kit 
% \cite{YBWD18} -> Extracting Commonsense Properties from Embeddings with Limited Human Guidance  
% \cite{winn2018lighter} ->  ’Lighter’Can Still Be Dark: Modeling Comparative Color Descriptions 
% \cite{gao2018action} -> What action causes this? towards naive physical action-effect prediction 
% \cite{wang2017integrating} -> What action causes this? towards naive physical action-effect prediction 
% \cite{ForbesCh17} -> Verb Physics: Relative Physical Knowledge of Actions and Objects 
% \cite{lin2015don} -> Don't just listen, use your imagination: Leveraging visual commonsense for non-visual tasks
% \cite{mostafazadeh2016corpus} -> A Corpus and Cloze Evaluation for Deeper Understanding of Commonsense Stories 
% \cite{ZRDD17} -> Ordinal commonsense Inference 
% SWAG~\cite{ZBSC18}, -> SWAG: A Large-Scale Adversarial Dataset for Grounded Commonsense Inference 
% ReCoRD~\cite{zhang2018record}, -> ReCoRD: Bridging the Gap between Human and Machine Commonsense Reading Comprehension  
% QuaRel~\cite{tafjord2018quarel}, -> QuaRel: A Dataset and Models for Answering Questions about Qualitative Relationships 

\begin{comment}
commonsense understanding has a long history as a critical part of machine reasoning as well, for both vision \cite{lin2015don} and NLP communities. Early work to address commonsense in languages are mostly focusing on acquiring commonsense information. \cite{LiuSi04} proposed a large knowledge base of commonsense relations between entities. \cite{ForbesCh17} proposed a way to generate large scale commonsense knowledge of physical properties. \cite{williams2012extracting} proposed an early work on acquiring large-scale temporal duration information. With the acquired information, there has been recent successes in applying commonsense information for downstream tasks. \cite{YBWD18} proposed a model to learn physical relationships among properties, \cite{NFWR18} ...
\end{comment}

There have also been many works trying to understand time in natural language but not necessarily with respect to commonsense, such as the extraction and normalization of temporal expressions~\cite{LADZ14}, temporal relation extraction \cite{NZFPR18}, and timeline construction \cite{LeeuwenbergMo18}. Among these, some works are implicitly on temporal commonsense, such as event durations \cite{Williams12,VempalaBlPa18}, typical temporal ordering \cite{ChklovskiPa04,NWPR18}, and script learning (i.e., what happens next after certain events) \cite{Granroth-WildingCl16,LiDiLi18}. 
However, either in terms of datasets or approaches, existing works did not study all five types of temporal commonsense in a unified framework as we do here.

% old
\ignore{
\paragraph{Temporal reasoning.}
The field has already studied some tasks related to \emph{time}:
the extraction and normalization of temporal expressions~\cite{LADZ14}, temporal ordering~\cite{NZFPR18}, and duration expressed in text~\cite{VempalaBlPa18}.
There have been some works conceptually relevant to commonsense, independently spreading over many subareas, including \citet{ChklovskiPa04,NWPR18} on temporal ordering of verbs, \citet{Williams12} on duration, and \citet{Granroth-WildingCl16,LiDiLi18} on script learning (i.e., what happens next after certain events). 
All these works were intended to provide prior knowledge for certain aspects of temporal reasoning, but none of them systematically studies a broad range of aspects to the temporal commonsense, which is what this paper is aiming for.
% \todo{Daniel: I don't udnderstand the previous two sentences}
}

% \benchange{ DROP: However, all these works were aimed for providing ``prior'' for specific tasks other than commonsense; they also were not intended to study all these facets of temporal commonsense systematically.}
%in addition, the phenomena of {\em frequency}, {\em transient vs. stationary}, and {\em absolute point} are never studied in those.

\ignore{
% The field of temporal reasoning has flourished in many different levels, 
This area has advanced in multiple interrelated directions. With respect to harnessing temporal patterns in the wild, there are many proposals~\cite{williams2012extracting,DivyeKhilnaniJu11}. 
% with respect to harnessing temporal patterns in the wild. 
In parallel, there is a line of work on
% there are progresses towards 
creating richer temporal reasoning formalism~\cite{NFWR18,leeuwenberg2018temporal}. 
Unfortunately, majority the work in this area has not explored 
% such works have not carefully studied 
the extent to which these ideas apply to scenarios which involve commonsense understanding/reasoning with respect to \emph{time}. Our dataset is an opportunity for this area to do such explorations. }
% to test such ideas in a natural medium. 
% script generation \cite{leeuwenberg2018temporal} 
% \cite{NFWR18} -> Joint reasoning for temporal and causal relations 
% \cite{granroth2016happens} -> What happens next? event prediction using a compositional neural network model 
% \cite{kuzey2016time} -> As time goes by: comprehensive tagging of textual phrases with temporal scopes 

% \cite{williams2012extracting} --> Extracting fine-grained durations for verbs from Twitter
% \cite{leeuwenberg2018temporal} -> Temporal Information Extraction by Predicting Relative Time-lines 
% \cite{DivyeKhilnaniJu11} -> Using Query Patterns to Learn the Duration of Events 

% QA dataset 

Instead of working on each individual aspect of temporal commonsense, we formulate the problem as a machine reading comprehension task in the format of question-answering (QA). The past few years have also seen significant progress on QA \cite{CCEKSST18,ORMTP18,MHBSZ18}, but mainly on {\em general} natural language comprehension tasks without tailoring it to test {\em specific} reasoning capabilities such as temporal commonsense. Therefore, a new dataset like \datasetname{} is strongly desired.


% \qiangcomment{If you are trying to argue why we are collecting a new dataset instead of using an existing one, I would suggest moving this somewhere in our ``second contribution''.}
\ignore{
\paragraph{Machine Reading Comprehension.}
This area has witnessed many recent datasets in the past few years. 
Many of the proposals provide general natural language comprehension tasks, without tailoring it to any specific reasoning ability.   
% Many such works create challenge sets with general language problems. 
To name a few, 
\namecite{CCEKSST18,ORMTP18,MHBSZ18} are among such works. 
While these are 
% While such tasks could be 
helpful to measure general language 
% reasoning, 
understanding,
they are not very useful when evaluating narrow 
% abilities
aspects of language. 
% such as temporal commonsense. 
% Even the most granular annotation on the reasoning task, such as \cite{sugawara2018makes}, usually do not distinguish different \emph{sub-types} of commonsense reasoning. 
Our reading comprehension dataset, while being naturally generated by 
% crowd-workers, 
crowdsourcers,
it is 
focused on class of language understanding problems (various properties of time)
% tailored to narrow reasoning class} 
and contains 
% \emph{temporal} commonsense, in addition to 
granular annotations for the required skills. 
% annotate the commonsense phenomenon up to a coarse level. 
% \cite{sugawara2017evaluation}
}

% MutliRC~\cite{khashabi2018looking}, ARC~\cite{CCEKSST18}, \cite{ORMTP18} 
% \cite{MHBSZ18}

% \cite{mihaylov2018knowledgeable}



% \section{Temporal commonsense QA}
\begin{table}[]
\centering
\footnotesize
\resizebox{0.65\textwidth}{!}{
\begin{tabular}{lcc}
\toprule
\multicolumn{2}{l}{Measure}                            & Value         \\
\cmidrule(r){1-2}  \cmidrule(r){3-3}
\multicolumn{2}{l}{\# of unique questions}             & 1893              \\
\multicolumn{2}{l}{\# of unique question-answer pairs}             & 13,225              \\
\multicolumn{2}{l}{avg. sentence length}            & 17.8              \\
\multicolumn{2}{l}{avg. question length}               & 8.2              \\
\multicolumn{2}{l}{avg. answer length}                 & 3.3              \\
\midrule
Category                           & \# questions & avg \# of candidate \\
\cmidrule(r){1-1} \cmidrule(r){2-2} \cmidrule(r){3-3}
\emph{event frequency}                    & 433 & 8.5 \\
\emph{event duration}                     & 440 & 9.4 \\
\emph{event stationarity}                 & 279 & 3.1 \\
\emph{event ordering}                     & 370 & 5.4 \\
\emph{event typical time}                 & 371 & 6.8 \\
\bottomrule
\end{tabular}
}
\caption{\small Statistics of \datasetname. }
    \label{tab:statistics}
\end{table}

\section{Construction of \datasetname}
\label{sec:tacoqa}
\ignore{
In the next steps we describe  a
% our efforts to \ben{generate data suitable for our purposes, and at the same time contain minimal noise.} deal with the noise in the data and making appropriate changes to make it suitable for our purpose. 
% The 
multi-step crowdsourcing scheme, 
% process described above is the result 
resulting from 
 detailed analysis and substantial refinements after multiple pilots studies. 
}
We describe our crowdsourcing scheme for \datasetname{} that is designed after extensive pilot studies. The multi-step scheme asks annotators to generate questions, validate questions, and then label candidate answers.
We use Amazon Mechanical Turk 
%(AMT)  % never used
and restrict our tasks to English-speakers only. Before working on our task, annotators need to read through our guidelines and pass a qualification test designed to ensure their understandings.\footnote{
Our dataset and some related details (such as, our annotation interfaces, guidelines and qualification tests) are available at the following link: { \url{https://bit.ly/2tZ1mkd}}
}

%We use crowdsourcing to annotate different aspects of the dataset. We used Amazon Mechanical Turk (AMT) for our annotations, restricting the task to workers in five English-speaking countries.
% (USA, UK, Canada, and Australia), more than 10$k$ finished HITs and at least a 98\% acceptance rate. \ben{not always true across all stages... I had to lift these on phase 2 to get everything going.}
% Additionally, for each instance of this task, we require the annotators to read through our instructions and 
% For any of the annotations steps describe below, the users are guided to an external platform where first first read the instructions and
% evaluate their understanding by taking a qualification test. 
% step to make sure they have understood the instructions. 
% Only the annotaters that pass the test 
% after successful completion they are allowed
% are allowed to work on the task.


% to start the annotation tasks. 
% The screen-shots of the annotation interfaces for each step are included in Appendix (Section~\ref{sec:supp:screenshots}).
% are provided in the link provided (see Footnote~1). 


\paragraph{Step 1: Question generation.}
In the first step, we ask crowdsourcers to generate questions given a sentence.
%, with respect to given sentences. 
We randomly select 630 sentences from MultiRC~\cite{KCRUR18} (70 from each of the 9 domains) as input sentences. 
To make sure that the questions indeed require temporal commonsense knowledge, we instruct annotators to follow two requirements when generating questions:
% We provide detailed instructions to the annotators and specify two 
%critical  
% requirements for our target questions: 
(a) ``temporal'' questions, from one of our five categories
%the following five categories: \emph{event duration,  stationarity, event ordering, typical time, event frequency} 
(see Fig.~\ref{fig:intro:example}); (b) not having direct answers mentioned in the given sentence.  
% Both requirements are essential to acquire questions that require temporal commonsense knowledge to infer. 
% We also ask annotators to 
% We give the sentences to annotators and ask them to   
% generate one question and one corresponding correct answer for each of the five categories above. Asking for correct answers is to make sure the question is answerable by the annotators themselves.
We also ask annotators to provide a correct answer for each of their questions to make sure that the questions are answerable at least by themselves.
% , and at the same time not having direct answers mentioned in the given sentence. \ben{are we introducing the 5 categories anywhere?} 
%We also ask annotators to provide one correct answer to each of the questions they generate. This is useful to make sure the annotators generate question that they can answer themselves (and not any random question that is not answerable). 
% let themselves validate if the generated question can be answered or not.

\paragraph{Step 2: Question verification.}
To improve the quality of the questions generated in Step~1, we further ask two different annotators to check (a) whether the two requirements above are satisfied and (b) whether there exist grammatical or logical errors.
% In this step, we ask two different annotators to validate the quality of the questions generated in \qiang{Step~1}. Specifically, we ask if each of the questions meet our two requirements (a) and (b) in \qiang{Step~1}. Additionally, we ask for grammatical or logical errors. 
We keep a question if and only if both annotators agree on its quality; since the annotator who provided the question in Step~1 also agrees on it, this leads to a [3/3] agreement for each question. For the questions that we keep, we continue to ask annotators to give one correct answer and one incorrect answer,
% for each question, 
which serve as a seed set for automatic answer expansion in the next step.


\paragraph{Step 3: Candidate answer expansion.}
In the previous steps, we have collected 3 positive and 2 negative answers for each question.\footnote{One positive answer from Step~1; one positive and one negative answer from each of the two annotators in Step~2.} Step~3 aims to automatically expand this set of candidate answers by three approaches. First, we use a set of rules to extract temporal terms (e.g. ``a.m.", ``1990", ``afternoon", ``day"), or numbers and quantities (``2", ``once"), which are replaced by terms randomly selected from a list of temporal units (``second''), adjectives (``early''), points ( ``a.m.'') and adverbs (``always'').
% see the appendix for more details.
% In this step, we expand the collection of 3 positive and 2 negative answers from previous steps.
% For each candidate answer, we use a set of rules to discover temporal terms (e.g. ``a.m.", ``1990", ``afternoon", ``day"), or numbers and quantities (``2", ``once"). We perturb the extracted terms by randomly selecting from a list of possible replacements, sourced from a hard-coded list of temporal units (``second''), adjectives (``early''), points ( ``a.m.'') and adverbs (``always''). 
Examples are ``2 a.m." $\rightarrow$ ``3 p.m.", ``1 day" $\rightarrow$ ``10 days", ``once a week"$\rightarrow$ ``twice a month". 
Second, we mask each individual token in a candidate answer and use \bert{}~\cite{DCLT18} to predict them; we rank those predictions by the confidence level of \bert{} and keep the top ones.
Third, for those candidates representing events, typically there are no temporal terms in them.
We then create a pool of $60k$ event phrases using PropBank~\cite{KingsburyPa02},
% in conjunction with all human generated candidate answers, 
and retrieve the most similar ones to a given candidate answer using an information retrieval (\emph{IR}) system.\footnote{\url{www.elastic.co}} 
We use the three approaches sequentially to expand the candidate answer set to 20 candidates per question.

% \qiangcomment{cite?} % footnote should be put after the period
% This is an industrial system; I don't think people cite anything for this. 
% We can cite sth, but it wouldn't be very accurate. 
% Lucene \ben{cite?} f
% to index them and expand the answer set with events that are similar to either one of the positive or negative answer seeds.

% we use an information retrieval (IR) system\footnote{\url{www.elastic.co}} to generate the best candidates for the task at hand.
% \todo{Clarify: examples of the perturbations}

\paragraph{Step 4: Answer labeling.}
In this step, we ask annotators to label each answer with three options: ``likely'', ``unlikely'', or ``garbage'' (incomplete or meaningless phrases). 
We keep a candidate answer if and only if all 4 annotators agree on ``likely'' or ``unlikely'', and ``garbage'' is not marked by any annotator.
We also discard any questions that end up with no valid candidate answers. 
\ignore{
\qiang{
Before asking annotators to label the candidates, we allow them to filter out illegitimate ones (incomplete or meaningless phrases), and discard a candidate answer if any annotator thinks so. This procedure is important since the set of candidate answers augmented by Step~3 is noisy.
}
% We expand the candidate answer set to a set of 20 in step 3, and prune the illegitimate ones in this step. 
% and in this step 
% We ask annotators to mark all the \emph{likely} answers to the given questions. 
% give each answers a binary label, positive or negative. 
% In addition, we ask annotators to mark any ``garbage'' answers (incomplete or meaningless phrases), and discard an candidate answers if any of the annotations marks it as so.
% that are clearly . 
% Finally, 
% As a result, 
We \qiang{only keep those} candidate answers with complete agreement (\qiang{[4/4]}),
\qiang{and we also discard any questions that end up with no valid candidate answers.}
% We also 
% We then 
% discard questions without any valid candidate answers.
% as our final dataset.
}
Finally, the statistics of \datasetname{} is in Table~\ref{tab:statistics}.
% We provide a summary of the statistics about our dataset in Table~\ref{tab:statistics}. 

% \subsection{Statistics.}
% We provide brief insights into our generated dataset. 
% Table~\ref{tab:statistics}
\ignore{
\begin{table}[]
    \centering
    \footnotesize
    \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{lc}
        \toprule 
         Measure & Value \\ 
         \cmidrule(lr){1-1} \cmidrule(lr){2-2}
        %   \# of unique sentences & 509 \\ % updated but commented
          \# of unique questions & 1,893 \\
          \# of unique question-answer pairs & 13,225 \\
          avg. sentence length & 17.8 \\
          avg. question length & 8.2 \\
          avg. answer length & 3.3 \\
          \midrule 
          \# of \emph{event frequency} questions & 433 \\
          \# of \emph{event duration} questions & 440 \\
          \# of \emph{event stationarity} questions & 279 \\
          \# of \emph{event ordering} questions & 370 \\
          \# of \emph{event typical time} questions & 371 \\
          \midrule
          avg candidate size for \emph{event frequency} questions & 8.5 \\
          avg candidate size for \emph{event duration} questions & 9.4 \\
          avg candidate size for \emph{event stationarity} questions & 3.1\\
          avg candidate size for \emph{event ordering} questions & 5.4  \\
          avg candidate size for \emph{event typical time} questions & 6.8 \\
%           Stationarity	3.1
% Frequency	8.5
% Ordering	5.4
% Typical Time	6.8
% Duration	9.4
        %   \# of ``freq.'' questions \ben{what's this?}\\ 
        %   \# of ``freq.'' questions \\ 
        \bottomrule 
    \end{tabular}
    }
    \caption{\small Statistics of \datasetname. }
    \label{tab:statistics}
\end{table}
}




\section{Experiments}
\label{sec:exp}
We assess the quality of our dataset using a couple of baseline systems. We create a uniform split of 30\%/70\% of the data to dev/test.
The rationale behind this split is that, a successful system has to bring in a huge amount of world knowledge and derive commonsense understandings {\em prior} to the current task evaluation. We therefore believe that it make no sense to expect a system to {\em train} solely on this data, and we think of the development data as only providing a {\em definition} of the task. Indeed, the gains from our development data are marginal after a certain number of observations.
This intuition has been studied and verified in the appendix of~\cite{ZKNR19}.
% mention that question with the same sentence fall in the same category. 

\paragraph{Evaluation metrics.}
Two question-level metrics are adopted in this work: exact match (\emph{EM}) and {\em F1}. EM measures in how many questions a system is able to correctly label all candidate answers, while {\em F1} measures the average overlap between one's predictions and the ground truth (see the appendix of~\cite{ZKNR19} for full definition).
% To measure the quality of all the systems, we use two question-level metrics: 
% EM measures percentage of questions with \emph{all} the candidates answers predicted correctly; \emph{F1} is a looser metric that measures the average overlap between the prediction and ground truth predictions (see the appendix of~\cite{ZKNR19} for full definition).

\paragraph{Human performance.}
An expert annotator also worked on \datasetname{} to gain a better understanding of the human performance on it.
The expert specifically answered 100 questions randomly sampled from the test set, and could only see a single answer at a time, with its corresponding question and sentence.
% We randomly sampled 100 questions from the test set and an expert annotator (one of the authors) answered them. 
\begin{comment}
asked three human annotators on AMT to label each instance. 
% through Mechanical Turk. 
Each annotator could only see a single answer at a time, with its corresponding question and sentence. 
We used the majority vote between three annotators as the label in our evaluation. 
% During inference, we choose their majority vote as the human prediction. 
\end{comment}

\paragraph{Systems.} 
We propose to use two state-of-the-art systems in machine reading comprehension that are suitable for our task.
% To get a better sense of the strength of the challenge we use of the following recent systems. 
\emph{ESIM}~\cite{CZLWJI17} is a neural model effective on natural language inference. We initialize the word embeddings in {\em ESIM} via either \emph{GloVe}~\cite{PenningtonSoMa14} or \emph{ELMo}~\cite{PNIGCLZ18} to demonstrate the effect of pre-training in this task.
% It has been shown effective on several language inference tasks like the SNLI \cite{snli:emnlp2015}. We use the same settings as the model used for SNLI. Here we do not use ELMo in combination to show the impact of large pre-trained language models. 
\bert{} is a recent state-of-the-art contextualized representation used in a broad range of high-level tasks~\cite{DCLT18}. 
We also add unit normalization to \bert{}, which extracts and converts temporal expressions in candidate answers to their most proper units. For example, ``30 months'' will be converted to ``2.5 years".
%, because ``month'' progresses to ``year'' at the value of 12. % QN: redundant
% This systems has shown significant improvements in a few keys task, including one claimed to be a commonsense one~\cite{ZBSC18}. 


\begin{comment}
\paragraph{ESIM} (Supervision baseline without heavy pre-training). 
\emph{ESIM}~\cite{CZLWJI17} is a neural model proposed for natrual language inference. It has been shown effective on several language inference tasks like the SNLI~\cite{snli:emnlp2015}. We use the same settings as the model used for SNLI. Here we do not use \emph{ELMo} in combination to show the impact of large pre-trained language models. 
    
\paragraph{BERT} (Contextual representations). A recent state-of-the-art contextualized representations which has been used across a broad range of high-level tasks~\cite{DCLT18}. 
% This systems has shown significant improvements in a few keys task, including one claimed to be a commonsense one~\cite{ZBSC18}. 
We use \emph{BERT}-base sequence pair classification model with the same parameters as in in BERT's MRPC experiment.\footnote{{github.com/huggingface/pytorch-pretrained-BERT}}
\end{comment}
    

\paragraph{Experimental setting.}
In both \emph{ESIM} baselines, we model the process as a sentence-pair labeling task, following the \emph{SNLI} setting provided in AllenNLP.\footnote{{https://github.com/allenai/allennlp}}
In both versions of \emph{BERT}, we use the same sequence pair classification model and the same parameters as in \emph{BERT}'s \emph{GLUE} experiment.\footnote{{github.com/huggingface/pytorch-pretrained-BERT}}
A system receives two phrases at a time: (a) the concatenation of the sentence and question, and (b) the answer. The system makes a binary prediction on each instance, positive or negative. 

% We train fine-tune with train and dev set, test on the test set.

% We argue that it is reasonable to model over per-question performances, as all the questions has a reasonable range of answers without having any options to choose from. Thus, a system demonstrate a true understanding of the questions only when it correctly predicts the binary label on all answers.

\begin{table}[]
    \centering
    \small 
    \begin{tabular}{ccc}
        \toprule 
         System & \emph{F1} & \emph{EM}  \\ 
         \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} 
         Random  & 36.2 & 8.1 \\ 
         Always Positive & 49.8 & 12.1  \\
         Always Negative & 17.4 & 17.4 \\
         \midrule
         \emph{ESIM + GloVe} & 50.3 & 20.9 \\
         \emph{ESIM + ELMo} & 54.9 & 26.4\\
         \emph{BERT} & 66.1 & 39.6  \\
         \emph{BERT + unit normalization} & \textbf{69.9} & \textbf{42.7}  \\
         \midrule 
         Single Human & 87.1 & 75.8  \\ 
        \bottomrule 
    \end{tabular}
    \caption{\small Summary of the performances for different baselines. All numbers are in percentages. 
    % Best machine performances indicated with \textbf{bold}. 
    % commented out for space 
    }
    \label{tab:performance}
\end{table}

\paragraph{Results and discussion.}
Table~\ref{tab:performance} provides a summary of the results on \datasetname{}, where we compare the {\em ESIM} and \bert{} baselines, along with a few naive baselines (always-positive, always-negative, uniformly random), to the human performance.
The significant improvement brought by contextualized pre-training such as \bert{} and \emph{ELMo} indicates that a significant portion of commonsense knowledge is actually acquired via pre-training.
% To get a better sense of the edge cases we have provided the performance of a few trivial baselines (always-positive, always-negative, uniformly random). 
% \paragraph{Random Baselines} We also compare with 3 instance independent baselines: predicting positive or negative on all potential answers, and uniform selection from positive or negative at each prediction. We repeated the random guessing baseline 1000 times and calculated an average.
We can also see that human annotators achieved a very high performance under both metrics, indicating the high agreement level humans are on for this task. 
Our baselines, including \emph{BERT}, still fall behind the human performance with a significantly margin. 

% \paragraph{Discussion.}
% \section{Discussion}
\begin{comment}
 - error analysis 
    - spreadsheet 
    - more focused on \emph{BERT} 
    - \emph{BERT} doing well on answer-only models
    - over-fitting to data 
 - extended questions: 
     - humans vs \emph{BERT} 
\end{comment}
% \paragraph{BERT analysis}
\begin{figure}
    \centering
    \includegraphics[scale=0.4,trim=1.6cm 0cm 0cm 0cm, clip=false]{figures_temporal_common_sense/performance-per-category-vert-large.pdf}
    \caption{\small \emph{BERT + unit normalization} performance per temporal reasoning category (top), performance gain over random baseline per category (bottom)}
    \label{fig:bert-per-category}
\end{figure}
% Another important \qiang{read from Table~\ref{tab:performance}} is that the significant improvement brought by contextualized pre-training such as \bert{} and \emph{ELMo} indicates that a significant portion of commonsense knowledge is actually acquired via pre-training.
\ignore{
In this section we provide further 
% in-depth 
intuition into our results. 
A major takeaway from the experiments, as expected, is the importance of \emph{contextual pre-training} for a task like ours, which involves much commonsense understanding (unlike tasks where answers are part of the input) \qiangcomment{not sure about the ``unlike'' part}. The best system in our results strongly relies on BERT. Additionally, the combination of \emph{ESIM} with \emph{ELMo} (a contextual pre-trained representation), is much stronger than using \emph{GloVe} as the underlying representations. This indicates the importance of using large amount of world knowledge in this task. \qiangcomment{a bit wordy; can just say ``the significant improvement brought by contextualized pre-training such as \emph{BERT} and \emph{ELMo} indicates that a significant portion of commonsense knowledge is actually acquired via pre-training.''}
}

Further analysis shows that \emph{BERT}, as a language model, is good at associating surface-forms (e.g. associating ``sunrise'' and ``morning'' since they often co-occur), which is highly sensitive to \emph{units} (\emph{days, years, etc}). To address the high sensitivity, we added unit normalization on top of \bert{}, but even with normalization, \emph{BERT+unit normalization} is still far behind the human performance. This implies that the information acquired by \bert{} is still not sufficient to solve this task. Moreover, the low EM scores show that the current systems do not truly understand time in those questions.
% We further analyzed BERT's performance, and we show that language models only understand the surface forms of the temporal knowledge, which is far from actually solving the task. 

\ignore{
However, the system can be brittle when a candidate answer is not mentioned with the typical units (and hence fail to generalize to deeper temporal understanding) \qiangcomment{``deeper'' not clear}.   
}
% However, even with all temporal expressions normalized, in which case maximum support of such association is provided, \emph{BERT+unit normalization} is still far behind human performance. This shows that the information acquired by \bert{} is not sufficient to solve this task. Moreover, low EM scores show that none of the current systems truly understands the question and can produce a sensible range of possible answers.
%without seeing the answers.
% \emph{BERT} does not understand the temporal meaning of phrases, rather it can only rely on signal words like days, years as a proxy of representing the true meanings. 

% observations in the previous section. 
Figure~\ref{fig:bert-per-category} reveals that the performance of \emph{BERT} is not uniform across different categories, which could stem from the nature of those different types of temporal commonsense, quality of the candidate answers, etc. For example, the number of candidates for stationarity questions are much smaller than those for other questions, leading to a relatively easy task, but the performance gain from a random baseline to \bert{}+normalization is not large, indicating that further improvement on stationarity is still difficult.
% Measuring performance per reasoning category reveals that the quality of \emph{BERT} is not uniform across different categories (Figure~\ref{fig:bert-per-category}). Such discrepancy could stem from the nature of the questions, quality of the candidate answers, etc. To show the actual performance on each category, we also provide the gains over a random baseline. As we can see, ordering and duration questions are especially hard. \ben{More on this?}



\begin{comment}
\ben{Drop the next sentences?}
Not surprisingly, 
% That being said, 
 perturbing numbers confuses the system (e.g., ``8 am'' $\rightarrow$ ``3 am'') . Our analysis shows that around $80\%$ of the \emph{BERT} mistakes  can be avoided by incorporating proper handling of the numerical candidate answers. 
%  \todo{clarify this point so that it does not cause misunderstanding}
%  modifying the numbers in the answers to reasonable values, meaning that \emph{BERT} is not considering the actual value of them during inference. 


Moreover, we see that \emph{BERT} has a strong bottom performance when only seeing the answers, which means that it is potentially over-fitting to the data, instead of understanding the questions.
\end{comment}

% \todo{How can we show that ``We need to show that quantity extraction and normalization is not going to be important here. ''?}
\ignore{
\paragraph{Beyond this work.}\qiangcomment{keep it for some time and I'll try to go over it again}
% \daniel{reworded this paragraph: read it? } \benchange{I like the change, but I still think we should drop this.}
% \todo{Drop this or keep it? }
While this work takes a positive step towards the temporal commonsense problem, 
% Even though humans are achieving significant better results on the proposed dataset, 
% this dataset only partially covers the temporal commonsense realm. 
\begin{comment}
it 
% dataset 
only partially covers the full complexity of this problem. 
\end{comment}
there are aspects of this problem that are not covered by our crowdsourced dataset. 
% temporal commonsense realm.
% There are relativley easy ways to extend these questions to make them require higher level reasoning capabilities, where existing systems are far from adequate.
To demonstrate this, one of the authors created a toy dataset of 55 question-answer pairs (20 questions) that require \emph{composing} temporal commonsense of potentially multiple events, rather than just making inferences about isolated events (examples in the appendix of~\cite{ZKNR19}).
% To show this, we manually created a small test set consisting 20 questions 
% and 55 answers. 
% Each of the questions requires a \emph{compositional} understanding of more than one temporal commonsense signals (examples in the appendix of ~\cite{ZKNR19}).
The fine-tuned \emph{BERT} (previous section) achieves \emph{F1}/\emph{EM} of 38.1/0.0; while a human annotator achieves \emph{F1}/\emph{EM} of 69.0/57.1. 
This highlights the necessity of, not only acquiring temporal commonsense, but also being able to \emph{compose} them and make inferences. 
% BERT, as indicated in Table~\ref{tab:extended} significantly suffers with all these problems. This highlights the necessity of developing richer challenges and better representations. 
}

% \begin{table}[h]
%     \centering
%     \small 
%     \begin{tabular}{ccc}
%         \toprule 
%          System & \emph{F1} & \emph{EM}  \\ 
%          \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} 
%          \emph{BERT} & 38.1 & 0.0  \\
%          \midrule 
%          Human & 69.0 & 57.1  \\ 
%         \bottomrule 
%     \end{tabular}
%     \caption{Comparison on the extended questions}
%     \label{tab:extended}
% \end{table}

% \todo{
% Daniel: I am still not a fan of this section; 
% Written in this form, it like punching ourselves. 
% It has to rewriten to convey the point without mis-representing us. 
% }



\section{Summary}
This chapter has focused on the challenge of temporal commonsense.
%understanding. 
Specifically, we framed it as a QA task, defined five categories of questions that capture such ability, and developed a novel crowdsourcing scheme to generate a high-quality dataset for temporal commonsense.
% On top of it, 
We then showed that systems equipped with state-of-the-art language models such as {\em ELMo} and \bert{} are still far behind humans, thus motivating future research in this area. Our analysis sheds light on the capabilities as well as limitations of current models. 
We hope that this study will inspire further research on temporal commonsense. 

%The work addressed the challenge of temporal commonsense understanding. In order to facilitate research in this direction we proposed a challenge oriented towards \emph{temporal understanding} in the form of QA task, a first of its kind in the field. We showed that the state-of-the-art has a significant distance with human performance on our task. Additionally, we provided new analysis that sheds light on capabilities and limitations of these models. 
%We hope that this resource will encourage our community to invest more effort to inducing temporal understanding in natural language models. 
% To the best of our knowledge, this is the first work creating su


==> Daniel K - thesis - dissertation/6.theory_new.tex <==
\chapter{Capabilities and Limitations of Reasoning in Natural Language}
\label{chapter:limits}
% \epigraph{ 
% ``You don't have to believe in God, but you should believe in The Book.''
% }{--- \textup{Paul Erd\H{o}s}, 1985 }
\epigraph{ 
``Language is froth on the surface of thought.''
}{--- \textup{John McCarthy} }




% \title{On the Power and Limitations of Graph-based Reasoning}
% \title{On the Power and Limitations of Reasoning on Graphical Knowledge}
% \title{On Capabilities and Limitations of Reasoning}
% \title{On Possibilities and Limitations of Reasoning}
% \title{On Possibilities and Limitations of Reasoning Over ``Natural'' Information}
% \title{A Little Reasoning is Probably Necessary (and Enough)}
% \title{Few Reasoning Steps Might be Necessary (and Enough)}
% \title{Reasoning on ``The Book"}
% \title{On Capabilities and Limitations of Reasoning \\ in the Presence of Symbol-Grounding Problem}
% \title{On the Capabilities and Limits of multi-hop Reasoning\\ Under Symbol-Grounding Uncertainty}
% \title{On the Capabilities and Limitations of Reasoning\\ for Natural Language Understanding}


\newif\iftacl
% \tacltrue


\section{Introduction}

Reasoning can be defined as the process 
of combining facts and beliefs, in order to make decisions~\citep{Johnson-Laird80}. 
In particular, in natural language processing (NLP), it has been 
studied under various settings, such as question-answering (QA)~\citep{HLBB99}. 



\begin{wrapfigure}{r}{0.5\textwidth}
% \begin{figure}
    \centering
    % \includegraphics[trim=0.3cm 0.1cm 0cm 1cm, clip=false, scale=0.41]{figures/intro-figure-9.png}
    \includegraphics[trim=0.31cm 0.05cm 0cm 1.3cm, clip=false, scale=0.31]{figures_theory/intro-figure-11.png}
    \vspace{-0.2cm}
    % \vspace{-0.2cm}
    \caption{
    The interface between meanings and symbols: each \colorbox{lightred}{meaning} (top) can be \colorbox{lightyellow}{\emph{uttered}} in many ways into \colorbox{lightgreen}{symbolic} forms (bottom). 
    % the \emph{symbol space} (bottom) is how we express knowledge; the \emph{meaning space} (top) is the level at which we abstract.
    }
    \label{fig:intro-figure}
% \end{figure}
\end{wrapfigure}
While there is a rich literature on reasoning, 
there is little understanding of the 
nature of the problem and its limitations, especially in the context of natural language. 
\begin{comment}
Early reasoning formalisms in AI were 
mostly based on models of symbolic representations of world knowledge~\citep{McCarthy63}. 
Later on, effort shifted towards a softer notion of symbols, by incorporating uncertainty into symbolic models~\citep{Zadeh75,Pearl1989ProbabilisticRI,SelmanLe90}. 
\end{comment}
In particular, there remains a sizable gap between empirical understanding of reasoning algorithms for language and the theoretical guarantees for their quality, often due to the complexity of the reality they operate on.
An important challenge in many language understanding problems 
% One such complication 
is 
the \emph{symbol grounding problem}~\citep{Harnad90}, %which is 
the problem of accurately mapping symbols into its underlying meaning representation.
Practitioners often address this challenging by enriching their representations; 
% circumvent this challenge via empirical solutions that appear to work well for the domain at hand;
for example by mapping textual information to Wikipedia entries~\citep{MihalceaCs07,RRDA11}, or grounding text to executable rules via semantic parsing~\citep{RTPSL17}. 
{
Building upon such representations, 
%the community 
has produced various reasoning systems that essentially work by combining local information. 
}


This work introduces a formalism that incorporates elements of the symbol-grounding problem, via the two spaces illustrated in Figure~\ref{fig:intro-figure}, and sheds theoretical light on existing %empirical
intuitions.\footnote{This chapter is based on the following publication: \cite{KSKSR19}.} The formalism consists of (A) an abstract model of linguistic knowledge, and (B) a reasoning model.


\noindent
\textbf{(A) Linguistically-inspired abstract model:}
We propose a theoretical framework to model and study the capabilities/limitations of reasoning, especially when taking into account key difficulties that arise when formalizing linguistic reasoning. Our model uses two spaces; cf.~Figure~\ref{fig:intro-figure}. We refer to the internal conceptualization in the human mind as the \colorbox{lightred}{\emph{meaning space}}. We assume the information in this space is free of noise and uncertainty.
In contrast to human thinking in this space, \emph{human expression} of thought via the \colorbox{lightyellow}{utterance} of language introduces many imperfections. 
The information in this linguistic space---which we refer to as the \colorbox{lightgreen}{\emph{symbol space}}---has many language-specific properties. 
The symbolic space is often redundant (e.g., multiple symbols ``CPU'' and ``computer processor'' express the same meaning), ambiguous (e.g., a symbol like ``chips'' could refer to multiple meanings ), incomplete (relations between some symbolic nodes might be missing), and inaccurate (there might be incorrect edges).
% While human brain functions in the meaning space, a machine reasoning algorithm operates in the symbol space. 
Importantly, this noisy symbol space is also what a machine reasoning algorithm operates in.


% ``\emph{present day spoons are made from metal such as steel ...}''. 
% While variability of language makes it difficult to map symbols to their meaning, it also results in \emph{redundancy} of popular facts. We model this phenomenon by mapping each unit of meaning 
% to potentially multiple items in the symbol space. 

\noindent
\textbf{(B) Reasoning model:}
We define reasoning as the ability to infer the existence of properties of interest  
 in the \colorbox{lightred}{\emph{meaning} space}, by observing only its 
 %noisy 
 representation in the \colorbox{lightgreen}{\emph{symbol} space}. 
The target property 
in the meaning graph is what characterizes the nature of the reasoning algorithm, e.g., are two nodes connected. 
While there are many flavors of reasoning (including \emph{multi-hop reasoning}), 
in this first study, we explore a
common primitive shared among various reasoning formalisms; namely, the \emph{connectivity problem} between a pair of nodes in an undirected graph in the \colorbox{lightred}{meaning space}, while observing its noisy version in the \colorbox{lightgreen}{symbol space}.
This simplification clarifies 
%helps with the clarity of 
the exposition and the analysis,and we expect similar results to hold for a broader class of reasoning algorithms
%as well, 
that rely on connectivity. %sub-routine as a main ingredient. 
% \dan{moved the comment on the figure after the Reasoning part}

\begin{figure*}
    \centering
    \includegraphics[trim=0cm 1.1cm 0cm 0cm, clip=false, scale=0.287]{figures_theory/intro-example-6.png}
    \caption{
    \small
    The \colorbox{lightred}{meaning space} contains [clean and unique] symbolic representation and the facts, while the \colorbox{lightgreen}{symbol space} contains [noisy, incomplete and variable] representation of the facts. We show sample meaning and symbol space nodes to answer the question: \textit{Is a metal spoon a good conductor of heat?}.
    }
    \label{fig:ny-example}
\end{figure*}

Figure~\ref{fig:ny-example} illustrates a reasoning setting where the semantics of the edges is included. Most humans understand that \emph{\textbf{V1}:``present day spoons''} and \emph{\textbf{V2}:``the metal spoons''} are equivalent nodes (have the same meaning). However, a machine has to infer this understanding. % Similarly the equivalence of the  \emph{\textbf{V3}}, \emph{\textbf{V4}} nodes 
The semantics of the connection between nodes are expressed through natural language sentences. 
For example, connectivity could express the semantic relation between two nodes: {\tt \small \textbf{has-property(metal,thermal-conductor)}}. However a machine may find it difficult to infer this fact from, say, reading text over the Internet as it may be expressed in many different ways, e.g., 
can be found in a sentence like \emph{``dense materials such as [\textbf{V3:}]metals and stones are [\textbf{V5:}]good conductors of heat''}. 

\begin{sloppypar}
To ground this in existing efforts, consider \emph{multi-hop} reasoning for QA systems~\citep{KKSCER16,JWMM18}. Here the reasoning task is to connect local information, via multiple local ``hops'', in order to arrive at a conclusion. In the meaning graph, one can trace a path of locally connected nodes to verify the correctness of a query; for example the query {\tt \small \textbf{has-property(metal-spoon, thermal-conductor)}}
% \footnote{This is a reformulation of a multiple-choice question from OpenBookQA~\citep{openqa2018}.} 
can be verified by tracing a sequence of nodes, as shown in Figure~\ref{fig:ny-example}. 
% However, there is no path supporting the query {\tt \small \textbf{has-property(blue-jeans, thermal-conductor)}}. 
In other words, answering queries can be cast as inferring the existence of {a 
% \erfan{Why length of the path matters in theoretical view?} 
% short-enough 
path} connecting two nodes $m$ and $m'$.
\footnote{This particular grounding is meant to help relate our graph-based formalism to existing applications, and is 
not the only way of realizing reasoning on graphs.}
While doing so on the \colorbox{lightred}{meaning graph} is straightforward, doing so on the noisy \colorbox{lightgreen}{symbol graph} is not. Intuitively, each local ``hop'' introduces more noise, allowing reliable inference to be performed only when it does not require too many steps in the underlying \colorbox{lightred}{meaning space}. To study this issue, one must quantify the effect of noise accumulation for long-range reasoning.
\end{sloppypar}


% We formally show that for any reasoning algorithms there is a logarithmic barrier on the maximum number  
% and knowing the representative nodes to $m$ and $m'$ in the symbol graph.  
% For example, if the event-of-interest is defined as the connectivity of the a node-pair in the meaning graph, which can be thought of multi-hop reasoning~\citep{tableilp2016:ijcai}. 

% \paragraph{Contributions.}
\textbf{Contributions.}
We believe that this is the first work to provide a mathematical study of the 
challenges
%possibilities 
and limitations of reasoning algorithms in the presence of the symbol-meaning mapping challenge.
We make three main contributions.

First, we establish a novel, linguistically motivated formal framework for analyzing the problem of reasoning about the ground truth (the meaning space) while operating over a noisy and incomplete linguistic representation (the symbol space). This framework allows one to derive rigorous intuitions about what various classes of reasoning algorithms \emph{can} and \emph{cannot} achieve.
%with noisy graphical knowledge~\citep{quillian1967word}.
% \dan{commented out something here: graphical knowledge is just a way to visualize things, not inherent issue. note also additions/clarifications below.}

Second, we study in detail the \emph{connectivity reasoning} problem, in particular the interplay between the noise level in the symbol space (due to ambiguity, variability, and missing information) and the distance (in terms of inference steps, or hops) between two elements in the meaning space. We prove that under low noise levels, it is indeed possible to perform reliable connectivity reasoning up to a few hops (Theorem~\ref{the:reasoning:possiblity}). On the flip side, even a moderate increase in the noise level makes it difficult to assess the connectivity of elements if they are logarithmic distance apart in the meaning space (Theorems~\ref{th:multi-hop:impossiblity} and~\ref{theorem:impossiblity:general:reasoning}). This finding is aligned with empirical observations of 
% Interestingly, many such empirical efforts have independently observed  
``semantic drift'', i.e., substantial drop in performance beyond a few (usually 2-3) hops~\citep{FJHSC15,Jansen16}.
% \ignore{This is usually referred to as 
% with the
% \emph{small-world phenomenon}~\citep{newman2002random} observed often, for example in social networks.}
% \dan{commented out previous sentence; I think it's not true; this phenomenon is an observation about data, not about ease of inference}

Third, we apply the framework to a subset of a real-world knowledge-base, FB15k237, treated as the meaning graph, illustrating how key noise parameters influence the possibility (or not) of accurately solving the connectivity problem.





%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}

\paragraph{Classical views on reasoning.}
%
Philosophers, all the way from Aristotle and Avicenna, were the first ones to notice reasoning and rationalism
% , almost right from the beginning of Philosophy
~\citep{KirkRaSc83,Davidson92}. 
% . 
% thousands of years ago. We encourage readers to refer to existing literature reviews
% locke1836essay,
In modern philosophy, the earlier notions were mixed with mathematical logic, resulting in formal theories of reasoning, such as deductive,
% ~\citep{EvansNeBy93}, 
inductive,
% ~\citep{HHNT89}, 
and abductive reasoning~\citep{Peirce83}.
Our treatment of reasoning applies to all these, that can be 
modeled and executed using graphical representations. 
%on graphical knowledge. 
% Specifically our approach to multi-hop reasoning is closely related to abductive learning, i.e.,
% \emph{finding the best simplest explanation}/
% {\emph{finding the simplest and the most likely explanation}.}
% \tushar{typo?}. 
% However, the framework can be applicable to other forms of classical reasoning with some modification. \tushar{Interesting history on reasoning but seems too long to just say "we do abductive reasoning too"}


\paragraph{Reasoning in AI literature.}
The AI literature has seen a  variety of formalisms for automated reasoning. 
These include, reasoning with logical representations~\citep{McCarthy63}, semantic networks~\citep{Quillan66}, frame-semantic based systems~\citep{Fillmore77}, Bayesian networks~\citep{Pearl88}, among others.
%just to name a few. 
% AI literature is rich with variations of formal logic in the form of automated reasoning. 
% A prime example is \emph{logic programming} a paradigm in which facts and rules about some problem domain are expressed in atomic logical clauses and inference rules, which are later solved by a logic-based deduction system~\citep{green1969applications}. 
% This was used to build landmark natural-language applications like SHRDLU~\citep{winograd1971procedures}. 

It is widely believed that a key obstacle to progress has been the \emph{symbol grounding problem}~\citep{Harnad90,TaddeoFl05}. 
%, which is the issue connecting symbols to their actual meaning. 
\begin{comment}
While human brain is adept in mapping sequences of symbols to meaningful thoughts -- often based on personal experiences-- for computers it is unclear how symbols (e.g., sequences of words) should be connected to their actual meaning. 
\cite{TaddeoFl05} provide an analysis of the requirement that must be satisfied by any hypothesis algorithm seeking to solve the symbol-grounding problem.
The authors also show how a collection of existing algorithms do not 
% analyze a few approaches and conclude that none 
satisfy the requirements, hence none will solve the symbol grounding problem. 
% \tushar{What was a positive conclusion of this paper i.e., we know that x can only go as far as y ?}
\end{comment}
Our formalism is directly relevant to this issue. 
We assume that symbols available to reasoning systems are results of communication meaning n natural language. This results in ambiguity since a given symbol could be mapped to multiple actual meanings but also in variablity (redundancy).  
%of utterances of meanings. Such utterance could result in ambiguity since it might be unclear how to map the symbols to their actual meanings, however the redundancy of the utterances could help the reasoners to cope with the issue. 

% This issue had major consequences on the strategies for containing the knowledge (also known as \emph{knowledge representation}).
% \cite{stanfill1986toward} argued reasoning should be on ``memories of specific episodes'', rather than rules. The \emph{connectionist} paradigm~\citep{clark1989connectionism,Shastri1993FROMSA} favored a distributed representation of notions, rather than explicit representation, which laid the foundation for neural networks. 

\begin{comment}
The uncertainty of real problems~\citep{schutze1996ambiguity} pushed for development of systems which rely on relative truths. This resulted in theories like fuzzy-logic~\citep{Zadeh75}, or probabilistic Bayesian networks~\citep{Neapolitan1990ProbabilisticRI,Dechter13}, default reasoning~\citep{HSME88,SelmanLe90,Poole90}. 
% , and the theory of PAC-learning~\citep{valiatnt1984theory}. 
% approximate learning of concepts with probabilistic guarantees 
In this work we disregard the issue of uncertainty and focus on the scenarios where the correct (but hidden) decision is certain. 
\end{comment}

\paragraph{Reasoning for natural language comprehension.}
%In the context of natural-language applications, the linguistic views are reasoning are mixed with AI literature. 
In the context of natural language applications (such as QA) flavors of linguistic theories are blended with the foundation provided by AI. 
A major roadblock has been 
% part of these combinations concern 
the problem of \emph{symbol grounding}, or grounding free-form texts to a higher-level meaning. Example proposals to deal with this issue are, extracting semantic parses~\citep{KaplanBrot82,SteedmanBa11,BBCGGHKPS13}, linking to the knowledge bases~\citep{MihalceaCs07}, mapping to semantic frames~\citep{PunyakanokRoYi04}, etc. These methods can be thought of as approximate solutions for grounding symbolic information to some \emph{meaning}. \citep{RothYi04} suggested a general abductive framework that addresses it by connecting reasoning to models learned from data; it has been used in multiple NLP reasoning problems~\citep{KKSR18}.

% \dan{Added reference to Roth, Yih; we could have cut a lot of this section, I think.}

On the execution of reasoning with the disambiguated inputs there are varieties of proposals, e.g., using executable formulas~\citep{RTPSL17,AngeliMa14}, chaining relations to infer new relations~\citep{SCMN13,MNDB17,KhotSaCl17}, 
% learning-theoretic frameworks~\citep{Schmidhuber2015DeepLI} 
and possible combinations of the aforementioned paradigms~\citep{GardnerTaMi15,CEKSTTK16}. 
Our analysis covers any algorithm for inferring patterns that can be formulated in graph-based knowledge, e.g.,  
% In our work we study a special family of algorithms where the discovery of the event of interest can be formulated as a 
chaining local information, often referred to as \emph{multi-hop} reasoning~\citep{JBSC16,JWMM18,LinSoXi18}. 
% for  result and an impossibility result, which lays theoretical justifications for what has already been observed empirically. 
% Our formal findings shed light on some existing empirical intuitions. 
For example, \cite{JSSC17} propose a structured multi-hop reasoning by aggregating sentential information from multiple knowledge bases. The work shows that while this strategy improves over baselines with no reasoning (showing the effectiveness of reasoning), with aggregation of more than 2-3 sentences the quality declines (showing a limitation for reasoning). Similar observations were also made in~\citep{KKSCER16}. These empirical observations support the theoretical intuition proven in this work. 

% \citep{Bottou2013FromML}

% It is noteworthy that there are other proposals that deviated from the \emph{reasoning-on-top-of-knowledge} design: for example 
% \daniel{talk about reasonign, multi-hop and chaining}
% Inference on graphical-models
% \citep{Dechter2013ReasoningWP}
% Entailment by logical-entailment rules 
% \citep{AngeliMa14}
% Reasoning about quantities 
% \citep{Roy2015ReasoningAQ}
% Roy2015ReasoningAQ 


%% not used: 
% matthew effects \citep{stanovich2009matthew}
% Reasoning is often loosely defined as the ability to chain the atomic facts to make a cohrent conclusion. 
% \citep{CCEKSST18}
% \citep{Johnsonlaird2015LogicPA}
% World knowledge is limited: 
% \citep{Angeli2015LeveragingLS}
% \citep{Etzioni2011OpenIE}
% \citep{JBSC16}
% \citep{JWMM18}
% \citep{jain2016question}
% \citep{Zhang2018VariationalRF}
% \citep{karp1990transitive}
% \todo{have a section on multi-hop reasoning}
% \citep{das2018reasoning}

%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Background and Notation}
\label{sec:background}
We start with basic definitions and notation. 
% We follow the standard notation for asymptotic comparison of functions: 
% $O(.), o(.), \Theta(.), \Omega(.),$ and $\omega(.)$~\citep{CLRS09}.

\paragraph{Graph Theory.}
%
We denote an undirected graph with $G(V, E)$ where $V$ and $E$ are the sets of nodes and edges, resp. We use the notations $V_G$ and $E_G$ to  refer to the nodes and edges of a graph $G$, respectively. 
Let $\dist(v_i, v_j)$ be the distance between nodes $v_i$ and $v_j$ in $G$. 
A \emph{simple path} (henceforth referred to as just a \emph{path}) is a sequence of adjacent nodes that does not have repeating nodes. Let $v_i \pathk{d} v_j$ denote the existence of a path of length $d$ between $v_i$ and $v_j$. Similarly, $v_i \npathk{} v_j$ denotes that there is no path between $v_i$ and $v_j$. We define the notion of $d$-\emph{neighborhood} in order to analyze local properties of the graphs:  
%
\begin{definition}
For a graph $G = (V,E)$, $s \in V$, and $d \in \mathbb{N}$, the \emph{$d$-neighbourhood} of $s$ is $\{v \mid \dist(s,v) \leq d\}$, i.e., the `ball' of radius $d$ around $s$. $\ball(s,d)$ denotes the number of nodes in this $d$-neighborhood, and $\ball(d) = \max_{s \in V} \ball(s,d)$.
\end{definition}

Finally, a \emph{cut} $C = (S,T)$ in $G$ is a partition of the nodes $V$ into subsets $S$ and $T$. The \emph{size} of the cut $C$ is the number of edges in $E$ with one endpoint in $S$ and the other in $T$.

\paragraph{Probability Theory.}
$X \sim f(\theta)$ denotes a random variable $X$ distributed according to probability distribution $f(\theta)$, paramterized by $\theta$. 
% The mean and variance of $X$ are denoted as 
% $\mathbb{E}_{X \sim f(\theta)}[X]$ and $\mathbb{V}[X]$, resp.
% $\bern{p}$ and $\bin{n,p}$ denote the Bernoulli and Binomial distributions, resp.

Given random variables $X\sim\bern{p}$ and $Y\sim\bern{q}$, their disjunction $X \vee Y$ is another Bernoulli $\bern{p \oplus q }$, where  
$p \oplus q \triangleq 1 - (1-p)(1-q) = p + q - pq$. We will make extensive use of this notation throughout this work. 
% , which indicates the disjunction between two Bernoulli random variables with probabilities $p$ and $q$. 


%%%%%%%%%%%%%%%%%%%%%%%%
\section{The Meaning-Symbol Interface}
\label{sec:framework}

We introduce two notions of knowledge spaces: 
\begin{itemize}
\itemsep0em 
    \item The \emph{meaning space}, $M$, is a conceptual hidden space where all the facts are accurate and complete. 
    We assume the knowledge in this space can be represented as an undirected graph, denoted \Gm. 
    This 
    knowledge is 
    % supposed to be 
    hidden, and representative of the information that exists within human minds. 

    \item The \emph{symbol space}, $S$, 
    is the space of written sentences, curated knowledge-based, etc., in which knowledge is represented for human and machine consumption. We assume access to a knowledge graph \Gs\ in this space that is an incomplete, noisy, redundant, and ambiguous approximation of $G_M$.
\end{itemize}

There are interactions between the two spaces: when we read a sentence, we are reading from the \emph{symbol space} and interpreting it 
%to our understanding, i.e., 
in the \emph{meaning space}. 
When writing out our thoughts, we symbolize our thought process, by moving them from \emph{meaning space} to the \emph{symbol space}. 
Figure~\ref{fig:intro-figure} provides a high-level view of the framework. A reasoning system is not aware of the exact structure and information encoded in the meaning graph.

The only information given is the ball-assumption, i.e., we assume that each node $m$ is connected to at most $\ball(m, d)$ many nodes, within distance at most $d$. If this bound holds for all the nodes in a graph, we'd simply write it as $\ball(d)$. The ball assumption is a simple understanding of the maximum-connectivity in the meaning-graph, without knowing the details of the connections. 


\paragraph{Meaning-Symbol mapping.}
We define an oracle function $\oracle: M \rightarrow  2^S$ that map nodes in the meaning space to those in the symbol space. When $s\in \oracle(m)$, with some abuse of notation, we write $\oracle^{-1}(s)=m$. 

% \todo{maybe use this notation everywhere }

\paragraph{Generative Modeling of Symbol Graphs.}
We now explain a generative process for constructing symbol graphs. Starting with \gm, we sample a symbol graph $G_S \leftarrow \alg{G_M}$ using a stochastic process, detailed in Algorithm~\ref{al:sampling}. Informally, the algorithm simulates the process of transforming conceptual information into linguistic utterances (web-pages, conversations, knowledge-bases).

Our stochastic process has three main parameters: (a) the distribution $r(\lambda)$ of the number of replicated symbols to be created for each node in the meaning space; (b) the edge retention probability $p_+$; and (c) the noisy edge creation probability $p_-$. We will discuss later the regimes under which Algorithm~\ref{al:sampling} generates interesting symbol graphs.

{
\begin{algorithm}[t]
% \SetAlgoLined
\footnotesize
\KwIn{Meaning graph \Gm, discrete distribution $r(\lambda)$, edge retention probability $p_+$, edge creation probability $p_-$}
\KwOut{Symbol graph \Gs}
 \ForEach{$v \in \vm$}{
     sample $k \sim r(\lambda)$ \\
     construct a collection of new nodes $U$ s.t.\ $|U| = k$ \\
    %  (the size of $U$ follows a discrete distribution). \\ 
     $\vs \leftarrow \vs  \cup U$  \\ 
    %  For any $u \in U$, \oracle$(v, u) = 1$. 
    \oracle$(v) \leftarrow U$
 }
 
 \ForEach{$(m_1,  m_2) \in (\vm \times \vm), m_1 \neq m_2$}{
    $S_1 \leftarrow \oracle(m_1)$, $S_2 \leftarrow \oracle(m_2)$  \\ 
    \ForEach{$e \in S_1 \times S_2$}{
        \eIf{$(m_1,  m_2) \in \emm$}{
            with probability $p_+$: $\es \leftarrow \es  \cup \{ e \} $   
        }{ 
            with probability $p_-$: $\es \leftarrow \es  \cup \{ e \} $
        }
    }
 }
 \caption{
%  \fontsize{10pt}{10pt}\selectfont
 Generative construction of knowledge graphs; sampling a symbol knowledge graph \gs\ given a meaning graph \gm. 
 }
 \label{al:sampling}
\end{algorithm}
}

This construction models a few key properties of linguistic representation of meaning. Each node in the meaning space is potentially mapped to multiple nodes in the symbol space, which models redundancy. 
Incompleteness of knowledge is modeled by the fact that not all meaning space edges appear in the symbol space {(controlled by parameter $p_+$ in Algorithm~\ref{al:sampling})}.  {There are also edges in the symbol space that do not correspond to any edges in the meaning space and account for the noise (controlled by parameter $p_-$ in Algorithm~\ref{al:sampling}).}
% \erfan{Not super clear} 
%\tushar{Rather than oscillating between handling ambiguity or not, how about the following insteadTo deal with ambiguity, i.e., a single node in the symbol graph mapping to multiple meaning nodes, we define linguistic similarity connections between nodes in symbol graph. Nodes with these similarity connections are assumed to have the same meaning. We can then introduce ambiguity by adding a connection between two symbol nodes that originate from different meaning nodes. }
%\daniel{We model ambiguity by introducing ... }

Next, we introduce a linguistic similarity based connection to model ambiguity, i.e., a single node in the symbol graph mapping to multiple nodes in the meaning graph.
{
The ambiguity phenomena is modelled indirectly via the linguistic similarity based connections (discussed next). 
We view ambiguity as treating (or confusing) two symbol nodes as the same even when they originate from different nodes in the meaning space.
}

\paragraph{Noisy Similarity Metric.}
Similarity metrics are typically used to judge the equivalence of symbolic assertions. Let $\rho: V_S \times V_S \rightarrow \{0, 1\}$ be such a metric, where $\rho(s, s')=1$ denotes the equivalence of two nodes in the symbol graph. Specifically, we define the similarity to be a noisy version of the true node similarity between node pairs:
\vspace{-0.05cm}
\begin{align*}
\rho(s, s') \triangleq &
  \begin{cases}
  1 - \text{Bern}(\varepsilon_+) &  \text{if\ } \oracle^{-1}(s) = \oracle^{-1}(s') \\ 
  \text{Bern}(\varepsilon_-) &  \text{otherwise}
  \end{cases}, 
  \vspace{-0.05cm}
\end{align*}
where $\varepsilon_+, \varepsilon_- \in (0, 1)$ are the noise parameters of the similarity function, both typically close to zero. 
{
Intuitively, the  similarity function is a \emph{perturbed} version of ground-truth similarities, with small random noise (parameterized with $\varepsilon_+$ and $\varepsilon_-$). Specifically with a high probability $1-\varepsilon_{+/-}$, it returns the correct similarity decision (i.e., whether two symbols have the same meaning); and with a low probability $\varepsilon_{+/-}$ it returns an incorrect similarity decision. In particular, $\varepsilon_+ = \varepsilon_- = 0$ models the perfect similarity metric. In practice, even the best entailment/similarity systems have some noise (modeled as $\varepsilon_{+/-} > 0$). 
}

We assume algorithms have access to the symbol graph $\gs$ and the similarity function $\rho$, and that they use the following procedure to verify the existence of a connection  
% \ashish{I think you mean a direct connection, not a path. Right?} 
between two nodes: 
\FrameSep0pt
\begin{framed}
  \begin{algorithmic}
        \Function{NodePairConnectivity}{$s, s'$}
         \State \textbf{return} $(s, s') \in E_S$ or $\rho(s, s') = 1$ 
        \EndFunction
    \end{algorithmic}
\end{framed}


There are many corner cases that result in uninteresting meaning or symbol graphs. 
Below we define the regime of realistic instances:

\begin{definition}[Nontrivial Graph Instances]
\label{defn:nontrivial}
    A pair ($\gm, \gs$) of a meaning graph and a symbol graph sampled from it is \emph{non-trivial} if it satisfies: 
    \begin{enumerate}
        \itemsep0em 
        \item non-zero noise, i.e., $p_-, \varepsilon_-, \varepsilon_+ > 0$; 
        
        \item incomplete information, i.e., $p_+ < 1$;
        
        \item noise content does not dominate the actual information, i.e., $p_- \ll p_+, \varepsilon_+ < 0.5$ and $p_+ > 0.5$; 
        
        \item \gm\ is not overly-connected, i.e., $\ball(d) \in o(n)$, where $n$ is the number of nodes in $\gm$;
        
        \item \gm\ is not overly-sparse, i.e., $|E_{G_M}| \in \omega(1)$. 
    \end{enumerate}
\end{definition}
%
Henceforth, we will only consider sampling parameters satisfying the above conditions.

\paragraph{Reasoning About Meaning, through Symbols.}
%
While the reasoning engine only sees the symbol graph $G_S$, it must make inferences about the potential latent meaning graph. Given a pair of nodes $\tuple:= \{s, s'\} \subset V_S$ in the symbol graph, the reasoning algorithm must then predict properties about the corresponding nodes $\tuplem =\{m, m'\} = \{ \oracle^{-1}(s), \oracle^{-1}(s') \}$ in the meaning graph. 

We use a hypothesis testing setup to assess the likelihood of two disjoint hypotheses defined over these meaning nodes:
$H^{\circled{1}}_M(\tuplem)$ and $H^{\circled{2}}_M(\tuplem)$. Given observations about the symbol nodes, defined as $X_S(\tuple)$, the goal of a reasoning algorithm is to identify which of the two hypotheses about the meaning graph has a higher likelihood of resulting in these observations under the sampling process of Algorithm~\ref{al:sampling}. Formally, we are interested in:
\vspace{-0.05cm}
\begin{equation}
\label{eq:decision}
\underset{h \in \{ H^{\circled{1}}_M(\tuplem), 
% H^{\circled{2}}_M(\tuplem)\}}{\text{argmax}}  \prob{e |  E_S(\tuple)}.
H^{\circled{2}}_M(\tuplem)\}}{\text{argmax}}  \probTwo{h}{X_S(\tuple)}
\end{equation}
\vspace{-0.03cm}
where $\probTwo{h}{x}$ denotes the probability of an event $x$ in the sample space induced by Algorithm~\ref{al:sampling} on the latent meaning graph $\gm$ when it satisfies hypothesis $h$.

Since we start with two disjoint hypotheses on $\gm$, the resulting probability spaces are generally different, making it plausible to identify the correct hypothesis with high confidence. At the same time, with sufficient noise in the sampling process, it can also become difficult for an algorithm to distinguish the two resulting probability spaces (corresponding to the two hypotheses)  especially depending on the observations $X_S(\tuple)$ used by the algorithm. For example, the distance between the symbolic nodes can often be an insufficient indicator for distinguishing these hypotheses. We will explore these two contrasting behaviors in the next section.


\begin{definition}[Reasoning Problem]
    The input for an instance $\ins$ of the \emph{reasoning problem} is a collection of parameters that characterize how a symbol graph $\gs$ is generated from a (latent) meaning graph $\gm$, two hypotheses $H^{\circled{1}}_M(\tuplem), H^{\circled{2}}_M(\tuplem)$ about $\gm$, and available observations $X_S(\tuple)$ in $\gs$.
    The reasoning problem, $\ins(p_+$, $p_-$, $\varepsilon_+$, $\varepsilon_-$, $\ball(d)$, n, $\lambda$, $H^{\circled{1}}_M(\tuplem)$, $H^{\circled{2}}_M(\tuplem)$, $X_S(\tuple))$, is to map the input to the hypothesis $h$ as per Eq.~(\ref{eq:decision}).
\end{definition}



We use the following notion to measure the effectiveness of the observation $X_S$ in distinguishing between the two hypotheses as in Eq.~(\ref{eq:decision}):
\vspace{-0.05cm}
\begin{definition}[$\gamma$-Separation]
\label{defn:gamma-separation}
    For $\gamma \in [0,1]$ and a problem instance $\ins$ with two hypotheses $h_1 = H^{\circled{1}}_M(\tuplem)$ and $h_2 = H^{\circled{2}}_M(\tuplem)$, we say an observation $X_S(\tuple)$ in the symbol space $\gamma$-separates $h_1$ from $h_2$ if: 
    $$
        \probTwo{ h_1 }{ X_S(\tuple) } - \probTwo{ h_2 }{ X_S(\tuple) } \, \geq \, \gamma.
    $$
    %  \begin{align}
    %     \label{eq:reasoning:probs}
    %      \begin{cases}
    %      \probTwo{ h_1 }{ X_S(\tuple) } > 1 - \delta \\ 
    %      \probTwo{ h_2 }{ X_S(\tuple) } < \delta 
    %      \end{cases}
    %  \end{align}
\end{definition}
\vspace{-0.05cm}
We can view $\gamma$ as the \emph{gap} between the likelihoods of the observation $X_S(\tuple)$ having originated from a meaning graph satisfying hypothesis $h_1$ vs.\ one satisfying hypothesis $h_2$. When $\gamma = 1$, $X_S(\tuple)$ is a perfect discriminator for distinguishing $h_1$ and $h_2$. In general, any positive 
% value of 
$\gamma$ bounded away from $1$ yields a valuable observation.\footnote{If the above probability gap is negative, one can instead use the complement of $X_S(\tuple)$ for $\gamma$-separation.}

Given an observation $X_S$ that $\gamma$-separates $h_1$ and $h_2$, there is a simple algorithm that distinguishes $h_1$ from $h_2$:
%
\FrameSep0pt
\begin{framed}
  \small 
  \begin{algorithmic}
        \Function{Separator$_{X_S}$}{$\gs, \tuple=\{s, s'\}$}
         \State \textbf{if} $X_S(\tuple) = 1$
            {\textbf{then} return $h_1$}
            {\textbf{else} return $h_2$}
        \EndFunction
    \end{algorithmic}
\end{framed}

Importantly, this algorithm does \emph{not} compute the probabilities in Definition~\ref{defn:gamma-separation}. Rather, it works with a particular instantiation \gs\ of the symbol graph. We refer to such an algorithm $\mathcal{A}$ as \textbf{$\gamma$-accurate} for $h_1$ and $h_2$ if, under the sampling choices of Algorithm~\ref{al:sampling}, it outputs the `correct' hypothesis with probability at least $\gamma$; that is, for both $i \in \{1,2\}$: 
$\probTwo{h_i}{\mathcal{A} \text{\ outputs\ } h_i} \geq \gamma.$

\begin{proposition}
If observation $X_S$ $\gamma$-separates $h_1$ and $h_2$, then algorithm \textsc{Separator}$_{X_S}$ is $\gamma$-accurate for $h_1$ and $h_2$.
\end{proposition}
\begin{proof}
Let $\mathcal{A}$ denote \textsc{Separator}$_{X_S}$ for brevity. Combining $\gamma$-separation of $X_S$ with how $\mathcal{A}$ operates, we obtain:
{
\small
\begin{align*}
    \probTwo{h_1}{\mathcal{A} \text{\ outputs\ } h_1} - \probTwo{h_2}{\mathcal{A} \text{\ outputs\ } h_1} & \geq \gamma \\
    \Rightarrow \probTwo{h_1}{\mathcal{A} \text{\ outputs\ } h_1} + \probTwo{h_2}{\mathcal{A} \text{\ outputs\ } h_2} & \geq 1 + \gamma
\end{align*}
}
% \erfan{The above expression goes into the right column}
Since each term on the left is bounded above by $1$, each of them must also be at least $\gamma$. 
% , as desired.
% dropped for space 
\end{proof}

In the rest of work, we will analyze when one can obtain a $\gamma$-accurate algorithm, using $\gamma$-separation of the underlying observation as a tool for the analysis.


We will assume that the replication factor (i.e., the number of symbol nodes corresponding to each meaning node) is a constant, i.e., $r$ is  such that $\prob{|U| = \lambda} = 1$. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Connectivity Reasoning Algorithm}
One simple but often effective approach for reasoning is to focus on connectivity (as described in Figure~\ref{fig:ny-example}). Specifically, we consider reasoning chains as valid if they correspond to a short path in the meaning space, and invalid if they correspond to disconnected nodes. Given nodes $m, m' \in \gm$, this corresponds to two possible hypotheses: 
$$h_1 = m \eone m'\text{, and}\; h_2 = m \etwo m'$$
% \daniel{$\leq$ is missing here. }\tushar{isn't that only on s and s' or do we have that on the meaning graph too ?}
We refer to distinguishing between these two worlds as the \textbf{$d$-connectivity reasoning problem}. While we consider two extreme hypotheses for our analysis, we find that with a small amount of noise, even these extreme hypotheses can be difficult to distinguish. 

For the reasoning algorithm, one natural observation that can be used is the connectivity of the symbol nodes in $\gs$. Existing models of multi-hop reasoning~\citep{KhotSaCl17} use similar features %in their programs 
to identify valid reasoning chains. Specifically, we consider the observation that there is a path of length at most $\tilde{d}$ between $s$ and $s'$: 
\vspace{-0.05cm}
$$
 X^{\tilde{d}}_S(s, s') = \; s \pathk{\leq \tilde{d}} s'
 \vspace{-0.05cm}
$$
The corresponding \textbf{connectivity algorithm} is \textsc{Separator}$_{X^{\tilde{d}}_S}$, which we would like to be $\gamma$-accurate for the two hypotheses under consideration.
Next, we derive bounds on $\gamma$ for these specific hypotheses and observation. Note that while the space of possible hypotheses and observations is large, the above natural and simple choices still allow us to derive valuable intuitions for the limits of reasoning.

\begin{comment}

multi-hop reasoning algorithms operate by combining local information along one or more paths connecting two nodes. Such algorithms must be able to determine basic properties of paths, such as the existence of one of length $d$ between two nodes in the meaning space. 
For two fixed nodes $m, m' \in \gm$, consider two possible worlds, one where the two nodes are connected, $H^{\circled{1}}_M(m, m') = m \eone m'$, and another where they are not, $H^{\circled{2}}_M(m, m') = m \etwo m'$. 
We will refer to distinguishing between these two worlds as the \textbf{$d$-connectivity problem}.
% This can be thought of an abductive reasoning, where the goal is to find the best simple explanation. 
We consider the reasoning setting from Equation~(\ref{eq:decision}), i.e., we would like to make an inference about $\gm$ based on observations $X_S(s, s')$ made in the symbol graph $\gs$, where $s, s'$ are symbol graph nodes associated with $m, m'$, resp. 


For a fixed choice for the type of observation $X_S(s, s')$ one can make, we can assess the quality of the corresponding algorithm.
% For a choice of $E_S(s, s')$ we show that one can solve the decision rule in  Equation~\ref{eq:decision:distance}. 
For example, let $X_S = \;\; s \pathk{\leq \tilde{d}} s'$, i.e., that there is a path of length at most $\tilde{d}$ between $s$ and $s'$. This reduces Eq.~(\ref{eq:decision}) to: 
\begin{equation}
\label{eq:decision:distance}
% \underset{e \in \{ m \eone m', m \etwo m'\}}{\text{argmax}} \prob{  s \pathk{\tilde{d}} s' | e} 
\underset{h \in \{ m \eone m', m \etwo m'\}}{\text{argmax}} \probTwo{h}{  s \pathk{\leq \tilde{d}} s'} 
\end{equation}

\end{comment}


%%%%%%%%%%%%%%%
% \subsection{Possibility of accurate connectivity reasoning}
\subsection{Possibility of accurate connectivity}

We begin by defining the following accuracy threshold, $\gamma^*$, as a function of the parameters for sampling a symbol graph:
%
\begin{definition}
Given $n, d \in \mathbb{N}$ and symbol graph sampling parameters $p_+, \varepsilon_+, \lambda$, define $ \gamma^*(n, d, p_+, \varepsilon_+, \varepsilon_-, \lambda) $ as
{
% \color{red}
\small
\begin{align*}
       \left( 1 - \left( 1- (p_+ \oplus \varepsilon_-) \right)^{\lambda^2} \right)^{d} 
       \cdot \left( 1 - 2 e^3 \varepsilon_+ ^{\lambda/2} \right)^{d+1}  
        - 2en (\lambda\ball(d))^2 p_-.
        % }
    % \right\}
\end{align*}
}
\vspace{-0.05cm}
\end{definition}
%
This expression is somewhat difficult to follow. Nevertheless,
as one might expect, the accuracy threshold $\gamma^*$ increases (higher accuracy) as $p_+$ increases (higher edge retention) or $\varepsilon_+$ decreases (fewer dropped connections between replicas). As $\lambda$ increases (higher replication), the impact of the noise on edges between node cluster
or $d$ decreases (shorter paths), the accuracy threshold will also increase.
%\tushar{If $p_+ = 1$, we would have a zero-accurate algorithm even if we didn't sample any similarity edges right since every replicated node would be connected to its true neighbours? I understand these bounds won't be tight, but I wanted to see how loose do they become because of $\varepsilon_+$. For a graph with limited replication($\lambda=3$) and 2-hop reasoning($d=2$), this lower-bound jumps to one at $\varepsilon_+>0.36$. But this goes down, for higher values of $\lambda$. It might be worth pointing out this relation to $\lambda$ i.e. higher redundancy increases the accuracy of the reasoning.}

% \iftacl 
% 	The following theorem establishes the possibility of a $\gamma$-accurate algorithm for the connectivity problem:\footnote{Details of the proofs are skipped. 
% 	% due to space limitation 
% 	We will incorporate them in our revision upon having more space. }
% \else
	The following theorem (see Appendix for a proof) establishes the possibility of a $\gamma$-accurate algorithm for the connectivity problem:
% \fi 


%
\begin{theorem}
\label{the:reasoning:possiblity:detailed}
Let $p_+, p_-, \varepsilon_+, \varepsilon_-, \lambda$ be parameters of the sampling process in Algorithm~\ref{al:sampling} on a meaning graph with $n$ nodes. Let $d \in \mathbb{N}$ and $\tilde{d} = d (1+\lambda)$. If $p_-$ and $d$ satisfy
% $ p_- \cdot \ball^2(\tilde{d}) < 1 \big/ (\lambda^2n)$,
% $ p_- \cdot \ball^2(\tilde{d}) < \frac{1}{\lambda^2n}$,
\vspace{-0.05cm}
$$
    % p_- \cdot \ball^2(\tilde{d}) < 1 \big/ (\lambda^2n),
    { (p_- \oplus \varepsilon_-) } \cdot \ball^2(d) < \frac{1}{{2e}\lambda^2n},
    %  \left[1-\left(1-p_-\right)\left(1-\varepsilon_-\right) \right] 
    \vspace{-0.05cm}
$$
and $\gamma = \max \{ 0, \gamma^*(n, d, p_+, \varepsilon_+, \varepsilon_-, \lambda) \}$, then the connectivity algorithm \textsc{Separator}$_{X^{\tilde{d}}_S}$ is $\gamma$-accurate for the $d$-connectivity problem.
\end{theorem}
\begin{proof}[Proof idea]
\small
The proof consists of two steps: first show that for the assumed choice of parameters, connectivity in the meaning space is recoverable in the symbol space, with high-probability. Then show that 
%Additionally, 
spurious connectivity in the symbol space (with no meaning space counterparts) has low probability. 
\end{proof}

\begin{corollary}
\label{the:reasoning:possiblity}
(Informal) If $p_-, \varepsilon_-, d,$ and $\gamma$ are small enough, then the connectivity algorithm \textsc{Separator}$_{X^{\tilde{d}}_S}$ with $\tilde{d} = d (1+\lambda)$ is $\gamma$-accurate for the $d$-connectivity problem.
\end{corollary}


%%%%%%%%%%%%%
\subsection{Limits of connectivity algorithm}
We show that as $d$, the distance between two nodes in the meaning space, increases, it is unlikely that we will be able to make any inference about their connectivity by assessing connectivity of the corresponding symbol-graph nodes. More specifically, if $d$ is at least logarithmic in the number of nodes in the graph, then, even for relatively small amounts of noise, the algorithm will see all node-pairs as connected within distance $d$;
% , and hence will be unable to perform any informative inference.
% ; hence won't be able to perform any informative inference.
hence any informative inference will be unlikely.


\begin{theorem}
\label{th:multi-hop:impossiblity}
Let $c > 1$ be a constant and $p_-, \varepsilon_-, \lambda$ be parameters of the sampling process in Algorithm~\ref{al:sampling} on a meaning graph $\gm$ with $n$ nodes. Let $d \in \mathbb{N}$ and $\tilde{d} = \lambda d$. If
$$
    \vspace{-0.04cm}
    {p_- \oplus \varepsilon_-} \geq \frac{c}{\lambda n} \ \ \ \text{and} \ \ \ d \in \Omega (\log n),
    \vspace{-0.05cm}
$$
% {1-(1-p_-)(1- \varepsilon_-)} 
then the connectivity algorithm \textsc{Separator}$_{X^{\tilde{d}}_S}$ almost-surely infers any node-pair in $\gm$ as connected, and is thus not $\gamma$-accurate for any $\gamma > 0$ for the $d$-connectivity problem.
\end{theorem}
\begin{proof}[Proof idea]
\small
One can show that, for the given choice of parameters, noisy edges would dominate over informative ones and the symbol-graph would be a densely connected graph (i.e., one cannot distinguish actual connectivities from the spurious ones). 
\end{proof}


This result exposes an inherent limitation to multi-hop reasoning: even for small values of noise, the diameter of the symbol graph becomes very small, namely, logarithmic in $n$. 
This has a resemblance to similar observations in various contexts, commonly known as the \emph{small-world phenomenon}. This principle states that in many real-world graphs, nodes are all linked by short chains of acquaintances, such as ``six degrees of separation"~\citep{Milgram67,WattsSt98}. Our result affirms that if NLP reasoning algorithms are not designed carefully, such macro behaviors 
% in noisy graphs 
will necessarily become bottlenecks. 

We note that the preconditions of Theorems~\ref{the:reasoning:possiblity:detailed} and~\ref{th:multi-hop:impossiblity} are disjoint, that is, both results do not apply simultaneously. Since $\ball(.) \geq 1$ and $\lambda \geq 1$, Theorem~\ref{the:reasoning:possiblity:detailed} requires ${p_- \oplus \varepsilon_-} 
\leq { \frac{1}{{2e}\lambda^2 n} < \frac{1}{\lambda^2 n}}$, whereas Theorem~\ref{th:multi-hop:impossiblity} applies when ${p_- \oplus \varepsilon_-} \geq \frac{c}{\lambda n} > \frac{1}{\lambda^2 n}$. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Limits of General Algorithms}

While in the previous section we showed limitations of multi-hop reasoning in inferring long-range relations, here we extend the argument to prove the difficulty for \emph{any} reasoning algorithm. 

Our exposition is algorithm independent; in other words, we do not make any assumption on the choice of $E_S(s, s')$ in Equation~\ref{eq:decision}.
In our analysis we use the spectral properties of the graph to quantify local information within graphs. 

\begin{wrapfigure}{r}{0.42\textwidth}
% \begin{figure}
    \centering
    % \includegraphics[scale=0.28]{figures_theory/laplacian-sampling.png}
    % \includegraphics[scale=0.38]{figures_theory/laplacian-sampling-2.png}
    \includegraphics[scale=0.19, trim=0cm 1.0cm 0cm 0cm]{figures_theory/laplacian-sampling-5.png}
    \caption{
    \small
    The construction considered in Definition~\ref{cut:construction}. 
    The node-pair $m$-$m'$ is connected with distance $d$ in $G_M$, and disconnected in $G_M'$, after dropping the edges of a cut $C$. For each symbol graph, we consider it ``local'' Laplacian. 
    }
    \label{fig:laplacians}
% \end{figure}
\end{wrapfigure}
Consider a meaning graph $G_M$ in which two nodes $m$ and $m'$ are connected. 
We drop edges in a min-cut $C$ to make the two nodes disconnected and get $G_M'$ (Figure~\ref{fig:laplacians}). 



\begin{definition}
\label{cut:construction}
Define a pair of meaning-graphs $G$ and $G'$, both with size $n$ and satisfying the ball assumption $\ball(d)$, with the following properties: (1) $m \pathk{d} m'$ in $G$, (2) $m \npathk{} m'$ in $G'$, (3) $E_{G'} \subset E_G$, (4) $C = E_G \setminus E_{G'}$, an $(m, m')$ min-cut of $G$. 
% \tushar{dropped itemize to save space}
% \begin{multicols}{2}
% \begin{itemize}
%     \item $m \pathk{d} m'$ in $G$
%     \item $m \npathk{} m'$ in $G'$
%     \item $E_{G'} \subset E_G $ 
%     \item $C = E_G \setminus E_{G'}$, an $(m, m')$ min-cut of $G$. 
% \end{itemize}
% \end{multicols}
\end{definition}
We define a uniform distribution over all the instances that satisfy the construction explained in Definition~\ref{cut:construction}: 
\begin{definition}
\label{def:distribution}
We define a distribution $\mathcal{G}$ over pairs of possible meaning graphs $G, G'$ and pairs of nodes $m,m'$ which satisfies the requirements of Definition \ref{cut:construction}. Formally, \(\mathcal{G}\) is a uniform distribution over the following set:
\vspace{-0.05cm}
{
\small
$$ 
\{(G,G',m,m') \mid G,G',m,m' \text{satisfy Definition \ref{cut:construction}}\}.
$$
}
\end{definition}

For the meaning graphs, we sample a symbol graph $G_S$ and $G'_S$, as denoted in Figure~\ref{fig:laplacians}. 
In the sampling of $G_S$ and $G'_S$, all the edges share the randomization, except for the ones that correspond to $C$ (i.e., the difference between the $G_M$ and $G'_M$).  
Let $\mathcal{U}$ be the union of the nodes involved in $\tilde{d}$-neighborhood of $s, s'$, in $G_S$ and $G'_S$. 
Define $L, L'$ to be the Laplacian matrices corresponding to the nodes of $\mathcal{U}$. As $n$ grows, the two Laplacians become less distinguishable whenever {$p_- \oplus  \varepsilon_-$} and $d$ are large enough: 
 
\begin{comment}
    \begin{theorem}
    \label{theorem:impossiblity:general:reasoning}
    For any meaning-graphs $G$ and $G'$ constructed according to Definition~\ref{cut:construction} there is no $\gamma$-accurate algorithm satisfying the conditions of Lemma~\ref{lemma:impossiblity:general:reasoning}, to distinguish $G$ from $G'$, 
    % {\color{red} with high probability}, 
    in computational models with limited numerical precision.
    \end{theorem}
    \begin{proof}[Proof of Theorem~\ref{theorem:impossiblity:general:reasoning}]
    If there is an algorithm that can distinguish $G$ and $G'$ with a high-probability, it should also be able to distinguish $L$ and $L'$ with a high probability as well, which would require higher precision computations (for larger $n$), which contradicts the assumptions of the theorem. 
    \end{proof}
\end{comment}

\begin{lemma}
\label{lem:normLaplacianClose}
Let $c > 0$ be a constant and $p_-, \lambda$ be parameters of the sampling process in Algorithm~\ref{al:sampling} on a pair of meaning graphs $G$ and $G'$ on $n$ nodes constructed according to Definition~\ref{cut:construction}. Let $d \in \mathbb{N}, \tilde{d} \geq \lambda d,$ and $L, L'$ be the Laplacian matrices for the $\tilde{d}$-neighborhoods of the corresponding nodes in the sampled symbol graphs $\gs$ and $\gs'$. If
${ p_- \oplus \varepsilon_-} \geq \frac{c \log n}{n}$ and 
$d > \log n,$
then, with a high probability, the two Laplacians are close:
$$
\vspace{-0.05cm}
\norm{\tilde{L}-\tilde{L'}} \leq \frac{ \sqrt{2\lambda}\, \ball(1)}{ \sqrt{n \log (n \lambda)} } 
\vspace{-0.05cm}
$$
\end{lemma}

This can be used to show 
% (see Lemma~\ref{lemma:improbable:recovery} in Appendix) 
that, for such large enough $p_-$ and $d$, the two symbol graphs, $G_S$ and $G'_S$ sampled as above, are indistinguishable by any 
% ``reasonable'' 
function operating over a $\lambda d$-neighborhood of $s, s'$ in \gs, with a high probability.

A reasoning function can be thought of a mapping defined on normalized Laplacians, 
% (or the normalized Laplacians), 
since they encode all the information in a graph.  
For a reasoning function $f$ with limited precision, the input space can be partitioned into regions where the function is constant; and for large enough values of $n$ both $\tilde{L}, \tilde{L}'$ (with a high probability) fall into regions where $f$ is constant.

Note that a reasoning algorithm is oblivious to the the details of $C$, i.e. it does not know where $C$ is, or where it has to look for the changes. Therefore a realistic algorithm ought to use the neighborhood information collectively. 


In the next lemma, we define a function $f$ to characterize the reasoning function, which uses Laplacian information and maps it to binary decisions. We then prove that for any such functions, there are regimes that the function won't be able to distinguish $\tilde{L}$ and $\tilde{L}'$: 

\begin{lemma}
\label{lemma:improbable:recovery}
Let meaning and symbol graphs be constructed under the conditions of Lemma~\ref{lem:normLaplacianClose}. Let $\beta > 0$ and $f: \mathbb{R}^{\dimm \times \dimm} \rightarrow \{0, 1\}$ be the indicator function of an open set.
%\footnote{\url{https://en.wikipedia.org/wiki/Indicator_function}}
Then there exists $n_0 \in \mathbb{N}$ such that for all $n \geq n_0$: 
$$
\mathbb{P}_{ \substack{ (G,G',m,m') \sim \mathcal{G} \\ G_S \leftarrow \alg{G}, \\G'_S \leftarrow \alg{G'}  } }\left[ f(\tilde{L}) = f(\tilde{L}') \right] \geq 1 - \beta.
$$
\end{lemma}

This yields the following result:

\begin{theorem}
\label{theorem:impossiblity:general:reasoning}
Let $c > 0$ be a constant and $p_-, \varepsilon_-, \lambda$ be parameters of the sampling process in Algorithm~\ref{al:sampling} on a meaning graph $\gm$ with $n$ nodes. Let $d \in \mathbb{N}$. If
$$
    {p_- \oplus \varepsilon_-} > \frac{c \log n}{\lambda n} \ \ \ \text{and} \ \ \ d > \log n,
$$
then there exists $n_0 \in \mathbb{N}$ such that for all $n \geq n_0$, \emph{any} algorithm cannot distinguish, with a high probability, between two nodes in \gm\ having a $d$-path vs.\ being disconnected, and is thus not $\gamma$-accurate for any $\gamma > 0$ for the $d$-connectivity problem.
\end{theorem}
\begin{proof}[Proof idea]
\small
The proof uses Lemma~\ref{lemma:improbable:recovery} to show that for the given choice of parameters, the informative paths are indistinguishable from the spurious ones, with high probability. 
\end{proof}


This reveals a fundamental limitation: under noisy conditions, our ability to infer interesting phenomena in the meaning space is limited to a small, logarithmic neighborhood.


%%%%%%%%%%%%%%%%%%%%%%
\section{Empirical Analysis}

Our formal analysis thus far provides worst-case bounds for two regions in the rather large spectrum of noisy sampling parameters for the symbol space, namely, when $p_- \oplus \varepsilon_-$ and $d$ are either both small (Theorem~\ref{the:reasoning:possiblity}), or both large (Theorem~\ref{th:multi-hop:impossiblity}).

This section complements the theoretical findings in two ways: (a) by grounding the formalism empirically into a real-world knowledge graph, and (b) by quantifying the impact of noisy sampling parameters on the success of the connectivity algorithm. 
% \iftacl 
    % DanielK: I dropped this sentence, since without Remark 1 it could be confusing what it really means. 
    % 	We use $\varepsilon_- = 0$ for this experiments, but the effect turns out to be identical as long as {$p_- \oplus \varepsilon_-$} stays unchanged.
% \else
    We use $\varepsilon_- = 0$ for this experiments, but the effect turns out to be identical as long as {$p_- \oplus \varepsilon_-$} stays unchanged (see Remark~\ref{remark:folding} in Appendix).	
% \fi 

Specifically, we consider FB15k237~\citep{ToutanovaCh15} containing a set of $\langle$head, relation, target$\rangle$ triples from a curated knowledge base, FreeBase~\citep{BEPST08}. For scalability, we use a subset that relates to the movies domain,\footnote{Specifically, relations beginning with {\tt /film/}.} resulting in 2855 distinct entity nodes and 4682 relation edges. 
%  use this curated graph 
We treat this as the meaning graph and sample a symbol graph as per Algorithm~\ref{al:sampling} to simulate the observed graph derived from text.

We sample symbol graphs for various values of $p_-$ and plot the resulting symbol and meaning graph distances in Figure~\ref{fig:emp:distance:pm}. For every value of $p_-$ ($y$-axis), we sample points in the meaning graph separated by distance $d$ ($x$-axis). For these points, we compute the average distance between the corresponding symbol nodes, and indicate that in the heat map using color shades.

We make two observations from this simulation. First, for lower values of $p_-$, disconnected nodes in the meaning graph (rightmost column)
% still stay disconnected and
are clearly distinguishable from meaning nodes with short paths (small $d$) as predicted by Theorem~\ref{the:reasoning:possiblity}, but harder to distinguish from nodes at large distances (large $d$). Second, and in contrast, for higher values of $p_-$, almost every pair of symbol nodes is connected with a very short path (dark color), making it impossible for a distance-based reasoning algorithm to confidently assess $d$-connectivity in the meaning graph. This simulation also confirms our finding in Theorem~\ref{th:multi-hop:impossiblity}: any graph with $p_- \geq 1/\lambda n$, which is $\sim 0.0001$ in this case, cannot distinguish disconnected meaning nodes from nodes with paths of short (logarithmic) length (top rows). 

\begin{figure}
    \centering
    % \includegraphics[scale=0.25,trim=0cm 1.4cm 0cm 0cm, clip=false]{figures_theory/pminusvsDistances-2.png}
    \includegraphics[scale=0.27,trim=1.9cm 1.4cm 0.5cm 0cm, clip=false]{figures_theory/pminusvsDistances-4.png}
    \caption{ 
    % \ashish{depth? may be `various colors in the figure'?} 
    Various colors in the figure depict the average distance between node-pairs in the symbol graph, for each true meaning-graph distance $d$ (x-axis), as the noise parameter $p_-$ (y-axis) is varied. {The goal is to distinguish squares in the column for a particular $d$ with the corresponding squares in the right-most column, which corresponds to node-pairs being disconnected. This is easy in the bottom-left regime and becomes progressively harder as we move upward (more noise) or rightward (higher meaning-graph distance).} ($\varepsilon_+=0.7, \lambda = 3
    % , \varepsilon_-=0
    $)}
    \label{fig:emp:distance:pm}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%
{
\section{Summary, Discussion and Practical Lessons}
Our work is inspired by empirical observations of ``semantic drift'' of reasoning algorithms, as the number of hops is increased. There are series of works sharing this empirical observation; for example, \cite{FJHSC15} show modest benefits up to 2-3 hops, and then decreasing performance; \cite{Jansen16,JWMM18} made similar observations in graphs built out of larger structures such as sentences, where the performance drops off around 2 hops. This pattern has interestingly been observed in a number of results with a variety of representations, including word-level representations, graphs, and traversal methods. 
The question we are after in this work is whether the field might be hitting a fundamental limit on multi-hop information aggregation using existing methods and noisy knowledge sources.

Our ``impossibility'' results are reaffirmations of the empirical intuition in the field. This means that multi-hop inference (and any algorithm that can be cast in that form), as we've been approaching it, is exceptionally unlikely to breach the few-hop barrier predicted in our analysis. 

% For \emph{multi-hop} connectivity reasoning, we prove the existence of high-quality algorithms. On the other hand, we show the reasoning algorithms face fundamental limitations, when they require long-range information. 

There are at least two practical lessons: 
\begin{enumerate}[leftmargin=.55cm]
% \itemsep0em 
    \item 
    There are several efforts in the field pursuing ``very long'' multi-hop reasoning. Our results suggest that such efforts, especially without a careful understanding of the limitations, are unlikely to succeed, unless some fundamental building blocks are altered.
    
    \item 
    A corollary of this observation suggests that, due to the limited number of hops, practitioners must focus on richer representations that allow reasoning with only a ``few'' hops. This, in part, requires higher-quality abstraction and grounding mechanisms. It also points to alternatives, such as offline KB completion/expansion, which indirectly reduce the number of steps needed at inference time. It basically suggests that ambiguity and variability must be handled well to reduce the number of hops needed.
\end{enumerate}
% \dan{rephrased/added text above}

Finally, we note that our proposed framework applies to any machine comprehension task over natural text that requires multi-step decision making, such as multi-hop QA or textual entailment.
}


\begin{comment}
\section{Conclusion}

Language is a complex set of phenomena. 
Meanings and how they are connected to the physical world can be taken for granted. Studying natural language without its variability, ambiguity, and incompleteness can result in misleading conclusions. At the same time, `thinking' (or \emph{reasoning}) with noisy, expressed, language, is a fundamental
%and millennial-long problem standing between us and our understanding of general intelligence. 
challenge for understanding general intelligence.

{
This work presents the first attempt to develop a formal framework for understanding the behavior of complex NLP reasoning in presence of key linguistic noise phenomena. 
The importance of this work is two-fold: we propose a graph-theoretic paradigm for studying reasoning, inspired by the symbol-meaning problem in the presence of variability, ambiguity, and incompleteness of language. 
Second, we show how this framework can be used to study and analyze a class of reasoning algorithms. 
% \erfan{connectivity reasoning?}
% Our findings are compatible with existing empirical intuitions that, while reasoning algorithms help, they are limited to few steps~\citep{JSSC17}. 
Our results have important implications on how problems in language comprehension, need to be studied. 

% \dan{rephrased some of the text above; can kill the last paragraph is needed (I assume not needed)}
% An interesting direction for future work is to relax some of the assumptions we made in this first attempt. For example, the independence assumption while sampling (Algorithm~\ref{al:sampling}) is a widely used simplification in areas such as PAC analysis~\citep{valiant1984theory}, which have proven insightful despite such assumptions. General results without such assumptions would be valuable, so would formal results covering a wider spectrum of the broad empirical trend depicted in Figure~\ref{fig:emp:distance:pm}.

}

% for  result and an impossibility result, which lays theoretical justifications for what has already been observed empirically. 
% Our formal findings shed light on some existing empirical intuitions. For example, \cite{JSSC17} proposes a structured multi-hop reasoning by aggregating sentential information from multiple knowledge bases. The work shows that while this aggregation strategy improves over the trivial baseline of non-aggregation (possibly of reasoning), with aggregation of more than 2-3 sentences the quality quality declines (impossibility of reasoning). Similar observations were also made in~\citep{tableilp2016:ijcai}. 
% % This is compatible with empirical that QA solvers generally struggle to meaningfully aggregate more than few freetext sentences~\citep{JSSC17}. 
% Another way of looking at this result is that in many existing datasets that multi-hop system achieve an acceptable performance is because the target queries likely needed only minimal reasoning (i.e., the datasets are easy). For example, in the elementary science domain, where multi-hop reasoning systems have been tested and achieved superior results, \cite{JBSC16} has estimated that, an average, at most 4-6 sentences are required to explain the answer of a given question. 
% corolary for representation 
% This issue had major consequences on the strategies for containing the knowledge (also known as \emph{knowledge representation}).
% \cite{stanfill1986toward} argued reasoning should be on ``memories of specific episodes'', rather than rules. The \emph{connectionist} paradigm~\citep{clark1989connectionism,Shastri1993FROMSA} favored a distributed representation of notions, rather than explicit representation, which laid the foundation for neural networks. 
% }

% the strategies for containing the knowledge (also known as \emph{knowledge representation}).
% \cite{stanfill1986toward} argued reasoning should be on ``memories of specific episodes'', rather than rules. The \emph{connectionist} paradigm~\citep{clark1989connectionism,Shastri1993FROMSA} favored a distributed representation of notions, rather than explicit representation, which laid the foundation for neural networks. 

% what is ignore and future work 
% Our contribution is just tip of the iceberg. Many other psychological, social and cultural issues all contribute to the contribute to the completely of language understanding, that are mostly ignored in our formalism. In terms of reasoning formalism, we explored only a single class, and there is much to be explored in this framework.  
% We believe there is much has to be done in this direction. 
% Meanings and how they are connected to the physical world can be taken for granted are in fact only the tip of a huge iceberg. 

\end{comment}

% \section{Discussion}





==> Daniel K - thesis - dissertation/7.conclusion_new.tex <==
\chapter{Summary and Future Work}
\label{chapter:conclusion:summary:future}
\epigraph{ 
\includegraphics[scale=0.55,trim=4.4cm 22.3cm 2.2cm 3cm, clip=true]{figures_conclusion/persian_poetry.pdf}
}{--- \textup{Omar Khayyam}, Rubaiyat, 1120 CE}

This thesis aims at progressing towards natural language understanding, by means of the task of question answering. 
% In terms of techniques, this thesis has been a pioneer in introducing a multiple novel approaches . 
% This problem is challenges for machines, due to its linguistic richness and diversity, its need for reasoning over linguistic concepts, and many other factors. 
This chapter, gives a summary of our contributions across this document and provides a few angles along which we would like to extend this work. 

% Question answering is challenging in the presence of linguistic richness and diversity, especially when arriving at the correct answer requires some level of reasoning. 
% \todo{talk about the recent progress towards NLU}
% Answering real science questions is a challenging task because they are posed in natural language, require extensive domain knowledge, and often require combining multiple facts together.
% Answering science questions posed in natural language is an important AI challenge. Answering such questions often requires non-trivial inference and knowledge that goes beyond factoid retrieval. Yet, most systems for this task are based on relatively shallow Information Retrieval (IR) and statistical correlation techniques operating on large unstructured corpora. 

\section{Summary of Contributions}
% \todo{talk about the intro and chapter}
We start the discussion in Chapter 2 by providing a thorough review of the past literature concerning NLU, highlighting the ones that are related to the works in this thesis. 
% Our review covers many interrelated highlights in the field. 
% realm of language \emph{representation} and \emph{reasoning}. 


Chapter 3 studies reasoning systems for question answering on elementary-school science exams, using a semi-structured knowledge base. We treat QA as a subgraph selection problem and then formulate this as an ILP optimization. 
Most importantly, this formulation allows multiple, semi-formally expressed facts to be combined to answer questions, a capability outside the scope of IR-based QA systems.
In our experiments, this approach significantly outperforms both the previous best attempt at structured reasoning for this task,  and an IR engine provided with the same knowledge. 
% It also significantly boosts performance {when combined with} unstructured methods (IR and PMI). 
% These results suggest that the approach is both viable and promising for natural language question answering.
Our effort has had great impacts since publication. Our work has inspired others to to build systems based on our design and to improve the state of the art in other domains; for instance, \cite{KhotSaCl17} uses similar ideas to reasoning with OpenIE tuples~\citep{EBSW08}.
In addition, the system has been incorporated into Allen Institute's reading-comprehension project\footnote{\url{https://allenai.org/aristo/}} and is shown to give a significant boost to their performance~\citep{CEKSTTK16}. 
Even after a couple of years, the system has been shown to be 
% The system was later on, after a two years, shown to be 
among the best systems on a recently-proposed reading comprehension task~\citep{CCEKSST18}.  
% Previous work has examined the use of Markov Logic Networks (MLNs) to represent the requisite background knowledge and interpret test questions, but did not improve upon an information retrieval (IR) baseline.

% formulated as an Integer Linear Program (ILP), that answers natural language questions using a semi-structured knowledge base derived from text, including questions requiring multi-step inference and a combination of multiple facts. On a dataset of real, unseen science questions, our system significantly outperforms (+14\%) the best previous attempt at structured reasoning for this task, which used Markov Logic Networks (MLNs). {It also improves upon a previous ILP formulation by 17.7\%.} When combined with unstructured inference methods, the ILP system significantly boosts overall performance (+10\%).  Finally, we show our approach is substantially more robust to {a simple answer} perturbation compared to statistical correlation methods.
% We presented \tableilp, a system that can answer such questions, 




Chapter 4 extends our abductive reasoning system (from Chapter 3) to consume raw text as input knowledge. This is the first system to successfully use a wide range of semantic abstractions to perform a high-level NLP task like Question Answering. 
    % The system makes use of a wide range of semantic abstractions of the text, which are derived using off-the-shelf and general-purpose natural language modules such as semantic-role labelers. This is the first system that †hat successfully uses a wide  
Departing from the currently popular paradigm of generating a very large dataset and learning ``everything'' from it in an end-to-end fashion, we  demonstrate that one can successfully leverage pre-trained NLP modules to extract a sufficiently complete linguistic abstraction of the text that allows answering interesting questions about it. This approach is particularly valuable in settings where there is a small amount of data. Instead of exploiting peculiarities of a large but homogeneous dataset, as many state-of-the-art QA systems end up doing, we focus on confidently performing certain kinds of reasoning, as captured by our semantic graphs and the ILP formulation of support graph search over them. 
% Bringing these ideas to practice, our system, \textilp, achieves state-of-the-art performance on two domains with very different characteristics. 
% , outperforming both traditional and neural models.
    
    % We propose a novel method for exploiting the semantic structure of text to answer multiple-choice questions. The approach is especially suitable for domains that require reasoning over a diverse set of linguistic constructs but have limited training data. To address these challenges, we present the first system, to the best of our knowledge, that reasons over a wide range of semantic abstractions of the text, which are derived using off-the-shelf, general-purpose, pre-trained natural language modules such as semantic role labelers, coreference resolvers, and dependency parsers. Representing multiple abstractions as a family of graphs, we translate question answering (QA) into a search for an optimal subgraph that satisfies certain global and local properties. This formulation generalizes several prior structured QA systems. Our system, \textilp, demonstrates strong performance on two domains simultaneously. In particular, on a collection of challenging science QA datasets, it outperforms various state-of-the-art approaches, including neural models, broad coverage information retrieval, and specialized techniques using structured knowledge bases, by 2\%-6\%. 

Chapter 5 introduces the concept of essential question terms and demonstrates its importance for question answering. 
% via two empirical findings: (a) humans becomes substantially worse at QA even when a few essential question terms are dropped, and (b) state-of-the-art QA systems can be improved by incorporating this notion. While text summarization has been studied before, questions have different characteristics, requiring new training data to learn a reliable model of essentiality. 
We introduce a dataset for this task and show that our classifier trained on this dataset substantially outperforms several baselines in identifying and ranking question terms by the degree of essentiality.
Since the publication, this work has been picked up by others to significantly improve their systems~\citep{NZCM18}. 

%     Question answering (QA) systems are easily distracted by irrelevant or redundant words in questions, especially when faced with long or multi-sentence questions in difficult domains. This paper introduces and studies the notion of {\em essential question terms} with the goal of improving such QA solvers.  We illustrate the importance of essential question terms by showing that humans' ability to answer questions drops significantly when essential terms are eliminated from questions. We then develop a classifier that reliably (90\% mean average precision) identifies and ranks essential terms in questions. Finally, we use the classifier to demonstrate that the notion of question term essentiality allows state-of-the-art QA solvers for elementary-level science questions to make better and more informed decisions, improving performance by up to 5\%.

% We also introduce a new dataset of over 2,200 crowd-sourced essential terms annotated science questions. 



%%% MultiRC 
Chapter 6 presents a reading comprehension dataset in which questions require \emph{reasoning over multiple sentences}. This dataset contains $\sim6k$ questions from different domains and wide variety of complexities.
% extracted from about +800 paragraphs. For each question, there are multiple answer-options out of which one or more can be correct. The paragraphs (and questions) originate from different domains and hence are amenable to a wide variety and complexity of required reasoning phenomena. We found that human performance on this corpus is about $88\%$, at least $20\%$ ahead of the best baseline systems in the field.
% while state-of-the-art machine comprehension models do not exceed a F1-score of $60\%$.
We have shown a significant performance different between human and state-of-the-art systems and we hope that this performance gap will encourage the community to work towards more sophisticated reasoning systems. It is encouraging to see that 
% since its publication, 
the work is already been used in a couple of works   
% this dataset has been used by a couple of works 
\citep{SYYC19,TKKSB19,WYSCYRM19}.  



%     To motivate the community to work on more challenging forms of natural language comprehension, we propose a dataset that requires reasoning over multiple sentences. 
%     % An additional important aspect of this work is that we challenged the community to change the harmful ``fixed'' test set methodology, and committed to updating the test set every few months.  
% We present a reading comprehension challenge in which questions can only be answered by taking into account information from multiple sentences. We solicit and verify questions and answers for this challenge through a 4-step crowdsourcing experiment.
% Our challenge dataset contains $\sim$6$k$ questions for $+800$ paragraphs across 7 different domains (elementary school science, news, travel guides, fiction stories, etc) bringing in linguistic diversity to the texts and to the questions wordings. On a subset of our dataset, we found human solvers to achieve an F1-score of $86.4\%$.
% We analyze a range of baselines, including a recent state-of-art reading comprehension system, and demonstrate the difficulty of this challenge,
% despite a high human performance.
% The dataset is the first to study multi-sentence inference at scale, with an open-ended set of question types that requires reasoning skills.


Chapter 7 offers a question answering dataset dedicated to \emph{temporal common sense understanding}. 
We show that systems equipped with the state-of-the-art techniques are still far behind human performance. 
% Subsequent error analysis sheds light on the capabilities as well as limitations of those models. 
We hope that the dataset will bring more attention to the study of common sense (especially in the context of understanding of \emph{time}). 

% and our discoveries will encourage a broad audience to work on the understanding of ``time''. 
% can be found interesting to a broad audience.

% focuses on the challenge of temporal common sense understanding. Specifically, we have developed a new crowdsourcing scheme that generates high-quality QA dataset dedicated to the study of the challenges in temporal common sense. On top of it, we are able to show that baseline systems equipped with the state-of-the-art techniques still have a much poorer performance as compared to humans. Subsequent error analysis sheds light on the capabilities as well as limitations of those models. We hope that the dataset and our discoveries will encourage a broad audience to work on the understanding of ``time''. 
% can be found interesting to a broad audience.

% The need to reason with respect to common sense knowledge is ubiquitous in natural language understanding and a key challenge to current natural language processing technologies.
% {\em Temporal common sense}, the ability to reason about multiple temporal aspects such as events' duration, order, and frequency is an important part of the common sense challenge.
% Unfortunately, a major impediment to progress is the lack of \emph{natural end-tasks} dedicated to temporal common sense, those that can provide an objective measure of progress in the field. 

% In this work, we describe a new crowdsourced natural language question-answering dataset defined so that performing well on it requires significant progress on multiple temporal common sense tasks.
% We show that human solvers score well-above current state-of-the-art systems on these tasks, and hope that this will motivate more research on temporal common sense reasoning.


In Chapter 8, we develop 
% \emph{Formalizing limitations of multi-step reasoning.  } We developed 
a theoretical formalism to investigate fundamental limitations pertaining to multi-step reasoning in the context of natural language problems.
% Recent systems for natural language understanding are strong at overcoming linguistic variability for lookup style reasoning. Yet, their accuracy drops dramatically as the number of reasoning steps increases. 
We present the first analysis of reasoning 
% formal framework 
% to study such empirical observations, 
% in relation to the 
in the context of properties like 
ambiguity, variability, incompleteness, and inaccuracy. 
% that the use of language introduces when representing a hidden conceptual space. 
% Our formal model works with two related spaces: a conceptual \emph{meaning space} that is unambiguous and complete but hidden, and a linguistic \emph{symbol space} that captures a noisy grounding of the meaning space in the symbols or words of a language.
% We apply this framework to study the \emph{connectivity problem} in undirected graphs---a core reasoning problem that forms the basis of more complex multi-hop reasoning.
% And within this formalism we characterize the regimes for successful and failed inferences. 
% We show that it is indeed possible to construct a high-quality algorithm for detecting connectivity in the (latent) meaning graph, based on an observed noisy symbol graph, as long as the noise is below {our quantified noise level} and only a few hops are needed. 
% On the other hand, we also prove an impossibility result: if a query requires a large number (specifically, logarithmic in the size of the meaning graph) of hops, \emph{no} reasoning system operating over the symbol graph is likely to recover any useful property of the meaning graph. 
% This highlights a fundamental barrier for a class of reasoning problems and systems, and suggests the need to limit the distance between the two spaces, rather than investing in multi-hop reasoning with ``many'' hops.
% This highlights a fundamental barrier for a class of reasoning problems and systems, and suggests the need to limit the amount of noise or desired hops for successful multi-hop reasoning.
% Language is a complex phenomenon. 
% Meanings and how they are connected to the physical world can be taken for granted. Studying natural language without its variability, ambiguity, and incompleteness can result in misleading conclusions. At the same time, `thinking' with noisy language, or \emph{reasoning}, is a fundamental
%and millennial-long problem standing between us and our understanding of general intelligence.  
% problem for understanding general intelligence.
% This work presents the first attempt to develop a formal framework for understanding the behavior of complex NLP reasoning in presence of key linguistic noise phenomena. 
% The importance of this work is two-fold: we propose a graph-theoretic paradigm for studying reasoning, inspired by the symbol-meaning problem in the presence of noise, ambiguity, and incompleteness of language. 
% Second, we show how this framework can be used to study and analyze a class of reasoning algorithms. 
% \erfan{connectivity reasoning?}
% Our findings are compatible with existing empirical intuitions that, while reasoning algorithms help, they are limited to few steps~\citep{JSSC17}. 
% Our results have important implications as to how the problems, especially in language comprehension, need to be treated. 
We show that a multi-hop inference (and any algorithm that can be cast in that
form), as we've been approaching it, is exceptionally unlikely to breach the few-hop barrier predicted in our analysis.
% There are at least two practical lessons: There are several
% ongoing efforts in the field on “very long” multi-hop reasoning. 
Our results suggest that such efforts, especially without
a careful understanding of the limitations, are unlikely to succeed, unless some fundamental building blocks are altered.
A corollary of this observation suggests that, practitioners must focus on richer representations that allow reasoning
with only a ``few'' hops. 
This, in part, requires higher-quality abstraction and grounding mechanisms.
% It also points to alternatives, such as offline KB completion/expansion, which indirectly reduce the number of steps needed at inference time. 
In other words, ambiguity and variability must be handled well to reduce the number of hops needed.


% An interesting direction for future work is to relax some of the assumptions we made in this first attempt. For example, the independence assumption while sampling (Algorithm~\ref{al:sampling}) is a widely used simplification in areas such as PAC analysis~\citep{valiant1984theory}, which have proven insightful despite such assumptions. General results without such assumptions would be valuable, so would formal results covering a wider spectrum of the broad empirical trend depicted in Figure~\ref{fig:emp:distance:pm}.



\section{Discussion and Future Directions}
This thesis has taken a noticeably distinct approach towards a few important problems in the field and has shown progress on multiple ends. 
For example, the formalism of Chapter 3 and 4 are novel and provide general ways to formalize and implement reasoning algorithms. The datasets of Chapter 6 and 7 are distinct from the many QA datasets in the field. The theoretical analysis of Chapter 8 takes a uniquely distinct formal analysis of reasoning in the context of natural language.  

All these said, 
% That said, 
there are many issues that 
are not addressed 
% we do not address directly or 
as extensively as we could have (or should have), or there are aspects that turned out slightly differently from  what we initially expected. 
% In some cases, there are fundamental reasons for why 

Looking back at the reasoning formalism of Chapter 4, we underestimated the hardness of extracting the underlying semantic representations. Even though the field has made significant progress in low-level NLP tasks (like SRL or Coreference), such tasks still suffer from brittleness and lack of transfer across domains.  And brittleness in the extraction of such annotations, result in exponentially bigger errors when 
% creating local chains for 
reasoning with them (as also justified by the theoretical observations of Chapter 8); in practice, it worked well only for short-ranged chains (1, 2, and sometimes 3 hops). 
% (for which many neural networks also did well). 
With more recent progress in unsupervised representations and improvement of semantic extraction systems, my hope is to redo these ideas in the coming years and revisit the remaining challenges. 


A vision that I would like to pursue 
% (which I have inherited from Dan) 
(influenced by discussions with my advisor)
is reasoning with \emph{minimal} data. We (humans) are able to perform the same  reasoning on many high-level concepts and are able to transfer them in all sorts of domains: for instance, an average human uses the same inductive reasoning to conclude \emph{the sky is blue} and inferring that  \emph{there is another number after every number}.  
% In other words, it's likely that we will end up creating effective reasoning with supervised datasets, since the datasets (even the humongous ones) represent limited expressively. 
Effective (unsupervised) representation could potentially need a huge amount of data (and many parameters), but successful reasoning systems will likely need very minimal data (and very simple, but general definitions). 


Over the past years, the field has witnessed a wave of activity on unsupervised language models~\citep{PNIGCLZ18,DCLT18}. There are many questions with respect  to the success of such models on several datasets: for instance, what kinds of reasoning are they capable of? what is it that they are missing? And how we can address them by possibly creating hybrid systems.  
What is clear is that these systems will offer increasingly richer representations of meaning; we need better ways to effectively understand what these systems are capable of and what are the scenarios they are used to represent. And in conjunction to understanding their capabilities and limitations, we have to build reasoning algorithms on top of them. It's unlikely that these tools will ever be enough to solve all of our challenges; one has to equip these representations with the ability to reason, especially when they face an unusual/unseen scenario. 


In Chapter 5 (essential terms) an initial motivation was to model \emph{knowing what we don't know}~\citep{RajpurkarJiLi18}; basically, systems should be able to infer whether they have enough confidence about the answer to a given query before acting. 
% in order to make a decision. 
% In practice, we divided it into multiple steps, namely deciding what is a essential in questions.  
In hindsight, I think our supervised system 
% Another issue is that the final systems 
ended up using too many shallow features, which didn't end up generalizing to tricky instances. 
Additionally, it would have been better if the decision of essentiality was more involved within reasoning systems (rather than an independently supervised classifier, which limited its domain transfer). 
% Another limitation of the model we study is that it is tailored specifically to science exams domain. 
% One way go beyond this limitation is to resort to unsupervised baselines we discussed here, which were shown to achieve competitive results compared to the supervised systems. 


The datasets of Chapter 6 and 7 are critical 
% I think this is a critical 
parts of this thesis which, I suspect, are likely to be remembered longer than the rest of the chapters. In general, the construction of datasets (including the ones we described) is a menial task. 
It's unfortunate that many small empirical details are usually left out. 
% Such issues make me more concerned, in particular with respect to the progress of the field, since at the this point such datasets are used to argue the progress in the field. 
It is not clear to me whether using static datasets is the best way for the road ahead. 
In the future, I hope that the field discovers more effective ways of measuring the progress towards NLU. 


A key issue contributing to the complexity of NLU (and Question Answering) is the set of implied information  (common sense). 
% of details omitted because they sound redundant for humans. 
We touch upon a class of such understanding in Chapter 7, where we introduce a dataset for such problems. A natural next step is addressing such questions and exploring the many ways we can incorporate such understanding in the models. 

The analysis of Chapter 8 is uniquely distinct within the field. That said, there are many issues that make me feel unsatisfied about our current attempt. In particular, there are many assumptions that may or may not stand the test of time (e.g., the generative construction of symbol graph from the meaning graph or the connectivity reasoning as a proxy for the actual reasoning in language). 
And there are some important reasoning phenomena missing from this formalism: 
% And these assumptions don't cover some important phenomena: 
conditional reasoning, transitivity and directionality, inductive reasoning, just to name a few. 
% There are reasons that we haven't been able to provide formalism here. 
In general, our (the field's) understanding of ``reasoning'' (and its formalisms) is very limited. 
% What bothers me is we do not really understand much on formalism of reasoning. 
And the existing formalisms are not easily applicable, since 
those who formalized reasoning were not intimately aware of the complexity of NLU; they were philosophers and mathematicians. In practice, it's really hard to make the existing theories of reasoning work in the existence of many of the properties of language. 
In the coming years, 
I would like to see more efforts on reconciling the issues in the interface of ``language'' and ``reasoning''. 


